Localizing an Unknown Number of mmW Transmitters Under Path Loss Model Uncertainties

This work estimates the position and the transmit power of multiple co-channel wireless transmitters under model uncertainties. The model uncertainties include the number of the targets and the parameters of the path-loss model which enable the system to cope with changes in the weather conditions and in mmW ranges. The problem is solved by an unbiased estimator. The underlying complicated optimization problem has a combinatorial nature that selects the best grid points as the location of the targets. The combinatorial problem is converted to a convex form by means of l1-regularization, which enables locating off-grid targets. Simulations show that the proposed algorithm solves the problem with very high accuracy in the absence of noise and shadowing.

==> figures/alpha_N_2_K_20_G_5_SNR_1000_I_20_Pratio_2_Nratio_1_cs.tex <==
\addplot [color=blue,line width=0.6pt]
  table[row sep=crcr]{%
5.2245789394125e-14	1\\
5.2245789394125e-14	0.99922480620155\\
1.0449157878825e-13	0.998449612403101\\
3.65720525758875e-13	0.997674418604651\\
6.40010920078031e-13	0.996899224806201\\
6.92256709472156e-13	0.996124031007752\\
8.09809735608938e-13	0.995348837209302\\
1.09716157727663e-12	0.994573643410853\\
1.13634591932222e-12	0.993798449612403\\
1.18859170871634e-12	0.993023255813953\\
1.26696039280753e-12	0.992248062015504\\
1.28002184015606e-12	0.991472868217054\\
1.29308328750459e-12	0.990697674418604\\
1.39757486629284e-12	0.989922480620155\\
1.55431223447522e-12	0.989147286821705\\
2.089831575765e-12	0.988372093023256\\
2.16820025985619e-12	0.987596899224806\\
2.67759670644891e-12	0.986821705426356\\
2.7167810484945e-12	0.986046511627907\\
2.82127262728275e-12	0.985271317829457\\
2.88657986402541e-12	0.984496124031008\\
2.89964131137394e-12	0.983720930232558\\
3.05637867955631e-12	0.982945736434108\\
3.06944012690484e-12	0.982170542635659\\
3.23923894243575e-12	0.981395348837209\\
3.343730521224e-12	0.98062015503876\\
3.48740644205784e-12	0.97984496124031\\
3.60495946819463e-12	0.97906976744186\\
3.82700407311966e-12	0.978294573643411\\
4.07517157274175e-12	0.977519379844961\\
4.11435591478735e-12	0.976744186046512\\
4.16660170418147e-12	0.975968992248062\\
4.29721617766678e-12	0.975193798449612\\
4.50619933524328e-12	0.974418604651163\\
4.75436683486538e-12	0.972868217054264\\
4.8066126242595e-12	0.972093023255814\\
5.10702591327572e-12	0.971317829457364\\
5.2637632814581e-12	0.970542635658915\\
5.48580788638313e-12	0.969767441860465\\
5.59029946517138e-12	0.968992248062016\\
5.79928262274788e-12	0.968217054263566\\
5.81234407009641e-12	0.967441860465116\\
6.03438867502144e-12	0.966666666666667\\
6.34786341138619e-12	0.965891472868217\\
6.37398630608325e-12	0.965116279069767\\
6.687461042448e-12	0.964341085271318\\
6.84419841063038e-12	0.963565891472868\\
6.9356285420701e-12	0.962790697674419\\
6.94868998941863e-12	0.961240310077519\\
7.01399722616128e-12	0.96046511627907\\
7.53645512010253e-12	0.95968992248062\\
7.54951656745106e-12	0.958914728682171\\
7.69319248828491e-12	0.958139534883721\\
8.01972867199819e-12	0.957364341085271\\
8.20258893487763e-12	0.956589147286822\\
8.34626485571147e-12	0.955813953488372\\
8.54218656593944e-12	0.955038759689923\\
8.5683094606365e-12	0.954263565891473\\
8.64667814472769e-12	0.953488372093023\\
8.67280103942475e-12	0.952713178294574\\
8.73810827616741e-12	0.951937984496124\\
8.79035406556153e-12	0.951162790697675\\
8.84259985495566e-12	0.950387596899225\\
8.90790709169832e-12	0.949612403100775\\
9.07770590722922e-12	0.948837209302326\\
9.18219748601747e-12	0.948062015503876\\
9.60016380117047e-12	0.947286821705427\\
9.6524095905646e-12	0.946511627906977\\
9.96588432692935e-12	0.945736434108527\\
1.00834373530661e-11	0.944961240310078\\
1.01356831424603e-11	0.944186046511628\\
1.01748674845058e-11	0.943410852713178\\
1.02924205106426e-11	0.942635658914729\\
1.03054819579912e-11	0.941860465116279\\
1.05144651155677e-11	0.94108527131783\\
1.08540627466295e-11	0.94031007751938\\
1.0867124193978e-11	0.93953488372093\\
1.10238615621604e-11	0.938759689922481\\
1.12459061670854e-11	0.937984496124031\\
1.17553026136781e-11	0.937209302325582\\
1.18075484030723e-11	0.936434108527132\\
1.18206098504208e-11	0.935658914728682\\
1.1898978534512e-11	0.934883720930233\\
1.19381628765576e-11	0.934108527131783\\
1.21079616920885e-11	0.933333333333333\\
1.22777605076194e-11	0.932558139534884\\
1.24606207704988e-11	0.931782945736434\\
1.24998051125444e-11	0.931007751937985\\
1.28785870856518e-11	0.930232558139535\\
1.29961401117886e-11	0.929457364341086\\
1.32965534008048e-11	0.928682170542636\\
1.35055365583813e-11	0.927906976744186\\
1.37275811633063e-11	0.927131782945737\\
1.39757486629284e-11	0.925581395348837\\
1.40671787943682e-11	0.924806201550388\\
1.42761619519447e-11	0.924031007751938\\
1.440677642543e-11	0.923255813953489\\
1.46418824777035e-11	0.922480620155039\\
1.47724969511888e-11	0.921705426356589\\
1.51512789242963e-11	0.92015503875969\\
1.51774018189933e-11	0.919379844961241\\
1.52035247136904e-11	0.918604651162791\\
1.5242709055736e-11	0.917829457364342\\
1.52557705030845e-11	0.917054263565892\\
1.52818933977816e-11	0.916279069767442\\
1.59088428705111e-11	0.915503875968993\\
1.60655802386934e-11	0.914728682170543\\
1.6078641686042e-11	0.913953488372093\\
1.69015128689994e-11	0.913178294573644\\
1.70582502371818e-11	0.912403100775194\\
1.71888647106671e-11	0.911627906976745\\
1.72019261580157e-11	0.910852713178295\\
1.74762165523348e-11	0.910077519379845\\
1.78549985254422e-11	0.909302325581396\\
1.81162274724128e-11	0.908527131782946\\
1.8168473261807e-11	0.907751937984497\\
1.81815347091555e-11	0.906976744186047\\
1.82076576038526e-11	0.906201550387597\\
1.84558251034747e-11	0.905426356589148\\
1.84819479981717e-11	0.904651162790698\\
1.87039926030968e-11	0.903875968992249\\
1.87692998398394e-11	0.903100775193799\\
1.89129757606733e-11	0.902325581395349\\
1.90697131288556e-11	0.9015503875969\\
1.91742047076439e-11	0.90077519379845\\
1.92656348390836e-11	0.9\\
1.93048191811292e-11	0.899224806201551\\
1.93962493125689e-11	0.898449612403101\\
1.96052324701454e-11	0.897674418604652\\
1.97358469436307e-11	0.896899224806202\\
1.97750312856763e-11	0.896124031007752\\
1.98533999697675e-11	0.895348837209303\\
1.99056457591616e-11	0.894573643410853\\
2.0062383127344e-11	0.893798449612404\\
2.0284427732269e-11	0.893023255813954\\
2.10681145731809e-11	0.892248062015504\\
2.1316282072803e-11	0.891472868217055\\
2.15644495724251e-11	0.890697674418605\\
2.16297568091678e-11	0.889922480620156\\
2.17081254932589e-11	0.889147286821706\\
2.17473098353045e-11	0.888372093023256\\
2.24656894394738e-11	0.887596899224807\\
2.27399798337929e-11	0.886821705426357\\
2.27530412811414e-11	0.886046511627907\\
2.28052870705356e-11	0.885271317829458\\
2.31318232542488e-11	0.884496124031008\\
2.31710075962944e-11	0.883720930232558\\
2.32754991750827e-11	0.882170542635659\\
2.38763257531151e-11	0.881395348837209\\
2.4020001673949e-11	0.88062015503876\\
2.41898004894799e-11	0.87984496124031\\
2.44118450944049e-11	0.879069767441861\\
2.45947053572844e-11	0.878294573643411\\
2.48036885148608e-11	0.877519379844962\\
2.49343029883462e-11	0.876744186046512\\
2.49865487777403e-11	0.875968992248062\\
2.51563475932712e-11	0.875193798449613\\
2.5717989829258e-11	0.874418604651163\\
2.58747271974404e-11	0.873643410852714\\
2.58877886447889e-11	0.872868217054264\\
2.64102465387302e-11	0.872093023255814\\
2.64755537754729e-11	0.871317829457365\\
2.65931068016096e-11	0.870542635658915\\
2.68543357485803e-11	0.869767441860465\\
2.77163912735833e-11	0.868992248062016\\
2.78600671944172e-11	0.868217054263566\\
2.80821117993422e-11	0.867441860465117\\
2.81082346940393e-11	0.866666666666667\\
2.82519106148731e-11	0.865891472868217\\
2.89702902190423e-11	0.865116279069768\\
2.92184577186644e-11	0.864341085271318\\
2.95319324550292e-11	0.862790697674419\\
2.99368373228336e-11	0.862015503875969\\
3.01066361383645e-11	0.86124031007752\\
3.08250157425338e-11	0.86046511627907\\
3.10731832421559e-11	0.859689922480621\\
3.17131941622339e-11	0.858914728682171\\
3.18699315304163e-11	0.858139534883722\\
3.22487135035237e-11	0.857364341085272\\
3.26144340292825e-11	0.856589147286822\\
3.27189256080708e-11	0.855813953488373\\
3.27319870554193e-11	0.855038759689923\\
3.34895510016341e-11	0.854263565891473\\
3.35026124489827e-11	0.853488372093024\\
3.35156738963312e-11	0.852713178294574\\
3.35679196857253e-11	0.851937984496125\\
3.3659349817165e-11	0.851162790697675\\
3.36985341592106e-11	0.850387596899225\\
3.39597631061813e-11	0.849612403100776\\
3.47303884997446e-11	0.848837209302326\\
3.50569246834579e-11	0.848062015503876\\
3.530509218308e-11	0.847286821705427\\
3.5331215077777e-11	0.846511627906977\\
3.53703994198226e-11	0.845736434108528\\
3.55401982353535e-11	0.844961240310078\\
3.60887790239919e-11	0.844186046511628\\
3.61279633660374e-11	0.843410852713179\\
3.6167147708083e-11	0.842635658914729\\
3.62847007342198e-11	0.841860465116279\\
3.63500079709625e-11	0.84108527131783\\
3.63761308656595e-11	0.84031007751938\\
3.66765441546758e-11	0.83953488372093\\
3.67418513914184e-11	0.838759689922481\\
3.73688008641479e-11	0.837984496124031\\
3.74471695482391e-11	0.837209302325582\\
3.74994153376332e-11	0.835658914728682\\
3.82831021785451e-11	0.834883720930233\\
3.83614708626363e-11	0.834108527131783\\
3.85051467834701e-11	0.833333333333334\\
3.85573925728643e-11	0.832558139534884\\
3.86618841516525e-11	0.831782945736434\\
3.89231130986231e-11	0.831007751937985\\
3.93280179664276e-11	0.830232558139535\\
3.95500625713526e-11	0.829457364341086\\
4.05949783592351e-11	0.828682170542636\\
4.0764777174766e-11	0.827906976744186\\
4.07778386221146e-11	0.827131782945737\\
4.20056146728765e-11	0.826356589147287\\
4.2214597830453e-11	0.825581395348838\\
4.23060279618927e-11	0.824806201550388\\
4.26195026982575e-11	0.824031007751938\\
4.2632564145606e-11	0.823255813953489\\
4.29460388819708e-11	0.822480620155039\\
4.32595136183355e-11	0.82170542635659\\
4.33509437497752e-11	0.82093023255814\\
4.34031895391694e-11	0.82015503875969\\
4.38342173016709e-11	0.819379844961241\\
4.40562619065959e-11	0.818604651162791\\
4.47093342740225e-11	0.817829457364342\\
4.49052559842505e-11	0.817054263565892\\
4.60024175615271e-11	0.816279069767442\\
4.62375236138006e-11	0.815503875968993\\
4.63550766399374e-11	0.814728682170543\\
4.64203838766801e-11	0.813953488372094\\
4.65771212448624e-11	0.813178294573644\\
4.67077357183478e-11	0.812403100775195\\
4.67207971656963e-11	0.811627906976745\\
4.69036574285757e-11	0.810852713178295\\
4.70865176914552e-11	0.810077519379846\\
4.72563165069861e-11	0.809302325581396\\
4.72824394016831e-11	0.808527131782946\\
4.78963274270641e-11	0.807751937984497\\
4.79485732164582e-11	0.806976744186047\\
4.79616346638068e-11	0.806201550387598\\
4.86277684785819e-11	0.805426356589148\\
4.90587962410834e-11	0.804651162790698\\
4.91632878198716e-11	0.803875968992249\\
4.91763492672202e-11	0.803100775193799\\
4.97510529505555e-11	0.802325581395349\\
4.98163601872982e-11	0.8015503875969\\
4.99861590028291e-11	0.80077519379845\\
5.11747507115455e-11	0.800000000000001\\
5.15404712373043e-11	0.799224806201551\\
5.19976218945029e-11	0.798449612403101\\
5.26115099198839e-11	0.797674418604652\\
5.26506942619295e-11	0.796899224806202\\
5.2663755709278e-11	0.796124031007753\\
5.27290629460207e-11	0.795348837209303\\
5.3303766629356e-11	0.794573643410853\\
5.42441908384503e-11	0.793798449612404\\
5.43486824172385e-11	0.793023255813954\\
5.48842017585283e-11	0.792248062015505\\
5.49103246532254e-11	0.791472868217055\\
5.5811564520274e-11	0.790697674418605\\
5.60336091251991e-11	0.789922480620156\\
5.62948380721697e-11	0.789147286821706\\
5.63601453089124e-11	0.788372093023257\\
5.63862682036094e-11	0.787596899224807\\
5.66736200452771e-11	0.786821705426357\\
5.74442454388405e-11	0.786046511627908\\
5.77446587278567e-11	0.785271317829458\\
5.82148708324038e-11	0.784496124031009\\
5.83585467532377e-11	0.783720930232559\\
5.88287588577848e-11	0.782945736434109\\
5.95993842513481e-11	0.78217054263566\\
5.96908143827878e-11	0.78139534883721\\
6.00173505665011e-11	0.780620155038761\\
6.00957192505923e-11	0.779844961240311\\
6.01479650399864e-11	0.779069767441861\\
6.15455399062793e-11	0.778294573643412\\
6.16108471430219e-11	0.777519379844962\\
6.16239085903705e-11	0.776744186046513\\
6.21463664843117e-11	0.775968992248063\\
6.25904556941618e-11	0.775193798449613\\
6.35570027979531e-11	0.774418604651164\\
6.38966004290149e-11	0.773643410852714\\
6.50460077956856e-11	0.772868217054265\\
6.5176622269171e-11	0.772093023255815\\
6.58296946365975e-11	0.771317829457365\\
6.60256163468255e-11	0.770542635658916\\
6.66917501616006e-11	0.769767441860466\\
6.69007333191771e-11	0.768992248062017\\
6.70182863453139e-11	0.768217054263567\\
6.70835935820565e-11	0.767441860465118\\
6.79195262123625e-11	0.766666666666668\\
6.90036263422906e-11	0.765891472868218\\
6.91211793684274e-11	0.765116279069769\\
6.9160363710473e-11	0.764341085271319\\
6.93954697627466e-11	0.76356589147287\\
6.94085312100951e-11	0.76279069767442\\
6.94215926574436e-11	0.76201550387597\\
7.0192218051007e-11	0.761240310077521\\
7.02575252877496e-11	0.760465116279071\\
7.05971229188114e-11	0.759689922480622\\
7.09367205498732e-11	0.758914728682172\\
7.17204073907851e-11	0.758139534883722\\
7.18510218642704e-11	0.757364341085273\\
7.20730664691955e-11	0.756589147286823\\
7.22689881794234e-11	0.755813953488374\\
7.26216472578338e-11	0.755038759689924\\
7.26608315998794e-11	0.754263565891474\\
7.27392002839706e-11	0.753488372093025\\
7.34575798881398e-11	0.752713178294575\\
7.44502498866282e-11	0.751937984496126\\
7.5625780147996e-11	0.751162790697676\\
7.62266067260284e-11	0.750387596899226\\
7.63310983048166e-11	0.749612403100777\\
7.67621260673182e-11	0.748837209302327\\
7.70102935669403e-11	0.748062015503878\\
7.70494779089859e-11	0.747286821705428\\
7.710172369838e-11	0.746511627906978\\
7.80160250127772e-11	0.745736434108529\\
7.85907286961126e-11	0.744961240310079\\
7.89172648798258e-11	0.744186046511629\\
7.91001251427053e-11	0.74341085271318\\
7.9387476984373e-11	0.74263565891473\\
7.97140131680862e-11	0.74186046511628\\
8.04323927722555e-11	0.741085271317831\\
8.04846385616496e-11	0.740310077519381\\
8.05499457983922e-11	0.739534883720932\\
8.11638338237732e-11	0.738759689922482\\
8.13728169813497e-11	0.737984496124032\\
8.18691519805939e-11	0.737209302325583\\
8.19475206646851e-11	0.736434108527133\\
8.21303809275645e-11	0.735658914728684\\
8.2731207505597e-11	0.734883720930234\\
8.2757330400294e-11	0.734108527131784\\
8.29271292158249e-11	0.733333333333335\\
8.41940896086325e-11	0.732558139534885\\
8.47557318446193e-11	0.731782945736436\\
8.53826813173488e-11	0.730232558139536\\
8.54218656593944e-11	0.729457364341087\\
8.57222789484106e-11	0.728682170542637\\
8.57875861851533e-11	0.727906976744188\\
8.62186139476548e-11	0.727131782945738\\
8.62839211843975e-11	0.726356589147288\\
8.6714948946899e-11	0.725581395348839\\
8.76031273665991e-11	0.724806201550389\\
8.87394732859213e-11	0.72403100775194\\
8.88439648647096e-11	0.72325581395349\\
8.92749926272111e-11	0.721705426356591\\
8.93533613113023e-11	0.720930232558141\\
8.95623444688788e-11	0.720155038759692\\
8.95754059162273e-11	0.719379844961242\\
8.99672493366833e-11	0.718604651162792\\
9.00717409154715e-11	0.717829457364343\\
9.01631710469112e-11	0.717054263565893\\
9.02937855203966e-11	0.716279069767444\\
9.08684892037319e-11	0.715503875968994\\
9.11035952560055e-11	0.714728682170544\\
9.14301314397188e-11	0.713953488372095\\
9.16782989393409e-11	0.712403100775196\\
9.18089134128262e-11	0.711627906976746\\
9.24097399908586e-11	0.710852713178296\\
9.24228014382071e-11	0.710077519379847\\
9.25926002537381e-11	0.709302325581397\\
9.26187231484351e-11	0.708527131782948\\
9.36113931469235e-11	0.707751937984498\\
9.37681305151059e-11	0.706976744186048\\
9.39379293306368e-11	0.706201550387599\\
9.41730353829103e-11	0.705426356589149\\
9.42514040670015e-11	0.7046511627907\\
9.52571355128384e-11	0.70387596899225\\
9.58187777488253e-11	0.7031007751938\\
9.63542970901151e-11	0.702325581395351\\
9.63934814321606e-11	0.701550387596901\\
9.65894031423886e-11	0.700775193798452\\
9.73469670886034e-11	0.700000000000002\\
9.80131009033785e-11	0.699224806201552\\
9.80653466927727e-11	0.698449612403103\\
9.85616816920168e-11	0.697674418604653\\
9.96849661639905e-11	0.696899224806204\\
9.99984409003553e-11	0.696124031007754\\
1.00181301163235e-10	0.695348837209304\\
1.00808250635964e-10	0.694573643410855\\
1.01069479582935e-10	0.693798449612405\\
1.01160909714375e-10	0.693023255813956\\
1.01213155503769e-10	0.692248062015506\\
1.01435200108694e-10	0.691472868217056\\
1.02036026686726e-10	0.690697674418607\\
1.03028696685215e-10	0.689922480620157\\
1.03080942474609e-10	0.689147286821707\\
1.03446663000368e-10	0.688372093023258\\
1.0395605944696e-10	0.687596899224808\\
1.04347902867416e-10	0.686821705426359\\
1.06385488653787e-10	0.686046511627909\\
1.0680345496894e-10	0.685271317829459\\
1.07077745363259e-10	0.68449612403101\\
1.07443465889018e-10	0.68372093023256\\
1.07561018915155e-10	0.682945736434111\\
1.0778306352008e-10	0.682170542635661\\
1.08344705756067e-10	0.681395348837211\\
1.09846772201148e-10	0.680620155038762\\
1.1196272667161e-10	0.679844961240312\\
1.13882759431844e-10	0.679069767441862\\
1.14392155878437e-10	0.678294573643413\\
1.14457463115179e-10	0.677519379844963\\
1.15045228245863e-10	0.676744186046514\\
1.15097474035257e-10	0.675968992248064\\
1.15881160876169e-10	0.675193798449614\\
1.15972591007609e-10	0.674418604651165\\
1.16011775349655e-10	0.673643410852715\\
1.16129328375791e-10	0.672868217054266\\
1.16155451270488e-10	0.672093023255816\\
1.1667790916443e-10	0.671317829457366\\
1.17422411663296e-10	0.670542635658917\\
1.17605271926175e-10	0.669767441860467\\
1.18584880477315e-10	0.668992248062017\\
1.18767740740195e-10	0.668217054263568\\
1.18950601003074e-10	0.667441860465118\\
1.19420813107621e-10	0.666666666666669\\
1.19891025212168e-10	0.665891472868219\\
1.20256745737927e-10	0.665116279069769\\
1.20713896395126e-10	0.66434108527132\\
1.20805326526566e-10	0.66356589147287\\
1.21288600078461e-10	0.662790697674421\\
1.22320454418995e-10	0.662015503875971\\
1.22490253234526e-10	0.661240310077521\\
1.22503314681875e-10	0.660465116279072\\
1.22751482181497e-10	0.659689922480622\\
1.23051895470513e-10	0.658914728682173\\
1.23678844943242e-10	0.658139534883723\\
1.25207034283021e-10	0.657364341085274\\
1.25990721123932e-10	0.656589147286824\\
1.26304195860297e-10	0.655813953488374\\
1.26800530859541e-10	0.655038759689925\\
1.27388295990225e-10	0.654263565891475\\
1.27584217700453e-10	0.653488372093026\\
1.28198105725834e-10	0.652713178294576\\
1.2947812756599e-10	0.651937984496126\\
1.29869970986446e-10	0.651162790697677\\
1.30627534932661e-10	0.650387596899227\\
1.34480661900478e-10	0.649612403100778\\
1.35016181241768e-10	0.648837209302328\\
1.35238225846693e-10	0.648062015503878\\
1.35786806635331e-10	0.647286821705429\\
1.37955006895187e-10	0.646511627906979\\
1.38790939525493e-10	0.64573643410853\\
1.3979667097133e-10	0.64496124031008\\
1.3988810110277e-10	0.64418604651163\\
1.39992592681558e-10	0.643410852713181\\
1.40136268602392e-10	0.642635658914731\\
1.41050569916789e-10	0.641860465116282\\
1.41599150705427e-10	0.641085271317832\\
1.42500390572476e-10	0.640310077519382\\
1.42513452019825e-10	0.639534883720933\\
1.42539574914522e-10	0.638759689922483\\
1.43427753334222e-10	0.637984496124034\\
1.44537976358847e-10	0.637209302325584\\
1.45269417410365e-10	0.636434108527134\\
1.45713506620215e-10	0.635658914728685\\
1.46131472935368e-10	0.634883720930235\\
1.47006589907719e-10	0.634108527131785\\
1.47542109249009e-10	0.633333333333336\\
1.47855583985374e-10	0.632558139534886\\
1.48260488853178e-10	0.631782945736437\\
1.48678455168331e-10	0.631007751937987\\
1.4913560582553e-10	0.630232558139537\\
1.49357650430455e-10	0.629457364341088\\
1.49775616745608e-10	0.628682170542638\\
1.51147068717204e-10	0.627906976744189\\
1.51695649505842e-10	0.627131782945739\\
1.52440152004708e-10	0.62635658914729\\
1.53772419634258e-10	0.62558139534884\\
1.54399369106988e-10	0.62480620155039\\
1.54543045027822e-10	0.624031007751941\\
1.54752028185398e-10	0.623255813953491\\
1.5544428489487e-10	0.622480620155042\\
1.5553571502631e-10	0.621705426356592\\
1.56123480156994e-10	0.620930232558142\\
1.56567569366844e-10	0.620155038759693\\
1.56632876603587e-10	0.619379844961243\\
1.59075367257762e-10	0.618604651162794\\
1.59610886599052e-10	0.617829457364344\\
1.59663132388446e-10	0.617054263565894\\
1.59976607124811e-10	0.616279069767445\\
1.60472942124055e-10	0.615503875968995\\
1.61922762779742e-10	0.614728682170546\\
1.6247134356838e-10	0.613953488372096\\
1.63934225671416e-10	0.613178294573646\\
1.64313007644523e-10	0.612403100775197\\
1.64495867907403e-10	0.611627906976747\\
1.64770158301722e-10	0.610852713178298\\
1.65240370406269e-10	0.610077519379848\\
1.65292616195663e-10	0.609302325581399\\
1.66024057247181e-10	0.608527131782949\\
1.671865260612e-10	0.607751937984499\\
1.67251833297943e-10	0.60697674418605\\
1.68140011717643e-10	0.6062015503876\\
1.70360457766893e-10	0.605426356589151\\
1.72032323027505e-10	0.604651162790701\\
1.73024993025994e-10	0.603875968992251\\
1.74357260655544e-10	0.603100775193802\\
1.76238109073732e-10	0.602325581395352\\
1.76264231968429e-10	0.601550387596903\\
1.76891181441159e-10	0.600775193798453\\
1.77883851439647e-10	0.600000000000003\\
1.7848467801768e-10	0.599224806201554\\
1.78628353938513e-10	0.598449612403104\\
1.78732845517302e-10	0.597674418604655\\
1.79007135911621e-10	0.596899224806205\\
1.79830007094578e-10	0.596124031007755\\
1.81214520513523e-10	0.595348837209306\\
1.82063514591177e-10	0.594573643410856\\
1.82194129064662e-10	0.593798449612407\\
1.82899447221483e-10	0.593023255813957\\
1.83356597878682e-10	0.592248062015508\\
1.86530529584375e-10	0.591472868217058\\
1.88293824976427e-10	0.590697674418608\\
1.89090573264687e-10	0.589922480620159\\
1.89234249185521e-10	0.589147286821709\\
1.89782829974159e-10	0.58837209302326\\
1.90017936026433e-10	0.58759689922481\\
1.90893052998784e-10	0.58682170542636\\
1.952033306238e-10	0.586046511627911\\
1.96013140359409e-10	0.585271317829461\\
1.96613966937441e-10	0.584496124031011\\
1.98050726145779e-10	0.583720930232562\\
1.98142156277219e-10	0.582945736434112\\
1.99343809433284e-10	0.582170542635663\\
1.99356870880633e-10	0.581395348837213\\
1.99487485354118e-10	0.580620155038764\\
2.01969160350339e-10	0.579844961240314\\
2.0240018811284e-10	0.579069767441864\\
2.02504679691629e-10	0.578294573643415\\
2.03484288242768e-10	0.577519379844965\\
2.05717795739367e-10	0.576744186046516\\
2.06971694684826e-10	0.575968992248066\\
2.08395392445816e-10	0.575193798449616\\
2.08460699682559e-10	0.574418604651167\\
2.08957034681803e-10	0.573643410852717\\
2.09583984154533e-10	0.572868217054268\\
2.1183055309848e-10	0.572093023255818\\
2.13097513491287e-10	0.571317829457368\\
2.13646094279926e-10	0.570542635658919\\
2.14090183489776e-10	0.569767441860469\\
2.14351412436746e-10	0.56899224806202\\
2.14847747435991e-10	0.56821705426357\\
2.1556612704016e-10	0.56744186046512\\
2.16088584934101e-10	0.566666666666671\\
2.16232260854935e-10	0.565891472868221\\
2.17682081510622e-10	0.565116279069772\\
2.1778657308941e-10	0.564341085271322\\
2.20176817954191e-10	0.563565891472873\\
2.20346616769722e-10	0.562790697674423\\
2.21352348215559e-10	0.562015503875973\\
2.2259318571367e-10	0.561240310077524\\
2.23585855712158e-10	0.560465116279074\\
2.24003822027311e-10	0.559689922480625\\
2.24160559395493e-10	0.558914728682175\\
2.24656894394738e-10	0.558139534883725\\
2.25727933077317e-10	0.557364341085276\\
2.27007954917473e-10	0.556589147286826\\
2.27151630838307e-10	0.555813953488377\\
2.29633305834528e-10	0.555038759689927\\
2.31083126490215e-10	0.554263565891477\\
2.31200679516352e-10	0.553488372093028\\
2.32154165172795e-10	0.552713178294578\\
2.33238265302723e-10	0.551937984496129\\
2.35406465562579e-10	0.551162790697679\\
2.35863616219777e-10	0.550387596899229\\
2.37169760954631e-10	0.54961240310078\\
2.38475905689484e-10	0.54883720930233\\
2.38711011741757e-10	0.548062015503881\\
2.40800843317522e-10	0.547286821705431\\
2.42472708578134e-10	0.546511627906981\\
2.43896406339124e-10	0.545736434108532\\
2.44079266602004e-10	0.544961240310082\\
2.44797646206173e-10	0.544186046511633\\
2.44954383574355e-10	0.543410852713183\\
2.46835231992544e-10	0.542635658914734\\
2.50296515539904e-10	0.541860465116284\\
2.52360224220972e-10	0.541085271317834\\
2.53796983429311e-10	0.540310077519385\\
2.54371687112646e-10	0.539534883720935\\
2.55481910137271e-10	0.538759689922486\\
2.56056613820607e-10	0.537984496124036\\
2.58146445396372e-10	0.537209302325586\\
2.60719550524032e-10	0.536434108527137\\
2.63162041178208e-10	0.535658914728687\\
2.65473917358898e-10	0.534883720930238\\
2.6563065472708e-10	0.534108527131788\\
2.71560551823313e-10	0.533333333333338\\
2.72618529058544e-10	0.532558139534889\\
2.75204695633554e-10	0.531782945736439\\
2.79214559969553e-10	0.53100775193799\\
2.81983586807441e-10	0.53023255813954\\
2.83877496672978e-10	0.52945736434109\\
2.84060356935858e-10	0.528682170542641\\
2.87521640483219e-10	0.527906976744191\\
2.88174712850645e-10	0.527131782945742\\
2.89572287716938e-10	0.526356589147292\\
2.89689840743075e-10	0.525581395348843\\
2.89715963637772e-10	0.524806201550393\\
2.93686643631725e-10	0.524031007751943\\
2.94078487052181e-10	0.523255813953494\\
2.95502184813171e-10	0.522480620155044\\
2.97056497047646e-10	0.521705426356595\\
2.9720017296848e-10	0.520930232558145\\
2.97356910336663e-10	0.520155038759695\\
3.02437813355241e-10	0.519379844961246\\
3.02594550723424e-10	0.518604651162796\\
3.02685980854863e-10	0.517829457364347\\
3.05376639008661e-10	0.517054263565897\\
3.06526046375331e-10	0.516279069767447\\
3.07479532031774e-10	0.515503875968998\\
3.07688515189351e-10	0.514728682170548\\
3.08158727293898e-10	0.513953488372099\\
3.11241228868151e-10	0.513178294573649\\
3.11384904788985e-10	0.512403100775199\\
3.15486199256424e-10	0.51162790697675\\
3.22108353062129e-10	0.5108527131783\\
3.23871648454181e-10	0.510077519379851\\
3.2405450871706e-10	0.509302325581401\\
3.25465145030702e-10	0.508527131782951\\
3.25648005293581e-10	0.507751937984502\\
3.26732105423509e-10	0.506976744186052\\
3.27816205553437e-10	0.506201550387603\\
3.28573769499652e-10	0.505426356589153\\
3.30350126339052e-10	0.504651162790703\\
3.30833399890948e-10	0.503875968992254\\
3.32361589230726e-10	0.503100775193804\\
3.32701186861788e-10	0.502325581395355\\
3.39780491324692e-10	0.501550387596905\\
3.40198457639845e-10	0.500775193798455\\
3.40799284217877e-10	0.500000000000006\\
3.44338936449329e-10	0.499224806201556\\
3.48675336969042e-10	0.498449612403107\\
3.50308017887608e-10	0.497674418604657\\
3.51026397491777e-10	0.496899224806208\\
3.57413445245209e-10	0.496124031007758\\
3.59620829847111e-10	0.495348837209308\\
3.60482885372114e-10	0.494573643410859\\
3.62363733790303e-10	0.493798449612409\\
3.63552325499019e-10	0.493023255813959\\
3.65616034180087e-10	0.49224806201551\\
3.69717328647526e-10	0.49147286821706\\
3.70971227592985e-10	0.49069767441861\\
3.71741852986548e-10	0.489922480620161\\
3.75242320875954e-10	0.489147286821711\\
3.78742788765361e-10	0.488372093023262\\
3.78873403238846e-10	0.487596899224812\\
3.81080787840748e-10	0.486821705426362\\
3.82112642181282e-10	0.486046511627913\\
3.82778775996057e-10	0.485271317829463\\
3.83327356784695e-10	0.484496124031013\\
3.83340418232044e-10	0.483720930232564\\
3.89505421380551e-10	0.482945736434114\\
3.92718537428289e-10	0.482170542635665\\
3.93489162821853e-10	0.481395348837215\\
3.96832893343077e-10	0.480620155038765\\
4.01704813204079e-10	0.479844961240316\\
4.0222727109802e-10	0.479069767441866\\
4.06707347538566e-10	0.478294573643417\\
4.08078799510162e-10	0.477519379844967\\
4.08144106746905e-10	0.476744186046517\\
4.0818329108895e-10	0.475968992248068\\
4.0827472122039e-10	0.475193798449618\\
4.10090262401836e-10	0.474418604651168\\
4.13303378449574e-10	0.473643410852719\\
4.14021758053744e-10	0.472868217054269\\
4.15079735288975e-10	0.47209302325582\\
4.1663404752345e-10	0.47131782945737\\
4.17143443970043e-10	0.47054263565892\\
4.1805774528444e-10	0.469767441860471\\
4.18789186335958e-10	0.468992248062021\\
4.19768794887097e-10	0.468217054263572\\
4.2366110619696e-10	0.467441860465122\\
4.24314178564386e-10	0.466666666666672\\
4.24405608695826e-10	0.465891472868223\\
4.26221149877272e-10	0.465116279069773\\
4.2695259092879e-10	0.464341085271323\\
4.27422803033337e-10	0.463565891472874\\
4.32582074736007e-10	0.462790697674424\\
4.32699627762143e-10	0.462015503875975\\
4.32856365130326e-10	0.461240310077525\\
4.34319247233361e-10	0.460465116279075\\
4.34449861706847e-10	0.459689922480626\\
4.35821313678442e-10	0.458914728682176\\
4.40105468408761e-10	0.458139534883726\\
4.42835310904604e-10	0.457364341085277\\
4.43710427876955e-10	0.456589147286827\\
4.45199432874688e-10	0.455813953488378\\
4.48634593527351e-10	0.455038759689928\\
4.51769340890999e-10	0.454263565891478\\
4.53336714572823e-10	0.453488372093029\\
4.55152255754269e-10	0.452713178294579\\
4.55308993122451e-10	0.45193798449613\\
4.55609406411467e-10	0.45116279069768\\
4.57294333119428e-10	0.45038759689923\\
4.61447873376261e-10	0.449612403100781\\
4.64452006266423e-10	0.448837209302331\\
4.66136932974383e-10	0.448062015503882\\
4.67573692182722e-10	0.447286821705432\\
4.71740293886903e-10	0.446511627906982\\
4.7337297480547e-10	0.445736434108533\\
4.75710973880857e-10	0.444961240310083\\
4.82254759002471e-10	0.444186046511634\\
4.84514389393767e-10	0.443410852713184\\
4.88720175439994e-10	0.442635658914734\\
4.90143873200984e-10	0.441860465116285\\
4.92965145828267e-10	0.441085271317835\\
4.93983938721452e-10	0.440310077519386\\
4.94336597799862e-10	0.439534883720936\\
4.94754564115015e-10	0.438759689922486\\
4.97588898189647e-10	0.437984496124037\\
4.97941557268057e-10	0.437209302325587\\
4.98594629635484e-10	0.436434108527137\\
5.00109757527913e-10	0.435658914728688\\
5.00162003317307e-10	0.434883720930238\\
5.0120691910519e-10	0.434108527131789\\
5.0378002423285e-10	0.433333333333339\\
5.10715652774921e-10	0.432558139534889\\
5.135630482969e-10	0.43178294573644\\
5.24168943543908e-10	0.43100775193799\\
5.25357535252624e-10	0.430232558139541\\
5.31026203401887e-10	0.429457364341091\\
5.34004213397352e-10	0.428682170542641\\
5.41018210623513e-10	0.427906976744192\\
5.43369271146249e-10	0.427131782945742\\
5.48724464559147e-10	0.425581395348843\\
5.51519614291732e-10	0.424806201550393\\
5.54053535077347e-10	0.424031007751943\\
5.69975439395207e-10	0.423255813953494\\
5.71464444392939e-10	0.422480620155044\\
5.76009828070228e-10	0.421705426356595\\
5.80124183985016e-10	0.420930232558145\\
5.80986239510019e-10	0.420155038759695\\
5.81848295035022e-10	0.419379844961246\\
5.82409937271009e-10	0.418604651162796\\
5.86001835291855e-10	0.417829457364346\\
5.88588001866864e-10	0.417054263565897\\
5.91814179361951e-10	0.416279069767447\\
5.97221618564243e-10	0.415503875968998\\
6.01375158821076e-10	0.414728682170548\\
6.02380890266913e-10	0.413953488372098\\
6.02485381845701e-10	0.413178294573649\\
6.0845446328398e-10	0.412403100775199\\
6.15729689457112e-10	0.411627906976749\\
6.16003979851431e-10	0.4108527131783\\
6.27889896938594e-10	0.41007751937985\\
6.31155258775727e-10	0.4093023255814\\
6.33023045746567e-10	0.408527131782951\\
6.34760218243922e-10	0.407751937984501\\
6.3549165929544e-10	0.406976744186052\\
6.35792072584456e-10	0.405426356589152\\
6.44517119413275e-10	0.404651162790703\\
6.48788212696244e-10	0.403875968992253\\
6.48892704275033e-10	0.403100775193803\\
6.49885374273521e-10	0.402325581395354\\
6.51648669665573e-10	0.401550387596904\\
6.57173661894001e-10	0.400775193798454\\
6.57238969130744e-10	0.400000000000005\\
6.60765559914848e-10	0.399224806201555\\
6.63547648200085e-10	0.398449612403106\\
6.63939491620541e-10	0.397674418604656\\
6.74480079630805e-10	0.396899224806206\\
6.77954424625515e-10	0.396124031007757\\
6.79704658570218e-10	0.395348837209307\\
6.82343070934621e-10	0.394573643410858\\
6.84890053167585e-10	0.393798449612408\\
6.86614164217591e-10	0.393023255813958\\
6.91799558814958e-10	0.392248062015509\\
6.93523669864964e-10	0.391472868217059\\
6.9480369170512e-10	0.390697674418609\\
6.94816753152469e-10	0.38992248062016\\
7.02118102220298e-10	0.38914728682171\\
7.06075720766902e-10	0.388372093023261\\
7.07995753527137e-10	0.387596899224811\\
7.11574590100634e-10	0.386821705426361\\
7.11914187731696e-10	0.386046511627912\\
7.20822094823394e-10	0.385271317829462\\
7.23356015609009e-10	0.384496124031012\\
7.29181421126454e-10	0.383720930232563\\
7.29925923625321e-10	0.382945736434113\\
7.46069872548105e-10	0.382170542635663\\
7.48133581229173e-10	0.381395348837214\\
7.48982575306828e-10	0.380620155038764\\
7.49361357279935e-10	0.379844961240315\\
7.51059345435244e-10	0.379069767441865\\
7.52901009511387e-10	0.378294573643415\\
7.52992439642827e-10	0.377519379844966\\
7.63846502389456e-10	0.376744186046516\\
7.64264468704609e-10	0.375968992248066\\
7.71931538298197e-10	0.375193798449617\\
7.78971658419056e-10	0.374418604651167\\
7.80852506837244e-10	0.373643410852718\\
7.86377499065673e-10	0.372868217054268\\
7.87278738932721e-10	0.372093023255818\\
7.91223296031978e-10	0.371317829457369\\
7.91353910505463e-10	0.370542635658919\\
7.94828255500172e-10	0.36976744186047\\
7.9805443299526e-10	0.36899224806202\\
8.03083090224444e-10	0.36821705426357\\
8.06818664166124e-10	0.367441860465121\\
8.08059501664235e-10	0.366666666666671\\
8.0952238376727e-10	0.365891472868222\\
8.33568508335916e-10	0.365116279069772\\
8.34391379518874e-10	0.364341085271322\\
8.38270629381387e-10	0.363565891472873\\
8.426070299011e-10	0.362790697674423\\
8.54649684356446e-10	0.362015503875973\\
8.55368063960615e-10	0.361240310077524\\
8.64720060262163e-10	0.360465116279074\\
8.6563436157656e-10	0.359689922480624\\
8.71707934593627e-10	0.358914728682175\\
8.79845216291762e-10	0.358139534883725\\
8.84442845758445e-10	0.357364341085276\\
8.96524684555837e-10	0.356589147286826\\
8.99123912578194e-10	0.355813953488376\\
9.02781117835783e-10	0.355038759689927\\
9.03316637177073e-10	0.354263565891477\\
9.10448187429371e-10	0.353488372093028\\
9.10735539271039e-10	0.352713178294578\\
9.13334767293396e-10	0.351937984496128\\
9.1632583873621e-10	0.351162790697679\\
9.2300023833131e-10	0.350387596899229\\
9.25508036222228e-10	0.34961240310078\\
9.32809385290057e-10	0.34883720930233\\
9.38765405280987e-10	0.34806201550388\\
9.41913214091983e-10	0.347286821705431\\
9.43232420274184e-10	0.346511627906981\\
9.46236553164347e-10	0.345736434108531\\
9.53786069731798e-10	0.344961240310082\\
9.58644928145451e-10	0.344186046511632\\
9.72790475623911e-10	0.343410852713183\\
9.7404437456937e-10	0.342635658914733\\
9.84375979422058e-10	0.341860465116283\\
1.01304585635208e-09	0.341085271317834\\
1.01552753134831e-09	0.340310077519384\\
1.01632427963657e-09	0.339534883720934\\
1.04042264999461e-09	0.338759689922485\\
1.05054527168972e-09	0.337984496124035\\
1.05374532629011e-09	0.337209302325586\\
1.07429098296935e-09	0.336434108527136\\
1.07699470257049e-09	0.335658914728686\\
1.09370029372926e-09	0.334883720930237\\
1.10259513937361e-09	0.334108527131787\\
1.11129406330774e-09	0.333333333333337\\
1.12464286249793e-09	0.332558139534888\\
1.12820863762408e-09	0.331782945736438\\
1.12897926301765e-09	0.331007751937989\\
1.14036884510557e-09	0.330232558139539\\
1.15271191284993e-09	0.329457364341089\\
1.15848507257798e-09	0.32868217054264\\
1.16222064651966e-09	0.32790697674419\\
1.17035792821779e-09	0.32713178294574\\
1.17080201742764e-09	0.326356589147291\\
1.17311389360833e-09	0.325581395348841\\
1.17409350215947e-09	0.324806201550392\\
1.1818781247792e-09	0.324031007751942\\
1.1840593864864e-09	0.323255813953492\\
1.189440702794e-09	0.322480620155043\\
1.2001249667251e-09	0.321705426356593\\
1.20046456435616e-09	0.320930232558144\\
1.20777897487134e-09	0.320155038759694\\
1.20843204723876e-09	0.319379844961244\\
1.22170247774487e-09	0.318604651162795\\
1.240145241401e-09	0.317829457364345\\
1.2418954753457e-09	0.317054263565895\\
1.24295345258093e-09	0.316279069767446\\
1.25917577018781e-09	0.315503875968996\\
1.27345193213975e-09	0.314728682170547\\
1.2752674733212e-09	0.313953488372097\\
1.28424068764964e-09	0.313178294573647\\
1.29863440262772e-09	0.312403100775198\\
1.29949645815272e-09	0.311627906976748\\
1.30810395195541e-09	0.310852713178298\\
1.31745594825695e-09	0.310077519379849\\
1.32200133193424e-09	0.309302325581399\\
1.32535812390281e-09	0.30852713178295\\
1.32881940745018e-09	0.3077519379845\\
1.33298600915436e-09	0.30697674418605\\
1.34425803821614e-09	0.306201550387601\\
1.34855525439381e-09	0.305426356589151\\
1.36199548371545e-09	0.304651162790702\\
1.36319713687151e-09	0.303875968992252\\
1.38348156460378e-09	0.303100775193802\\
1.3846179105231e-09	0.302325581395353\\
1.3971046541883e-09	0.301550387596903\\
1.39988674247353e-09	0.300775193798453\\
1.40204188128604e-09	0.300000000000004\\
1.42257447651793e-09	0.299224806201554\\
1.42615331309143e-09	0.298449612403105\\
1.43963272675511e-09	0.297674418604655\\
1.44136989925247e-09	0.296899224806205\\
1.44221889333012e-09	0.296124031007756\\
1.46238576803626e-09	0.295348837209306\\
1.47505537196433e-09	0.294573643410856\\
1.47547333827948e-09	0.293798449612407\\
1.48281387168936e-09	0.293023255813957\\
1.4860008648424e-09	0.292248062015507\\
1.48703271918293e-09	0.291472868217058\\
1.4953659225913e-09	0.290697674418608\\
1.51406991519439e-09	0.289922480620159\\
1.52199821373495e-09	0.289147286821709\\
1.52984814359142e-09	0.288372093023259\\
1.53505966108348e-09	0.28759689922481\\
1.56963331221505e-09	0.28682170542636\\
1.59840768072386e-09	0.286046511627911\\
1.61592308161824e-09	0.285271317829461\\
1.61614512622317e-09	0.284496124031011\\
1.62029866648e-09	0.283720930232562\\
1.62928494225579e-09	0.282945736434112\\
1.63601158764028e-09	0.282170542635662\\
1.63956430131908e-09	0.281395348837213\\
1.65662255155626e-09	0.280620155038763\\
1.69881102649202e-09	0.279844961240313\\
1.71128470870987e-09	0.279069767441864\\
1.71622193580761e-09	0.278294573643414\\
1.7389880385361e-09	0.277519379844965\\
1.739471312088e-09	0.276744186046515\\
1.74050316642853e-09	0.275968992248065\\
1.74653755510355e-09	0.275193798449616\\
1.74916290602061e-09	0.274418604651166\\
1.76942121085818e-09	0.273643410852717\\
1.78135937373474e-09	0.272868217054267\\
1.78462473557187e-09	0.272093023255817\\
1.78918318069651e-09	0.271317829457368\\
1.79473429581963e-09	0.270542635658918\\
1.81427422105304e-09	0.269767441860468\\
1.81718692381176e-09	0.268992248062019\\
1.82434459695875e-09	0.268217054263569\\
1.82451439577429e-09	0.267441860465119\\
1.84242164008912e-09	0.26666666666667\\
1.84452453311224e-09	0.26589147286822\\
1.84458984034898e-09	0.265116279069771\\
1.85766434914486e-09	0.264341085271321\\
1.87494464398696e-09	0.263565891472871\\
1.884427254762e-09	0.262790697674422\\
1.91723761050151e-09	0.262015503875972\\
1.94368704138228e-09	0.261240310077522\\
1.94453603545994e-09	0.260465116279073\\
1.94686097308798e-09	0.259689922480623\\
1.9479711961126e-09	0.258914728682174\\
1.95138023387057e-09	0.258139534883724\\
1.98494815355629e-09	0.257364341085274\\
1.9866722646063e-09	0.256589147286825\\
1.98925843118131e-09	0.255813953488375\\
1.99015967104836e-09	0.255038759689926\\
1.99717366827452e-09	0.254263565891476\\
2.00363908471204e-09	0.253488372093026\\
2.00585953076129e-09	0.252713178294577\\
2.01566867772004e-09	0.251937984496127\\
2.01642624166625e-09	0.251162790697677\\
2.02106305547498e-09	0.250387596899228\\
2.02858644914774e-09	0.249612403100778\\
2.04373772807203e-09	0.248837209302329\\
2.05208399292775e-09	0.248062015503879\\
2.06080903975656e-09	0.247286821705429\\
2.06173640251831e-09	0.24651162790698\\
2.07215943750244e-09	0.24573643410853\\
2.07257740381759e-09	0.24496124031008\\
2.07312598460623e-09	0.244186046511631\\
2.07332190631646e-09	0.243410852713181\\
2.13290822912046e-09	0.242635658914732\\
2.15687598500501e-09	0.241860465116282\\
2.16114707828798e-09	0.241085271317832\\
2.17159623616681e-09	0.240310077519383\\
2.17257584471795e-09	0.239534883720933\\
2.17623304997553e-09	0.238759689922483\\
2.1774085802369e-09	0.237984496124034\\
2.17948535036532e-09	0.237209302325584\\
2.18602913548693e-09	0.236434108527135\\
2.19723585731197e-09	0.235658914728685\\
2.19863343217827e-09	0.234883720930235\\
2.22277098687835e-09	0.234108527131786\\
2.22454734371775e-09	0.233333333333336\\
2.23194012291702e-09	0.232558139534886\\
2.23302422304695e-09	0.231782945736437\\
2.23472221120226e-09	0.231007751937987\\
2.23682510422537e-09	0.230232558139538\\
2.24698691026253e-09	0.229457364341088\\
2.24967756841633e-09	0.228682170542638\\
2.26613499207548e-09	0.227906976744189\\
2.26758481273116e-09	0.227131782945739\\
2.27066731430542e-09	0.22635658914729\\
2.27568291008725e-09	0.22558139534884\\
2.29976821899794e-09	0.22480620155039\\
2.30872837187904e-09	0.224031007751941\\
2.34057218051476e-09	0.223255813953491\\
2.34432081590378e-09	0.222480620155041\\
2.35649408483261e-09	0.221705426356592\\
2.38046184071717e-09	0.220930232558142\\
2.40158220107974e-09	0.220155038759693\\
2.4064149365987e-09	0.219379844961243\\
2.42348624828323e-09	0.218604651162793\\
2.43419663510903e-09	0.217829457364344\\
2.44488089904013e-09	0.217054263565894\\
2.44891688627082e-09	0.216279069767444\\
2.45506882797198e-09	0.215503875968995\\
2.46274895901292e-09	0.214728682170545\\
2.47426915557432e-09	0.213953488372096\\
2.4833076771395e-09	0.213178294573646\\
2.51050161051915e-09	0.212403100775196\\
2.53453467364044e-09	0.211627906976747\\
2.56286495293941e-09	0.210852713178297\\
2.56622174490798e-09	0.210077519379847\\
2.5776374498906e-09	0.209302325581398\\
2.5927103601308e-09	0.208527131782948\\
2.61183231904905e-09	0.207751937984499\\
2.61379153615133e-09	0.206976744186049\\
2.61486257483391e-09	0.206201550387599\\
2.61960388022143e-09	0.20542635658915\\
2.63320084691125e-09	0.2046511627907\\
2.65434733016852e-09	0.20387596899225\\
2.71045930797781e-09	0.203100775193801\\
2.71377691560434e-09	0.202325581395351\\
2.72332483361612e-09	0.201550387596902\\
2.72580650861234e-09	0.200775193798452\\
2.73069148992069e-09	0.200000000000002\\
2.73391766741577e-09	0.199224806201553\\
2.7581466522473e-09	0.198449612403103\\
2.76049771277003e-09	0.197674418604654\\
2.76338429263406e-09	0.196899224806204\\
2.78445240720724e-09	0.196124031007754\\
2.79313826969401e-09	0.195348837209305\\
2.80049186455124e-09	0.194573643410855\\
2.81828155583994e-09	0.193798449612405\\
2.83135606463582e-09	0.193023255813956\\
2.84141337909419e-09	0.192248062015506\\
2.84221012738245e-09	0.191472868217057\\
2.87082775852308e-09	0.190697674418607\\
2.91331664674785e-09	0.189922480620157\\
2.92179352607705e-09	0.189147286821708\\
2.94593108077713e-09	0.188372093023258\\
2.94644047722373e-09	0.187596899224808\\
3.01809557737777e-09	0.186821705426359\\
3.02329403342248e-09	0.186046511627909\\
3.06895685335295e-09	0.18527131782946\\
3.07088994756053e-09	0.18449612403101\\
3.08039868123026e-09	0.18372093023256\\
3.09233684410682e-09	0.182945736434111\\
3.1130000538122e-09	0.182170542635661\\
3.13780374232706e-09	0.181395348837212\\
3.16775364109724e-09	0.180620155038762\\
3.17590398424272e-09	0.179844961240312\\
3.19318427908483e-09	0.179069767441863\\
3.1983435507875e-09	0.178294573643413\\
3.23807647362173e-09	0.177519379844963\\
3.24830358689563e-09	0.176744186046514\\
3.25581391912104e-09	0.175968992248064\\
3.26499611660705e-09	0.175193798449615\\
3.2939141610367e-09	0.174418604651165\\
3.31443369482125e-09	0.173643410852715\\
3.32246648494059e-09	0.172868217054266\\
3.33803573018004e-09	0.172093023255816\\
3.3401516846505e-09	0.171317829457367\\
3.35417967910283e-09	0.170542635658917\\
3.36187287159111e-09	0.169767441860467\\
3.36566069132218e-09	0.168992248062018\\
3.38006746774761e-09	0.168217054263568\\
3.38523980089763e-09	0.167441860465118\\
3.43995420384063e-09	0.166666666666669\\
3.46481013814489e-09	0.165891472868219\\
3.47966100378017e-09	0.16511627906977\\
3.54370128013001e-09	0.16434108527132\\
3.56864864456571e-09	0.16356589147287\\
3.56883150482859e-09	0.162790697674421\\
3.57372954758429e-09	0.162015503875971\\
3.57392546929452e-09	0.161240310077521\\
3.58103089665212e-09	0.160465116279072\\
3.58259827033394e-09	0.159689922480622\\
3.58366930901652e-09	0.158914728682173\\
3.60388842951205e-09	0.158139534883723\\
3.6523202762804e-09	0.157364341085273\\
3.70546730554157e-09	0.156589147286824\\
3.71092699053326e-09	0.155813953488374\\
3.71582503328896e-09	0.155038759689925\\
3.72931750839999e-09	0.154263565891475\\
3.74781251784551e-09	0.153488372093025\\
3.7608086579573e-09	0.152713178294576\\
3.78452824634223e-09	0.151937984496126\\
3.80141669776388e-09	0.151162790697676\\
3.84287373164812e-09	0.150387596899227\\
3.85790745754628e-09	0.149612403100777\\
3.85836460820348e-09	0.148837209302328\\
3.94364279794204e-09	0.148062015503878\\
3.94740449477842e-09	0.147286821705428\\
4.00547568968999e-09	0.146511627906979\\
4.03492925346093e-09	0.145736434108529\\
4.03647050424805e-09	0.14496124031008\\
4.0547042847466e-09	0.14418604651163\\
4.10030179744033e-09	0.14341085271318\\
4.15867340564091e-09	0.142635658914731\\
4.16758131273261e-09	0.141860465116281\\
4.18138726258001e-09	0.141085271317831\\
4.18486160757472e-09	0.140310077519382\\
4.28569598110538e-09	0.139534883720932\\
4.29291896148912e-09	0.138759689922483\\
4.44036964060668e-09	0.137984496124033\\
4.4504922623018e-09	0.137209302325583\\
4.52795970652594e-09	0.136434108527134\\
4.53101608520549e-09	0.135658914728684\\
4.53557453033013e-09	0.134883720930234\\
4.54008072966537e-09	0.134108527131785\\
4.60971130548039e-09	0.133333333333335\\
4.63438437952177e-09	0.132558139534886\\
4.66373345171392e-09	0.131782945736436\\
4.71836948597282e-09	0.131007751937986\\
4.71942746320805e-09	0.130232558139537\\
4.74165804659526e-09	0.129457364341087\\
4.75035697052938e-09	0.128682170542637\\
4.80385665886896e-09	0.127906976744188\\
4.83709804237097e-09	0.127131782945738\\
4.83873072328954e-09	0.126356589147289\\
4.87271660929042e-09	0.125581395348839\\
4.8791428413859e-09	0.124806201550389\\
4.93315192617207e-09	0.12403100775194\\
4.95079794153994e-09	0.12325581395349\\
4.99229415976622e-09	0.12248062015504\\
5.01362350328637e-09	0.121705426356591\\
5.03146544036447e-09	0.120930232558141\\
5.05496298414447e-09	0.120155038759692\\
5.12698380482428e-09	0.119379844961242\\
5.23621668900004e-09	0.118604651162792\\
5.23828039768111e-09	0.117829457364343\\
5.24255149096408e-09	0.117054263565893\\
5.29987818337678e-09	0.116279069767444\\
5.3321791426697e-09	0.115503875968994\\
5.33365508622009e-09	0.114728682170544\\
5.35007332553719e-09	0.113953488372095\\
5.39544879362599e-09	0.113178294573645\\
5.40690368295065e-09	0.112403100775195\\
5.45031993393717e-09	0.111627906976746\\
5.45729474682128e-09	0.110852713178296\\
5.45920171813417e-09	0.110077519379846\\
5.57236609796184e-09	0.109302325581397\\
5.57576207427246e-09	0.108527131782947\\
5.60859855290667e-09	0.107751937984498\\
5.61046633987751e-09	0.106976744186048\\
5.62317512814763e-09	0.106201550387598\\
5.63285366063289e-09	0.105426356589149\\
5.69152568212249e-09	0.104651162790699\\
5.76152197846327e-09	0.103875968992249\\
5.82626757296994e-09	0.1031007751938\\
5.8542190702958e-09	0.10232558139535\\
5.87961052394134e-09	0.101550387596901\\
5.92787257189417e-09	0.100775193798451\\
5.940907896348e-09	0.100000000000001\\
5.97764974773942e-09	0.0992248062015518\\
6.14466647498509e-09	0.0984496124031022\\
6.25823575968057e-09	0.0976744186046525\\
6.37190953595483e-09	0.0968992248062029\\
6.38622488224883e-09	0.0961240310077534\\
6.40618277379738e-09	0.0953488372093036\\
6.42773416192246e-09	0.0945736434108541\\
6.44949453320511e-09	0.0937984496124045\\
6.45575096648506e-09	0.0930232558139549\\
6.47753746066241e-09	0.0922480620155052\\
6.5064685665394e-09	0.0914728682170556\\
6.54266183714218e-09	0.090697674418606\\
6.5909500079897e-09	0.0899224806201564\\
6.64968733671605e-09	0.0891472868217067\\
6.69821061361584e-09	0.0883720930232571\\
6.76410561548918e-09	0.0875968992248075\\
6.78513454572032e-09	0.0868217054263579\\
6.88573381319871e-09	0.0860465116279082\\
6.93211501273334e-09	0.0852713178294586\\
6.94286458390118e-09	0.084496124031009\\
6.95704931572169e-09	0.0837209302325594\\
7.00059618118169e-09	0.0829457364341097\\
7.00873346287982e-09	0.0821705426356601\\
7.24052190752686e-09	0.0813953488372106\\
7.31938692661729e-09	0.0806201550387609\\
7.36004721221327e-09	0.0798449612403113\\
7.42177561238243e-09	0.0790697674418617\\
7.44495968142607e-09	0.0782945736434121\\
7.45188224852079e-09	0.0775193798449625\\
7.59935905053306e-09	0.0767441860465128\\
7.6252337777305e-09	0.0759689922480632\\
7.63906585047259e-09	0.0751937984496136\\
7.7021787640607e-09	0.0744186046511639\\
7.78009029749469e-09	0.0736434108527143\\
7.79618200062808e-09	0.0728682170542647\\
7.81365821718041e-09	0.0720930232558151\\
7.81764195862171e-09	0.0713178294573654\\
8.2015048347477e-09	0.0705426356589158\\
8.38188342263092e-09	0.0697674418604662\\
8.40352624088743e-09	0.0689922480620166\\
8.57952924390889e-09	0.0682170542635669\\
8.63421752395719e-09	0.0674418604651174\\
8.68118648862251e-09	0.0666666666666678\\
8.73754663393142e-09	0.0658914728682181\\
8.8978105928979e-09	0.0651162790697685\\
8.91897013760252e-09	0.0643410852713189\\
8.93721697954842e-09	0.0635658914728692\\
9.04767763977495e-09	0.0627906976744196\\
9.25825429392797e-09	0.06201550387597\\
9.28388085362579e-09	0.0612403100775204\\
9.3904883868845e-09	0.0604651162790707\\
9.47357225346851e-09	0.0596899224806211\\
9.48688186831666e-09	0.0589147286821715\\
9.49888533842996e-09	0.0581395348837219\\
9.50627811762923e-09	0.0573643410852722\\
9.6981377177318e-09	0.0565891472868226\\
9.76425476421007e-09	0.055813953488373\\
9.87201170483545e-09	0.0550387596899233\\
9.88219963376731e-09	0.0542635658914737\\
9.90173955900071e-09	0.0534883720930242\\
9.9454431618289e-09	0.0527131782945746\\
1.00439134133895e-08	0.0519379844961249\\
1.0132300227597e-08	0.0511627906976753\\
1.02176176016776e-08	0.0503875968992257\\
1.02786929294793e-08	0.049612403100776\\
1.03181646233666e-08	0.0488372093023264\\
1.05206039958215e-08	0.0480620155038768\\
1.05319152092253e-08	0.0472868217054272\\
1.06498992631246e-08	0.0465116279069775\\
1.06751992866387e-08	0.0457364341085279\\
1.15449349426827e-08	0.0449612403100783\\
1.15819249615737e-08	0.0441860465116286\\
1.1713101077295e-08	0.043410852713179\\
1.17610104661694e-08	0.0426356589147294\\
1.17774548283812e-08	0.0418604651162797\\
1.19207650286893e-08	0.0410852713178301\\
1.19827285349108e-08	0.0403100775193805\\
1.2192900284196e-08	0.0395348837209308\\
1.22258020700669e-08	0.0387596899224812\\
1.24142526324115e-08	0.0379844961240317\\
1.25652429637606e-08	0.0372093023255819\\
1.27232864766778e-08	0.0364341085271324\\
1.30535843572274e-08	0.0356589147286828\\
1.30602718182699e-08	0.0348837209302332\\
1.35423306555621e-08	0.0341085271317835\\
1.3642198481989e-08	0.0333333333333339\\
1.37277901464639e-08	0.0325581395348843\\
1.45266805120895e-08	0.0317829457364346\\
1.45269548024838e-08	0.031007751937985\\
1.47271084216527e-08	0.0302325581395354\\
1.50985106770082e-08	0.0294573643410857\\
1.54212851638851e-08	0.0286821705426361\\
1.54403287541192e-08	0.0279069767441865\\
1.55033110532339e-08	0.0271317829457369\\
1.55603373323576e-08	0.0263565891472872\\
1.61069980882356e-08	0.0255813953488376\\
1.62248907120035e-08	0.024806201550388\\
1.64127796321121e-08	0.0240310077519383\\
1.75731847374503e-08	0.0232558139534887\\
1.82258522000091e-08	0.0224806201550392\\
1.90393844481123e-08	0.0217054263565895\\
1.91908188686712e-08	0.0209302325581399\\
1.94013824613769e-08	0.0201550387596903\\
1.9922037875584e-08	0.0193798449612407\\
2.33107258985817e-08	0.018604651162791\\
2.35666257750341e-08	0.0178294573643414\\
2.42255627323202e-08	0.0170542635658918\\
2.57000695234959e-08	0.0162790697674421\\
2.57203800741228e-08	0.0155038759689925\\
2.57487756606585e-08	0.0147286821705429\\
3.24560509187343e-08	0.0139534883720932\\
3.55702656871499e-08	0.0131782945736436\\
4.42779930367846e-08	0.012403100775194\\
5.2743952995998e-08	0.0116279069767444\\
6.09705227482075e-08	0.0108527131782947\\
7.68518843334973e-08	0.0100775193798451\\
1.12917544595682e-07	0.00930232558139554\\
1.698012854506e-06	0.00852713178294584\\
2.80609112416929e-06	0.00775193798449625\\
3.49254616469227e-05	0.00697674418604666\\
0.000151487820379385	0.00620155038759695\\
0.000256810698497661	0.00542635658914736\\
0.000341239733398273	0.00465116279069777\\
0.000386135043573641	0.00387596899224818\\
0.000618118073274629	0.00310077519379848\\
0.004059450447817	0.00232558139534889\\
0.00466525552684652	0.00155038759689929\\
0.0117928782360303	0.000775193798449592\\
0.0141262953617481	0\\
};
\addlegendentry{$K=20$, $G=\;\,5$, $\lrmse =0.001$, $\prmse =0.001$, $\gamma \rightarrow \infty$}


==> figures/alpha_N_2_K_20_G_5_SNR_40_I_20_Pratio_2_Nratio_1_cs.tex <==
\addplot [color=blue, dashed,line width=0.6pt]
  table[row sep=crcr]{%
0.000291964610435948	1\\
0.000291964610435948	0.997787610619469\\
0.000534001838578056	0.995575221238938\\
0.00166107867596691	0.993362831858407\\
0.00237399868620885	0.991150442477876\\
0.00309731094788928	0.988938053097345\\
0.00365333579994556	0.986725663716814\\
0.00442611228639442	0.984513274336283\\
0.00497152372609258	0.982300884955752\\
0.00574451999843027	0.980088495575221\\
0.00584935837130217	0.97787610619469\\
0.00619626263354643	0.975663716814159\\
0.00696647627569249	0.973451327433628\\
0.00747265212051302	0.971238938053097\\
0.00750015975002056	0.969026548672566\\
0.00753519385666897	0.966814159292036\\
0.00762215488795991	0.964601769911505\\
0.00779891570216772	0.962389380530974\\
0.00824253531833359	0.960176991150443\\
0.00841965940456824	0.957964601769911\\
0.00995944694622242	0.955752212389381\\
0.0119603915464427	0.95353982300885\\
0.0119801411847335	0.951327433628319\\
0.0121282833559826	0.949115044247788\\
0.0124436873524716	0.946902654867257\\
0.0135498385009271	0.944690265486726\\
0.0135875791763878	0.942477876106195\\
0.013956634886798	0.940265486725664\\
0.013959434636498	0.938053097345133\\
0.0142179380163372	0.935840707964602\\
0.0142697057835082	0.933628318584071\\
0.01445248354642	0.93141592920354\\
0.0146040698337333	0.929203539823009\\
0.0148007712531474	0.926991150442478\\
0.0151036477783669	0.924778761061947\\
0.0151347227168194	0.922566371681416\\
0.0155876365753936	0.920353982300885\\
0.015627560528622	0.918141592920354\\
0.0169831438192864	0.915929203539823\\
0.0170768442560163	0.913716814159292\\
0.0173474919231045	0.911504424778761\\
0.0178867017269833	0.90929203539823\\
0.0184533283304249	0.907079646017699\\
0.0191230574785513	0.904867256637168\\
0.0191865679552591	0.902654867256637\\
0.0193763269120945	0.900442477876107\\
0.0196321972498486	0.898230088495576\\
0.0196860123561675	0.896017699115045\\
0.0205464220311783	0.893805309734514\\
0.0208321831048059	0.891592920353983\\
0.0211157370658622	0.889380530973452\\
0.0213043058243003	0.887168141592921\\
0.0219367391911137	0.88495575221239\\
0.0224096574063036	0.882743362831859\\
0.0226701605928029	0.880530973451328\\
0.0228091477090242	0.878318584070797\\
0.0242163042836196	0.876106194690266\\
0.024958638817724	0.873893805309735\\
0.0251542618464802	0.871681415929204\\
0.0254902989400955	0.869469026548673\\
0.0264884693318358	0.867256637168142\\
0.0267178361368228	0.865044247787611\\
0.0270943287246606	0.86283185840708\\
0.0271195474122825	0.860619469026549\\
0.0278211837085612	0.858407079646018\\
0.0281768192899633	0.856194690265487\\
0.0291017253013112	0.853982300884957\\
0.0306710084830656	0.851769911504425\\
0.0310572105536246	0.849557522123895\\
0.0311110137593584	0.847345132743364\\
0.0317871743202858	0.845132743362833\\
0.0318858215348004	0.842920353982302\\
0.0320355352287524	0.840707964601771\\
0.0323368358012179	0.83849557522124\\
0.0333337681975266	0.836283185840709\\
0.0334226633448483	0.834070796460178\\
0.0335465910197939	0.831858407079647\\
0.0340125610102562	0.829646017699116\\
0.0359650420822533	0.827433628318585\\
0.0364152224598696	0.825221238938054\\
0.0368678465540483	0.823008849557523\\
0.0368771193938515	0.820796460176992\\
0.0372369408147196	0.818584070796461\\
0.0378614438296023	0.81637168141593\\
0.0384322886106419	0.814159292035399\\
0.0387264261595737	0.811946902654868\\
0.0389236077223638	0.809734513274337\\
0.0401742947801389	0.807522123893806\\
0.0402349661036857	0.805309734513275\\
0.0402419395996363	0.803097345132744\\
0.0403114106854485	0.800884955752213\\
0.0424288492626826	0.798672566371682\\
0.043246181869193	0.796460176991151\\
0.0439392434097819	0.79424778761062\\
0.0443628497380973	0.792035398230089\\
0.0445657909408942	0.789823008849558\\
0.0450870234541365	0.787610619469027\\
0.0456394463244734	0.785398230088496\\
0.0456509574679628	0.783185840707965\\
0.0457856844585201	0.780973451327434\\
0.0460321405415259	0.778761061946903\\
0.0460787678967446	0.776548672566372\\
0.0462548618519138	0.774336283185841\\
0.0463002890882002	0.77212389380531\\
0.0465943776659388	0.76991150442478\\
0.0471510604519116	0.767699115044248\\
0.0473672352217481	0.765486725663717\\
0.047631507903434	0.763274336283186\\
0.047788252831151	0.761061946902655\\
0.0478227547138352	0.758849557522124\\
0.0484851755295909	0.756637168141594\\
0.0488006047218208	0.754424778761063\\
0.0497354876088211	0.752212389380532\\
0.0498438546343833	0.750000000000001\\
0.0517950524852171	0.74778761061947\\
0.0519087889714462	0.745575221238939\\
0.0527166815694561	0.743362831858408\\
0.0529737177174821	0.741150442477877\\
0.0533111425050049	0.738938053097346\\
0.0538600773840864	0.736725663716815\\
0.0547907797787945	0.734513274336284\\
0.0554711408967091	0.732300884955753\\
0.0555163078172396	0.730088495575222\\
0.0556047379730911	0.727876106194691\\
0.0561646580563699	0.72566371681416\\
0.0562034299476753	0.723451327433629\\
0.0563426180974001	0.721238938053098\\
0.0566103254320794	0.719026548672567\\
0.0568595439508033	0.716814159292036\\
0.0580133357962149	0.714601769911505\\
0.0581956977418768	0.712389380530974\\
0.0592743646925912	0.710176991150443\\
0.0593198061934017	0.707964601769912\\
0.0593917387211269	0.705752212389381\\
0.0598505513557047	0.70353982300885\\
0.0605483147159201	0.701327433628319\\
0.0609599545830149	0.699115044247788\\
0.0610653427529313	0.696902654867257\\
0.0617352349354933	0.694690265486726\\
0.0621187011846135	0.692477876106195\\
0.0624918086343469	0.690265486725664\\
0.0629197248990308	0.688053097345133\\
0.0633316560496197	0.685840707964602\\
0.0639754346736505	0.683628318584071\\
0.0642167148658684	0.681415929203541\\
0.0647366229850654	0.67920353982301\\
0.0649419315845853	0.676991150442479\\
0.0654653066608697	0.674778761061948\\
0.0654806916412966	0.672566371681417\\
0.0662645950516114	0.670353982300886\\
0.0678260316258584	0.668141592920355\\
0.0678744776926375	0.665929203539824\\
0.0681678328480598	0.663716814159293\\
0.0683557370306656	0.661504424778762\\
0.0684105215963862	0.659292035398231\\
0.0686558772751536	0.6570796460177\\
0.0701436244338115	0.654867256637169\\
0.0702043596579294	0.652654867256638\\
0.0702842332880577	0.650442477876107\\
0.0711934798532605	0.648230088495576\\
0.0712662882768774	0.646017699115045\\
0.0715631067490181	0.643805309734514\\
0.0716987938859039	0.641592920353983\\
0.0717544944130749	0.639380530973452\\
0.0718640032818192	0.637168141592921\\
0.0720601490071673	0.63495575221239\\
0.0721060966825703	0.632743362831859\\
0.0724368295293138	0.630530973451328\\
0.072650201457257	0.628318584070797\\
0.0732431076363906	0.626106194690266\\
0.0732623657531912	0.623893805309735\\
0.0745360427059867	0.621681415929204\\
0.0746335913399284	0.619469026548673\\
0.0757137903742009	0.617256637168142\\
0.0766152418482821	0.615044247787611\\
0.0770128163575833	0.61283185840708\\
0.077450766189016	0.610619469026549\\
0.0775214066973346	0.608407079646018\\
0.078571188174402	0.606194690265487\\
0.0786391592019797	0.603982300884956\\
0.0787995705108431	0.601769911504425\\
0.0791039019937986	0.599557522123894\\
0.0794441795269427	0.597345132743363\\
0.0794782342452691	0.595132743362833\\
0.0796106920307411	0.592920353982301\\
0.0806139867269132	0.590707964601771\\
0.080652830556517	0.58849557522124\\
0.0806605023939046	0.586283185840708\\
0.0808278491809207	0.584070796460178\\
0.0819411837907706	0.581858407079647\\
0.0820366742714698	0.579646017699116\\
0.0821062652021087	0.577433628318585\\
0.0826558284981166	0.575221238938054\\
0.0836044944859344	0.573008849557523\\
0.084645261142321	0.570796460176992\\
0.0853812303994009	0.568584070796461\\
0.0862699184571844	0.56637168141593\\
0.0864682192470124	0.564159292035399\\
0.0868924506401643	0.561946902654868\\
0.0869958070425552	0.559734513274337\\
0.0896656878225181	0.557522123893806\\
0.089668506319196	0.555309734513275\\
0.0898848053122916	0.553097345132744\\
0.089996929149526	0.550884955752213\\
0.0903551864316278	0.548672566371682\\
0.0905388692815123	0.546460176991151\\
0.0909067327645599	0.54424778761062\\
0.0924557243541823	0.542035398230089\\
0.0929284915815748	0.539823008849558\\
0.0934074548794736	0.537610619469027\\
0.0937293529425281	0.535398230088497\\
0.0938567457850906	0.533185840707966\\
0.0939083921704681	0.530973451327435\\
0.0943804323709643	0.528761061946904\\
0.0944379584966312	0.526548672566373\\
0.094633763215632	0.524336283185842\\
0.0948728484273912	0.522123893805311\\
0.0953520566736914	0.51991150442478\\
0.0957390857637881	0.517699115044249\\
0.0958297246502368	0.515486725663718\\
0.0958443782921576	0.513274336283187\\
0.0960048342493453	0.511061946902656\\
0.0964239058476705	0.508849557522125\\
0.0967383036031735	0.506637168141594\\
0.0983323147457834	0.504424778761063\\
0.0988819786590313	0.502212389380532\\
0.0996621955205282	0.500000000000001\\
0.100383765450805	0.49778761061947\\
0.100726884043272	0.495575221238939\\
0.101070876498825	0.493362831858408\\
0.101420936846057	0.491150442477877\\
0.101702806212767	0.488938053097346\\
0.101926050650801	0.486725663716815\\
0.102307276335521	0.484513274336285\\
0.103041789955225	0.482300884955754\\
0.103590948614425	0.480088495575222\\
0.103701955842214	0.477876106194692\\
0.104110110807752	0.475663716814161\\
0.104663280855912	0.47345132743363\\
0.105204468758508	0.471238938053099\\
0.105941466878426	0.469026548672568\\
0.106231327803349	0.466814159292037\\
0.106688648467745	0.464601769911506\\
0.107020623983868	0.462389380530975\\
0.107152253059795	0.460176991150444\\
0.107646209482801	0.457964601769913\\
0.108967431982586	0.455752212389382\\
0.109147717127033	0.453539823008851\\
0.109491430801497	0.45132743362832\\
0.109711552442882	0.449115044247789\\
0.111492435946071	0.446902654867258\\
0.111981938662706	0.444690265486727\\
0.112437422624143	0.442477876106196\\
0.112705035948715	0.440265486725665\\
0.113588849570898	0.438053097345134\\
0.113659115297991	0.435840707964603\\
0.114970284521434	0.433628318584072\\
0.115660651526932	0.431415929203541\\
0.118157719506798	0.42920353982301\\
0.118559371737894	0.426991150442479\\
0.118851366976954	0.424778761061948\\
0.119055920775115	0.422566371681417\\
0.119258440751982	0.420353982300886\\
0.120415395811163	0.418141592920355\\
0.121418747277427	0.415929203539824\\
0.121543170575679	0.413716814159293\\
0.121551219561928	0.411504424778762\\
0.12318714049035	0.409292035398231\\
0.123202035183998	0.4070796460177\\
0.123911591907402	0.404867256637169\\
0.124171530114191	0.402654867256638\\
0.124721581579482	0.400442477876107\\
0.125787079853903	0.398230088495576\\
0.125851714312459	0.396017699115045\\
0.126064002692197	0.393805309734514\\
0.126306835709133	0.391592920353983\\
0.127306667957487	0.389380530973452\\
0.128301223494067	0.387168141592921\\
0.128428912515593	0.384955752212391\\
0.12877029409183	0.38274336283186\\
0.128890078354965	0.380530973451328\\
0.129110788468236	0.378318584070798\\
0.129755519173282	0.376106194690267\\
0.13291427091885	0.373893805309736\\
0.132925813982884	0.371681415929205\\
0.134140567217213	0.369469026548674\\
0.135457407211881	0.367256637168143\\
0.135599807994641	0.365044247787612\\
0.135964652703099	0.362831858407081\\
0.136047332235836	0.36061946902655\\
0.136338759441223	0.358407079646019\\
0.136755290510885	0.356194690265488\\
0.137745438911893	0.353982300884957\\
0.137929131308442	0.351769911504426\\
0.138197758505073	0.349557522123895\\
0.138300182154843	0.347345132743364\\
0.138369126096392	0.345132743362833\\
0.139811367885264	0.342920353982302\\
0.140846156591229	0.340707964601771\\
0.140879957736523	0.33849557522124\\
0.140923328790696	0.336283185840709\\
0.142389710103647	0.334070796460178\\
0.143046852030652	0.331858407079647\\
0.143102414565473	0.329646017699116\\
0.145216824205201	0.327433628318585\\
0.145585028899164	0.325221238938054\\
0.147045010909158	0.323008849557523\\
0.147174652344001	0.320796460176992\\
0.147424173555706	0.318584070796461\\
0.149149190006591	0.31637168141593\\
0.149893185397363	0.314159292035399\\
0.149999098878329	0.311946902654868\\
0.150039814229851	0.309734513274337\\
0.150457370366851	0.307522123893806\\
0.151989383953862	0.305309734513275\\
0.152793039551931	0.303097345132744\\
0.155570240393503	0.300884955752213\\
0.15679935885561	0.298672566371682\\
0.157473421846564	0.296460176991151\\
0.158325686576934	0.29424778761062\\
0.158535237446937	0.292035398230089\\
0.158631433721334	0.289823008849558\\
0.160170301906894	0.287610619469028\\
0.161531328124856	0.285398230088497\\
0.162639496795984	0.283185840707965\\
0.163306533105478	0.280973451327435\\
0.164058934317479	0.278761061946904\\
0.16447654484855	0.276548672566373\\
0.165051014827418	0.274336283185842\\
0.165794089116551	0.272123893805311\\
0.16714923984856	0.26991150442478\\
0.167932818742827	0.267699115044249\\
0.169962758817095	0.265486725663718\\
0.170194343886268	0.263274336283187\\
0.171223970008082	0.261061946902656\\
0.171876898350468	0.258849557522125\\
0.171927334083117	0.256637168141594\\
0.172959056719396	0.254424778761063\\
0.173540484574643	0.252212389380532\\
0.174319287532323	0.250000000000001\\
0.174637816856808	0.24778761061947\\
0.174891082940403	0.245575221238939\\
0.174985651417544	0.243362831858408\\
0.176134436145634	0.241150442477877\\
0.176770414049386	0.238938053097346\\
0.178575863343166	0.236725663716815\\
0.181250682529989	0.234513274336284\\
0.188393406144483	0.232300884955753\\
0.189392978197155	0.230088495575222\\
0.191331590661164	0.227876106194691\\
0.191946435961249	0.22566371681416\\
0.192563241437016	0.223451327433629\\
0.1939852059412	0.221238938053098\\
0.194385445368696	0.219026548672567\\
0.197143460065464	0.216814159292036\\
0.198085757151327	0.214601769911505\\
0.198496904805498	0.212389380530974\\
0.200353205153769	0.210176991150443\\
0.201718345201035	0.207964601769912\\
0.202553539716439	0.205752212389381\\
0.204629835506744	0.20353982300885\\
0.204733921670641	0.201327433628319\\
0.205422460427109	0.199115044247788\\
0.205981567420635	0.196902654867257\\
0.206284795282606	0.194690265486726\\
0.206298093202142	0.192477876106195\\
0.206635598820563	0.190265486725664\\
0.208253537891922	0.188053097345134\\
0.208325166004109	0.185840707964603\\
0.21092423608273	0.183628318584071\\
0.212241357340829	0.181415929203541\\
0.215899322462184	0.17920353982301\\
0.216829837716014	0.176991150442479\\
0.220177017134929	0.174778761061948\\
0.223740832647012	0.172566371681417\\
0.225991536426231	0.170353982300886\\
0.226727631528201	0.168141592920355\\
0.228282360031068	0.165929203539824\\
0.229266906934223	0.163716814159293\\
0.231410947830158	0.161504424778762\\
0.233209298778942	0.159292035398231\\
0.235073844120059	0.1570796460177\\
0.236575974049626	0.154867256637169\\
0.237533554648088	0.152654867256638\\
0.237558185290829	0.150442477876107\\
0.238866678611557	0.148230088495576\\
0.240714350485475	0.146017699115045\\
0.245477022209392	0.143805309734514\\
0.245641262196819	0.141592920353983\\
0.247696569456916	0.139380530973452\\
0.248422018856148	0.137168141592921\\
0.2507601177069	0.13495575221239\\
0.254364158306257	0.132743362831859\\
0.257317885515901	0.130530973451328\\
0.262934346327182	0.128318584070797\\
0.266978454543827	0.126106194690266\\
0.267508567467424	0.123893805309735\\
0.26871062454884	0.121681415929204\\
0.272912575869497	0.119469026548673\\
0.273013955350372	0.117256637168142\\
0.273325552200525	0.115044247787611\\
0.275700518587764	0.11283185840708\\
0.277176917455853	0.110619469026549\\
0.278371739476156	0.108407079646018\\
0.27852576564506	0.106194690265487\\
0.28119216008898	0.103982300884956\\
0.281196930999287	0.101769911504425\\
0.284522858798966	0.0995575221238942\\
0.284991972643991	0.0973451327433632\\
0.28512578630204	0.0951327433628323\\
0.286769181155758	0.0929203539823013\\
0.287548093382044	0.0907079646017703\\
0.29305243607336	0.0884955752212393\\
0.294155374008212	0.0862831858407083\\
0.298495716747965	0.0840707964601773\\
0.298982059858494	0.0818584070796463\\
0.301039897228269	0.0796460176991154\\
0.304240371289595	0.0774336283185844\\
0.304308638963736	0.0752212389380534\\
0.305876860849054	0.0730088495575224\\
0.313107696247353	0.0707964601769915\\
0.325087800536724	0.0685840707964605\\
0.33816016993819	0.0663716814159295\\
0.339632590242592	0.0641592920353985\\
0.343237376420215	0.0619469026548676\\
0.345034129274009	0.0597345132743365\\
0.345715032176044	0.0575221238938056\\
0.347382606891809	0.0553097345132746\\
0.348749668741217	0.0530973451327437\\
0.350338317005699	0.0508849557522126\\
0.352819652062248	0.0486725663716816\\
0.355339940018815	0.0464601769911507\\
0.355907751609293	0.0442477876106196\\
0.356131294872226	0.0420353982300887\\
0.357668842515378	0.0398230088495577\\
0.358029073890892	0.0376106194690268\\
0.358235382843519	0.0353982300884957\\
0.360085440485374	0.0331858407079647\\
0.36029423224165	0.0309734513274338\\
0.363737250626949	0.0287610619469028\\
0.364808961156198	0.0265486725663718\\
0.367425756615277	0.0243362831858408\\
0.375971282081353	0.0221238938053099\\
0.378846368934352	0.0199115044247788\\
0.385612480895728	0.0176991150442478\\
0.388869758553051	0.0154867256637169\\
0.393584247177105	0.0132743362831859\\
0.399498982639246	0.0110619469026549\\
0.426960976715717	0.00884955752212391\\
0.451979788976728	0.00663716814159299\\
0.881349932404597	0.00442477876106195\\
1.0558012434278	0.00221238938053103\\
1.06114252844253	0\\
};
\addlegendentry{$K=20$, $G=\;\,5$, $\lrmse =0.297$, $\prmse =0.025$, $\gamma=40$}


==> figures/mse_N_1_K_20_G_5_SNR_1000_I_20_Pratio_2_Nratio_2_alpha_2_cs.tex <==
\addplot [color=red,line width=0.1pt]
  table[row sep=crcr]{%
0	1\\
4.54747350886464e-13	0.863\\
6.9153003668114e-13	0.7522\\
9.09494701772928e-13	0.6756\\
1.07251948202891e-12	0.6038\\
1.22444471506572e-12	0.5622\\
1.36897080878865e-12	0.5132\\
1.48229501182928e-12	0.475\\
1.60777467769219e-12	0.447000000000001\\
1.731626322422e-12	0.410400000000001\\
1.83314517660132e-12	0.382400000000001\\
1.93601708428178e-12	0.358200000000001\\
2.03369197834017e-12	0.3412\\
2.13598175697097e-12	0.322000000000001\\
2.23359196574944e-12	0.301800000000001\\
2.29917400431039e-12	0.291400000000001\\
2.3982264690095e-12	0.2762\\
2.4829580147345e-12	0.264\\
2.56489196833138e-12	0.2524\\
2.65160992732731e-12	0.2432\\
2.7379416175773e-12	0.2346\\
2.8239224658078e-12	0.2258\\
2.9118037843695e-12	0.2132\\
3.00141864100717e-12	0.2054\\
3.07795434552665e-12	0.1966\\
3.15877605077044e-12	0.189\\
3.21956628306595e-12	0.1844\\
3.29887782949002e-12	0.178600000000001\\
3.36674313415662e-12	0.1694\\
3.44078806629604e-12	0.1652\\
3.55169034988042e-12	0.1568\\
3.63264582771773e-12	0.152\\
3.71183607906335e-12	0.1458\\
3.78425215264843e-12	0.1394\\
3.87203416856355e-12	0.1346\\
3.95950218427697e-12	0.1308\\
4.04827319806938e-12	0.1258\\
4.11948143027836e-12	0.1222\\
4.207949023867e-12	0.119\\
4.29760306620569e-12	0.115\\
4.3750972974735e-12	0.1118\\
4.45704603951359e-12	0.1068\\
4.57298150675314e-12	0.1034\\
4.67776785886621e-12	0.0996000000000001\\
4.78701241978054e-12	0.0964\\
4.92147155953566e-12	0.0930000000000001\\
5.03313086055156e-12	0.0906\\
5.10958785849749e-12	0.0878\\
5.16743883843606e-12	0.0852000000000001\\
5.28490968425533e-12	0.0826\\
5.39264020773381e-12	0.0796\\
5.48649427947278e-12	0.0772\\
5.61571552463123e-12	0.0746000000000001\\
5.74540480033342e-12	0.0724\\
5.82582650864377e-12	0.0696\\
5.95745064246053e-12	0.0674\\
6.0936569221928e-12	0.0646\\
6.25277607468888e-12	0.0626\\
6.36747789255444e-12	0.0601999999999999\\
6.48413753497116e-12	0.0579999999999999\\
6.6911247675135e-12	0.0554\\
6.83635170315616e-12	0.0529999999999999\\
7.00997134548197e-12	0.0509999999999999\\
7.19916906700181e-12	0.0484\\
7.41844728557928e-12	0.0464\\
7.62634491877562e-12	0.0444\\
7.91083960262531e-12	0.0422\\
8.13873899873917e-12	0.04\\
8.36197411828529e-12	0.0378000000000001\\
8.77232274609033e-12	0.0356000000000001\\
9.35415411309996e-12	0.0336000000000001\\
9.78301496532636e-12	0.0316000000000001\\
1.02419159061858e-11	0.0296000000000001\\
1.09906423300408e-11	0.0274000000000001\\
1.20148217459759e-11	0.0254000000000001\\
1.28993236293175e-11	0.0234000000000001\\
1.46342827111139e-11	0.0214000000000001\\
1.66841002400838e-11	0.0194000000000001\\
1.84810185001253e-11	0.0174000000000001\\
2.0857119983844e-11	0.0154000000000001\\
2.63951850840235e-11	0.0134000000000001\\
1.79748525876163e-10	0.0114000000000001\\
1.63759016406385e-07	0.00940000000000007\\
3.2597931160879e-07	0.00740000000000007\\
9.48591813510358e-07	0.00540000000000007\\
2.09537673069437e-06	0.00340000000000007\\
0.00315878290745627	0.00139999999999996\\
};
\addlegendentry{$N=1$,~, $\lrmse =5.493$, $\prmse =0.003$, $\gamma \rightarrow \infty$}


==> figures/mse_N_1_K_20_G_5_SNR_1000_I_20_Pratio_2_Nratio_2_alpha_3.4_cs.tex <==
\addplot [color=red,line width=0.6pt]
  table[row sep=crcr]{%
4.90625200475339e-09	1\\
8.58481777489609e-09	0.99899879855827\\
1.15308078910689e-08	0.99799759711654\\
1.36352797164578e-08	0.99699639567481\\
1.45359485089858e-08	0.99599519423308\\
1.5845034307008e-08	0.99499399279135\\
1.63358478627729e-08	0.99399279134962\\
2.04010422244924e-08	0.99299158990789\\
2.21465717447851e-08	0.99199038846616\\
2.43887073628345e-08	0.99098918702443\\
2.54729922146118e-08	0.9899879855827\\
2.74019007915865e-08	0.98898678414097\\
2.86313880840734e-08	0.98798558269924\\
2.95623386656453e-08	0.98698438125751\\
3.01125924851509e-08	0.985983179815779\\
3.078647217145e-08	0.984981978374049\\
3.12362512562464e-08	0.983980776932319\\
3.16100701370568e-08	0.982979575490589\\
3.26928817635394e-08	0.981978374048859\\
3.36975968219353e-08	0.980977172607129\\
3.4308582322339e-08	0.979975971165399\\
3.47256285064212e-08	0.978974769723669\\
3.59720795899486e-08	0.977973568281939\\
3.6438707975859e-08	0.976972366840209\\
3.74258747412957e-08	0.975971165398479\\
3.80683889017908e-08	0.974969963956749\\
3.87262762676284e-08	0.973968762515019\\
3.907753756673e-08	0.972967561073289\\
3.97340476822562e-08	0.971966359631559\\
4.06702420349096e-08	0.970965158189829\\
4.1063091236352e-08	0.969963956748099\\
4.20634429329165e-08	0.968962755306369\\
4.23618466576465e-08	0.967961553864639\\
4.29182063080157e-08	0.966960352422909\\
4.33273330291304e-08	0.965959150981178\\
4.394135145542e-08	0.964957949539448\\
4.43349110881807e-08	0.963956748097718\\
4.47720758501336e-08	0.962955546655988\\
4.55658007922629e-08	0.961954345214258\\
4.63291638110819e-08	0.960953143772528\\
4.74274858832239e-08	0.959951942330798\\
4.79347885649556e-08	0.958950740889068\\
4.81428080345167e-08	0.957949539447338\\
4.88145622803465e-08	0.956948338005608\\
4.90691174057677e-08	0.955947136563878\\
5.00963521618793e-08	0.954945935122147\\
5.0496830389964e-08	0.953944733680417\\
5.0718757847069e-08	0.952943532238687\\
5.15002659218606e-08	0.951942330796957\\
5.17310944503478e-08	0.950941129355227\\
5.22916492496711e-08	0.949939927913497\\
5.28213700859133e-08	0.948938726471767\\
5.30283855886371e-08	0.947937525030037\\
5.37471321858476e-08	0.946936323588307\\
5.4744794751588e-08	0.945935122146577\\
5.53136624146625e-08	0.944933920704847\\
5.59412264989557e-08	0.943932719263116\\
5.66589610668949e-08	0.942931517821386\\
5.68973264761033e-08	0.941930316379656\\
5.78772864124725e-08	0.940929114937926\\
5.84966399667474e-08	0.939927913496196\\
5.93058984758708e-08	0.938926712054466\\
6.03412041650064e-08	0.937925510612736\\
6.10949150661158e-08	0.936924309171006\\
6.19076899465195e-08	0.935923107729276\\
6.23448217367055e-08	0.934921906287546\\
6.29516557640516e-08	0.933920704845816\\
6.33387789217402e-08	0.932919503404086\\
6.35464002265042e-08	0.931918301962356\\
6.39322798111992e-08	0.930917100520626\\
6.43363279402924e-08	0.929915899078895\\
6.47887770644537e-08	0.928914697637165\\
6.51541663350315e-08	0.927913496195435\\
6.55396829129328e-08	0.926912294753705\\
6.60882955238887e-08	0.925911093311975\\
6.66275176273092e-08	0.924909891870245\\
6.72421051713529e-08	0.923908690428515\\
6.73739108707354e-08	0.922907488986785\\
6.76429235236877e-08	0.921906287545055\\
6.81485662470637e-08	0.920905086103325\\
6.84599760952437e-08	0.919903884661595\\
6.86303273248519e-08	0.918902683219865\\
6.90370342414302e-08	0.917901481778134\\
6.94503990622325e-08	0.916900280336404\\
7.00694574664155e-08	0.915899078894674\\
7.04305498449356e-08	0.914897877452944\\
7.08579163972929e-08	0.913896676011214\\
7.11514000558221e-08	0.912895474569484\\
7.17063808760466e-08	0.911894273127754\\
7.23990162421128e-08	0.910893071686024\\
7.28711597719717e-08	0.909891870244294\\
7.31363254229238e-08	0.908890668802564\\
7.3300204758588e-08	0.907889467360834\\
7.36748091360663e-08	0.906888265919104\\
7.43853493551904e-08	0.905887064477374\\
7.46522645535254e-08	0.904885863035643\\
7.48120857200022e-08	0.903884661593913\\
7.53888143699839e-08	0.902883460152183\\
7.55556676819559e-08	0.901882258710453\\
7.64419736501843e-08	0.900881057268723\\
7.7076376727791e-08	0.899879855826993\\
7.77837472458852e-08	0.898878654385262\\
7.81651218189727e-08	0.897877452943532\\
7.85065327735734e-08	0.896876251501802\\
7.88930233751963e-08	0.895875050060072\\
7.94563367157044e-08	0.894873848618342\\
7.9765135418656e-08	0.893872647176612\\
8.02189924828278e-08	0.892871445734882\\
8.06091385648319e-08	0.891870244293152\\
8.09121759906289e-08	0.890869042851422\\
8.11978692465867e-08	0.889867841409692\\
8.14641824534789e-08	0.888866639967962\\
8.16711123026492e-08	0.887865438526232\\
8.20430720279882e-08	0.886864237084501\\
8.23302832492839e-08	0.885863035642771\\
8.28253018799889e-08	0.884861834201041\\
8.32472719856805e-08	0.883860632759311\\
8.33819508090249e-08	0.882859431317581\\
8.41776186457955e-08	0.881858229875851\\
8.42907807171801e-08	0.880857028434121\\
8.44612155892638e-08	0.879855826992391\\
8.4858857622725e-08	0.878854625550661\\
8.50736731421578e-08	0.877853424108931\\
8.5602886293094e-08	0.876852222667201\\
8.57547397032724e-08	0.875851021225471\\
8.60601989821709e-08	0.874849819783741\\
8.64941074616559e-08	0.873848618342011\\
8.68401482204196e-08	0.872847416900281\\
8.70926667035021e-08	0.871846215458551\\
8.74604184745639e-08	0.870845014016821\\
8.79433538435173e-08	0.869843812575091\\
8.81068776044088e-08	0.868842611133361\\
8.82442211155023e-08	0.867841409691631\\
8.85145593559416e-08	0.866840208249901\\
8.87707434629353e-08	0.865839006808171\\
8.89885658695272e-08	0.864837805366441\\
8.92241950198563e-08	0.863836603924711\\
8.94595038666038e-08	0.862835402482981\\
8.97788503715984e-08	0.86183420104125\\
9.05125997236836e-08	0.86083299959952\\
9.08732662300281e-08	0.85983179815779\\
9.1057801512724e-08	0.85883059671606\\
9.14670147799598e-08	0.85782939527433\\
9.18011583133567e-08	0.8568281938326\\
9.20505039239463e-08	0.85582699239087\\
9.22812746759532e-08	0.85482579094914\\
9.25215360593779e-08	0.85382458950741\\
9.27752295062819e-08	0.85282338806568\\
9.30663330300899e-08	0.85182218662395\\
9.36094228589397e-08	0.85082098518222\\
9.37524248969104e-08	0.849819783740489\\
9.41273808491825e-08	0.848818582298759\\
9.43958098156163e-08	0.847817380857029\\
9.48739665169017e-08	0.846816179415299\\
9.53426817199476e-08	0.845814977973569\\
9.6341254570104e-08	0.844813776531839\\
9.6490612424353e-08	0.843812575090109\\
9.68166604850817e-08	0.842811373648379\\
9.70961304614387e-08	0.841810172206649\\
9.76151316752086e-08	0.840808970764918\\
9.79467511780276e-08	0.839807769323188\\
9.87960360452268e-08	0.838806567881459\\
9.93153625543725e-08	0.837805366439728\\
9.97462404901964e-08	0.836804164997998\\
1.0005186078214e-07	0.835802963556268\\
1.00232860002421e-07	0.834801762114538\\
1.0041384009862e-07	0.833800560672808\\
1.00778155351231e-07	0.832799359231078\\
1.01044076233322e-07	0.831798157789348\\
1.01504437852842e-07	0.830796956347618\\
1.0196142731147e-07	0.829795754905888\\
1.02430488203668e-07	0.828794553464158\\
1.0300508270567e-07	0.827793352022428\\
1.03239892156079e-07	0.826792150580697\\
1.03538441141662e-07	0.825790949138967\\
1.03785651625399e-07	0.824789747697237\\
1.04863424066524e-07	0.823788546255507\\
1.05436387094524e-07	0.822787344813777\\
1.05535692659157e-07	0.821786143372047\\
1.05700137486912e-07	0.820784941930317\\
1.05918044709721e-07	0.819783740488587\\
1.0615231180459e-07	0.818782539046857\\
1.06673437829683e-07	0.817781337605127\\
1.06842668798051e-07	0.816780136163397\\
1.07090073813731e-07	0.815778934721667\\
1.07542117125119e-07	0.814777733279937\\
1.07733671866408e-07	0.813776531838207\\
1.08232388749142e-07	0.812775330396477\\
1.08491579990918e-07	0.811774128954747\\
1.08783676828071e-07	0.810772927513017\\
1.09003408441901e-07	0.809771726071287\\
1.09316802680627e-07	0.808770524629556\\
1.09679443020976e-07	0.807769323187826\\
1.09825777516976e-07	0.806768121746096\\
1.10254244402892e-07	0.805766920304366\\
1.10726441110993e-07	0.804765718862636\\
1.10960284839096e-07	0.803764517420906\\
1.1122949302125e-07	0.802763315979176\\
1.11518103734994e-07	0.801762114537446\\
1.12439381944712e-07	0.800760913095716\\
1.12674709249982e-07	0.799759711653986\\
1.13155317096097e-07	0.798758510212256\\
1.13571004933404e-07	0.797757308770525\\
1.141667559171e-07	0.796756107328796\\
1.14436883370528e-07	0.795754905887066\\
1.14521240167891e-07	0.794753704445335\\
1.15101917392832e-07	0.793752503003606\\
1.15530727655975e-07	0.792751301561875\\
1.15975540354176e-07	0.791750100120145\\
1.16392911332575e-07	0.790748898678415\\
1.16721924258128e-07	0.789747697236685\\
1.1718839312558e-07	0.788746495794955\\
1.17453245693267e-07	0.787745294353225\\
1.1764023835732e-07	0.786744092911495\\
1.17746017002857e-07	0.785742891469765\\
1.18023309278473e-07	0.784741690028035\\
1.18253163210122e-07	0.783740488586305\\
1.18567864488822e-07	0.782739287144575\\
1.18705202528683e-07	0.781738085702845\\
1.1922452980723e-07	0.780736884261114\\
1.19802519403692e-07	0.779735682819384\\
1.20100483319027e-07	0.778734481377654\\
1.20622652048519e-07	0.777733279935924\\
1.20933454739861e-07	0.776732078494194\\
1.21327307381869e-07	0.775730877052464\\
1.21489156612798e-07	0.774729675610734\\
1.21774099913813e-07	0.773728474169004\\
1.22418476093519e-07	0.772727272727274\\
1.22901511827174e-07	0.771726071285544\\
1.2306125346539e-07	0.770724869843814\\
1.23383781412421e-07	0.769723668402084\\
1.23899527070981e-07	0.768722466960354\\
1.24191601958873e-07	0.767721265518623\\
1.2447365400032e-07	0.766720064076893\\
1.2469315467861e-07	0.765718862635163\\
1.24877754700312e-07	0.764717661193433\\
1.25181850966808e-07	0.763716459751703\\
1.25301657943152e-07	0.762715258309973\\
1.257527288963e-07	0.761714056868243\\
1.2594278409746e-07	0.760712855426513\\
1.26183910771895e-07	0.759711653984783\\
1.26644352300778e-07	0.758710452543052\\
1.26833498692906e-07	0.757709251101322\\
1.26981088546028e-07	0.756708049659592\\
1.27088814270139e-07	0.755706848217862\\
1.27523715454003e-07	0.754705646776132\\
1.27965612565392e-07	0.753704445334402\\
1.2847891608049e-07	0.752703243892672\\
1.28862961877288e-07	0.751702042450942\\
1.29676612135448e-07	0.750700841009212\\
1.29970488551678e-07	0.749699639567482\\
1.3020698773718e-07	0.748698438125752\\
1.30501174517772e-07	0.747697236684022\\
1.31154705185334e-07	0.746696035242292\\
1.31588864332222e-07	0.745694833800562\\
1.31824861368545e-07	0.744693632358832\\
1.32004336485953e-07	0.743692430917102\\
1.32148174667773e-07	0.742691229475372\\
1.32399547619628e-07	0.741690028033642\\
1.32746078957783e-07	0.740688826591912\\
1.33063599733587e-07	0.739687625150181\\
1.33431090256131e-07	0.738686423708451\\
1.33708957632529e-07	0.737685222266721\\
1.34190930771675e-07	0.736684020824991\\
1.34332331139274e-07	0.735682819383261\\
1.34619091805277e-07	0.734681617941531\\
1.34979594987868e-07	0.733680416499801\\
1.353851932178e-07	0.732679215058071\\
1.35477873376078e-07	0.731678013616341\\
1.3618607585938e-07	0.730676812174611\\
1.36624134864734e-07	0.729675610732881\\
1.3676156799247e-07	0.728674409291151\\
1.36852135980135e-07	0.727673207849421\\
1.37232751344306e-07	0.726672006407691\\
1.37726901169744e-07	0.725670804965961\\
1.37988181098935e-07	0.724669603524231\\
1.38255806716893e-07	0.723668402082501\\
1.38651051685693e-07	0.722667200640771\\
1.39193144712065e-07	0.721665999199041\\
1.39835865432648e-07	0.720664797757311\\
1.40349994928166e-07	0.719663596315581\\
1.40770354318388e-07	0.718662394873851\\
1.41106805956864e-07	0.717661193432121\\
1.41411896962598e-07	0.716659991990391\\
1.41702799300841e-07	0.715658790548661\\
1.42041406600889e-07	0.714657589106931\\
1.42460689026845e-07	0.713656387665201\\
1.43007583466418e-07	0.712655186223471\\
1.43282681281889e-07	0.711653984781741\\
1.43375787989576e-07	0.710652783340011\\
1.43823771996544e-07	0.70965158189828\\
1.44109135152893e-07	0.70865038045655\\
1.44515290831173e-07	0.70764917901482\\
1.45171361392384e-07	0.70664797757309\\
1.45835993113866e-07	0.70564677613136\\
1.4631921225479e-07	0.70464557468963\\
1.46557424590636e-07	0.7036443732479\\
1.46694946227609e-07	0.70264317180617\\
1.47198511180467e-07	0.70164197036444\\
1.47491607924818e-07	0.70064076892271\\
1.47703881311385e-07	0.69963956748098\\
1.48033093683879e-07	0.69863836603925\\
1.48209639138437e-07	0.69763716459752\\
1.49075100758997e-07	0.69663596315579\\
1.49599628528461e-07	0.69563476171406\\
1.49856543552003e-07	0.69463356027233\\
1.50172658067572e-07	0.6936323588306\\
1.50557586651951e-07	0.69263115738887\\
1.51029108446172e-07	0.69162995594714\\
1.51433302143204e-07	0.69062875450541\\
1.51564287775305e-07	0.68962755306368\\
1.51741700146529e-07	0.68862635162195\\
1.52113392400208e-07	0.68762515018022\\
1.5249104176705e-07	0.68662394873849\\
1.52890894025646e-07	0.68562274729676\\
1.53190835364204e-07	0.68462154585503\\
1.53862293924791e-07	0.6836203444133\\
1.54309799715873e-07	0.68261914297157\\
1.54632889957899e-07	0.68161794152984\\
1.54835892172415e-07	0.68061674008811\\
1.55114554325771e-07	0.67961553864638\\
1.55414928949835e-07	0.67861433720465\\
1.55828851233046e-07	0.67761313576292\\
1.55976367657277e-07	0.676611934321189\\
1.5624698573607e-07	0.675610732879459\\
1.56543427688986e-07	0.67460953143773\\
1.5683398888594e-07	0.673608329996\\
1.57101633923677e-07	0.672607128554269\\
1.57375004156e-07	0.671605927112539\\
1.57803039215012e-07	0.670604725670809\\
1.58495787370059e-07	0.669603524229079\\
1.58747166786212e-07	0.668602322787349\\
1.58925267839974e-07	0.667601121345619\\
1.59525726613543e-07	0.666599919903889\\
1.60112288751851e-07	0.665598718462159\\
1.60485462097561e-07	0.664597517020429\\
1.6077095523706e-07	0.663596315578699\\
1.60963260170262e-07	0.662595114136969\\
1.61619593807201e-07	0.661593912695239\\
1.61787896662594e-07	0.660592711253509\\
1.62365424787294e-07	0.659591509811779\\
1.62642511423684e-07	0.658590308370049\\
1.62791403745544e-07	0.657589106928319\\
1.63089079066372e-07	0.656587905486589\\
1.63453075768145e-07	0.655586704044859\\
1.63789923814506e-07	0.654585502603129\\
1.64225056824719e-07	0.653584301161399\\
1.64562061186085e-07	0.652583099719669\\
1.64757122105295e-07	0.651581898277939\\
1.65157887164389e-07	0.650580696836209\\
1.65243714971673e-07	0.649579495394479\\
1.65770948656523e-07	0.648578293952749\\
1.66111665206089e-07	0.647577092511019\\
1.6640399978571e-07	0.646575891069289\\
1.66673861745652e-07	0.645574689627559\\
1.67109030948934e-07	0.644573488185829\\
1.67437818958093e-07	0.643572286744098\\
1.67984305004376e-07	0.642571085302368\\
1.68238159027522e-07	0.641569883860638\\
1.68639343072964e-07	0.640568682418908\\
1.69538282334765e-07	0.639567480977178\\
1.69612540917502e-07	0.638566279535448\\
1.70303766939077e-07	0.637565078093718\\
1.70450948298215e-07	0.636563876651988\\
1.70841810631894e-07	0.635562675210258\\
1.70978002872952e-07	0.634561473768528\\
1.71450107445548e-07	0.633560272326798\\
1.71931979815932e-07	0.632559070885068\\
1.72320839512413e-07	0.631557869443338\\
1.72734732277028e-07	0.630556668001608\\
1.72979512120044e-07	0.629555466559878\\
1.73331001298344e-07	0.628554265118148\\
1.73688408572235e-07	0.627553063676417\\
1.73922547744956e-07	0.626551862234687\\
1.74236278809796e-07	0.625550660792957\\
1.74632970673347e-07	0.624549459351227\\
1.75440760043612e-07	0.623548257909497\\
1.76406907038536e-07	0.622547056467767\\
1.76677549646057e-07	0.621545855026037\\
1.77196741782279e-07	0.620544653584307\\
1.77687603873088e-07	0.619543452142577\\
1.7819111452083e-07	0.618542250700847\\
1.78481002543552e-07	0.617541049259117\\
1.78941453937384e-07	0.616539847817387\\
1.7927277125821e-07	0.615538646375657\\
1.79590829313981e-07	0.614537444933927\\
1.80086671066572e-07	0.613536243492197\\
1.80422782511121e-07	0.612535042050467\\
1.80700976376209e-07	0.611533840608737\\
1.81482620668252e-07	0.610532639167007\\
1.81777265989588e-07	0.609531437725277\\
1.82436490357406e-07	0.608530236283547\\
1.82818033153792e-07	0.607529034841817\\
1.83299489674004e-07	0.606527833400086\\
1.8404323700089e-07	0.605526631958356\\
1.84673730631213e-07	0.604525430516626\\
1.85233904715143e-07	0.603524229074896\\
1.8556881505785e-07	0.602523027633166\\
1.8573820221736e-07	0.601521826191436\\
1.86140627634034e-07	0.600520624749706\\
1.87069843456059e-07	0.599519423307976\\
1.87964731012294e-07	0.598518221866246\\
1.88518213266446e-07	0.597517020424516\\
1.88862398073841e-07	0.596515818982786\\
1.89286152241924e-07	0.595514617541056\\
1.89596822771861e-07	0.594513416099326\\
1.89960756643935e-07	0.593512214657596\\
1.90429317617618e-07	0.592511013215866\\
1.9077049971881e-07	0.591509811774136\\
1.91001171763581e-07	0.590508610332406\\
1.91542767608979e-07	0.589507408890676\\
1.91800492350337e-07	0.588506207448946\\
1.92336663617894e-07	0.587505006007216\\
1.92895690881097e-07	0.586503804565486\\
1.93120763411746e-07	0.585502603123756\\
1.93577693948839e-07	0.584501401682026\\
1.94333974051785e-07	0.583500200240296\\
1.95114106845659e-07	0.582498998798566\\
1.96005886926925e-07	0.581497797356836\\
1.96604827226883e-07	0.580496595915106\\
1.97016024680338e-07	0.579495394473376\\
1.97491355019739e-07	0.578494193031646\\
1.97712610733349e-07	0.577492991589916\\
1.98313764852143e-07	0.576491790148186\\
1.98912073440723e-07	0.575490588706456\\
1.99520076540415e-07	0.574489387264726\\
2.00249589594517e-07	0.573488185822996\\
2.00692870102811e-07	0.572486984381266\\
2.0177480339968e-07	0.571485782939536\\
2.02259088134682e-07	0.570484581497806\\
2.02681020806711e-07	0.569483380056076\\
2.03001943916641e-07	0.568482178614346\\
2.03565208751457e-07	0.567480977172616\\
2.03839098017323e-07	0.566479775730886\\
2.04139706376678e-07	0.565478574289156\\
2.04645966307151e-07	0.564477372847426\\
2.05084688752662e-07	0.563476171405696\\
2.05376225645952e-07	0.562474969963966\\
2.06477341101317e-07	0.561473768522236\\
2.07335924104944e-07	0.560472567080506\\
2.07713256230883e-07	0.559471365638776\\
2.08100437049311e-07	0.558470164197046\\
2.08476115608333e-07	0.557468962755316\\
2.09339416031895e-07	0.556467761313586\\
2.09827241475924e-07	0.555466559871856\\
2.10176386397583e-07	0.554465358430126\\
2.10452228961708e-07	0.553464156988396\\
2.10982462180863e-07	0.552462955546666\\
2.1125930497593e-07	0.551461754104936\\
2.11639835898233e-07	0.550460552663206\\
2.12172901303856e-07	0.549459351221476\\
2.12726594059362e-07	0.548458149779746\\
2.13125516785094e-07	0.547456948338016\\
2.13323312877406e-07	0.546455746896286\\
2.13922310681728e-07	0.545454545454556\\
2.14365013759867e-07	0.544453344012826\\
2.14878886993931e-07	0.543452142571096\\
2.15234001723293e-07	0.542450941129366\\
2.16167850297047e-07	0.541449739687636\\
2.17331594316987e-07	0.540448538245906\\
2.17885992767216e-07	0.539447336804176\\
2.18322984762523e-07	0.538446135362446\\
2.18696039188486e-07	0.537444933920715\\
2.19023468956814e-07	0.536443732478985\\
2.19278043815719e-07	0.535442531037255\\
2.19737382047662e-07	0.534441329595525\\
2.20177495824842e-07	0.533440128153795\\
2.20557250791535e-07	0.532438926712065\\
2.20973728596085e-07	0.531437725270335\\
2.21484405803702e-07	0.530436523828605\\
2.21746829971642e-07	0.529435322386875\\
2.22251293734725e-07	0.528434120945145\\
2.22798339202476e-07	0.527432919503415\\
2.2343301278347e-07	0.526431718061685\\
2.23987382190076e-07	0.525430516619955\\
2.24363835723614e-07	0.524429315178225\\
2.25158628463338e-07	0.523428113736495\\
2.26054693746912e-07	0.522426912294765\\
2.26501102242282e-07	0.521425710853035\\
2.2750021722839e-07	0.520424509411305\\
2.27785736492101e-07	0.519423307969575\\
2.28676740385075e-07	0.518422106527845\\
2.29166189714341e-07	0.517420905086115\\
2.29799586239818e-07	0.516419703644385\\
2.30384642247461e-07	0.515418502202655\\
2.31093399211006e-07	0.514417300760925\\
2.31603581334585e-07	0.513416099319195\\
2.32194971751105e-07	0.512414897877465\\
2.32992896920135e-07	0.511413696435734\\
2.33826810944969e-07	0.510412494994005\\
2.34165944930765e-07	0.509411293552274\\
2.35089056619829e-07	0.508410092110544\\
2.35473441697437e-07	0.507408890668814\\
2.35711780068207e-07	0.506407689227084\\
2.35960351402455e-07	0.505406487785354\\
2.36788426041037e-07	0.504405286343624\\
2.37219655990826e-07	0.503404084901894\\
2.37629122117657e-07	0.502402883460164\\
2.38769215826574e-07	0.501401682018434\\
2.39214311843157e-07	0.500400480576704\\
2.39868840700653e-07	0.499399279134974\\
2.40625269517329e-07	0.498398077693244\\
2.41336698130974e-07	0.497396876251514\\
2.41929638997623e-07	0.496395674809784\\
2.42595558507778e-07	0.495394473368053\\
2.43318162234376e-07	0.494393271926323\\
2.43667383952855e-07	0.493392070484593\\
2.4437757611193e-07	0.492390869042863\\
2.44759780921667e-07	0.491389667601133\\
2.45173505867302e-07	0.490388466159403\\
2.46195594661852e-07	0.489387264717673\\
2.4704283001015e-07	0.488386063275943\\
2.47708670168704e-07	0.487384861834212\\
2.48386781239039e-07	0.486383660392482\\
2.48876487301643e-07	0.485382458950752\\
2.4962357423226e-07	0.484381257509022\\
2.5066163026705e-07	0.483380056067292\\
2.51433248376106e-07	0.482378854625562\\
2.51765270745723e-07	0.481377653183832\\
2.52181042026384e-07	0.480376451742102\\
2.53029903137465e-07	0.479375250300372\\
2.53993649714527e-07	0.478374048858642\\
2.54334185562248e-07	0.477372847416912\\
2.54925140431602e-07	0.476371645975181\\
2.56070021908689e-07	0.475370444533451\\
2.57469946684895e-07	0.474369243091721\\
2.58544139751594e-07	0.473368041649991\\
2.59246243137131e-07	0.472366840208261\\
2.60754994484621e-07	0.471365638766531\\
2.6191502284451e-07	0.470364437324801\\
2.62394092709351e-07	0.469363235883071\\
2.63087296811302e-07	0.468362034441341\\
2.63749725004047e-07	0.46736083299961\\
2.64997228603047e-07	0.46635963155788\\
2.65445147147088e-07	0.46535843011615\\
2.65768552005517e-07	0.46435722867442\\
2.66770119024453e-07	0.46335602723269\\
2.67162058528438e-07	0.46235482579096\\
2.67959770261712e-07	0.46135362434923\\
2.6899728229531e-07	0.4603524229075\\
2.69481039143995e-07	0.45935122146577\\
2.69794390006854e-07	0.45835002002404\\
2.70608972715969e-07	0.457348818582309\\
2.71773483322675e-07	0.456347617140579\\
2.72337916397397e-07	0.455346415698849\\
2.7392022672519e-07	0.454345214257119\\
2.75461540184961e-07	0.453344012815389\\
2.76928178781019e-07	0.452342811373659\\
2.77811061292019e-07	0.451341609931929\\
2.78461133408474e-07	0.450340408490199\\
2.79559970053364e-07	0.449339207048469\\
2.80407916576432e-07	0.448338005606739\\
2.81125959002138e-07	0.447336804165009\\
2.81956492198257e-07	0.446335602723278\\
2.83476182033135e-07	0.445334401281548\\
2.83934018329096e-07	0.444333199839818\\
2.84615671406415e-07	0.443331998398088\\
2.85508898987242e-07	0.442330796956358\\
2.86823539599712e-07	0.441329595514628\\
2.88016777660684e-07	0.440328394072898\\
2.89021105722242e-07	0.439327192631168\\
2.90118716665385e-07	0.438325991189437\\
2.9206562444055e-07	0.437324789747707\\
2.92744422222812e-07	0.436323588305977\\
2.93469442532978e-07	0.435322386864247\\
2.94290573824755e-07	0.434321185422517\\
2.94916896092756e-07	0.433319983980787\\
2.96308608677963e-07	0.432318782539057\\
2.97613993770165e-07	0.431317581097327\\
2.99007589987966e-07	0.430316379655596\\
2.99525595587975e-07	0.429315178213866\\
3.00763364657364e-07	0.428313976772136\\
3.01561649937614e-07	0.427312775330406\\
3.02887934542763e-07	0.426311573888676\\
3.03901644229165e-07	0.425310372446946\\
3.05406833173567e-07	0.424309171005216\\
3.06216939888023e-07	0.423307969563486\\
3.07320707332953e-07	0.422306768121755\\
3.07725272016294e-07	0.421305566680025\\
3.09449654526572e-07	0.420304365238295\\
3.10953915373409e-07	0.419303163796565\\
3.11563153994602e-07	0.418301962354835\\
3.1355012842921e-07	0.417300760913105\\
3.15620141809427e-07	0.416299559471375\\
3.17400877797661e-07	0.415298358029645\\
3.18700257279572e-07	0.414297156587915\\
3.20030828871492e-07	0.413295955146185\\
3.21339165948675e-07	0.412294753704455\\
3.23094131736939e-07	0.411293552262724\\
3.23980633423113e-07	0.410292350820994\\
3.25147111650034e-07	0.409291149379264\\
3.26869020278774e-07	0.408289947937534\\
3.28983414309871e-07	0.407288746495804\\
3.30288548561442e-07	0.406287545054074\\
3.31895218661022e-07	0.405286343612344\\
3.33170859264832e-07	0.404285142170613\\
3.34414576477506e-07	0.403283940728883\\
3.35452580469457e-07	0.402282739287153\\
3.36908730760434e-07	0.401281537845423\\
3.38257323536703e-07	0.400280336403693\\
3.39945211280872e-07	0.399279134961963\\
3.40788460228205e-07	0.398277933520233\\
3.42447164604935e-07	0.397276732078502\\
3.43816788394867e-07	0.396275530636772\\
3.45499575946889e-07	0.395274329195042\\
3.46838158360152e-07	0.394273127753312\\
3.48831041356453e-07	0.393271926311582\\
3.51106178384857e-07	0.392270724869852\\
3.53939895158994e-07	0.391269523428122\\
3.5513345671731e-07	0.390268321986392\\
3.56221067565031e-07	0.389267120544662\\
3.57101346834195e-07	0.388265919102932\\
3.60407150429553e-07	0.387264717661202\\
3.61634406837076e-07	0.386263516219471\\
3.62388250788218e-07	0.385262314777741\\
3.64411722625406e-07	0.384261113336011\\
3.65486054933678e-07	0.383259911894281\\
3.66012975112505e-07	0.382258710452551\\
3.66644805175301e-07	0.381257509010821\\
3.68256093204532e-07	0.380256307569091\\
3.70041067495725e-07	0.37925510612736\\
3.71695928385733e-07	0.378253904685631\\
3.73750377165609e-07	0.3772527032439\\
3.75898676253642e-07	0.37625150180217\\
3.77673046419524e-07	0.37525030036044\\
3.79279211555187e-07	0.37424909891871\\
3.80974489111125e-07	0.37324789747698\\
3.82238637555937e-07	0.37224669603525\\
3.84981588742785e-07	0.37124549459352\\
3.87099637391664e-07	0.370244293151789\\
3.89221453568321e-07	0.369243091710059\\
3.91308310190524e-07	0.368241890268329\\
3.91815662423493e-07	0.367240688826599\\
3.92989365928333e-07	0.366239487384869\\
3.9653312332467e-07	0.365238285943139\\
3.99861928826421e-07	0.364237084501409\\
4.02188968726024e-07	0.363235883059679\\
4.04198180848374e-07	0.362234681617948\\
4.06786550317439e-07	0.361233480176218\\
4.10556328584799e-07	0.360232278734488\\
4.12017413421233e-07	0.359231077292758\\
4.14580497841753e-07	0.358229875851028\\
4.16245269405261e-07	0.357228674409298\\
4.19761069014102e-07	0.356227472967568\\
4.21842666938919e-07	0.355226271525837\\
4.25204980111241e-07	0.354225070084107\\
4.3001939748193e-07	0.353223868642377\\
4.3520148475285e-07	0.352222667200647\\
4.37647475849895e-07	0.351221465758917\\
4.38854688214859e-07	0.350220264317187\\
4.40186287904945e-07	0.349219062875457\\
4.43323431522907e-07	0.348217861433726\\
4.4521361917006e-07	0.347216659991996\\
4.5188646672908e-07	0.346215458550266\\
4.5642067300043e-07	0.345214257108536\\
4.58214792440741e-07	0.344213055666806\\
4.61895596425009e-07	0.343211854225076\\
4.66204401785901e-07	0.342210652783346\\
4.70507944690401e-07	0.341209451341616\\
4.72819027302781e-07	0.340208249899885\\
4.78659268395137e-07	0.339207048458155\\
4.80487713615081e-07	0.338205847016425\\
4.81647222390579e-07	0.337204645574695\\
4.85231278448996e-07	0.336203444132965\\
4.86035070326173e-07	0.335202242691235\\
4.87963891628917e-07	0.334201041249505\\
4.89390720966658e-07	0.333199839807774\\
4.91837067202057e-07	0.332198638366044\\
4.9512817930211e-07	0.331197436924314\\
4.97338783683936e-07	0.330196235482584\\
4.99547356266906e-07	0.329195034040854\\
5.0606163066529e-07	0.328193832599124\\
5.12233108081489e-07	0.327192631157394\\
5.17981004801048e-07	0.326191429715663\\
5.18541996897365e-07	0.325190228273933\\
5.25779358245073e-07	0.324189026832203\\
5.33080476194726e-07	0.323187825390473\\
5.37282990953293e-07	0.322186623948743\\
5.41033953939024e-07	0.321185422507013\\
5.43607628879811e-07	0.320184221065283\\
5.50208870667187e-07	0.319183019623552\\
5.57629957755862e-07	0.318181818181822\\
5.644873891201e-07	0.317180616740092\\
5.6859350116351e-07	0.316179415298362\\
5.72846105292882e-07	0.315178213856632\\
5.7564368060031e-07	0.314177012414902\\
5.78141650601549e-07	0.313175810973171\\
5.84323984884322e-07	0.312174609531441\\
5.87061856991099e-07	0.311173408089711\\
5.92775156000332e-07	0.310172206647981\\
5.99656396541341e-07	0.309171005206251\\
6.02168399048016e-07	0.308169803764521\\
6.07435037959741e-07	0.307168602322791\\
6.12391157472327e-07	0.30616740088106\\
6.18426321280353e-07	0.30516619943933\\
6.21803848906426e-07	0.3041649979976\\
6.29212073457964e-07	0.30316379655587\\
6.38612923045236e-07	0.30216259511414\\
6.48620763761004e-07	0.30116139367241\\
6.52022297096863e-07	0.30016019223068\\
6.58088693461639e-07	0.299158990788949\\
6.66140467067774e-07	0.298157789347219\\
6.70064271039418e-07	0.297156587905489\\
6.79945782000455e-07	0.296155386463759\\
6.85657766964392e-07	0.295154185022029\\
6.88962720970011e-07	0.294152983580299\\
6.96754540345234e-07	0.293151782138569\\
7.10442842293197e-07	0.292150580696839\\
7.18455804316096e-07	0.291149379255108\\
7.24226989606485e-07	0.290148177813378\\
7.2916744045921e-07	0.289146976371648\\
7.36384194038231e-07	0.288145774929918\\
7.4518385251703e-07	0.287144573488188\\
7.62457829549353e-07	0.286143372046458\\
7.72381478983489e-07	0.285142170604727\\
7.78715905229745e-07	0.284140969162997\\
7.98693965527046e-07	0.283139767721267\\
8.0751455223007e-07	0.282138566279537\\
8.20605402751216e-07	0.281137364837807\\
8.28107310569704e-07	0.280136163396077\\
8.41860688648463e-07	0.279134961954347\\
8.51531442793758e-07	0.278133760512617\\
8.68024523125764e-07	0.277132559070886\\
8.73803363027927e-07	0.276131357629156\\
8.92363198049067e-07	0.275130156187426\\
9.09187226368906e-07	0.274128954745696\\
9.13706111835691e-07	0.273127753303966\\
9.33027320255022e-07	0.272126551862236\\
9.46123116478102e-07	0.271125350420506\\
9.69521926644819e-07	0.270124148978776\\
9.77736313764568e-07	0.269122947537045\\
1.00328807046847e-06	0.268121746095315\\
1.01358552304159e-06	0.267120544653585\\
1.02247249923398e-06	0.266119343211855\\
1.02738740980701e-06	0.265118141770125\\
1.04748318571134e-06	0.264116940328395\\
1.05631815891423e-06	0.263115738886665\\
1.07853552607429e-06	0.262114537444934\\
1.1011679893926e-06	0.261113336003204\\
1.11722345976012e-06	0.260112134561474\\
1.13674815566583e-06	0.259110933119744\\
1.16146960431632e-06	0.258109731678014\\
1.18561974277473e-06	0.257108530236284\\
1.19893421595494e-06	0.256107328794554\\
1.21314522519801e-06	0.255106127352824\\
1.23579867136712e-06	0.254104925911094\\
1.24709332757506e-06	0.253103724469363\\
1.27829487534684e-06	0.252102523027633\\
1.28782571317474e-06	0.251101321585903\\
1.31714775876833e-06	0.250100120144173\\
1.32745866755664e-06	0.249098918702443\\
1.34255469747653e-06	0.248097717260713\\
1.38767585730572e-06	0.247096515818983\\
1.39562329866747e-06	0.246095314377253\\
1.41582205099351e-06	0.245094112935523\\
1.45728271386066e-06	0.244092911493793\\
1.47441467695655e-06	0.243091710052062\\
1.50087261769598e-06	0.242090508610332\\
1.51564608303075e-06	0.241089307168602\\
1.54749189400165e-06	0.240088105726872\\
1.57777775284943e-06	0.239086904285142\\
1.63487719932836e-06	0.238085702843412\\
1.65637085825568e-06	0.237084501401682\\
1.67246707352985e-06	0.236083299959952\\
1.71310270142587e-06	0.235082098518222\\
1.74932683327698e-06	0.234080897076492\\
1.79457817515014e-06	0.233079695634762\\
1.83418765448313e-06	0.232078494193032\\
1.87558035554137e-06	0.231077292751302\\
1.91690750148638e-06	0.230076091309572\\
1.95516066612967e-06	0.229074889867841\\
1.98908158288265e-06	0.228073688426111\\
2.05064283617242e-06	0.227072486984381\\
2.08389078829712e-06	0.226071285542651\\
2.1434558932487e-06	0.225070084100921\\
2.18342865391941e-06	0.224068882659191\\
2.21500745887792e-06	0.223067681217461\\
2.25952373820764e-06	0.222066479775731\\
2.30542079703326e-06	0.221065278334001\\
2.32263787011395e-06	0.220064076892271\\
2.35957065921043e-06	0.219062875450541\\
2.4985281765187e-06	0.218061674008811\\
2.53092388176483e-06	0.21706047256708\\
2.58564196335745e-06	0.21605927112535\\
2.67560543094447e-06	0.21505806968362\\
2.75413560318862e-06	0.21405686824189\\
2.78044307835842e-06	0.21305566680016\\
2.81560365722551e-06	0.21205446535843\\
2.9413503153985e-06	0.2110532639167\\
2.99164369030742e-06	0.21005206247497\\
3.04485584544609e-06	0.20905086103324\\
3.13127034178707e-06	0.20804965959151\\
3.16341237596829e-06	0.20704845814978\\
3.22819351929122e-06	0.20604725670805\\
3.35339315711485e-06	0.205046055266319\\
3.4226114900859e-06	0.204044853824589\\
3.49781460551732e-06	0.203043652382859\\
3.574584276345e-06	0.202042450941129\\
3.67476348691285e-06	0.201041249499399\\
3.75888989126769e-06	0.200040048057669\\
3.85499048992552e-06	0.199038846615939\\
4.01980921052655e-06	0.198037645174209\\
4.26647077912608e-06	0.197036443732479\\
4.3852157906479e-06	0.196035242290749\\
4.57696892969812e-06	0.195034040849019\\
4.68543686710182e-06	0.194032839407289\\
4.82475754056626e-06	0.193031637965559\\
5.00589969261871e-06	0.192030436523829\\
5.21748460273085e-06	0.191029235082099\\
5.3499076506423e-06	0.190028033640369\\
5.62495212103438e-06	0.189026832198638\\
5.73249311209814e-06	0.188025630756908\\
5.99146048791082e-06	0.187024429315178\\
6.34192754582169e-06	0.186023227873448\\
6.56626932372438e-06	0.185022026431718\\
6.94349487690475e-06	0.184020824989988\\
7.15580333566734e-06	0.183019623548258\\
7.66122623808117e-06	0.182018422106528\\
8.01770597595262e-06	0.181017220664798\\
8.52224719178196e-06	0.180016019223068\\
8.74248485973434e-06	0.179014817781338\\
9.07258236540645e-06	0.178013616339608\\
9.50513684018024e-06	0.177012414897878\\
9.87176934379175e-06	0.176011213456148\\
1.01447792952193e-05	0.175010012014417\\
1.0647589261328e-05	0.174008810572687\\
1.11255608925785e-05	0.173007609130957\\
1.16708303025294e-05	0.172006407689227\\
1.21274645652959e-05	0.171005206247497\\
1.22536082034307e-05	0.170004004805767\\
1.26804434927888e-05	0.169002803364037\\
1.2827322642618e-05	0.168001601922307\\
1.30379702774115e-05	0.167000400480577\\
1.37540406261099e-05	0.165999199038847\\
1.42544757136142e-05	0.164997997597117\\
1.44455802208311e-05	0.163996796155387\\
1.48841190887663e-05	0.162995594713657\\
1.52509404652552e-05	0.161994393271927\\
1.58839742902546e-05	0.160993191830196\\
1.66401911890958e-05	0.159991990388466\\
1.73323275111984e-05	0.158990788946736\\
1.84114379965902e-05	0.157989587505006\\
1.90213208018537e-05	0.156988386063276\\
1.98106110353517e-05	0.155987184621546\\
2.03865561983665e-05	0.154985983179816\\
2.12290897174559e-05	0.153984781738086\\
2.16667614670448e-05	0.152983580296356\\
2.26181224902523e-05	0.151982378854626\\
2.44810204968206e-05	0.150981177412896\\
2.49880162677595e-05	0.149979975971166\\
2.52279675149313e-05	0.148978774529436\\
2.61597286573573e-05	0.147977573087706\\
2.7593744256392e-05	0.146976371645976\\
2.85844073465918e-05	0.145975170204245\\
2.96026844462452e-05	0.144973968762515\\
3.10575153375757e-05	0.143972767320785\\
3.18441661505937e-05	0.142971565879055\\
3.25504120366391e-05	0.141970364437325\\
3.33932721517809e-05	0.140969162995595\\
3.48933313044131e-05	0.139967961553865\\
3.55835852299637e-05	0.138966760112135\\
3.66724416452461e-05	0.137965558670405\\
3.76229470522915e-05	0.136964357228675\\
3.89438345458658e-05	0.135963155786945\\
3.95322876711899e-05	0.134961954345215\\
4.08402001937093e-05	0.133960752903485\\
4.2240125157788e-05	0.132959551461755\\
4.33262658833142e-05	0.131958350020025\\
4.38886247757871e-05	0.130957148578294\\
4.541662633317e-05	0.129955947136564\\
4.62786082134591e-05	0.128954745694834\\
4.70618373528781e-05	0.127953544253104\\
4.82547249687484e-05	0.126952342811374\\
4.89269430009801e-05	0.125951141369644\\
4.97277165955077e-05	0.124949939927914\\
5.06445714124557e-05	0.123948738486184\\
5.10287441873949e-05	0.122947537044454\\
5.14054472231234e-05	0.121946335602724\\
5.17010421576139e-05	0.120945134160994\\
5.3086061274624e-05	0.119943932719264\\
5.36223306204004e-05	0.118942731277534\\
5.4348386047217e-05	0.117941529835803\\
5.52610682694732e-05	0.116940328394073\\
5.64387023617519e-05	0.115939126952343\\
5.6912282863298e-05	0.114937925510613\\
5.73710349260348e-05	0.113936724068883\\
5.77625777121491e-05	0.112935522627153\\
5.85835388005789e-05	0.111934321185423\\
5.87508797508233e-05	0.110933119743693\\
5.90121952982047e-05	0.109931918301963\\
5.98873473490779e-05	0.108930716860233\\
6.05488505622432e-05	0.107929515418503\\
6.10878884455655e-05	0.106928313976772\\
6.21832937063602e-05	0.105927112535043\\
6.31778894254519e-05	0.104925911093312\\
6.36522649500173e-05	0.103924709651582\\
6.42138790739888e-05	0.102923508209852\\
6.54287265721836e-05	0.101922306768122\\
6.57565154723661e-05	0.100921105326392\\
6.64287483802952e-05	0.0999199038846619\\
6.70892843372404e-05	0.0989187024429319\\
6.79522791646772e-05	0.0979175010012018\\
6.89351333872488e-05	0.0969162995594717\\
6.97132784316602e-05	0.0959150981177416\\
7.05712716383886e-05	0.0949138966760115\\
7.11915225587451e-05	0.0939126952342815\\
7.20004307702493e-05	0.0929114937925514\\
7.3312634418068e-05	0.0919102923508213\\
7.39875260693371e-05	0.0909090909090912\\
7.42349769333672e-05	0.0899078894673611\\
7.52723640638227e-05	0.088906688025631\\
7.59021552956805e-05	0.0879054865839008\\
7.69055605917315e-05	0.0869042851421709\\
7.79924919758142e-05	0.0859030837004408\\
7.88533272935879e-05	0.0849018822587106\\
7.93598829727581e-05	0.0839006808169805\\
8.0127876532936e-05	0.0828994793752504\\
8.2546665242216e-05	0.0818982779335203\\
8.35130326597117e-05	0.0808970764917902\\
8.46994505140901e-05	0.0798958750500602\\
8.54701136162059e-05	0.0788946736083301\\
8.68357736874921e-05	0.0778934721666\\
8.76894094424133e-05	0.0768922707248699\\
8.8961107680143e-05	0.0758910692831398\\
8.92997293003558e-05	0.0748898678414097\\
9.04538680879458e-05	0.0738886663996796\\
9.10190527295208e-05	0.0728874649579496\\
9.15592792323967e-05	0.0718862635162195\\
9.24711475299683e-05	0.0708850620744894\\
9.2971890955539e-05	0.0698838606327593\\
9.37487050269877e-05	0.0688826591910292\\
9.43960830813267e-05	0.0678814577492991\\
9.50112825099327e-05	0.066880256307569\\
9.62328952490879e-05	0.0658790548658389\\
9.74830839011967e-05	0.0648778534241088\\
9.86847823290151e-05	0.0638766519823788\\
9.99515802420152e-05	0.0628754505406487\\
0.000100616262005852	0.0618742490989186\\
0.000101884619256199	0.0608730476571885\\
0.000102675943367344	0.0598718462154585\\
0.000103834579452998	0.0588706447737284\\
0.000105328296340681	0.0578694433319983\\
0.000106789856872196	0.0568682418902682\\
0.000107243038062594	0.0558670404485382\\
0.000108109433902756	0.0548658390068081\\
0.000108951937615123	0.053864637565078\\
0.00011018703546922	0.0528634361233479\\
0.000110560769127107	0.0518622346816179\\
0.000111444400654173	0.0508610332398878\\
0.000112735406774431	0.0498598317981577\\
0.000113881702912245	0.0488586303564276\\
0.000114430677517968	0.0478574289146976\\
0.000115094563516836	0.0468562274729675\\
0.000116344012284702	0.0458550260312375\\
0.000117253026652017	0.0448538245895074\\
0.000119092165166988	0.0438526231477773\\
0.00012165992858945	0.0428514217060473\\
0.000123266997960143	0.0418502202643172\\
0.000124257589003672	0.0408490188225871\\
0.00012474872072799	0.039847817380857\\
0.000125151221636534	0.038846615939127\\
0.00012690920901955	0.0378454144973969\\
0.000128071103744286	0.0368442130556668\\
0.000130648207274323	0.0358430116139367\\
0.000132796358198663	0.0348418101722067\\
0.000136074613493565	0.0338406087304766\\
0.000139525145083084	0.0328394072887465\\
0.000142199948641709	0.0318382058470164\\
0.000145108043147802	0.0308370044052864\\
0.000147867583473772	0.0298358029635563\\
0.000153243362890533	0.0288346015218262\\
0.000158858510375597	0.027833400080096\\
0.00016385211680172	0.0268321986383661\\
0.000170785991509773	0.025830997196636\\
0.000186644629553245	0.0248297957549058\\
0.000199955668257303	0.0238285943131757\\
0.000211154729971368	0.0228273928714458\\
0.000221669493785487	0.0218261914297156\\
0.000233778233324608	0.0208249899879855\\
0.00025999918896392	0.0198237885462555\\
0.000308131645468499	0.0188225871045254\\
0.000356059574752119	0.0178213856627953\\
0.00046987603536196	0.0168201842210652\\
0.000665009569425474	0.0158189827793352\\
0.00107225864007527	0.0148177813376051\\
0.00166937183482503	0.013816579895875\\
0.00291636498333204	0.0128153784541449\\
0.00442146023663127	0.0118141770124149\\
0.00739643437302355	0.0108129755706848\\
0.0098532209086821	0.00981177412895473\\
0.0127915152829252	0.00881057268722463\\
0.0190069225763982	0.00780937124549463\\
0.0245840969817472	0.00680816980376453\\
0.0505772466612439	0.00580696836203443\\
0.142396849866701	0.00480576692030432\\
0.393059606434248	0.00380456547857433\\
82.0772957296053	0.00280336403684422\\
361.652513905046	0.00180216259511412\\
636.095260879805	0.000800961153384017\\
};
\addlegendentry{$N=1$,~, $\lrmse =26.52$, $\prmse =0.012$, $\armse =0.032$, $\brmse =1\hspace{-3pt}\times\hspace{-3pt}10^{-4}$, $\gamma \rightarrow \infty$}


==> figures/mse_N_1_K_20_G_5_SNR_40_I_20_Pratio_2_Nratio_2_alpha_2_cs.tex <==
\addplot [color=red, dashed,line width=0.6pt]
  table[row sep=crcr]{%
0.000877313702955488	1\\
0.0125198436914985	0.998\\
0.0197299214324539	0.996\\
0.0242885983037307	0.994\\
0.0265560435987167	0.992\\
0.0315124067891384	0.99\\
0.0341553260031352	0.988\\
0.0381556412449297	0.986\\
0.0399475769071952	0.984\\
0.041769352712526	0.982\\
0.045840257837466	0.98\\
0.047470853068204	0.978\\
0.0491115129015274	0.976\\
0.0511141468703334	0.974\\
0.0530635535159526	0.972\\
0.0546314410347305	0.970000000000001\\
0.0565479274675989	0.968\\
0.0578560719283227	0.966000000000001\\
0.0601754572754482	0.964000000000001\\
0.061889789840069	0.962000000000001\\
0.0631753359680068	0.960000000000001\\
0.0643005341294343	0.958000000000001\\
0.0663077351057073	0.956000000000001\\
0.0678589707459699	0.954000000000001\\
0.0692886350599342	0.952000000000001\\
0.0715872609302271	0.950000000000001\\
0.0736801453465872	0.948000000000001\\
0.075396528834672	0.946000000000001\\
0.0769711633429068	0.944000000000001\\
0.0780909158525662	0.942000000000001\\
0.0796978124168583	0.940000000000001\\
0.0820756111037591	0.938000000000001\\
0.0834894047913341	0.936000000000001\\
0.0845916040395363	0.934000000000001\\
0.0863124808933795	0.932000000000001\\
0.087575681275894	0.930000000000001\\
0.0886676473926321	0.928000000000001\\
0.0901236987731214	0.926000000000001\\
0.0918848181400624	0.924000000000001\\
0.0930446004832928	0.922000000000001\\
0.0947974131963511	0.920000000000001\\
0.096357643619682	0.918000000000001\\
0.0975275303769013	0.916000000000001\\
0.0989062433821962	0.914000000000001\\
0.101078670485123	0.912000000000001\\
0.103265955851937	0.910000000000001\\
0.103581213377945	0.908000000000001\\
0.105054496605045	0.906000000000001\\
0.105701152703992	0.904000000000001\\
0.106876897534009	0.902000000000001\\
0.108244848765012	0.900000000000001\\
0.109147637667686	0.898000000000001\\
0.110278970087055	0.896000000000001\\
0.11117336808747	0.894000000000001\\
0.113079374278358	0.892000000000001\\
0.114373766911595	0.890000000000001\\
0.115986837341479	0.888000000000001\\
0.117464745237626	0.886000000000001\\
0.118214160890289	0.884000000000001\\
0.119972252597635	0.882000000000001\\
0.121272972775826	0.880000000000001\\
0.122315344263849	0.878000000000001\\
0.123364473838786	0.876000000000001\\
0.12434947393664	0.874000000000001\\
0.125808226332393	0.872000000000001\\
0.126922482791864	0.870000000000001\\
0.128269015515751	0.868000000000002\\
0.129380644253769	0.866000000000001\\
0.130233450603524	0.864000000000001\\
0.131508166273369	0.862000000000002\\
0.132295904539767	0.860000000000001\\
0.133617922143804	0.858000000000001\\
0.134573423467238	0.856000000000001\\
0.136388763706584	0.854000000000002\\
0.137473473461874	0.852000000000001\\
0.138288499102529	0.850000000000001\\
0.139297597690476	0.848000000000001\\
0.140017264193774	0.846000000000001\\
0.141273162187461	0.844000000000001\\
0.142596875793271	0.842000000000001\\
0.143829944058201	0.840000000000001\\
0.144758894460774	0.838000000000002\\
0.145736938496725	0.836000000000002\\
0.14640690623123	0.834000000000001\\
0.147320401367808	0.832000000000001\\
0.148493455211357	0.830000000000001\\
0.149236982608006	0.828000000000001\\
0.149817072654102	0.826000000000002\\
0.151815242810114	0.824000000000002\\
0.152696965986531	0.822000000000002\\
0.153398282084462	0.820000000000002\\
0.154321693076908	0.818000000000002\\
0.155134152688594	0.816000000000002\\
0.15566878130123	0.814000000000002\\
0.156257371947322	0.812000000000002\\
0.157376487544799	0.810000000000002\\
0.158162624237714	0.808000000000002\\
0.159377437863578	0.806000000000002\\
0.161105284116394	0.804000000000002\\
0.162823419085711	0.802000000000002\\
0.163480051712243	0.800000000000002\\
0.16476646742753	0.798000000000002\\
0.165977619414058	0.796000000000002\\
0.167537812600772	0.794000000000002\\
0.168932310831987	0.792000000000002\\
0.171247076652069	0.790000000000002\\
0.173657903639463	0.788000000000002\\
0.174679225468417	0.786000000000002\\
0.175273677655668	0.784000000000002\\
0.175879148808832	0.782000000000002\\
0.177091343575502	0.780000000000002\\
0.178172647897384	0.778000000000002\\
0.179367044270591	0.776000000000002\\
0.180109716749033	0.774000000000002\\
0.181688732310654	0.772000000000002\\
0.182507267784544	0.770000000000003\\
0.183697795885522	0.768000000000003\\
0.184326144545151	0.766000000000003\\
0.185394472586235	0.764000000000003\\
0.187423212126264	0.762000000000003\\
0.188815057422239	0.760000000000003\\
0.19038762092383	0.758000000000003\\
0.19135186938994	0.756000000000003\\
0.192313477208194	0.754000000000004\\
0.19340471489493	0.752000000000004\\
0.194911701671932	0.750000000000004\\
0.195944150766149	0.748000000000004\\
0.19721869053434	0.746000000000004\\
0.198404780515713	0.744000000000004\\
0.198988429945702	0.742000000000004\\
0.200066619266235	0.740000000000004\\
0.201242795649655	0.738000000000005\\
0.20255823647741	0.736000000000005\\
0.203562119335	0.734000000000005\\
0.204569341259536	0.732000000000005\\
0.205175477064341	0.730000000000005\\
0.206149215252547	0.728000000000005\\
0.207248520475453	0.726000000000005\\
0.208371152373446	0.724000000000006\\
0.209424535437761	0.722000000000006\\
0.210206892164327	0.720000000000006\\
0.210960070179131	0.718000000000006\\
0.212055242536216	0.716000000000006\\
0.212701640223248	0.714000000000006\\
0.214275377124449	0.712000000000006\\
0.214972472973723	0.710000000000006\\
0.216220448822367	0.708000000000006\\
0.21730777232738	0.706000000000007\\
0.217823146789736	0.704000000000007\\
0.218946025503082	0.702000000000007\\
0.21987495990811	0.700000000000007\\
0.220720286647403	0.698000000000007\\
0.221781489448211	0.696000000000007\\
0.223071462292844	0.694000000000007\\
0.224152559915212	0.692000000000007\\
0.225195799045695	0.690000000000007\\
0.226110138854425	0.688000000000007\\
0.226809959208939	0.686000000000007\\
0.227947881444465	0.684000000000007\\
0.229216554694056	0.682000000000007\\
0.231211695517824	0.680000000000007\\
0.232100800565177	0.678000000000008\\
0.23376132415558	0.676000000000008\\
0.234819017058377	0.674000000000008\\
0.236364176862086	0.672000000000008\\
0.23848560784167	0.670000000000008\\
0.239408366200393	0.668000000000008\\
0.240570998561131	0.666000000000008\\
0.242022293316945	0.664000000000008\\
0.242685283448382	0.662000000000009\\
0.243884657316819	0.660000000000009\\
0.244830432384903	0.658000000000009\\
0.245510001668868	0.656000000000009\\
0.246155096843778	0.654000000000009\\
0.246781049837172	0.652000000000009\\
0.24843966041252	0.650000000000009\\
0.24910382305046	0.64800000000001\\
0.250194287668772	0.64600000000001\\
0.251356533455802	0.64400000000001\\
0.252830316564859	0.64200000000001\\
0.254471094493899	0.64000000000001\\
0.255099236142017	0.63800000000001\\
0.256612930580483	0.63600000000001\\
0.258124079913347	0.63400000000001\\
0.258912207388947	0.63200000000001\\
0.260194816017596	0.630000000000011\\
0.261042266183867	0.628000000000011\\
0.262769643362535	0.626000000000011\\
0.26400888315426	0.624000000000011\\
0.264769511100547	0.622000000000011\\
0.265589283106728	0.620000000000011\\
0.26675359729089	0.618000000000011\\
0.26811945209619	0.616000000000012\\
0.269210142788617	0.614000000000012\\
0.271584515517882	0.612000000000012\\
0.2732894871455	0.610000000000012\\
0.273938819865464	0.608000000000012\\
0.275317662644017	0.606000000000012\\
0.276550429864133	0.604000000000013\\
0.277077759329979	0.602000000000013\\
0.278202219975413	0.600000000000013\\
0.278761478459066	0.598000000000013\\
0.279783273056496	0.596000000000013\\
0.280988835530772	0.594000000000014\\
0.281772589244557	0.592000000000014\\
0.283043075802483	0.590000000000014\\
0.284706953153654	0.588000000000014\\
0.285356992354204	0.586000000000014\\
0.286268661796213	0.584000000000014\\
0.288533005368151	0.582000000000015\\
0.289771679927106	0.580000000000015\\
0.291496570423748	0.578000000000015\\
0.293163302683063	0.576000000000015\\
0.294428656286555	0.574000000000015\\
0.296652489733848	0.572000000000015\\
0.297783654200594	0.570000000000015\\
0.299275738581318	0.568000000000016\\
0.301526148689263	0.566000000000016\\
0.301889463100016	0.564000000000016\\
0.303492721053853	0.562000000000016\\
0.305480718975995	0.560000000000016\\
0.306818543953169	0.558000000000016\\
0.308501428736579	0.556000000000017\\
0.310072017145933	0.554000000000017\\
0.310999152472381	0.552000000000017\\
0.312569783206967	0.550000000000017\\
0.313293514797934	0.548000000000017\\
0.31484882804534	0.546000000000018\\
0.315613882737641	0.544000000000018\\
0.316638024685108	0.542000000000018\\
0.317588818491312	0.540000000000018\\
0.318379992823985	0.538000000000018\\
0.31917500673966	0.536000000000018\\
0.320095263011995	0.534000000000018\\
0.320957841068361	0.532000000000018\\
0.322110298510469	0.530000000000019\\
0.323213191339544	0.528000000000019\\
0.324109258232886	0.526000000000019\\
0.325533505033234	0.524000000000019\\
0.327595254949651	0.522000000000019\\
0.329664642198705	0.520000000000019\\
0.330951529971185	0.518000000000019\\
0.332388246122134	0.51600000000002\\
0.333208303528081	0.51400000000002\\
0.335214855210917	0.51200000000002\\
0.336661639380387	0.51000000000002\\
0.337281378492062	0.50800000000002\\
0.338964333605701	0.506000000000021\\
0.340730998545068	0.504000000000021\\
0.342050064741368	0.502000000000021\\
0.34349114737793	0.500000000000021\\
0.345291619255463	0.498000000000021\\
0.347110062945845	0.496000000000021\\
0.348095624187838	0.494000000000021\\
0.349091210742508	0.492000000000021\\
0.351278935043974	0.490000000000021\\
0.353169380691698	0.488000000000021\\
0.354158694461769	0.48600000000002\\
0.355516700574984	0.48400000000002\\
0.356713447555487	0.48200000000002\\
0.357841986985652	0.48000000000002\\
0.358702232162968	0.47800000000002\\
0.360017962768544	0.47600000000002\\
0.361078885026139	0.47400000000002\\
0.362512213847169	0.47200000000002\\
0.363807076082449	0.47000000000002\\
0.36578654664672	0.46800000000002\\
0.366997408064048	0.46600000000002\\
0.367762226181904	0.464000000000019\\
0.369569468833891	0.462000000000019\\
0.371088812279039	0.460000000000019\\
0.372787960360154	0.458000000000019\\
0.373601205238835	0.456000000000019\\
0.375403529327105	0.454000000000019\\
0.377743247287424	0.452000000000019\\
0.379696968368421	0.450000000000019\\
0.381506714695782	0.448000000000019\\
0.383369797204628	0.446000000000019\\
0.384856749269035	0.444000000000019\\
0.386221357510817	0.442000000000019\\
0.387990872015053	0.440000000000019\\
0.389525335322295	0.438000000000018\\
0.39058532649628	0.436000000000018\\
0.392064828910274	0.434000000000018\\
0.394370482365192	0.432000000000018\\
0.395588652742933	0.430000000000018\\
0.397141664231537	0.428000000000018\\
0.399321348198758	0.426000000000018\\
0.400391729237562	0.424000000000018\\
0.402715148935459	0.422000000000018\\
0.404806085722574	0.420000000000017\\
0.405600448118429	0.418000000000017\\
0.407947491875891	0.416000000000017\\
0.409910650445836	0.414000000000017\\
0.411005902720399	0.412000000000017\\
0.412821506219769	0.410000000000017\\
0.413520998002431	0.408000000000017\\
0.415422523381325	0.406000000000017\\
0.41741587623143	0.404000000000017\\
0.419523602176679	0.402000000000017\\
0.421773712831408	0.400000000000017\\
0.423335004950389	0.398000000000016\\
0.424779249001212	0.396000000000016\\
0.427362467114384	0.394000000000016\\
0.429582857264233	0.392000000000016\\
0.430653375908439	0.390000000000016\\
0.433362462540986	0.388000000000016\\
0.43571209035456	0.386000000000016\\
0.437579198789954	0.384000000000016\\
0.439534839377908	0.382000000000016\\
0.442470270431463	0.380000000000016\\
0.444090542125711	0.378000000000016\\
0.44525762319618	0.376000000000016\\
0.446310567358658	0.374000000000015\\
0.447868912584981	0.372000000000015\\
0.448744140792787	0.370000000000015\\
0.450154318217659	0.368000000000015\\
0.452364671486284	0.366000000000015\\
0.455465061538681	0.364000000000015\\
0.45790184536921	0.362000000000015\\
0.459285185995359	0.360000000000015\\
0.461209502159531	0.358000000000015\\
0.46417282792679	0.356000000000015\\
0.465519219124412	0.354000000000015\\
0.467415328790664	0.352000000000015\\
0.46970007056786	0.350000000000015\\
0.47241220668717	0.348000000000014\\
0.474169327731153	0.346000000000014\\
0.475505999445697	0.344000000000014\\
0.478270782470279	0.342000000000014\\
0.480661533993215	0.340000000000014\\
0.482638926149797	0.338000000000014\\
0.485053255613921	0.336000000000014\\
0.486605128533181	0.334000000000014\\
0.487740604893389	0.332000000000013\\
0.489873931237913	0.330000000000013\\
0.491038505791189	0.328000000000013\\
0.493656720016236	0.326000000000013\\
0.495630709991594	0.324000000000013\\
0.497834335806069	0.322000000000013\\
0.499429903695569	0.320000000000012\\
0.502638411300346	0.318000000000012\\
0.504524243107571	0.316000000000012\\
0.50648713717362	0.314000000000012\\
0.508925475491237	0.312000000000012\\
0.510259995874592	0.310000000000012\\
0.512186295242927	0.308000000000012\\
0.515528233530886	0.306000000000012\\
0.517620748979034	0.304000000000012\\
0.519634446206674	0.302000000000012\\
0.521543911916199	0.300000000000012\\
0.523555677444	0.298000000000011\\
0.526012147351733	0.296000000000011\\
0.530585814521172	0.294000000000011\\
0.534491179211346	0.292000000000011\\
0.536933536058799	0.290000000000011\\
0.54000141147228	0.288000000000011\\
0.541907301826367	0.28600000000001\\
0.546794018830921	0.28400000000001\\
0.549592984157424	0.28200000000001\\
0.553269938519241	0.28000000000001\\
0.555568792845192	0.27800000000001\\
0.558335021790562	0.27600000000001\\
0.561693280292982	0.27400000000001\\
0.562817805172509	0.27200000000001\\
0.56521637507474	0.27000000000001\\
0.567290347223632	0.26800000000001\\
0.570019814248935	0.26600000000001\\
0.572469364803538	0.26400000000001\\
0.575401166686047	0.262000000000009\\
0.577465231860447	0.260000000000009\\
0.579819897335303	0.258000000000009\\
0.582470684499454	0.256000000000009\\
0.584248015935951	0.254000000000009\\
0.587110683352482	0.252000000000009\\
0.589700770250258	0.250000000000009\\
0.592485335873164	0.248000000000009\\
0.594303251667276	0.246000000000009\\
0.596693709743105	0.244000000000009\\
0.599754841343466	0.242000000000009\\
0.604202583698836	0.240000000000009\\
0.608088819538291	0.238000000000008\\
0.611595062744344	0.236000000000008\\
0.615822204737887	0.234000000000008\\
0.618457140405583	0.232000000000008\\
0.622072138764212	0.230000000000008\\
0.623829200636923	0.228000000000008\\
0.626688541461989	0.226000000000008\\
0.630684381228068	0.224000000000008\\
0.63492848314816	0.222000000000008\\
0.637374030292664	0.220000000000008\\
0.640306788465068	0.218000000000008\\
0.642223850310279	0.216000000000008\\
0.644751962570579	0.214000000000008\\
0.647485204433763	0.212000000000008\\
0.651079678907313	0.210000000000008\\
0.653510340930289	0.208000000000008\\
0.659107740273898	0.206000000000008\\
0.662576491645689	0.204000000000008\\
0.66523728527064	0.202000000000007\\
0.668973286594039	0.200000000000007\\
0.673928555906905	0.198000000000007\\
0.678150846168301	0.196000000000007\\
0.684447580100564	0.194000000000007\\
0.687996306867153	0.192000000000007\\
0.690789970610403	0.190000000000007\\
0.694914167547575	0.188000000000007\\
0.702763396736168	0.186000000000007\\
0.709576136377965	0.184000000000007\\
0.713735065639057	0.182000000000007\\
0.718086253960258	0.180000000000007\\
0.722563898242883	0.178000000000007\\
0.726307107266071	0.176000000000007\\
0.730232679957096	0.174000000000007\\
0.736012095291169	0.172000000000007\\
0.738124299426206	0.170000000000006\\
0.741367355673116	0.168000000000006\\
0.74796817120988	0.166000000000006\\
0.751266724926842	0.164000000000006\\
0.757248843342062	0.162000000000006\\
0.760050925554929	0.160000000000006\\
0.762236073671538	0.158000000000006\\
0.765313477186219	0.156000000000006\\
0.770706452354321	0.154000000000006\\
0.774451431438777	0.152000000000006\\
0.779568065393894	0.150000000000006\\
0.784350903977016	0.148000000000006\\
0.790927427247757	0.146000000000006\\
0.795471855635838	0.144000000000006\\
0.798249096301696	0.142000000000006\\
0.80649647978471	0.140000000000006\\
0.81230715345724	0.138000000000006\\
0.818015831497273	0.136000000000005\\
0.821216647503085	0.134000000000005\\
0.828012020755958	0.132000000000005\\
0.832294591693645	0.130000000000005\\
0.839579611061808	0.128000000000005\\
0.845844762721781	0.126000000000005\\
0.851426364167988	0.124000000000005\\
0.858190395990033	0.122000000000005\\
0.864543189202318	0.120000000000005\\
0.870039410975486	0.118000000000005\\
0.882547015863416	0.116000000000005\\
0.893995988516501	0.114000000000005\\
0.902019781225294	0.112000000000005\\
0.91288278280855	0.110000000000005\\
0.924262757979847	0.108000000000005\\
0.93110885308075	0.106000000000004\\
0.938949697528187	0.104000000000004\\
0.94673474258004	0.102000000000004\\
0.955413294120093	0.100000000000004\\
0.961763222890242	0.0980000000000041\\
0.976466879655542	0.0960000000000041\\
0.98648702640269	0.094000000000004\\
0.993087946904921	0.0920000000000039\\
1.00105994616759	0.0900000000000039\\
1.01244107555344	0.0880000000000037\\
1.01775398475079	0.0860000000000037\\
1.03564838387222	0.0840000000000036\\
1.04629613352139	0.0820000000000036\\
1.05581718600128	0.0800000000000035\\
1.06899702618722	0.0780000000000034\\
1.08218076288973	0.0760000000000034\\
1.0880599480332	0.0740000000000033\\
1.10122745645209	0.0720000000000033\\
1.1098048793298	0.0700000000000032\\
1.12003551159735	0.0680000000000032\\
1.13287184875289	0.0660000000000031\\
1.14345209947238	0.0640000000000031\\
1.16152446054177	0.0620000000000029\\
1.17220607555108	0.0600000000000028\\
1.18738790304868	0.0580000000000027\\
1.20410017781473	0.0560000000000027\\
1.23259237086485	0.0540000000000026\\
1.24221373959041	0.0520000000000025\\
1.26928098954054	0.0500000000000024\\
1.28731859011538	0.0480000000000023\\
1.29981725609174	0.0460000000000023\\
1.3173980897196	0.0440000000000021\\
1.33793879154108	0.042000000000002\\
1.36578932741632	0.0400000000000019\\
1.38975954019901	0.0380000000000018\\
1.44089301027836	0.0360000000000017\\
1.45838524585687	0.0340000000000017\\
1.48161542856432	0.0320000000000016\\
1.51818768879169	0.0300000000000015\\
1.55667279332368	0.0280000000000014\\
1.59817266684136	0.0260000000000012\\
1.63075304754834	0.0240000000000011\\
1.69892794126171	0.0220000000000011\\
1.74825040628843	0.020000000000001\\
1.78886600861721	0.0180000000000009\\
1.87059657430025	0.0160000000000008\\
1.95490856686531	0.0140000000000007\\
2.09340721348208	0.0120000000000006\\
2.26284639826045	0.0100000000000005\\
2.37730222835733	0.00800000000000045\\
2.7880960963753	0.00600000000000034\\
3.56380115209949	0.00400000000000023\\
20.45477833266	0.00200000000000011\\
229.142658696892	0\\
};
\addlegendentry{$N=1$,~, $\lrmse =7.040$, $\prmse =0.006$, $\gamma=40$}


==> figures/mse_N_1_K_20_G_5_SNR_40_I_20_Pratio_2_Nratio_2_alpha_3.4_cs.tex <==
\addplot [color=red, dashed,line width=0.6pt]
  table[row sep=crcr]{%
0.000900321453254836	1\\
0.0048566035885791	0.998986623429266\\
0.00943685232189041	0.997973246858533\\
0.0112508850622624	0.996959870287799\\
0.0131947632329864	0.995946493717065\\
0.0143620918933516	0.994933117146331\\
0.0166174796468689	0.993919740575598\\
0.0175102207705013	0.992906364004864\\
0.0188203991097352	0.99189298743413\\
0.0190892964181925	0.990879610863397\\
0.0201835306507528	0.989866234292663\\
0.0203595654383993	0.988852857721929\\
0.0208531597861499	0.987839481151196\\
0.0220683307944402	0.986826104580462\\
0.0231250731534454	0.985812728009728\\
0.0238561070353856	0.984799351438994\\
0.0243391987630746	0.983785974868261\\
0.0249594051276625	0.982772598297527\\
0.0253796575489073	0.981759221726793\\
0.0266822379610475	0.980745845156059\\
0.027329482183321	0.979732468585326\\
0.028097642526047	0.978719092014592\\
0.0289615963711917	0.977705715443858\\
0.0295211893782931	0.976692338873125\\
0.0299606759777546	0.975678962302391\\
0.0301338743093905	0.974665585731657\\
0.0307895140118402	0.973652209160924\\
0.0312456741122992	0.97263883259019\\
0.0317847187124179	0.971625456019456\\
0.0324389290974898	0.970612079448722\\
0.0332681956575345	0.969598702877989\\
0.0335823100657887	0.968585326307255\\
0.0342708739084191	0.967571949736521\\
0.0349892228565041	0.966558573165787\\
0.0355783792687856	0.965545196595054\\
0.0361908374206055	0.96453182002432\\
0.0365174811540396	0.963518443453586\\
0.0373002771875489	0.962505066882853\\
0.0380358073445147	0.961491690312119\\
0.0384037947459712	0.960478313741385\\
0.0389637873186553	0.959464937170651\\
0.0392855842280086	0.958451560599918\\
0.0398742051682392	0.957438184029184\\
0.0403003214621767	0.95642480745845\\
0.040635008768526	0.955411430887717\\
0.0411474447703016	0.954398054316983\\
0.0417127806977279	0.953384677746249\\
0.0419566272654491	0.952371301175516\\
0.0423870591504807	0.951357924604782\\
0.0429139705618313	0.950344548034048\\
0.0433417906377576	0.949331171463315\\
0.0435814114176805	0.948317794892581\\
0.0439430344540959	0.947304418321847\\
0.0445632022448289	0.946291041751113\\
0.0449774589756795	0.94527766518038\\
0.0454998685779907	0.944264288609646\\
0.0460001555585596	0.943250912038912\\
0.0464188559006934	0.942237535468179\\
0.0471790488081085	0.941224158897445\\
0.0475878198192475	0.940210782326711\\
0.0479270437278581	0.939197405755977\\
0.048258941051868	0.938184029185244\\
0.0485391400833741	0.93717065261451\\
0.0488216728836907	0.936157276043776\\
0.049181946980105	0.935143899473043\\
0.0497382380690835	0.934130522902309\\
0.0499972616121758	0.933117146331575\\
0.0512097014009676	0.932103769760841\\
0.0518509237362947	0.931090393190108\\
0.0522972556634086	0.930077016619374\\
0.052667236052299	0.92906364004864\\
0.0529176088078734	0.928050263477907\\
0.0534740586494756	0.927036886907173\\
0.0544446097171305	0.926023510336439\\
0.0547912164786643	0.925010133765706\\
0.0552383996174002	0.923996757194972\\
0.0557231468165678	0.922983380624238\\
0.055953053475284	0.921970004053504\\
0.0563427922024292	0.920956627482771\\
0.0564895600986807	0.919943250912037\\
0.0566681395888761	0.918929874341303\\
0.057249472606032	0.91791649777057\\
0.0576982441748311	0.916903121199836\\
0.0581421453241429	0.915889744629102\\
0.0587717772445781	0.914876368058368\\
0.0590783922058851	0.913862991487635\\
0.0593484211381588	0.912849614916901\\
0.0596993257686592	0.911836238346167\\
0.0598096125595661	0.910822861775434\\
0.0602483124156368	0.9098094852047\\
0.0605782166138343	0.908796108633966\\
0.0606899663127608	0.907782732063233\\
0.0608447751326789	0.906769355492499\\
0.0614165752496656	0.905755978921765\\
0.061829734993567	0.904742602351031\\
0.0620301194553408	0.903729225780298\\
0.0622428993854159	0.902715849209564\\
0.0626680234102155	0.90170247263883\\
0.063097201486151	0.900689096068097\\
0.0632496701188289	0.899675719497363\\
0.0637232253236978	0.898662342926629\\
0.0640674377234275	0.897648966355895\\
0.0644331211527068	0.896635589785162\\
0.0646946943052402	0.895622213214428\\
0.0649569973639524	0.894608836643694\\
0.0653110657639176	0.89359546007296\\
0.0655980354787705	0.892582083502227\\
0.0659743451828963	0.891568706931493\\
0.0664609782464933	0.890555330360759\\
0.0666812322155262	0.889541953790026\\
0.0671213516169776	0.888528577219292\\
0.0672522398363243	0.887515200648558\\
0.06747691418572	0.886501824077824\\
0.0681785429988474	0.885488447507091\\
0.068575464718564	0.884475070936357\\
0.0687131747365533	0.883461694365623\\
0.0690578540857803	0.88244831779489\\
0.0697780663197552	0.881434941224156\\
0.0702016624997554	0.880421564653422\\
0.0705315118372571	0.879408188082689\\
0.0710185718276768	0.878394811511955\\
0.0714323704356462	0.877381434941221\\
0.0721226077008376	0.876368058370487\\
0.0724286624512204	0.875354681799754\\
0.0726828857006399	0.87434130522902\\
0.0731092796396985	0.873327928658286\\
0.073239862102965	0.872314552087553\\
0.073948030346387	0.871301175516819\\
0.0742115513619363	0.870287798946085\\
0.0748880820044037	0.869274422375351\\
0.0751252035872443	0.868261045804618\\
0.0754636989324907	0.867247669233884\\
0.0756543103905716	0.866234292663151\\
0.076123660282262	0.865220916092417\\
0.0762590893992216	0.864207539521683\\
0.0765935746201862	0.863194162950949\\
0.0770527875941732	0.862180786380216\\
0.0772596513650952	0.861167409809482\\
0.077437915406424	0.860154033238748\\
0.077707414828726	0.859140656668015\\
0.0778617503315101	0.858127280097281\\
0.0781027288056441	0.857113903526547\\
0.0784274625675988	0.856100526955814\\
0.0786798666317862	0.85508715038508\\
0.0793058678794612	0.854073773814346\\
0.0794952512379377	0.853060397243612\\
0.0800141401328589	0.852047020672879\\
0.0802738112245665	0.851033644102145\\
0.0804291704451183	0.850020267531411\\
0.0810228389768712	0.849006890960678\\
0.08140030189492	0.847993514389944\\
0.0819979224037663	0.84698013781921\\
0.0824529806808432	0.845966761248476\\
0.0828919276030988	0.844953384677743\\
0.0830633309269846	0.843940008107009\\
0.083265855724171	0.842926631536275\\
0.0839080214686893	0.841913254965541\\
0.0843745488828119	0.840899878394808\\
0.084668820415305	0.839886501824074\\
0.0849330305911412	0.83887312525334\\
0.0851310483048725	0.837859748682606\\
0.0854202747724232	0.836846372111873\\
0.0856673649382516	0.835832995541139\\
0.085989355552454	0.834819618970405\\
0.0864152307769265	0.833806242399672\\
0.0868002147606525	0.832792865828938\\
0.0869600352141782	0.831779489258204\\
0.0872352640131595	0.83076611268747\\
0.0874878674169414	0.829752736116737\\
0.0875528939265324	0.828739359546003\\
0.087894610958828	0.827725982975269\\
0.0880956327976142	0.826712606404535\\
0.0884377542626906	0.825699229833802\\
0.0886334180485701	0.824685853263068\\
0.0890430717383051	0.823672476692334\\
0.0892031413415574	0.822659100121601\\
0.0896143004140906	0.821645723550867\\
0.0901609597261136	0.820632346980133\\
0.0903291622834781	0.819618970409399\\
0.0909623013809202	0.818605593838666\\
0.0914765534302154	0.817592217267932\\
0.0916524072988921	0.816578840697198\\
0.0920022161196342	0.815565464126465\\
0.0926779140053128	0.814552087555731\\
0.0929465387522836	0.813538710984997\\
0.0934070033388386	0.812525334414263\\
0.0939586923762928	0.81151195784353\\
0.0942972795975449	0.810498581272796\\
0.0949823934640258	0.809485204702062\\
0.0951457550731034	0.808471828131328\\
0.0955484933800353	0.807458451560595\\
0.0956474678828621	0.806445074989861\\
0.0960990555678359	0.805431698419127\\
0.0965396591340604	0.804418321848393\\
0.0968006781725216	0.80340494527766\\
0.0969257284525035	0.802391568706926\\
0.0973720090394752	0.801378192136192\\
0.0977080477417911	0.800364815565458\\
0.098205509934408	0.799351438994725\\
0.0984045001660444	0.798338062423991\\
0.0987340967885294	0.797324685853257\\
0.098946608296009	0.796311309282523\\
0.0991434202913278	0.79529793271179\\
0.0994286324337963	0.794284556141056\\
0.0996939815481413	0.793271179570322\\
0.0999441812767255	0.792257802999588\\
0.100035514998246	0.791244426428855\\
0.100244886156414	0.790231049858121\\
0.100783200433254	0.789217673287387\\
0.101052173244586	0.788204296716654\\
0.101561811764269	0.78719092014592\\
0.102259072820223	0.786177543575186\\
0.102390232066522	0.785164167004452\\
0.102678128498647	0.784150790433719\\
0.102959292197479	0.783137413862985\\
0.103438899849568	0.782124037292251\\
0.103762187552865	0.781110660721517\\
0.104200605197993	0.780097284150784\\
0.104711327435936	0.77908390758005\\
0.104925198946192	0.778070531009316\\
0.105066445556988	0.777057154438582\\
0.105339843150409	0.776043777867849\\
0.105687740991275	0.775030401297115\\
0.105979923940371	0.774017024726381\\
0.106341949234734	0.773003648155647\\
0.107119061096273	0.771990271584914\\
0.10732511560298	0.77097689501418\\
0.107515959610997	0.769963518443446\\
0.107770307028435	0.768950141872712\\
0.107991633485032	0.767936765301979\\
0.108250595733822	0.766923388731245\\
0.108630832511898	0.765910012160511\\
0.10905691391746	0.764896635589777\\
0.109710497801606	0.763883259019044\\
0.109839061442334	0.76286988244831\\
0.110066549216825	0.761856505877576\\
0.110497583399426	0.760843129306843\\
0.110671189817913	0.759829752736109\\
0.110921802927884	0.758816376165375\\
0.111220738366351	0.757802999594641\\
0.111407785690142	0.756789623023908\\
0.111608235824506	0.755776246453174\\
0.111866682564328	0.75476286988244\\
0.112096566585819	0.753749493311706\\
0.11224628038208	0.752736116740973\\
0.112490081284369	0.751722740170239\\
0.113363059912509	0.750709363599505\\
0.113638713424425	0.749695987028771\\
0.11422513116529	0.748682610458038\\
0.114388262841488	0.747669233887304\\
0.114617390708127	0.74665585731657\\
0.114887944076312	0.745642480745837\\
0.115101854151598	0.744629104175103\\
0.115218630583564	0.743615727604369\\
0.115435592109054	0.742602351033635\\
0.115887339490185	0.741588974462902\\
0.116125560083897	0.740575597892168\\
0.116759817749139	0.739562221321434\\
0.117117516041448	0.7385488447507\\
0.117921350514034	0.737535468179967\\
0.118487339442187	0.736522091609233\\
0.118765623184906	0.735508715038499\\
0.118953164972178	0.734495338467765\\
0.119519772778298	0.733481961897032\\
0.119814105276836	0.732468585326298\\
0.120056174563416	0.731455208755564\\
0.120349452757016	0.73044183218483\\
0.120472917876509	0.729428455614097\\
0.120645550217239	0.728415079043363\\
0.121030525164299	0.727401702472629\\
0.121557827931718	0.726388325901895\\
0.121819593052216	0.725374949331162\\
0.122006510244324	0.724361572760428\\
0.122464766092562	0.723348196189694\\
0.122952104595208	0.72233481961896\\
0.123050768114856	0.721321443048227\\
0.123359258929765	0.720308066477493\\
0.123718219640137	0.719294689906759\\
0.124017791325715	0.718281313336025\\
0.124155904319961	0.717267936765292\\
0.124564854727583	0.716254560194558\\
0.124881324457167	0.715241183623824\\
0.125249921509033	0.71422780705309\\
0.125402924377712	0.713214430482357\\
0.125735512393868	0.712201053911623\\
0.126096999428823	0.711187677340889\\
0.126436092889537	0.710174300770155\\
0.126628801599331	0.709160924199422\\
0.126841388742807	0.708147547628688\\
0.127473224438941	0.707134171057954\\
0.127720184988088	0.70612079448722\\
0.12783077176705	0.705107417916487\\
0.128026492328021	0.704094041345753\\
0.128343374242187	0.703080664775019\\
0.128644811181573	0.702067288204285\\
0.128911128336057	0.701053911633552\\
0.129241716589711	0.700040535062818\\
0.129453612135661	0.699027158492084\\
0.129751509726395	0.69801378192135\\
0.130146394576344	0.697000405350617\\
0.13033182645721	0.695987028779883\\
0.130625187483608	0.694973652209149\\
0.130954727127234	0.693960275638415\\
0.131465938272233	0.692946899067682\\
0.131601637932961	0.691933522496948\\
0.132106357638768	0.690920145926214\\
0.132439688477744	0.68990676935548\\
0.13252379888095	0.688893392784747\\
0.132682366141296	0.687880016214013\\
0.132998705429164	0.686866639643279\\
0.133201871707916	0.685853263072545\\
0.133777566120675	0.684839886501812\\
0.133851964524241	0.683826509931078\\
0.134200339061401	0.682813133360344\\
0.134710118701098	0.68179975678961\\
0.134926151129808	0.680786380218877\\
0.135323554391024	0.679773003648143\\
0.135628390595869	0.678759627077409\\
0.135719492567711	0.677746250506675\\
0.136001892638387	0.676732873935942\\
0.136235300527928	0.675719497365208\\
0.136563399090415	0.674706120794474\\
0.136748252392171	0.67369274422374\\
0.137186048181828	0.672679367653007\\
0.137370859584361	0.671665991082273\\
0.137888744520164	0.670652614511539\\
0.13821490430537	0.669639237940805\\
0.13871191992698	0.668625861370072\\
0.139283466683872	0.667612484799338\\
0.139444865860756	0.666599108228604\\
0.139740420900171	0.66558573165787\\
0.140127307155952	0.664572355087137\\
0.140413019163286	0.663558978516403\\
0.141101100063553	0.662545601945669\\
0.141500010629883	0.661532225374936\\
0.141903079814476	0.660518848804202\\
0.142525412750792	0.659505472233468\\
0.142717137322908	0.658492095662734\\
0.142917842566692	0.657478719092001\\
0.143217292884844	0.656465342521267\\
0.143445334691778	0.655451965950533\\
0.143808234126824	0.654438589379799\\
0.143995847433062	0.653425212809066\\
0.144377572455883	0.652411836238332\\
0.144770759166055	0.651398459667598\\
0.14519683551496	0.650385083096864\\
0.145564491356425	0.649371706526131\\
0.146091935370734	0.648358329955397\\
0.146334846982768	0.647344953384663\\
0.146664632460133	0.646331576813929\\
0.146879798112381	0.645318200243196\\
0.147113878007294	0.644304823672462\\
0.147965282227509	0.643291447101728\\
0.148306814815161	0.642278070530994\\
0.148631672450606	0.641264693960261\\
0.149030565510026	0.640251317389527\\
0.149345075418468	0.639237940818793\\
0.14982899453187	0.638224564248059\\
0.150126673590294	0.637008512363179\\
0.150320690761698	0.635995135792445\\
0.150718065797011	0.634981759221711\\
0.150999944677249	0.633968382650978\\
0.151112787647961	0.632955006080244\\
0.151559686080618	0.63194162950951\\
0.15170379610527	0.630928252938776\\
0.152195665751929	0.629914876368043\\
0.152370670918923	0.628901499797309\\
0.152783635922143	0.627888123226575\\
0.152962663410479	0.626874746655841\\
0.15306029503071	0.625861370085108\\
0.153119859008243	0.624847993514374\\
0.153507422746853	0.62383461694364\\
0.153726163807806	0.622821240372906\\
0.154305335456678	0.621807863802173\\
0.154494845781297	0.620794487231439\\
0.154945291071563	0.619781110660705\\
0.15513483624872	0.618565058775825\\
0.155417913165498	0.617551682205091\\
0.155912327137181	0.616538305634357\\
0.156094735389355	0.615524929063623\\
0.156198294248606	0.61451155249289\\
0.156680044635838	0.613498175922156\\
0.156982587613953	0.612484799351422\\
0.157161982681737	0.611471422780688\\
0.157592729224223	0.610458046209955\\
0.157753980169581	0.609444669639221\\
0.158152663281502	0.608431293068487\\
0.15851753960795	0.607417916497753\\
0.15866783156366	0.60640453992702\\
0.158888725434778	0.605391163356286\\
0.159188414268712	0.604377786785552\\
0.159520613939149	0.603364410214818\\
0.160235613525763	0.602351033644085\\
0.160409831911007	0.601337657073351\\
0.160571481223773	0.600324280502617\\
0.160971927040317	0.599310903931883\\
0.161151523927969	0.59829752736115\\
0.161563468967901	0.597284150790416\\
0.161951901321922	0.596270774219682\\
0.162304027349943	0.595257397648948\\
0.162457237513275	0.594244021078215\\
0.162824002717275	0.593230644507481\\
0.163133357499428	0.592217267936747\\
0.163323021459548	0.591203891366013\\
0.1634510049195	0.59019051479528\\
0.163768359069743	0.589177138224546\\
0.164216142871231	0.588163761653812\\
0.164936384930508	0.587150385083078\\
0.165137720159409	0.586137008512345\\
0.165534963638267	0.585123631941611\\
0.165961491098483	0.584110255370877\\
0.166591367524797	0.583096878800143\\
0.166970430880311	0.58208350222941\\
0.167589247170653	0.581070125658676\\
0.167996266721832	0.580056749087942\\
0.168337200451731	0.579043372517208\\
0.168871406700711	0.578029995946475\\
0.169335148827944	0.577016619375741\\
0.169854257923313	0.576003242805007\\
0.170023971667922	0.574989866234273\\
0.170470546449304	0.57397648966354\\
0.170829967000611	0.572963113092806\\
0.171672274089238	0.571949736522072\\
0.172111263358812	0.570936359951338\\
0.172506716205694	0.569922983380605\\
0.173263390230974	0.568909606809871\\
0.173938363251299	0.567896230239137\\
0.174133364736342	0.566882853668403\\
0.174713389045964	0.56586947709767\\
0.174895993407963	0.564856100526936\\
0.175409893306206	0.563842723956202\\
0.175716359946854	0.562829347385468\\
0.176158632885199	0.561815970814735\\
0.176608713195609	0.560802594244001\\
0.176705643289118	0.559789217673267\\
0.177228724452053	0.558775841102533\\
0.177668608483178	0.5577624645318\\
0.17788810780083	0.556749087961066\\
0.178022285707482	0.555735711390332\\
0.178600296511694	0.554722334819598\\
0.178862107268841	0.553708958248865\\
0.179251174911458	0.552695581678131\\
0.179623430654879	0.551682205107397\\
0.179904907468824	0.550668828536663\\
0.180207945002362	0.54965545196593\\
0.180648066434044	0.548642075395196\\
0.181292544290977	0.547628698824462\\
0.181495761254143	0.546615322253728\\
0.181961880034606	0.545601945682995\\
0.18220921705054	0.544588569112261\\
0.182406501492295	0.543575192541527\\
0.182713251946834	0.542561815970793\\
0.183272112033095	0.54154843940006\\
0.184085652206408	0.540535062829326\\
0.184605027243375	0.539521686258592\\
0.184845833603011	0.538508309687858\\
0.185073497162409	0.537494933117125\\
0.185392211689492	0.536481556546391\\
0.185717651497787	0.535468179975657\\
0.185993868093366	0.534454803404923\\
0.186441366435889	0.53344142683419\\
0.186928245653925	0.532428050263456\\
0.187126603794488	0.531414673692722\\
0.187284499467102	0.530401297121988\\
0.187338811300203	0.529387920551255\\
0.187581544404773	0.528374543980521\\
0.188317439953614	0.527361167409787\\
0.188772047744066	0.526347790839053\\
0.18907983450062	0.52533441426832\\
0.189353763962234	0.524321037697586\\
0.189824715266928	0.523307661126852\\
0.190049928604501	0.522294284556118\\
0.190423486996609	0.521280907985385\\
0.190567812440337	0.520267531414651\\
0.191147214723512	0.519254154843917\\
0.191738790017764	0.518240778273183\\
0.191926506951408	0.51722740170245\\
0.192150751208721	0.516214025131716\\
0.192504955111216	0.515200648560982\\
0.192857194073977	0.514187271990248\\
0.192959179990032	0.513173895419515\\
0.193338611501135	0.512160518848781\\
0.193764446472906	0.511147142278047\\
0.194405499665661	0.510133765707314\\
0.194592041884916	0.50912038913658\\
0.194866898570163	0.508107012565846\\
0.195106649210249	0.507093635995112\\
0.195678959274882	0.506080259424379\\
0.195867517987321	0.505066882853645\\
0.196096589481544	0.504053506282911\\
0.19657022134612	0.503040129712177\\
0.196942408023218	0.502026753141444\\
0.197465589396269	0.50101337657071\\
0.197566219528031	0.499999999999976\\
0.197755245505672	0.498986623429242\\
0.198176604336139	0.497973246858509\\
0.198400862049982	0.496959870287775\\
0.19881792628626	0.495946493717041\\
0.199188122981027	0.494933117146308\\
0.199471291887773	0.493919740575574\\
0.199750373362765	0.492906364004841\\
0.200318629181816	0.491892987434107\\
0.200510385563248	0.490879610863373\\
0.200651630267165	0.48986623429264\\
0.201105765475905	0.488852857721906\\
0.201412998073579	0.487839481151172\\
0.201963549234357	0.486826104580439\\
0.202545024244545	0.485812728009705\\
0.203162351014144	0.484799351438971\\
0.20377868001581	0.483785974868238\\
0.204598464516837	0.482772598297504\\
0.204846360898978	0.481759221726771\\
0.205121245404802	0.480745845156037\\
0.20546601387894	0.479732468585303\\
0.205799450878601	0.47871909201457\\
0.206126497827487	0.477705715443836\\
0.206506031283541	0.476692338873102\\
0.207104354758102	0.475678962302369\\
0.207601241803945	0.474665585731635\\
0.207933854036456	0.473652209160901\\
0.208191756624522	0.472638832590168\\
0.208646729159374	0.471625456019434\\
0.20906146356679	0.4706120794487\\
0.209408066080505	0.469598702877967\\
0.209987579592118	0.468585326307233\\
0.210490614216435	0.4675719497365\\
0.210858472206744	0.466558573165766\\
0.211495334509803	0.465545196595032\\
0.211797714175913	0.464531820024299\\
0.212408681170212	0.463518443453565\\
0.212793748947646	0.462505066882831\\
0.213305646835382	0.461491690312098\\
0.213743456481388	0.460478313741364\\
0.213932026905166	0.459464937170631\\
0.214288441127086	0.458451560599897\\
0.214695217560117	0.457438184029163\\
0.215109414433784	0.45642480745843\\
0.215720409126537	0.455411430887696\\
0.216243328182568	0.454398054316963\\
0.216568402012812	0.453384677746229\\
0.217036202858287	0.452371301175495\\
0.217402134262838	0.451357924604762\\
0.217608815654786	0.450344548034028\\
0.217995076982562	0.449331171463294\\
0.218561246392169	0.448317794892561\\
0.218909361443558	0.447304418321827\\
0.219494865095621	0.446291041751093\\
0.220352493660312	0.44527766518036\\
0.220668199144846	0.444264288609626\\
0.220959644220975	0.443250912038893\\
0.221526848426692	0.442237535468159\\
0.222033037909869	0.441224158897425\\
0.222372248911599	0.440210782326691\\
0.222784043603497	0.439197405755958\\
0.223140524559781	0.438184029185224\\
0.223581749650868	0.437170652614491\\
0.223797765500125	0.436157276043757\\
0.224265917515751	0.435143899473023\\
0.224815722901429	0.434130522902289\\
0.225274730767493	0.433117146331556\\
0.225587459753366	0.432103769760822\\
0.226383259575362	0.431090393190088\\
0.226742488278683	0.430077016619355\\
0.227153868072574	0.429063640048621\\
0.227600280862172	0.428050263477888\\
0.227862219385594	0.427036886907154\\
0.228355451758772	0.42602351033642\\
0.228701978520608	0.425010133765687\\
0.229573449372839	0.423996757194953\\
0.230070662434557	0.42298338062422\\
0.230197840841427	0.421970004053486\\
0.230475479544188	0.420956627482752\\
0.230807300546515	0.419943250912019\\
0.231116609605614	0.418929874341285\\
0.23173952313827	0.417916497770552\\
0.232123426626138	0.416903121199818\\
0.23305319333404	0.415889744629084\\
0.233522728303719	0.41487636805835\\
0.233992850192809	0.413862991487617\\
0.234765768400008	0.412849614916883\\
0.235282790418819	0.41183623834615\\
0.23595219646304	0.410822861775416\\
0.236192223504376	0.409809485204682\\
0.23633118718021	0.408796108633949\\
0.236594946535933	0.407782732063215\\
0.237098259081839	0.406769355492481\\
0.237436278591445	0.405755978921748\\
0.237780254974327	0.404742602351014\\
0.238049229385623	0.40372922578028\\
0.238389808979706	0.402715849209547\\
0.238965696145907	0.401702472638813\\
0.239396328204701	0.400689096068079\\
0.240270947671267	0.399675719497346\\
0.240923496140918	0.398662342926612\\
0.241355579979006	0.397648966355879\\
0.242045644795846	0.396635589785145\\
0.24271359324211	0.395622213214412\\
0.242938772900316	0.394608836643678\\
0.243847931134258	0.393595460072944\\
0.244455268923867	0.39258208350221\\
0.244828670395223	0.391568706931477\\
0.245335873724085	0.390555330360743\\
0.246200189578494	0.38954195379001\\
0.246635785409003	0.388528577219276\\
0.247106412235906	0.387515200648542\\
0.247688239896762	0.386501824077809\\
0.24833653590583	0.385488447507075\\
0.248708560710055	0.384475070936341\\
0.249337007950613	0.383461694365608\\
0.249620273456743	0.382448317794874\\
0.250241409903943	0.381434941224141\\
0.250993971077551	0.380421564653407\\
0.25135595040325	0.379408188082673\\
0.251950492442821	0.37839481151194\\
0.252662850789633	0.377381434941206\\
0.253240759332128	0.376368058370472\\
0.254005892973157	0.375354681799738\\
0.254400721037887	0.374341305229005\\
0.254804537656305	0.373327928658271\\
0.255406426661948	0.372314552087538\\
0.256038852648159	0.371301175516804\\
0.256754312345817	0.37028779894607\\
0.257066514094437	0.369274422375337\\
0.257409349176629	0.368261045804603\\
0.258001740059255	0.367247669233869\\
0.258816328867893	0.366234292663136\\
0.259176522425846	0.365220916092402\\
0.259785027024936	0.364207539521668\\
0.260131941319851	0.363194162950935\\
0.260911878989855	0.362180786380201\\
0.26183821973913	0.361167409809467\\
0.262276954938871	0.360154033238734\\
0.262585379309968	0.359140656668\\
0.262911006528893	0.358127280097266\\
0.263645423910956	0.357113903526533\\
0.264483394051694	0.356100526955799\\
0.2650917337001	0.355087150385066\\
0.265564385366601	0.354073773814332\\
0.266007341370125	0.353060397243598\\
0.266467061583059	0.352047020672865\\
0.267101964456324	0.351033644102131\\
0.267579156651863	0.350020267531397\\
0.267989321771803	0.349006890960664\\
0.268334246323216	0.34799351438993\\
0.269091058751284	0.346980137819196\\
0.269314078451585	0.345966761248463\\
0.269956486184622	0.344953384677729\\
0.270370461591366	0.343940008106995\\
0.270635631349489	0.342926631536262\\
0.270987323732896	0.341913254965528\\
0.271691683721856	0.340899878394795\\
0.271991548343999	0.339886501824061\\
0.27321763875372	0.338873125253327\\
0.273609712853997	0.337859748682594\\
0.274109952627837	0.33684637211186\\
0.274497164906243	0.335832995541126\\
0.27500898647177	0.334819618970393\\
0.275753764499247	0.333806242399659\\
0.276844973703191	0.332792865828925\\
0.277745111558672	0.331779489258192\\
0.278166082652188	0.330766112687458\\
0.278652611785715	0.329752736116724\\
0.279280847286899	0.328739359545991\\
0.280139037313892	0.327725982975257\\
0.281004613156983	0.326712606404523\\
0.281594226636458	0.32569922983379\\
0.282121551663642	0.324685853263056\\
0.282975564624036	0.323672476692322\\
0.283802305185772	0.322659100121588\\
0.284240848000771	0.321645723550855\\
0.284637130070368	0.320632346980121\\
0.285458306856545	0.319618970409388\\
0.286115109008844	0.318605593838654\\
0.286453501272811	0.31759221726792\\
0.287060388603488	0.316578840697187\\
0.287852183941855	0.315565464126453\\
0.288218011699008	0.314552087555719\\
0.288610026085512	0.313538710984986\\
0.289065859524304	0.312525334414252\\
0.289895142778069	0.311511957843518\\
0.290761241505074	0.310498581272785\\
0.291440518604649	0.309485204702051\\
0.292035991639794	0.308471828131317\\
0.292333138863623	0.307458451560584\\
0.293119571937797	0.30644507498985\\
0.294021944598885	0.305431698419117\\
0.294268857405664	0.304418321848383\\
0.295250118226157	0.303404945277649\\
0.295796968891404	0.302391568706915\\
0.296383699648654	0.301378192136182\\
0.296955303607971	0.300364815565448\\
0.29767632130327	0.299351438994714\\
0.298517439664083	0.298338062423981\\
0.299657443789074	0.297324685853247\\
0.300308612751174	0.296311309282513\\
0.300837300014825	0.29529793271178\\
0.30154638788305	0.294284556141046\\
0.30241843244253	0.293271179570312\\
0.302943304980366	0.292257802999579\\
0.303451060592638	0.291244426428845\\
0.304481275046525	0.290231049858111\\
0.304853658940004	0.289217673287378\\
0.305740382064627	0.288204296716644\\
0.306531709358429	0.28719092014591\\
0.307162095158133	0.286177543575177\\
0.307882423918617	0.285164167004443\\
0.308571011230344	0.284150790433709\\
0.309685433963178	0.283137413862976\\
0.310900429950004	0.282124037292242\\
0.311152152827284	0.281110660721509\\
0.311973621767786	0.280097284150775\\
0.313283637653458	0.279083907580041\\
0.314264773059987	0.278070531009308\\
0.314619363411169	0.277057154438574\\
0.315523627639695	0.276043777867841\\
0.316283882982502	0.275030401297107\\
0.316791378645813	0.274017024726373\\
0.318348846195283	0.27300364815564\\
0.318925488156535	0.271990271584906\\
0.320388540752316	0.270976895014172\\
0.320857958516674	0.269963518443439\\
0.321782186633997	0.268950141872705\\
0.322448139421311	0.267936765301971\\
0.323155480324946	0.266923388731238\\
0.323963605026154	0.265910012160504\\
0.325745639369752	0.26489663558977\\
0.326323225384144	0.263883259019037\\
0.326987026835584	0.262869882448303\\
0.327773308199066	0.261856505877569\\
0.328715946872929	0.260843129306836\\
0.329491986757344	0.259829752736102\\
0.330019059344043	0.258816376165368\\
0.33094881670576	0.257802999594635\\
0.331524518558475	0.256789623023901\\
0.332070383321701	0.255776246453167\\
0.332778665396938	0.254762869882434\\
0.333462496705648	0.2537494933117\\
0.33490303450522	0.252736116740967\\
0.336268394106862	0.251722740170233\\
0.336835940106307	0.250709363599499\\
0.337738317644086	0.249695987028765\\
0.338516569457493	0.248682610458032\\
0.339105016961456	0.247669233887298\\
0.339850616698054	0.246655857316565\\
0.340466541200879	0.245642480745831\\
0.34139715569842	0.244629104175097\\
0.342041067370917	0.243615727604364\\
0.342982588531661	0.24260235103363\\
0.343921745980284	0.241588974462897\\
0.345076028589191	0.240575597892163\\
0.346497715644886	0.239562221321429\\
0.347326739792369	0.238548844750696\\
0.348398266375915	0.237535468179962\\
0.349431270631421	0.236522091609228\\
0.350110978585298	0.235508715038495\\
0.351171535003102	0.234495338467761\\
0.351804783524804	0.233481961897028\\
0.353402200513984	0.232468585326294\\
0.353982110826728	0.23145520875556\\
0.35557925499838	0.230441832184827\\
0.357063704983422	0.229428455614093\\
0.357831143276057	0.228415079043359\\
0.35924824014491	0.227401702472626\\
0.359716898252649	0.226388325901892\\
0.360366058158846	0.225374949331159\\
0.361069494721955	0.224361572760425\\
0.361598271992778	0.223348196189691\\
0.362506054078012	0.222334819618958\\
0.363438861390655	0.221321443048224\\
0.365175391491194	0.22030806647749\\
0.365618501077568	0.219294689906757\\
0.366289263139544	0.218281313336023\\
0.366914845992322	0.217267936765289\\
0.368504275129249	0.216254560194556\\
0.371996763944942	0.215241183623822\\
0.373375891717202	0.214227807053089\\
0.373878070794827	0.213214430482355\\
0.374993192024227	0.212201053911621\\
0.375658104135657	0.211187677340888\\
0.376314081665742	0.210174300770154\\
0.377752503258325	0.209160924199421\\
0.379289999954762	0.208147547628687\\
0.380313865644095	0.207134171057953\\
0.38275893290699	0.20612079448722\\
0.383304631449557	0.205107417916486\\
0.38474437710977	0.204094041345752\\
0.385808507650316	0.203080664775019\\
0.387591457801255	0.202067288204285\\
0.389933264487689	0.201053911633552\\
0.390259322063366	0.200040535062818\\
0.391313432401045	0.199027158492084\\
0.392746101479168	0.198013781921351\\
0.393345147949361	0.197000405350617\\
0.394733184159836	0.195987028779884\\
0.39776209674292	0.19497365220915\\
0.399424727186167	0.193960275638416\\
0.400499193836093	0.192946899067683\\
0.401752762848118	0.191933522496949\\
0.403337378652125	0.190920145926216\\
0.40444821564161	0.189906769355482\\
0.405898346939225	0.188893392784748\\
0.406263187340836	0.187880016214015\\
0.4071315781021	0.186866639643281\\
0.408119475870747	0.185853263072547\\
0.410185095724682	0.184839886501814\\
0.410684633774263	0.18382650993108\\
0.412712903575949	0.182813133360347\\
0.413700008940517	0.181799756789613\\
0.415210877060186	0.180786380218879\\
0.416937053190951	0.179773003648146\\
0.417639416555998	0.178759627077412\\
0.41894699272496	0.177746250506679\\
0.420585948586131	0.176732873935945\\
0.421582691150346	0.175719497365211\\
0.422901680882348	0.174706120794478\\
0.424226610939789	0.173692744223744\\
0.426177947918644	0.172679367653011\\
0.427389171811979	0.171665991082277\\
0.428355158423976	0.170652614511543\\
0.430049157578705	0.16963923794081\\
0.43242360591006	0.168625861370076\\
0.433437490835759	0.167612484799343\\
0.434484411145224	0.166599108228609\\
0.435905841266972	0.165585731657875\\
0.438422079052418	0.164572355087142\\
0.439636924903143	0.163558978516408\\
0.440635641370039	0.162545601945674\\
0.443930180259169	0.161532225374941\\
0.445268086546886	0.160518848804207\\
0.446541405271485	0.159505472233474\\
0.449396313520175	0.15849209566274\\
0.450485526018609	0.157478719092006\\
0.452656672092154	0.156465342521273\\
0.455157267373629	0.155451965950539\\
0.455722149273926	0.154438589379806\\
0.45707051245233	0.153425212809072\\
0.458181946788505	0.152411836238338\\
0.459847700397917	0.151398459667605\\
0.461777819314656	0.150385083096871\\
0.464630173384901	0.149371706526138\\
0.467090438674794	0.148358329955404\\
0.468784085978205	0.14734495338467\\
0.470809771703812	0.146331576813937\\
0.472332333179802	0.145318200243203\\
0.473585549684201	0.14430482367247\\
0.475234672463419	0.143291447101736\\
0.478304182172156	0.142278070531002\\
0.479050343910373	0.141264693960269\\
0.480045381639194	0.140251317389535\\
0.480507576759664	0.139237940818801\\
0.482868942501694	0.138224564248068\\
0.48525156372714	0.137211187677334\\
0.48851184356581	0.136197811106601\\
0.490157613045818	0.135184434535867\\
0.49260183983795	0.134171057965133\\
0.494566291812779	0.1331576813944\\
0.496581717795164	0.132144304823666\\
0.497547718522446	0.131130928252933\\
0.49868347760003	0.130117551682199\\
0.499463640934216	0.129104175111465\\
0.501839042417706	0.128090798540732\\
0.502945304522174	0.127077421969998\\
0.503819205686311	0.126064045399265\\
0.505318807285549	0.125050668828531\\
0.507832102976108	0.124037292257797\\
0.509356720807379	0.123023915687064\\
0.51073649201066	0.12201053911633\\
0.512016536509591	0.120997162545596\\
0.514415174288577	0.119983785974863\\
0.515686442436096	0.118970409404129\\
0.517640894734813	0.117957032833396\\
0.518614585192021	0.116943656262662\\
0.520811444877339	0.115930279691928\\
0.522099262253913	0.114916903121195\\
0.524031442956893	0.113903526550461\\
0.52729022907175	0.112890149979727\\
0.529537203469896	0.111876773408994\\
0.532612637350041	0.11086339683826\\
0.535417677602105	0.109850020267526\\
0.538689249532414	0.108836643696793\\
0.543428759815101	0.107823267126059\\
0.546013905791289	0.106809890555326\\
0.547687052819242	0.105796513984592\\
0.548573883649202	0.104783137413858\\
0.551014888774867	0.103769760843125\\
0.554130401702973	0.102756384272391\\
0.556159279813342	0.101743007701657\\
0.558391588297689	0.100729631130924\\
0.560119548936906	0.0997162545601901\\
0.562873123657831	0.0987028779894564\\
0.56493695217049	0.0976895014187228\\
0.570159839184915	0.0966761248479892\\
0.571447348722959	0.0956627482772555\\
0.57506829674372	0.0946493717065219\\
0.579626817163384	0.0936359951357882\\
0.582288569405617	0.0926226185650546\\
0.583952982003144	0.091609241994321\\
0.586288069941367	0.0905958654235873\\
0.589645958272912	0.0895824888528537\\
0.594317377536529	0.0885691122821201\\
0.598240845285198	0.0875557357113864\\
0.599581620738127	0.0865423591406528\\
0.60321858592863	0.0855289825699191\\
0.606281543566147	0.0845156059991855\\
0.609856946689039	0.0835022294284519\\
0.61468240582492	0.0824888528577182\\
0.615823490274101	0.0814754762869846\\
0.617802057907952	0.080462099716251\\
0.621644325049526	0.0794487231455174\\
0.625694225020512	0.0784353465747838\\
0.627562107791702	0.0774219700040502\\
0.630071286781923	0.0764085934333165\\
0.634196223343887	0.0753952168625829\\
0.639031695525717	0.0743818402918492\\
0.641218487184556	0.0733684637211156\\
0.644973917083647	0.072355087150382\\
0.646677454074956	0.0713417105796483\\
0.649177997185689	0.0703283340089147\\
0.652592613464278	0.0693149574381811\\
0.655854295054948	0.0683015808674474\\
0.659218205564665	0.0672882042967138\\
0.663381391965261	0.0662748277259801\\
0.667591475638103	0.0652614511552464\\
0.671183489305087	0.0642480745845128\\
0.673062583205027	0.0632346980137791\\
0.681419973688738	0.0622213214430456\\
0.689157009460432	0.0612079448723118\\
0.692541189153414	0.0601945683015782\\
0.696982279937049	0.0591811917308446\\
0.702659052832547	0.0581678151601109\\
0.70785346951987	0.0571544385893773\\
0.713497248857891	0.0561410620186437\\
0.717822107624458	0.05512768544791\\
0.72099050549701	0.0541143088771764\\
0.727259137133291	0.0531009323064427\\
0.730857703169633	0.0520875557357091\\
0.739427298259043	0.0510741791649755\\
0.741841050790577	0.0500608025942418\\
0.744891545940285	0.0490474260235082\\
0.749038839724629	0.0480340494527746\\
0.751042988197226	0.0470206728820409\\
0.756691522326885	0.0460072963113073\\
0.761351034321933	0.0449939197405737\\
0.767391115255018	0.04398054316984\\
0.770714927577815	0.0429671665991063\\
0.777376917873449	0.0419537900283726\\
0.781145285044837	0.040940413457639\\
0.78633859277437	0.0399270368869054\\
0.792364362194601	0.0389136603161717\\
0.803852628860369	0.0379002837454381\\
0.817475469979261	0.0368869071747044\\
0.825418503726919	0.0358735306039708\\
0.829439253049354	0.0348601540332372\\
0.834587651890271	0.0338467774625035\\
0.840039733442901	0.0328334008917699\\
0.846357478774647	0.0318200243210363\\
0.853169745870294	0.0308066477503026\\
0.870078473617542	0.029793271179569\\
0.889737953286404	0.0287798946088353\\
0.900242056555	0.0277665180381017\\
0.925293342281775	0.0267531414673681\\
0.939018223563663	0.0257397648966344\\
0.954015704711971	0.0247263883259008\\
0.973329720710817	0.0237130117551672\\
0.988531087273122	0.0226996351844335\\
1.00491288593386	0.0216862586136999\\
1.02562318106608	0.0206728820429662\\
1.04713109618831	0.0196595054722326\\
1.05972092191031	0.018646128901499\\
1.09779405696862	0.0176327523307653\\
1.1208815207673	0.0166193757600317\\
1.13385296761763	0.0156059991892981\\
1.15466884204118	0.0145926226185644\\
1.18147439618863	0.0135792460478308\\
1.19491829891421	0.0125658694770971\\
1.2322683844385	0.0115524929063635\\
1.27465755528294	0.0105391163356299\\
1.31334985601052	0.00952573976489623\\
1.42960930583567	0.0085123631941626\\
1.46902045104518	0.00749898662342896\\
1.57097185755334	0.00648561005269532\\
1.94652664825884	0.00547223348196169\\
2.73283339181503	0.00445885691122805\\
3.93408503043031	0.00344548034049441\\
5.94744648466883	0.00243210376976077\\
20.6575378996516	0.00141872719902714\\
467.727504545072	0.000405350628293499\\
};
\addlegendentry{$N=1$,~, $\lrmse =17.58$, $\prmse =0.024$, $\armse =0.020$, $\brmse =4\hspace{-3pt}\times\hspace{-3pt}10^{-5}$, $\gamma=40$}


==> figures/mse_N_2_K_10_G_5_SNR_1000_I_20_Pratio_2_Nratio_1_cs.tex <==
\addplot [color=red,line width=0.2pt]
  table[row sep=crcr]{%
2.7379416175773e-11	1\\
9.00606120445211e-11	0.999\\
1.3891334003428e-10	0.998\\
2.03580810663966e-10	0.997\\
2.20605383277542e-10	0.996\\
2.36195349694337e-10	0.995\\
2.55105385693905e-10	0.994\\
3.00083724823192e-10	0.993\\
3.43291926491236e-10	0.992\\
3.66236196890214e-10	0.991\\
4.02929734034097e-10	0.99\\
4.36561990238151e-10	0.989\\
4.52405857559307e-10	0.988\\
4.91748681293784e-10	0.987\\
5.44848321084091e-10	0.986\\
5.78929500923652e-10	0.985\\
6.16334861014491e-10	0.984\\
6.54104571359867e-10	0.983\\
6.70772574655725e-10	0.982\\
6.88391888442457e-10	0.981\\
6.99325516938518e-10	0.98\\
7.50791235352708e-10	0.979\\
7.715519964128e-10	0.978\\
7.94479820545393e-10	0.977\\
8.02747875111658e-10	0.976\\
8.36719099649614e-10	0.975\\
8.53422536140735e-10	0.974\\
8.68372045119621e-10	0.973\\
8.84276072730702e-10	0.972\\
9.08520425526462e-10	0.971\\
9.30848614730103e-10	0.970000000000001\\
9.6389823476744e-10	0.969\\
9.7647805590442e-10	0.968\\
9.91664681791429e-10	0.967000000000001\\
1.02861716136008e-09	0.966000000000001\\
1.06280655715962e-09	0.965000000000001\\
1.08390801240412e-09	0.964000000000001\\
1.09734891400712e-09	0.963000000000001\\
1.1161605972883e-09	0.962000000000001\\
1.12979440992908e-09	0.961000000000001\\
1.14797620589331e-09	0.960000000000001\\
1.17154827538267e-09	0.959000000000001\\
1.20913434599018e-09	0.958000000000001\\
1.23203888029126e-09	0.957000000000001\\
1.24543256176841e-09	0.956000000000001\\
1.25047566391855e-09	0.955000000000001\\
1.28912881689252e-09	0.954000000000001\\
1.30639187051004e-09	0.953000000000001\\
1.34286209843284e-09	0.952000000000001\\
1.36852364434778e-09	0.951000000000001\\
1.38402005581365e-09	0.950000000000001\\
1.41199784730717e-09	0.949000000000001\\
1.44735444908652e-09	0.948000000000001\\
1.47529647207397e-09	0.947000000000001\\
1.50160140683102e-09	0.946000000000001\\
1.51745167545127e-09	0.945000000000001\\
1.53734038458021e-09	0.944000000000001\\
1.54564530999937e-09	0.943000000000001\\
1.56278910261189e-09	0.942000000000001\\
1.57456311286613e-09	0.941000000000001\\
1.59587372029162e-09	0.940000000000001\\
1.61996446190388e-09	0.939000000000001\\
1.63420841641234e-09	0.938000000000001\\
1.67445952959854e-09	0.937000000000001\\
1.68578462159994e-09	0.936000000000001\\
1.70364115336177e-09	0.935000000000001\\
1.72203084518217e-09	0.934000000000001\\
1.75052120996362e-09	0.933000000000001\\
1.76668175294662e-09	0.932000000000001\\
1.77812376821404e-09	0.931000000000001\\
1.83914815198195e-09	0.930000000000001\\
1.86493832228598e-09	0.929000000000001\\
1.88187984959675e-09	0.928000000000001\\
1.90235027964069e-09	0.927000000000001\\
1.93001884444821e-09	0.926000000000001\\
1.96111373832754e-09	0.925000000000001\\
1.9748559690944e-09	0.924000000000001\\
1.99635402611172e-09	0.923000000000001\\
2.00251063044242e-09	0.922000000000001\\
2.01091339237848e-09	0.921000000000001\\
2.02280500787576e-09	0.920000000000001\\
2.02929994250146e-09	0.919000000000001\\
2.04438879153829e-09	0.918000000000001\\
2.05747093091971e-09	0.917000000000001\\
2.07680449158345e-09	0.916000000000001\\
2.09895047673955e-09	0.915000000000001\\
2.1210914572707e-09	0.914000000000001\\
2.13873142510852e-09	0.913000000000001\\
2.1568606097535e-09	0.912000000000001\\
2.16977221427089e-09	0.911000000000001\\
2.18559988755003e-09	0.910000000000001\\
2.20549681592889e-09	0.909000000000001\\
2.24266762095363e-09	0.908000000000001\\
2.26082565039669e-09	0.907000000000001\\
2.29057939335953e-09	0.906000000000001\\
2.31972692403313e-09	0.905000000000001\\
2.33843137446828e-09	0.904000000000001\\
2.35877484055249e-09	0.903000000000001\\
2.36551988930853e-09	0.902000000000001\\
2.3792252136833e-09	0.901000000000001\\
2.39471953437383e-09	0.900000000000001\\
2.41185842501354e-09	0.899000000000001\\
2.42250714297344e-09	0.898000000000001\\
2.43083197836391e-09	0.897000000000001\\
2.44492579364373e-09	0.896000000000001\\
2.47969550866485e-09	0.895000000000001\\
2.51325197525105e-09	0.894000000000001\\
2.51905805117689e-09	0.893000000000001\\
2.55953790014295e-09	0.892000000000001\\
2.56893178289058e-09	0.891000000000001\\
2.580410740118e-09	0.890000000000001\\
2.59043251121652e-09	0.889000000000001\\
2.59556227032778e-09	0.888000000000001\\
2.60365348105524e-09	0.887000000000001\\
2.61458757184885e-09	0.886000000000001\\
2.64095235180838e-09	0.885000000000001\\
2.66691396600891e-09	0.884000000000001\\
2.68921644349532e-09	0.883000000000001\\
2.72476710772498e-09	0.882000000000001\\
2.73308916942389e-09	0.881000000000001\\
2.75412975501787e-09	0.880000000000001\\
2.79823379258101e-09	0.879000000000001\\
2.82324352504397e-09	0.878000000000001\\
2.85565553782078e-09	0.877000000000001\\
2.87949039117912e-09	0.876000000000001\\
2.89913608506895e-09	0.875000000000001\\
2.92101930861775e-09	0.874000000000001\\
2.94743789537784e-09	0.873000000000001\\
2.97294477098417e-09	0.872000000000001\\
2.98080541790582e-09	0.871000000000001\\
3.00976584482453e-09	0.870000000000001\\
3.03285227404363e-09	0.869000000000001\\
3.07695218068929e-09	0.868000000000002\\
3.09861688207911e-09	0.867000000000001\\
3.125861571283e-09	0.866000000000001\\
3.15457934327899e-09	0.865000000000001\\
3.17448712942897e-09	0.864000000000001\\
3.18838066764842e-09	0.863000000000001\\
3.20508785963625e-09	0.862000000000002\\
3.24197807200924e-09	0.861000000000002\\
3.26585374284471e-09	0.860000000000001\\
3.28776808482493e-09	0.859000000000001\\
3.29893816470854e-09	0.858000000000001\\
3.31768328293309e-09	0.857000000000001\\
3.34221588729374e-09	0.856000000000001\\
3.35724894160778e-09	0.855000000000002\\
3.39422944627148e-09	0.854000000000002\\
3.41467914130818e-09	0.853000000000001\\
3.45702411682372e-09	0.852000000000001\\
3.48890755179481e-09	0.851000000000001\\
3.51274476007364e-09	0.850000000000001\\
3.52674239823788e-09	0.849000000000001\\
3.542259218925e-09	0.848000000000001\\
3.58572723729772e-09	0.847000000000001\\
3.60048104156287e-09	0.846000000000001\\
3.61679966135482e-09	0.845000000000001\\
3.63720717576755e-09	0.844000000000001\\
3.65997784186281e-09	0.843000000000001\\
3.68177908781281e-09	0.842000000000001\\
3.69664077875117e-09	0.841000000000001\\
3.71316394549142e-09	0.840000000000001\\
3.74513891856028e-09	0.839000000000001\\
3.76401394505537e-09	0.838000000000002\\
3.79833935114193e-09	0.837000000000002\\
3.81538118241806e-09	0.836000000000002\\
3.82589047689909e-09	0.835000000000001\\
3.85138556436029e-09	0.834000000000001\\
3.86796322158496e-09	0.833000000000001\\
3.89878052029202e-09	0.832000000000001\\
3.91691481558081e-09	0.831000000000001\\
3.92857687328604e-09	0.830000000000001\\
3.94704017197346e-09	0.829000000000001\\
3.9576109417825e-09	0.828000000000001\\
3.98814091088385e-09	0.827000000000001\\
4.02571950927403e-09	0.826000000000002\\
4.03040557173674e-09	0.825000000000002\\
4.05781045500552e-09	0.824000000000002\\
4.08771203319818e-09	0.823000000000002\\
4.12678156079298e-09	0.822000000000002\\
4.16814206293947e-09	0.821000000000002\\
4.1934858349527e-09	0.820000000000002\\
4.23020253278082e-09	0.819000000000002\\
4.23798062339819e-09	0.818000000000002\\
4.25066634328219e-09	0.817000000000002\\
4.27762646565589e-09	0.816000000000002\\
4.31024969058942e-09	0.815000000000002\\
4.32206498140166e-09	0.814000000000002\\
4.34407615868558e-09	0.813000000000002\\
4.367866586629e-09	0.812000000000002\\
4.37565456252717e-09	0.811000000000002\\
4.41115347562513e-09	0.810000000000002\\
4.42614770466791e-09	0.809000000000002\\
4.43994625971074e-09	0.808000000000002\\
4.47202917669497e-09	0.807000000000002\\
4.50585822170799e-09	0.806000000000002\\
4.52432051721603e-09	0.805000000000002\\
4.56506463938028e-09	0.804000000000002\\
4.59606535199698e-09	0.803000000000002\\
4.64400649812982e-09	0.802000000000002\\
4.66895026733819e-09	0.801000000000002\\
4.69551084060657e-09	0.800000000000002\\
4.72529754164242e-09	0.799000000000002\\
4.73467316778711e-09	0.798000000000002\\
4.75027554855798e-09	0.797000000000002\\
4.77533831325697e-09	0.796000000000002\\
4.8169474365994e-09	0.795000000000002\\
4.84844301744845e-09	0.794000000000002\\
4.87929902555846e-09	0.793000000000002\\
4.91847118004326e-09	0.792000000000002\\
4.96396533519484e-09	0.791000000000002\\
4.99038112380174e-09	0.790000000000002\\
5.01211604643716e-09	0.789000000000002\\
5.04908980240588e-09	0.788000000000002\\
5.08085023256705e-09	0.787000000000002\\
5.11181278686332e-09	0.786000000000002\\
5.12811736800428e-09	0.785000000000002\\
5.17241079420879e-09	0.784000000000002\\
5.19665912274463e-09	0.783000000000002\\
5.21628390496165e-09	0.782000000000002\\
5.236865931907e-09	0.781000000000002\\
5.25024381468646e-09	0.780000000000002\\
5.27168184163452e-09	0.779000000000002\\
5.29840023558207e-09	0.778000000000002\\
5.31683455977852e-09	0.777000000000002\\
5.33224673981642e-09	0.776000000000002\\
5.35441329439016e-09	0.775000000000002\\
5.36954594818466e-09	0.774000000000002\\
5.39096194419631e-09	0.773000000000002\\
5.41266902739999e-09	0.772000000000002\\
5.42814792790222e-09	0.771000000000003\\
5.4447363937967e-09	0.770000000000003\\
5.46266941772113e-09	0.769000000000003\\
5.50884103984107e-09	0.768000000000003\\
5.52525683497683e-09	0.767000000000003\\
5.55996043116263e-09	0.766000000000003\\
5.60132709767722e-09	0.765000000000003\\
5.63057314331848e-09	0.764000000000003\\
5.65791409369994e-09	0.763000000000003\\
5.68571986332409e-09	0.762000000000003\\
5.70903673209363e-09	0.761000000000003\\
5.74509989274604e-09	0.760000000000003\\
5.79089059918102e-09	0.759000000000003\\
5.81812294533062e-09	0.758000000000003\\
5.84169790546958e-09	0.757000000000003\\
5.85573116030627e-09	0.756000000000003\\
5.87350683803821e-09	0.755000000000004\\
5.88691474146002e-09	0.754000000000004\\
5.90889294670801e-09	0.753000000000004\\
5.94009996224406e-09	0.752000000000004\\
5.99164615234967e-09	0.751000000000004\\
6.02143374337868e-09	0.750000000000004\\
6.04580096117988e-09	0.749000000000004\\
6.05922887287451e-09	0.748000000000004\\
6.08795229889822e-09	0.747000000000004\\
6.09874782874248e-09	0.746000000000004\\
6.12325550525499e-09	0.745000000000004\\
6.15664467391286e-09	0.744000000000004\\
6.17034250173801e-09	0.743000000000004\\
6.19670768562369e-09	0.742000000000004\\
6.21724422801582e-09	0.741000000000004\\
6.2381274455467e-09	0.740000000000004\\
6.28202864620157e-09	0.739000000000004\\
6.32862317859949e-09	0.738000000000005\\
6.35123151911642e-09	0.737000000000005\\
6.37667107045083e-09	0.736000000000005\\
6.39568171900575e-09	0.735000000000005\\
6.40564106844937e-09	0.734000000000005\\
6.43597094085844e-09	0.733000000000005\\
6.45993892480044e-09	0.732000000000005\\
6.46695293372739e-09	0.731000000000005\\
6.47713265673216e-09	0.730000000000005\\
6.52112718059283e-09	0.729000000000005\\
6.53923897292419e-09	0.728000000000005\\
6.57184596689935e-09	0.727000000000005\\
6.60050536499202e-09	0.726000000000005\\
6.62141745532869e-09	0.725000000000006\\
6.69753631537369e-09	0.724000000000006\\
6.72634063017086e-09	0.723000000000006\\
6.76553067302679e-09	0.722000000000006\\
6.78866460821145e-09	0.721000000000006\\
6.82072343533273e-09	0.720000000000006\\
6.88833926739173e-09	0.719000000000006\\
6.90518150949634e-09	0.718000000000006\\
6.94781973423403e-09	0.717000000000006\\
6.99111274163062e-09	0.716000000000006\\
7.03406456426864e-09	0.715000000000006\\
7.05185353357799e-09	0.714000000000006\\
7.09796266960674e-09	0.713000000000006\\
7.14692375978662e-09	0.712000000000006\\
7.18726309439968e-09	0.711000000000006\\
7.24639034688107e-09	0.710000000000006\\
7.27273139571988e-09	0.709000000000006\\
7.32452877815705e-09	0.708000000000006\\
7.34652798809766e-09	0.707000000000007\\
7.39147664342913e-09	0.706000000000007\\
7.42083799100365e-09	0.705000000000007\\
7.43837934325185e-09	0.704000000000007\\
7.47634771003026e-09	0.703000000000007\\
7.50048341603077e-09	0.702000000000007\\
7.51973217741784e-09	0.701000000000007\\
7.55648339260617e-09	0.700000000000007\\
7.57411330712827e-09	0.699000000000007\\
7.63238591727999e-09	0.698000000000007\\
7.68163076138341e-09	0.697000000000007\\
7.70444711802924e-09	0.696000000000007\\
7.72142062135824e-09	0.695000000000007\\
7.74695974372605e-09	0.694000000000007\\
7.7761655389588e-09	0.693000000000007\\
7.82139417398487e-09	0.692000000000007\\
7.85612848458254e-09	0.691000000000007\\
7.90222221121514e-09	0.690000000000007\\
7.92230499827684e-09	0.689000000000007\\
7.97985299532704e-09	0.688000000000007\\
8.00893482085657e-09	0.687000000000007\\
8.03377645835405e-09	0.686000000000007\\
8.07083857705878e-09	0.685000000000007\\
8.09811497001422e-09	0.684000000000007\\
8.14436556875066e-09	0.683000000000007\\
8.1644737430995e-09	0.682000000000007\\
8.18153867809889e-09	0.681000000000007\\
8.21986058315827e-09	0.680000000000007\\
8.23693413188922e-09	0.679000000000008\\
8.24477059156135e-09	0.678000000000008\\
8.29333431085539e-09	0.677000000000008\\
8.3476906105149e-09	0.676000000000008\\
8.35737479163322e-09	0.675000000000008\\
8.42828024011862e-09	0.674000000000008\\
8.47371768276691e-09	0.673000000000008\\
8.50494036789954e-09	0.672000000000008\\
8.55129298147745e-09	0.671000000000008\\
8.56505020384839e-09	0.670000000000008\\
8.60741886840307e-09	0.669000000000008\\
8.65544732448241e-09	0.668000000000008\\
8.71447611597787e-09	0.667000000000008\\
8.73823510965204e-09	0.666000000000008\\
8.81642482495043e-09	0.665000000000008\\
8.83856491984601e-09	0.664000000000008\\
8.87937188945876e-09	0.663000000000009\\
8.90453915006403e-09	0.662000000000009\\
8.95839026550634e-09	0.661000000000009\\
8.98354600641112e-09	0.660000000000009\\
9.01732816665723e-09	0.659000000000009\\
9.04606903564618e-09	0.658000000000009\\
9.06289610079258e-09	0.657000000000009\\
9.09714691616707e-09	0.656000000000009\\
9.10490799068124e-09	0.655000000000009\\
9.14816792886049e-09	0.654000000000009\\
9.17706344965605e-09	0.653000000000009\\
9.2215135847258e-09	0.652000000000009\\
9.25498822508156e-09	0.651000000000009\\
9.27760746254389e-09	0.650000000000009\\
9.30358940694923e-09	0.649000000000009\\
9.32159393586884e-09	0.64800000000001\\
9.34726297689347e-09	0.64700000000001\\
9.36392420982665e-09	0.64600000000001\\
9.41109026532128e-09	0.64500000000001\\
9.50762106693504e-09	0.64400000000001\\
9.52963310001018e-09	0.64300000000001\\
9.5726309603123e-09	0.64200000000001\\
9.61197347820812e-09	0.64100000000001\\
9.63309914681539e-09	0.64000000000001\\
9.67373447459334e-09	0.63900000000001\\
9.68651261685564e-09	0.63800000000001\\
9.71145150495321e-09	0.63700000000001\\
9.73182389670731e-09	0.63600000000001\\
9.7637442704393e-09	0.63500000000001\\
9.81588288396723e-09	0.63400000000001\\
9.85736934937258e-09	0.63300000000001\\
9.89073240982015e-09	0.63200000000001\\
9.92212015899488e-09	0.63100000000001\\
9.95045896577085e-09	0.630000000000011\\
9.97854353869401e-09	0.629000000000011\\
1.00012819900763e-08	0.628000000000011\\
1.00446045355489e-08	0.627000000000011\\
1.01203880154674e-08	0.626000000000011\\
1.01946477835702e-08	0.625000000000011\\
1.02246385476711e-08	0.624000000000011\\
1.02893580583126e-08	0.623000000000011\\
1.03271362032533e-08	0.622000000000011\\
1.0378321834201e-08	0.621000000000011\\
1.04223986505898e-08	0.620000000000011\\
1.04698766023439e-08	0.619000000000011\\
1.04967969818908e-08	0.618000000000011\\
1.05635677999446e-08	0.617000000000011\\
1.06364794505851e-08	0.616000000000012\\
1.07281453041851e-08	0.615000000000012\\
1.07749018733054e-08	0.614000000000012\\
1.08108394814498e-08	0.613000000000012\\
1.08395923777552e-08	0.612000000000012\\
1.08780049312811e-08	0.611000000000012\\
1.09204422579985e-08	0.610000000000012\\
1.09504090730224e-08	0.609000000000012\\
1.10024301491172e-08	0.608000000000012\\
1.10184602779618e-08	0.607000000000012\\
1.10950003342026e-08	0.606000000000012\\
1.1128650559914e-08	0.605000000000013\\
1.11486490977222e-08	0.604000000000013\\
1.1200211245836e-08	0.603000000000013\\
1.12561108990757e-08	0.602000000000013\\
1.1338900146552e-08	0.601000000000013\\
1.14018106670081e-08	0.600000000000013\\
1.14479780552601e-08	0.599000000000013\\
1.14899639873794e-08	0.598000000000013\\
1.15262772933415e-08	0.597000000000013\\
1.15672697033634e-08	0.596000000000013\\
1.16446321926408e-08	0.595000000000013\\
1.17132715030576e-08	0.594000000000014\\
1.17437200381361e-08	0.593000000000014\\
1.18119410138054e-08	0.592000000000014\\
1.18389061304177e-08	0.591000000000014\\
1.1882010481768e-08	0.590000000000014\\
1.19674373742985e-08	0.589000000000014\\
1.21061635265034e-08	0.588000000000014\\
1.21632150659238e-08	0.587000000000014\\
1.22170382096206e-08	0.586000000000014\\
1.22386791357731e-08	0.585000000000014\\
1.22814211412443e-08	0.584000000000014\\
1.23695982289101e-08	0.583000000000015\\
1.24671673527288e-08	0.582000000000015\\
1.25207146854768e-08	0.581000000000015\\
1.26049125224655e-08	0.580000000000015\\
1.2667473626658e-08	0.579000000000015\\
1.2707602530475e-08	0.578000000000015\\
1.27616243580658e-08	0.577000000000015\\
1.28274263201885e-08	0.576000000000015\\
1.28839504187244e-08	0.575000000000015\\
1.29164354982628e-08	0.574000000000015\\
1.3001409804839e-08	0.573000000000015\\
1.30638595917199e-08	0.572000000000015\\
1.31300903901686e-08	0.571000000000015\\
1.31606254583557e-08	0.570000000000015\\
1.31897846906749e-08	0.569000000000015\\
1.32420073938872e-08	0.568000000000016\\
1.32562475526837e-08	0.567000000000015\\
1.33029749486667e-08	0.566000000000016\\
1.33582371149967e-08	0.565000000000016\\
1.3391524956304e-08	0.564000000000016\\
1.34979265021534e-08	0.563000000000016\\
1.35469325779846e-08	0.562000000000016\\
1.35933578979117e-08	0.561000000000016\\
1.36286059844785e-08	0.560000000000016\\
1.36615605204455e-08	0.559000000000016\\
1.38004410195139e-08	0.558000000000016\\
1.38832403113442e-08	0.557000000000017\\
1.39072664937827e-08	0.556000000000017\\
1.39855430098403e-08	0.555000000000017\\
1.40614407561377e-08	0.554000000000017\\
1.40839765107254e-08	0.553000000000017\\
1.41140565594848e-08	0.552000000000017\\
1.42153639584617e-08	0.551000000000017\\
1.42781505531968e-08	0.550000000000017\\
1.43070414316592e-08	0.549000000000017\\
1.4339172685043e-08	0.548000000000017\\
1.44029962505129e-08	0.547000000000018\\
1.44859724906033e-08	0.546000000000018\\
1.45524813894624e-08	0.545000000000018\\
1.46862020135505e-08	0.544000000000018\\
1.4747562458202e-08	0.543000000000018\\
1.47849632909918e-08	0.542000000000018\\
1.48666748311756e-08	0.541000000000018\\
1.48900284115199e-08	0.540000000000018\\
1.49303679598301e-08	0.539000000000018\\
1.50239478804235e-08	0.538000000000018\\
1.51285777018134e-08	0.537000000000018\\
1.51565904641731e-08	0.536000000000018\\
1.51899592247554e-08	0.535000000000018\\
1.53028007996133e-08	0.534000000000018\\
1.53776908651137e-08	0.533000000000018\\
1.54122831177548e-08	0.532000000000018\\
1.55162228858443e-08	0.531000000000018\\
1.56138572824452e-08	0.530000000000019\\
1.56960539474671e-08	0.529000000000019\\
1.58216923525553e-08	0.528000000000019\\
1.58817787600459e-08	0.527000000000019\\
1.59597173656407e-08	0.526000000000019\\
1.60148661470019e-08	0.525000000000019\\
1.60798803357416e-08	0.524000000000019\\
1.61650830033355e-08	0.523000000000019\\
1.6212731552862e-08	0.522000000000019\\
1.6272624744997e-08	0.521000000000019\\
1.6351780849398e-08	0.520000000000019\\
1.64351502777226e-08	0.519000000000019\\
1.65311065575523e-08	0.518000000000019\\
1.66235540942487e-08	0.51700000000002\\
1.67141632964814e-08	0.51600000000002\\
1.68446225181793e-08	0.51500000000002\\
1.68966492813889e-08	0.51400000000002\\
1.70043335154754e-08	0.51300000000002\\
1.70726596778234e-08	0.51200000000002\\
1.71397949713113e-08	0.51100000000002\\
1.71786502275764e-08	0.51000000000002\\
1.7278383004291e-08	0.50900000000002\\
1.73358855022239e-08	0.50800000000002\\
1.74259067229105e-08	0.507000000000021\\
1.75067392427414e-08	0.506000000000021\\
1.75806983379726e-08	0.505000000000021\\
1.76415705585502e-08	0.504000000000021\\
1.77300504591093e-08	0.503000000000021\\
1.77947245454268e-08	0.502000000000021\\
1.78660852026599e-08	0.501000000000021\\
1.80128727858826e-08	0.500000000000021\\
1.80626650346552e-08	0.499000000000021\\
1.81773942093344e-08	0.498000000000021\\
1.82632878962119e-08	0.497000000000021\\
1.835721012472e-08	0.496000000000021\\
1.8390439384376e-08	0.495000000000021\\
1.85127744832362e-08	0.494000000000021\\
1.86272074087464e-08	0.493000000000021\\
1.88497306276546e-08	0.492000000000021\\
1.89483124236883e-08	0.491000000000021\\
1.90534231701962e-08	0.490000000000021\\
1.92246470774782e-08	0.489000000000021\\
1.93346333642993e-08	0.488000000000021\\
1.94271944393733e-08	0.487000000000021\\
1.95361150630298e-08	0.48600000000002\\
1.96686049180213e-08	0.48500000000002\\
1.97993555967724e-08	0.48400000000002\\
1.99700022791135e-08	0.483000000000021\\
2.00958910405198e-08	0.48200000000002\\
2.01734406299567e-08	0.48100000000002\\
2.03037023276682e-08	0.48000000000002\\
2.03836289599655e-08	0.47900000000002\\
2.05588370156566e-08	0.47800000000002\\
2.06389665353256e-08	0.47700000000002\\
2.07537847893048e-08	0.47600000000002\\
2.08300521630881e-08	0.47500000000002\\
2.09386167175777e-08	0.47400000000002\\
2.10164013803641e-08	0.47300000000002\\
2.1192117219377e-08	0.47200000000002\\
2.13579379611003e-08	0.47100000000002\\
2.14946628229354e-08	0.47000000000002\\
2.15658229979046e-08	0.46900000000002\\
2.16593790530332e-08	0.46800000000002\\
2.1727062228766e-08	0.46700000000002\\
2.18657784117508e-08	0.46600000000002\\
2.19485210779132e-08	0.46500000000002\\
2.20298732898624e-08	0.464000000000019\\
2.21209911270245e-08	0.463000000000019\\
2.21647530481877e-08	0.462000000000019\\
2.22696552539308e-08	0.461000000000019\\
2.23592117052048e-08	0.460000000000019\\
2.25042730288661e-08	0.459000000000019\\
2.25663397233625e-08	0.458000000000019\\
2.26783644714617e-08	0.457000000000019\\
2.27755999461464e-08	0.456000000000019\\
2.29709157517848e-08	0.455000000000019\\
2.30716568449545e-08	0.454000000000019\\
2.31212558170966e-08	0.453000000000019\\
2.32116022173827e-08	0.452000000000019\\
2.33069736223986e-08	0.451000000000019\\
2.34989857555579e-08	0.450000000000019\\
2.36003128163213e-08	0.449000000000019\\
2.37179111452608e-08	0.448000000000019\\
2.3857940396564e-08	0.447000000000019\\
2.40612006879344e-08	0.446000000000019\\
2.40963732465345e-08	0.445000000000019\\
2.42794483659549e-08	0.444000000000019\\
2.43630807362201e-08	0.443000000000019\\
2.45520554717353e-08	0.442000000000019\\
2.46370456823262e-08	0.441000000000019\\
2.48296750165259e-08	0.440000000000019\\
2.49985314196103e-08	0.439000000000018\\
2.5145616852972e-08	0.438000000000018\\
2.51961170771695e-08	0.437000000000018\\
2.53569641761813e-08	0.436000000000018\\
2.54350895667647e-08	0.435000000000018\\
2.55559350916771e-08	0.434000000000018\\
2.56391378462303e-08	0.433000000000018\\
2.58193006731035e-08	0.432000000000018\\
2.59240074120895e-08	0.431000000000018\\
2.61321922157412e-08	0.430000000000018\\
2.62325704860624e-08	0.429000000000018\\
2.63301989364181e-08	0.428000000000018\\
2.64106231114073e-08	0.427000000000018\\
2.65172497390299e-08	0.426000000000018\\
2.65627158967359e-08	0.425000000000018\\
2.67715775155262e-08	0.424000000000018\\
2.68619438811673e-08	0.423000000000018\\
2.70289695183482e-08	0.422000000000018\\
2.71775930983805e-08	0.421000000000018\\
2.72683701064578e-08	0.420000000000017\\
2.75429876387348e-08	0.419000000000018\\
2.77764023550255e-08	0.418000000000017\\
2.79393069361548e-08	0.417000000000018\\
2.80986954848718e-08	0.416000000000017\\
2.82896075535876e-08	0.415000000000017\\
2.8442009573128e-08	0.414000000000017\\
2.85062891097838e-08	0.413000000000017\\
2.85457386179934e-08	0.412000000000017\\
2.87182588989477e-08	0.411000000000017\\
2.89044927466699e-08	0.410000000000017\\
2.91601827188339e-08	0.409000000000017\\
2.92376387766645e-08	0.408000000000017\\
2.93942755777873e-08	0.407000000000017\\
2.97527814233593e-08	0.406000000000017\\
2.98447876303166e-08	0.405000000000017\\
2.99972978403706e-08	0.404000000000017\\
3.01952403870325e-08	0.403000000000017\\
3.05574473942769e-08	0.402000000000017\\
3.06966252442294e-08	0.401000000000017\\
3.07702324121066e-08	0.400000000000017\\
3.09393938017589e-08	0.399000000000017\\
3.10939668878191e-08	0.398000000000016\\
3.11956350068287e-08	0.397000000000016\\
3.13084384704754e-08	0.396000000000016\\
3.14497050164565e-08	0.395000000000016\\
3.15227556087861e-08	0.394000000000016\\
3.17407113260199e-08	0.393000000000016\\
3.18744252420663e-08	0.392000000000016\\
3.20898311348437e-08	0.391000000000016\\
3.24251443351393e-08	0.390000000000016\\
3.25824236535915e-08	0.389000000000016\\
3.27264287972269e-08	0.388000000000016\\
3.30410664134524e-08	0.387000000000016\\
3.31986169154412e-08	0.386000000000016\\
3.33934723740811e-08	0.385000000000016\\
3.36710907510287e-08	0.384000000000016\\
3.38545176120244e-08	0.383000000000016\\
3.42378677638454e-08	0.382000000000016\\
3.44213842625741e-08	0.381000000000016\\
3.46413436517469e-08	0.380000000000016\\
3.48411703298223e-08	0.379000000000016\\
3.5096310167514e-08	0.378000000000016\\
3.52764007469607e-08	0.377000000000016\\
3.54028010853045e-08	0.376000000000016\\
3.56316419365405e-08	0.375000000000016\\
3.57349384134179e-08	0.374000000000015\\
3.58927753717099e-08	0.373000000000015\\
3.60813494707516e-08	0.372000000000015\\
3.62849419817454e-08	0.371000000000015\\
3.65107323693592e-08	0.370000000000015\\
3.67843879380701e-08	0.369000000000015\\
3.69512043897972e-08	0.368000000000015\\
3.71212694364702e-08	0.367000000000015\\
3.73082420969367e-08	0.366000000000015\\
3.74640702645491e-08	0.365000000000015\\
3.75790357845822e-08	0.364000000000015\\
3.77418438497415e-08	0.363000000000015\\
3.80860974688525e-08	0.362000000000015\\
3.82476157517317e-08	0.361000000000015\\
3.83494160447663e-08	0.360000000000015\\
3.84398744341963e-08	0.359000000000015\\
3.85604519648029e-08	0.358000000000015\\
3.88894717911203e-08	0.357000000000015\\
3.94731773037385e-08	0.356000000000015\\
3.97689649508857e-08	0.355000000000015\\
4.00132752217154e-08	0.354000000000015\\
4.01942873262286e-08	0.353000000000015\\
4.03534463825348e-08	0.352000000000015\\
4.04838807586913e-08	0.351000000000015\\
4.07177448650086e-08	0.350000000000015\\
4.12268075370829e-08	0.349000000000014\\
4.1653356029847e-08	0.348000000000014\\
4.18541572227328e-08	0.347000000000014\\
4.19847832430736e-08	0.346000000000014\\
4.24507465208336e-08	0.345000000000014\\
4.26585512247289e-08	0.344000000000014\\
4.29248778400043e-08	0.343000000000014\\
4.30143284291404e-08	0.342000000000014\\
4.31994945312886e-08	0.341000000000014\\
4.3348135104839e-08	0.340000000000014\\
4.34913933268772e-08	0.339000000000014\\
4.36707669237439e-08	0.338000000000014\\
4.39155918146663e-08	0.337000000000014\\
4.41102012290381e-08	0.336000000000014\\
4.425050622104e-08	0.335000000000014\\
4.44597250499203e-08	0.334000000000014\\
4.47538085239376e-08	0.333000000000014\\
4.53391236885221e-08	0.332000000000013\\
4.5735378843552e-08	0.331000000000013\\
4.60716681232449e-08	0.330000000000013\\
4.61609364669203e-08	0.329000000000013\\
4.62679656987739e-08	0.328000000000013\\
4.68158423590349e-08	0.327000000000013\\
4.70966965868618e-08	0.326000000000013\\
4.72780130131838e-08	0.325000000000013\\
4.77192288669833e-08	0.324000000000013\\
4.8031260484752e-08	0.323000000000013\\
4.83668973794982e-08	0.322000000000013\\
4.84677817622659e-08	0.321000000000013\\
4.87670169023081e-08	0.320000000000012\\
4.91449540476543e-08	0.319000000000012\\
4.92496659205495e-08	0.318000000000012\\
4.95969492326631e-08	0.317000000000012\\
5.03819706526882e-08	0.316000000000012\\
5.0713603806253e-08	0.315000000000012\\
5.15464080654467e-08	0.314000000000012\\
5.19670934647922e-08	0.313000000000012\\
5.2353512356758e-08	0.312000000000012\\
5.28932678473261e-08	0.311000000000012\\
5.32636312276978e-08	0.310000000000012\\
5.35845609380992e-08	0.309000000000012\\
5.40533066693086e-08	0.308000000000012\\
5.42224654309066e-08	0.307000000000012\\
5.44784265451825e-08	0.306000000000012\\
5.49146537201155e-08	0.305000000000012\\
5.51249604265888e-08	0.304000000000012\\
5.53711745231198e-08	0.303000000000012\\
5.56983507766783e-08	0.302000000000012\\
5.63544800221192e-08	0.301000000000012\\
5.69483965308529e-08	0.300000000000012\\
5.79295991155896e-08	0.299000000000011\\
5.84213308047429e-08	0.298000000000011\\
5.86131963081295e-08	0.297000000000011\\
5.93580609790121e-08	0.296000000000011\\
5.99190057729478e-08	0.295000000000011\\
6.00924159306134e-08	0.294000000000011\\
6.0523493584549e-08	0.293000000000011\\
6.07602362354398e-08	0.292000000000011\\
6.09071412278432e-08	0.291000000000011\\
6.11460148940271e-08	0.290000000000011\\
6.14577406462307e-08	0.289000000000011\\
6.18617634651624e-08	0.288000000000011\\
6.25092713267895e-08	0.287000000000011\\
6.3071197172284e-08	0.28600000000001\\
6.33519683276505e-08	0.28500000000001\\
6.36863243698434e-08	0.28400000000001\\
6.40451338337173e-08	0.28300000000001\\
6.43236079411647e-08	0.28200000000001\\
6.49736517243703e-08	0.28100000000001\\
6.57757343355194e-08	0.28000000000001\\
6.63875740165998e-08	0.27900000000001\\
6.67876487048282e-08	0.27800000000001\\
6.76422034947779e-08	0.27700000000001\\
6.81927805241539e-08	0.27600000000001\\
6.86029781190676e-08	0.27500000000001\\
6.91303445492774e-08	0.27400000000001\\
7.03131552630095e-08	0.27300000000001\\
7.08020163973201e-08	0.27200000000001\\
7.10757119909191e-08	0.27100000000001\\
7.23555389624986e-08	0.27000000000001\\
7.29941287708659e-08	0.26900000000001\\
7.36587659922218e-08	0.26800000000001\\
7.39929937411629e-08	0.26700000000001\\
7.46535991444801e-08	0.26600000000001\\
7.54428801040493e-08	0.26500000000001\\
7.59450328055576e-08	0.26400000000001\\
7.65749705287345e-08	0.263000000000009\\
7.72965957447895e-08	0.262000000000009\\
7.78084021065453e-08	0.261000000000009\\
7.85263761454387e-08	0.260000000000009\\
7.87878416584335e-08	0.259000000000009\\
7.91682740404806e-08	0.258000000000009\\
7.98356162883769e-08	0.257000000000009\\
8.05373678250574e-08	0.256000000000009\\
8.17517796476981e-08	0.255000000000009\\
8.22215548048296e-08	0.254000000000009\\
8.2708331091014e-08	0.253000000000009\\
8.3106090648245e-08	0.252000000000009\\
8.3482781854422e-08	0.251000000000009\\
8.3748804298802e-08	0.250000000000009\\
8.42798254638864e-08	0.249000000000009\\
8.47775321434653e-08	0.248000000000009\\
8.50949640155624e-08	0.247000000000009\\
8.57636957050795e-08	0.246000000000009\\
8.62903374337283e-08	0.245000000000009\\
8.69128028337344e-08	0.244000000000009\\
8.75366277265276e-08	0.243000000000009\\
9.04736665044993e-08	0.242000000000009\\
9.14946572937669e-08	0.241000000000009\\
9.19727292181716e-08	0.240000000000009\\
9.25823528584972e-08	0.239000000000008\\
9.30193996090916e-08	0.238000000000008\\
9.37536259099952e-08	0.237000000000008\\
9.4637469596813e-08	0.236000000000008\\
9.51264814572533e-08	0.235000000000008\\
9.59281838532452e-08	0.234000000000008\\
9.75437838776921e-08	0.233000000000008\\
9.85365885896535e-08	0.232000000000008\\
1.00153811394112e-07	0.231000000000008\\
1.01092332094149e-07	0.230000000000008\\
1.01616574464623e-07	0.229000000000008\\
1.02217762404769e-07	0.228000000000008\\
1.04048019036589e-07	0.227000000000008\\
1.04477025719746e-07	0.226000000000008\\
1.05391613682651e-07	0.225000000000008\\
1.07530173785565e-07	0.224000000000008\\
1.08723757668397e-07	0.223000000000008\\
1.10047874086508e-07	0.222000000000008\\
1.10445212549539e-07	0.221000000000008\\
1.1103831467882e-07	0.220000000000008\\
1.12134628772944e-07	0.219000000000008\\
1.13299396240781e-07	0.218000000000008\\
1.14040210228666e-07	0.217000000000008\\
1.15405517051039e-07	0.216000000000008\\
1.15632947295934e-07	0.215000000000008\\
1.15953708315383e-07	0.214000000000008\\
1.1690717790873e-07	0.213000000000008\\
1.18115824976747e-07	0.212000000000008\\
1.1903420231238e-07	0.211000000000008\\
1.20195322840712e-07	0.210000000000008\\
1.20963202221002e-07	0.209000000000008\\
1.21859689565709e-07	0.208000000000008\\
1.22724789265232e-07	0.207000000000008\\
1.2424853230213e-07	0.206000000000008\\
1.25200395860483e-07	0.205000000000008\\
1.25880494370414e-07	0.204000000000008\\
1.28423192504608e-07	0.203000000000007\\
1.29590350697016e-07	0.202000000000007\\
1.30851950241187e-07	0.201000000000007\\
1.31723442818768e-07	0.200000000000007\\
1.3313083681925e-07	0.199000000000007\\
1.33890694844182e-07	0.198000000000007\\
1.34393738033048e-07	0.197000000000007\\
1.35486875627318e-07	0.196000000000007\\
1.37077334313577e-07	0.195000000000007\\
1.39683590144504e-07	0.194000000000007\\
1.40828865624753e-07	0.193000000000007\\
1.43076131266039e-07	0.192000000000007\\
1.44129997794922e-07	0.191000000000007\\
1.45884143596643e-07	0.190000000000007\\
1.4643043064096e-07	0.189000000000007\\
1.47270553763842e-07	0.188000000000007\\
1.50269910715234e-07	0.187000000000007\\
1.54696273633469e-07	0.186000000000007\\
1.55423887426056e-07	0.185000000000007\\
1.56949696463673e-07	0.184000000000007\\
1.59355057617151e-07	0.183000000000007\\
1.60130926223154e-07	0.182000000000007\\
1.63622722654736e-07	0.181000000000007\\
1.64373259851437e-07	0.180000000000007\\
1.64985325316496e-07	0.179000000000007\\
1.66341012152326e-07	0.178000000000007\\
1.68913910554243e-07	0.177000000000007\\
1.69887030446981e-07	0.176000000000007\\
1.70220444948936e-07	0.175000000000007\\
1.72879515702413e-07	0.174000000000007\\
1.74128911630185e-07	0.173000000000007\\
1.75405732396977e-07	0.172000000000007\\
1.75598287811364e-07	0.171000000000006\\
1.77851077653146e-07	0.170000000000006\\
1.78905348960305e-07	0.169000000000006\\
1.80581461670882e-07	0.168000000000006\\
1.82241836335131e-07	0.167000000000006\\
1.86887425570172e-07	0.166000000000006\\
1.8873370021226e-07	0.165000000000006\\
1.89768269480523e-07	0.164000000000006\\
1.92953523418445e-07	0.163000000000006\\
1.94505382399267e-07	0.162000000000006\\
1.95333733228317e-07	0.161000000000006\\
1.99879653616246e-07	0.160000000000006\\
2.02267568046678e-07	0.159000000000006\\
2.04592618846736e-07	0.158000000000006\\
2.07756104515346e-07	0.157000000000006\\
2.09203846732217e-07	0.156000000000006\\
2.11384369728492e-07	0.155000000000006\\
2.13881787127734e-07	0.154000000000006\\
2.16858129879526e-07	0.153000000000006\\
2.1903944808136e-07	0.152000000000006\\
2.2301400158766e-07	0.151000000000006\\
2.26451255618981e-07	0.150000000000006\\
2.28111010613954e-07	0.149000000000006\\
2.31337900277074e-07	0.148000000000006\\
2.3354811931166e-07	0.147000000000006\\
2.36093891923893e-07	0.146000000000006\\
2.39217733072976e-07	0.145000000000006\\
2.40651952761508e-07	0.144000000000006\\
2.42447056549134e-07	0.143000000000006\\
2.46133746864336e-07	0.142000000000006\\
2.50708174523504e-07	0.141000000000006\\
2.53667659936367e-07	0.140000000000006\\
2.58322756581873e-07	0.139000000000006\\
2.62583204924991e-07	0.138000000000006\\
2.68924704731341e-07	0.137000000000006\\
2.71651000206035e-07	0.136000000000005\\
2.82490180191918e-07	0.135000000000005\\
2.87599660202192e-07	0.134000000000005\\
2.90338100531211e-07	0.133000000000005\\
2.95647977185306e-07	0.132000000000005\\
3.00999251492727e-07	0.131000000000005\\
3.02333178194241e-07	0.130000000000005\\
3.06399746798367e-07	0.129000000000005\\
3.11376554206895e-07	0.128000000000005\\
3.13390245172533e-07	0.127000000000005\\
3.1737012435575e-07	0.126000000000005\\
3.20341955338197e-07	0.125000000000005\\
3.23301257508488e-07	0.124000000000005\\
3.26588683635124e-07	0.123000000000005\\
3.27810366202482e-07	0.122000000000005\\
3.33682029692355e-07	0.121000000000005\\
3.49106964059056e-07	0.120000000000005\\
3.55584027924644e-07	0.119000000000005\\
3.70875385491906e-07	0.118000000000005\\
3.79501818177415e-07	0.117000000000005\\
3.82972612535608e-07	0.116000000000005\\
3.88743428284238e-07	0.115000000000005\\
3.94549715116879e-07	0.114000000000005\\
4.01535985830763e-07	0.113000000000005\\
4.05970591320365e-07	0.112000000000005\\
4.19193878735889e-07	0.111000000000005\\
4.25455066729713e-07	0.110000000000005\\
4.37034620773007e-07	0.109000000000005\\
4.45035097304334e-07	0.108000000000005\\
4.50694997306264e-07	0.107000000000005\\
4.62921270096179e-07	0.106000000000004\\
4.76117718493861e-07	0.105000000000004\\
4.80414440687331e-07	0.104000000000004\\
4.87480714810096e-07	0.103000000000004\\
4.96775234263436e-07	0.102000000000004\\
5.05389044511197e-07	0.101000000000004\\
5.08129660001653e-07	0.100000000000004\\
5.1779763047164e-07	0.0990000000000042\\
5.27649117634806e-07	0.0980000000000041\\
5.35186815167463e-07	0.0970000000000041\\
5.392824681698e-07	0.0960000000000041\\
5.50049711841478e-07	0.095000000000004\\
5.58284249815451e-07	0.094000000000004\\
5.64548728654078e-07	0.093000000000004\\
5.69033203427124e-07	0.0920000000000039\\
5.79699432353948e-07	0.0910000000000039\\
5.9078795065802e-07	0.0900000000000039\\
6.00004245328766e-07	0.0890000000000037\\
6.09454466541016e-07	0.0880000000000037\\
6.21276407476654e-07	0.0870000000000037\\
6.36684126104367e-07	0.0860000000000037\\
6.44408083340895e-07	0.0850000000000036\\
6.65546160140851e-07	0.0840000000000036\\
7.08828950144449e-07	0.0830000000000036\\
7.12769649902436e-07	0.0820000000000036\\
7.27667928662063e-07	0.0810000000000035\\
7.62912859104298e-07	0.0800000000000035\\
7.86164362035246e-07	0.0790000000000035\\
8.20039788867147e-07	0.0780000000000034\\
8.5099143367801e-07	0.0770000000000034\\
9.01556312958763e-07	0.0760000000000034\\
9.41772565595759e-07	0.0750000000000034\\
1.00834628896456e-06	0.0740000000000033\\
1.0242554053195e-06	0.0730000000000033\\
1.04641912273302e-06	0.0720000000000033\\
1.14643463206131e-06	0.0710000000000033\\
1.26209249621791e-06	0.0700000000000032\\
1.28592055984123e-06	0.0690000000000032\\
1.37765662787989e-06	0.0680000000000032\\
1.42496711475707e-06	0.0670000000000031\\
1.465262217793e-06	0.0660000000000031\\
1.52111588756063e-06	0.0650000000000031\\
1.56943950865115e-06	0.0640000000000031\\
1.64557485525655e-06	0.0630000000000029\\
1.72153484314957e-06	0.0620000000000029\\
1.8542467512607e-06	0.0610000000000029\\
1.89880457246067e-06	0.0600000000000028\\
2.00634133558308e-06	0.0590000000000028\\
2.16597214842943e-06	0.0580000000000027\\
2.34994739571406e-06	0.0570000000000027\\
2.53094657498016e-06	0.0560000000000027\\
2.77750771215715e-06	0.0550000000000026\\
3.09039467299193e-06	0.0540000000000026\\
3.16972022132303e-06	0.0530000000000025\\
3.47208889156047e-06	0.0520000000000025\\
3.87550567075414e-06	0.0510000000000024\\
4.19624385007442e-06	0.0500000000000024\\
4.66687557945923e-06	0.0490000000000024\\
5.02045517844739e-06	0.0480000000000023\\
5.47196810591564e-06	0.0470000000000023\\
7.65677655187312e-06	0.0460000000000023\\
8.38045295406627e-06	0.0450000000000021\\
9.78144652621341e-06	0.0440000000000021\\
1.30200272168709e-05	0.0430000000000021\\
1.77211089724723e-05	0.042000000000002\\
2.34462694081532e-05	0.041000000000002\\
3.7878769198967e-05	0.0400000000000019\\
7.21310118164012e-05	0.0390000000000019\\
0.00017353075422086	0.0380000000000018\\
0.000474918429514373	0.0370000000000018\\
0.00161552787121882	0.0360000000000017\\
0.0126805464210917	0.0350000000000017\\
0.0412374431013033	0.0340000000000017\\
0.0862203894197072	0.0330000000000016\\
0.32129914217548	0.0320000000000016\\
0.542841249231237	0.0310000000000015\\
1.92734328300136	0.0300000000000015\\
7.2543977853368	0.0290000000000014\\
26.7447252970088	0.0280000000000014\\
107.253138925217	0.0270000000000014\\
204.488593660588	0.0260000000000012\\
331.465189345042	0.0250000000000012\\
898.599668444785	0.0240000000000011\\
1038.87015429301	0.0230000000000011\\
1303.85732804278	0.0220000000000011\\
1874.1385635512	0.021000000000001\\
1942.82097399445	0.020000000000001\\
2095.16745367002	0.0190000000000009\\
2280.31074984745	0.0180000000000009\\
2638.97176348594	0.0170000000000008\\
2997.23104952662	0.0160000000000008\\
3246.97259347209	0.0150000000000008\\
3612.34056905413	0.0140000000000007\\
4049.58117129056	0.0130000000000007\\
4286.65155798188	0.0120000000000006\\
4444.14608257738	0.0110000000000006\\
4621.0971373901	0.0100000000000005\\
4998.03443820955	0.00900000000000045\\
5457.2511005282	0.00800000000000045\\
5619.43797530916	0.00700000000000034\\
6262.5103391018	0.00600000000000034\\
6837.35472860252	0.00500000000000023\\
13991.4368296983	0.00400000000000023\\
14476.3606107163	0.00300000000000011\\
14728.3070770089	0.00200000000000011\\
15300.4396564371	0.001\\
16715.3015197664	0\\
};
\addlegendentry{$K=10$, $G=\;\,5$, $\lrmse =841.9$, $\prmse =0.022$, $\armse =0.038$, $\brmse =3\hspace{-3pt}\times\hspace{-3pt}10^{-4}$, $\gamma \rightarrow \infty$}


==> figures/mse_N_2_K_10_G_5_SNR_40_I_20_Pratio_2_Nratio_1_cs.tex <==
\addplot [color=red, dashed,line width=0.6pt]
  table[row sep=crcr]{%
0.518851035775393	1\\
0.616386732919589	0.999\\
0.829234937291179	0.998\\
0.94955127072076	0.997\\
1.02527168526029	0.996\\
1.11894969495244	0.995\\
1.16495902089308	0.994\\
1.20394264152895	0.993\\
1.26370860989964	0.992\\
1.30610770774397	0.991\\
1.35607632474757	0.99\\
1.38570599112354	0.989\\
1.42310020263254	0.988\\
1.46197036986977	0.987\\
1.47596924565047	0.986\\
1.48684923471453	0.985\\
1.51381475811546	0.984\\
1.54649714801803	0.983\\
1.57871923732925	0.982\\
1.60794052983609	0.981\\
1.63305051618517	0.98\\
1.64885882529837	0.979\\
1.66685422189907	0.978\\
1.69611351208204	0.977\\
1.7161242613104	0.976\\
1.72778107395309	0.975\\
1.74965006363333	0.974\\
1.76268279473548	0.973\\
1.77016889362528	0.972\\
1.78146647039819	0.971\\
1.80047310087173	0.970000000000001\\
1.83016572041305	0.969\\
1.85097290548999	0.968\\
1.87157981540452	0.967000000000001\\
1.9004824454575	0.966000000000001\\
1.91088681577484	0.965000000000001\\
1.92925766223191	0.964000000000001\\
1.94422861443333	0.963000000000001\\
1.96552010439642	0.962000000000001\\
1.98948770426114	0.961000000000001\\
2.01396785365327	0.960000000000001\\
2.02760690714092	0.959000000000001\\
2.03883445680131	0.958000000000001\\
2.04320312560063	0.957000000000001\\
2.05499891604505	0.956000000000001\\
2.0817434849899	0.955000000000001\\
2.08721799567345	0.954000000000001\\
2.1050022768352	0.953000000000001\\
2.12084133955322	0.952000000000001\\
2.1456154325698	0.951000000000001\\
2.15741556880127	0.950000000000001\\
2.17488251993841	0.949000000000001\\
2.18458997845733	0.948000000000001\\
2.20600911491915	0.947000000000001\\
2.2183070295778	0.946000000000001\\
2.23110858829325	0.945000000000001\\
2.24333800317896	0.944000000000001\\
2.24983354757036	0.943000000000001\\
2.26266690228913	0.942000000000001\\
2.26596311495299	0.941000000000001\\
2.28055616701994	0.940000000000001\\
2.29333128538882	0.939000000000001\\
2.32029381406588	0.938000000000001\\
2.32917228843896	0.937000000000001\\
2.34003135211435	0.936000000000001\\
2.35918308651157	0.935000000000001\\
2.37459091803154	0.934000000000001\\
2.38167329345103	0.933000000000001\\
2.39974660295874	0.932000000000001\\
2.41299122175155	0.931000000000001\\
2.43050216541032	0.930000000000001\\
2.44146111304874	0.929000000000001\\
2.45257151968786	0.928000000000001\\
2.47038774583365	0.927000000000001\\
2.48524412494402	0.926000000000001\\
2.49490387037853	0.925000000000001\\
2.50494334043052	0.924000000000001\\
2.51657197159868	0.923000000000001\\
2.53700919452615	0.922000000000001\\
2.54899454716979	0.921000000000001\\
2.56184397487245	0.920000000000001\\
2.56852850841843	0.919000000000001\\
2.57502004923134	0.918000000000001\\
2.57997686683193	0.917000000000001\\
2.58885056307501	0.916000000000001\\
2.59870654681739	0.915000000000001\\
2.60888425407383	0.914000000000001\\
2.62917958814638	0.913000000000001\\
2.64218515352487	0.912000000000001\\
2.65628376445609	0.911000000000001\\
2.66129300973392	0.910000000000001\\
2.67198809096684	0.909000000000001\\
2.67878088196096	0.908000000000001\\
2.68754740181694	0.907000000000001\\
2.69891210172834	0.906000000000001\\
2.70800210637978	0.905000000000001\\
2.72317365027072	0.904000000000001\\
2.73634270792171	0.903000000000001\\
2.75210565020024	0.902000000000001\\
2.7751861591935	0.901000000000001\\
2.78314373145736	0.900000000000001\\
2.79447786632666	0.899000000000001\\
2.80815798184111	0.898000000000001\\
2.82386180256772	0.897000000000001\\
2.82929916057533	0.896000000000001\\
2.83559383914324	0.895000000000001\\
2.84493786134552	0.894000000000001\\
2.85201221655942	0.893000000000001\\
2.85829294426887	0.892000000000001\\
2.87799735507166	0.891000000000001\\
2.88604294727735	0.890000000000001\\
2.89515056438772	0.889000000000001\\
2.90660507243095	0.888000000000001\\
2.92004694089797	0.887000000000001\\
2.93757273348986	0.886000000000001\\
2.95085424146272	0.885000000000001\\
2.95889212189281	0.884000000000001\\
2.96823464828514	0.883000000000001\\
2.98758883645433	0.882000000000001\\
2.99457024202935	0.881000000000001\\
3.0056949289455	0.880000000000001\\
3.01266347322129	0.879000000000001\\
3.04094511226611	0.878000000000001\\
3.04903680704446	0.877000000000001\\
3.06186565807845	0.876000000000001\\
3.07084673375244	0.875000000000001\\
3.07743328731245	0.874000000000001\\
3.089113182525	0.873000000000001\\
3.09524580862925	0.872000000000001\\
3.11169770486206	0.871000000000001\\
3.12422431822854	0.870000000000001\\
3.14758925975223	0.869000000000001\\
3.15088682917363	0.868000000000002\\
3.16092682404624	0.867000000000001\\
3.16838760547468	0.866000000000001\\
3.17800763271467	0.865000000000001\\
3.20107089689975	0.864000000000001\\
3.21440808538893	0.863000000000001\\
3.21932862449825	0.862000000000002\\
3.22955567125123	0.861000000000002\\
3.23794505292986	0.860000000000001\\
3.24927832199903	0.859000000000001\\
3.25560439015422	0.858000000000001\\
3.26515435338902	0.857000000000001\\
3.28019889747521	0.856000000000001\\
3.30264782122099	0.855000000000002\\
3.31918200836283	0.854000000000002\\
3.32631306934429	0.853000000000001\\
3.33378455301625	0.852000000000001\\
3.34206077152924	0.851000000000001\\
3.34710528036181	0.850000000000001\\
3.35493595828468	0.849000000000001\\
3.3641988424626	0.848000000000001\\
3.38027986187725	0.847000000000001\\
3.38504784259956	0.846000000000001\\
3.39034564875241	0.845000000000001\\
3.39448733688726	0.844000000000001\\
3.40673469467607	0.843000000000001\\
3.4188674623687	0.842000000000001\\
3.44081079169704	0.841000000000001\\
3.44454704012351	0.840000000000001\\
3.4549135734342	0.839000000000001\\
3.46533051158646	0.838000000000002\\
3.48020291947662	0.837000000000002\\
3.48913153425825	0.836000000000002\\
3.49857556866458	0.835000000000001\\
3.5096638619646	0.834000000000001\\
3.52054987945519	0.833000000000001\\
3.52855495368405	0.832000000000001\\
3.54217464567374	0.831000000000001\\
3.55077446355448	0.830000000000001\\
3.56373657540659	0.829000000000001\\
3.57285688921628	0.828000000000001\\
3.58264999416629	0.827000000000001\\
3.59583825042032	0.826000000000002\\
3.60477065248101	0.825000000000002\\
3.61291724306898	0.824000000000002\\
3.62061711285041	0.823000000000002\\
3.63163154423552	0.822000000000002\\
3.64628308897298	0.821000000000002\\
3.65682968482947	0.820000000000002\\
3.66349026526786	0.819000000000002\\
3.67558858325698	0.818000000000002\\
3.68309159150606	0.817000000000002\\
3.68819860393302	0.816000000000002\\
3.70083009846296	0.815000000000002\\
3.70893963943004	0.814000000000002\\
3.7205238165755	0.813000000000002\\
3.72501308889905	0.812000000000002\\
3.72932076846226	0.811000000000002\\
3.74542542644087	0.810000000000002\\
3.75149622840997	0.809000000000002\\
3.75513214290124	0.808000000000002\\
3.76867088882012	0.807000000000002\\
3.7797746120176	0.806000000000002\\
3.7916789482485	0.805000000000002\\
3.81074165330941	0.804000000000002\\
3.82561259912902	0.803000000000002\\
3.84208283206246	0.802000000000002\\
3.86022005685047	0.801000000000002\\
3.86354687921619	0.800000000000002\\
3.87177554640261	0.799000000000002\\
3.87599053053252	0.798000000000002\\
3.88274258576229	0.797000000000002\\
3.89734348645451	0.796000000000002\\
3.90594671018922	0.795000000000002\\
3.91730569433392	0.794000000000002\\
3.92328478952369	0.793000000000002\\
3.93138798088442	0.792000000000002\\
3.94472338333452	0.791000000000002\\
3.9630745707574	0.790000000000002\\
3.98021040271328	0.789000000000002\\
3.98831652702056	0.788000000000002\\
3.99497457770059	0.787000000000002\\
4.01039414715137	0.786000000000002\\
4.01433819910267	0.785000000000002\\
4.02112286552039	0.784000000000002\\
4.0310341739195	0.783000000000002\\
4.03437289047714	0.782000000000002\\
4.04034876386863	0.781000000000002\\
4.05370336510972	0.780000000000002\\
4.06669003899281	0.779000000000002\\
4.07867391261571	0.778000000000002\\
4.08410282382201	0.777000000000002\\
4.09381299132261	0.776000000000002\\
4.10025504155579	0.775000000000002\\
4.11130081509313	0.774000000000002\\
4.11825187287342	0.773000000000002\\
4.13796607194313	0.772000000000002\\
4.15399188016648	0.771000000000003\\
4.16229022745984	0.770000000000003\\
4.16673034155223	0.769000000000003\\
4.18373613041955	0.768000000000003\\
4.19084639151963	0.767000000000003\\
4.20507589302727	0.766000000000003\\
4.21122601512168	0.765000000000003\\
4.21545410187816	0.764000000000003\\
4.23731604537504	0.763000000000003\\
4.25117059318357	0.762000000000003\\
4.26261759783225	0.761000000000003\\
4.26939985714975	0.760000000000003\\
4.27714498912079	0.759000000000003\\
4.29476450990707	0.758000000000003\\
4.3022259616073	0.757000000000003\\
4.30720470852041	0.756000000000003\\
4.32116259892286	0.755000000000004\\
4.33183801617947	0.754000000000004\\
4.34328083528147	0.753000000000004\\
4.35635420057434	0.752000000000004\\
4.36918018135136	0.751000000000004\\
4.38811093001386	0.750000000000004\\
4.40052742163951	0.749000000000004\\
4.4102820983062	0.748000000000004\\
4.42478936743572	0.747000000000004\\
4.43295060675604	0.746000000000004\\
4.44114158118033	0.745000000000004\\
4.4535754194219	0.744000000000004\\
4.46838673782943	0.743000000000004\\
4.47973578555413	0.742000000000004\\
4.49351394385572	0.741000000000004\\
4.50058511950211	0.740000000000004\\
4.51714019701305	0.739000000000004\\
4.52115129288266	0.738000000000005\\
4.53392883498349	0.737000000000005\\
4.54974692533733	0.736000000000005\\
4.55402897333754	0.735000000000005\\
4.56316762417717	0.734000000000005\\
4.57470865252093	0.733000000000005\\
4.58088689257098	0.732000000000005\\
4.58444175012804	0.731000000000005\\
4.60044133737271	0.730000000000005\\
4.60376320500988	0.729000000000005\\
4.60941333907751	0.728000000000005\\
4.61827262968009	0.727000000000005\\
4.62934981090158	0.726000000000005\\
4.63733857357836	0.725000000000006\\
4.64464710227434	0.724000000000006\\
4.66851159785551	0.723000000000006\\
4.68635385462766	0.722000000000006\\
4.70216903541672	0.721000000000006\\
4.71106776743376	0.720000000000006\\
4.72542459350485	0.719000000000006\\
4.74726146509352	0.718000000000006\\
4.75531782738842	0.717000000000006\\
4.770524675557	0.716000000000006\\
4.78113339263205	0.715000000000006\\
4.78909238578244	0.714000000000006\\
4.79717599152148	0.713000000000006\\
4.80984801420607	0.712000000000006\\
4.82096368824169	0.711000000000006\\
4.83583000698384	0.710000000000006\\
4.83905523377358	0.709000000000006\\
4.85295424800786	0.708000000000006\\
4.86670206326197	0.707000000000007\\
4.8809414236298	0.706000000000007\\
4.88757948625235	0.705000000000007\\
4.90134302875892	0.704000000000007\\
4.90595908904679	0.703000000000007\\
4.91451672715756	0.702000000000007\\
4.92384827064396	0.701000000000007\\
4.94115467086407	0.700000000000007\\
4.95572320827391	0.699000000000007\\
4.96066702301601	0.698000000000007\\
4.97456244862242	0.697000000000007\\
4.9919420230212	0.696000000000007\\
5.0024890064232	0.695000000000007\\
5.02428511674126	0.694000000000007\\
5.02881482993736	0.693000000000007\\
5.04245066904365	0.692000000000007\\
5.04885557764746	0.691000000000007\\
5.07169466798526	0.690000000000007\\
5.09582978020115	0.689000000000007\\
5.10367955694005	0.688000000000007\\
5.11542815206564	0.687000000000007\\
5.12607392570189	0.686000000000007\\
5.14632793491665	0.685000000000007\\
5.1652600619987	0.684000000000007\\
5.1701010430286	0.683000000000007\\
5.1836415367869	0.682000000000007\\
5.20015239143354	0.681000000000007\\
5.20869770966085	0.680000000000007\\
5.22492597412887	0.679000000000008\\
5.24629893896491	0.678000000000008\\
5.2553034561681	0.677000000000008\\
5.26362486122776	0.676000000000008\\
5.26975415212914	0.675000000000008\\
5.28237480626485	0.674000000000008\\
5.29215640615226	0.673000000000008\\
5.29768582438503	0.672000000000008\\
5.31161454095168	0.671000000000008\\
5.31818552355975	0.670000000000008\\
5.33331330808165	0.669000000000008\\
5.35435694316056	0.668000000000008\\
5.36445225520346	0.667000000000008\\
5.37549040181727	0.666000000000008\\
5.38290931505058	0.665000000000008\\
5.39840046358074	0.664000000000008\\
5.40732090185827	0.663000000000009\\
5.42052094124221	0.662000000000009\\
5.43670816851839	0.661000000000009\\
5.44731435511432	0.660000000000009\\
5.45694700388245	0.659000000000009\\
5.46496394879969	0.658000000000009\\
5.47378597039396	0.657000000000009\\
5.48863709807773	0.656000000000009\\
5.50717804951217	0.655000000000009\\
5.51026334781273	0.654000000000009\\
5.51748587849175	0.653000000000009\\
5.52552482704648	0.652000000000009\\
5.53711771652107	0.651000000000009\\
5.54967905191886	0.650000000000009\\
5.567219907733	0.649000000000009\\
5.58171168532031	0.64800000000001\\
5.59609544408603	0.64700000000001\\
5.61232306288951	0.64600000000001\\
5.6225300190236	0.64500000000001\\
5.62760681422251	0.64400000000001\\
5.64009099725983	0.64300000000001\\
5.65232392021328	0.64200000000001\\
5.66397204621318	0.64100000000001\\
5.68803166912958	0.64000000000001\\
5.7006936373263	0.63900000000001\\
5.71782032300558	0.63800000000001\\
5.73452155324895	0.63700000000001\\
5.75099041112212	0.63600000000001\\
5.7756708687009	0.63500000000001\\
5.79666227997381	0.63400000000001\\
5.80339466621529	0.63300000000001\\
5.81042363450219	0.63200000000001\\
5.82888476174119	0.63100000000001\\
5.84040736758763	0.630000000000011\\
5.84676459770232	0.629000000000011\\
5.86211012899849	0.628000000000011\\
5.86903637705196	0.627000000000011\\
5.88812505192386	0.626000000000011\\
5.91831747877593	0.625000000000011\\
5.92857550391998	0.624000000000011\\
5.93353368325777	0.623000000000011\\
5.94682694964237	0.622000000000011\\
5.97160583673739	0.621000000000011\\
5.98583537875148	0.620000000000011\\
5.99924385587212	0.619000000000011\\
6.00279066898435	0.618000000000011\\
6.02130884360488	0.617000000000011\\
6.03201913688867	0.616000000000012\\
6.04429085094187	0.615000000000012\\
6.0504379223292	0.614000000000012\\
6.06329135896795	0.613000000000012\\
6.08096760961583	0.612000000000012\\
6.08564227966929	0.611000000000012\\
6.09885169889206	0.610000000000012\\
6.10735305714821	0.609000000000012\\
6.11539718932142	0.608000000000012\\
6.1276195747121	0.607000000000012\\
6.15163861844377	0.606000000000012\\
6.15958842810096	0.605000000000013\\
6.17214526943251	0.604000000000013\\
6.18945682208548	0.603000000000013\\
6.19877430842301	0.602000000000013\\
6.21210985891302	0.601000000000013\\
6.22871427769501	0.600000000000013\\
6.24533169716937	0.599000000000013\\
6.25434373452673	0.598000000000013\\
6.27351061925967	0.597000000000013\\
6.28554583604046	0.596000000000013\\
6.3076841054315	0.595000000000013\\
6.32537491362977	0.594000000000014\\
6.33276547877945	0.593000000000014\\
6.3410312371179	0.592000000000014\\
6.36112714626819	0.591000000000014\\
6.37036235079815	0.590000000000014\\
6.39194444811516	0.589000000000014\\
6.40655280800717	0.588000000000014\\
6.41493851695883	0.587000000000014\\
6.42833408982159	0.586000000000014\\
6.44314977610962	0.585000000000014\\
6.46015688415654	0.584000000000014\\
6.47718581468997	0.583000000000015\\
6.49352703643676	0.582000000000015\\
6.50364276784213	0.581000000000015\\
6.52012134013902	0.580000000000015\\
6.52714820115128	0.579000000000015\\
6.54247052688222	0.578000000000015\\
6.55525125761697	0.577000000000015\\
6.57948694864235	0.576000000000015\\
6.59811617051296	0.575000000000015\\
6.62120936538841	0.574000000000015\\
6.63447345543433	0.573000000000015\\
6.64758774766464	0.572000000000015\\
6.6684038246022	0.571000000000015\\
6.68676641056993	0.570000000000015\\
6.69194826406064	0.569000000000015\\
6.71212126245524	0.568000000000016\\
6.74220000049791	0.567000000000015\\
6.77331279911136	0.566000000000016\\
6.78999207523028	0.565000000000016\\
6.80904253620402	0.564000000000016\\
6.82725963315467	0.563000000000016\\
6.83673013623766	0.562000000000016\\
6.84316662251344	0.561000000000016\\
6.85471593491919	0.560000000000016\\
6.86427124112343	0.559000000000016\\
6.87622136058258	0.558000000000016\\
6.88625885272308	0.557000000000017\\
6.89594374431027	0.556000000000017\\
6.91960648260889	0.555000000000017\\
6.93317536127159	0.554000000000017\\
6.95954710331572	0.553000000000017\\
6.97362283519428	0.552000000000017\\
6.98471580176119	0.551000000000017\\
7.00283698252485	0.550000000000017\\
7.01098923934202	0.549000000000017\\
7.02692975152537	0.548000000000017\\
7.03361062890343	0.547000000000018\\
7.05303115625174	0.546000000000018\\
7.06565275469128	0.545000000000018\\
7.08163851489635	0.544000000000018\\
7.09278591884773	0.543000000000018\\
7.11512633339857	0.542000000000018\\
7.12825733727031	0.541000000000018\\
7.1380352523984	0.540000000000018\\
7.15155976822835	0.539000000000018\\
7.17906988515071	0.538000000000018\\
7.19205781613856	0.537000000000018\\
7.21272050872802	0.536000000000018\\
7.25469846575233	0.535000000000018\\
7.28141009304205	0.534000000000018\\
7.3152353011819	0.533000000000018\\
7.32528293030226	0.532000000000018\\
7.35006298574883	0.531000000000018\\
7.36019655233164	0.530000000000019\\
7.38503902871604	0.529000000000019\\
7.40080683729565	0.528000000000019\\
7.41848042747015	0.527000000000019\\
7.45468772018006	0.526000000000019\\
7.46564056429043	0.525000000000019\\
7.47641722213389	0.524000000000019\\
7.50924362558352	0.523000000000019\\
7.53018348250563	0.522000000000019\\
7.54822155503371	0.521000000000019\\
7.55524298087245	0.520000000000019\\
7.58487305475487	0.519000000000019\\
7.60990488429965	0.518000000000019\\
7.61925021002756	0.51700000000002\\
7.63561894940328	0.51600000000002\\
7.65539949261474	0.51500000000002\\
7.6795304394614	0.51400000000002\\
7.69186180807852	0.51300000000002\\
7.71361663344523	0.51200000000002\\
7.72678053187958	0.51100000000002\\
7.75526035900518	0.51000000000002\\
7.77105056378384	0.50900000000002\\
7.78347802175381	0.50800000000002\\
7.79598063265441	0.507000000000021\\
7.80698042728865	0.506000000000021\\
7.81333886543129	0.505000000000021\\
7.83187190848469	0.504000000000021\\
7.84295830667753	0.503000000000021\\
7.85878400661028	0.502000000000021\\
7.86703034874922	0.501000000000021\\
7.91488658162387	0.500000000000021\\
7.9488583584964	0.499000000000021\\
7.96068594156034	0.498000000000021\\
7.99145333808956	0.497000000000021\\
8.00870808754548	0.496000000000021\\
8.03972920749063	0.495000000000021\\
8.06164903194167	0.494000000000021\\
8.08645222667543	0.493000000000021\\
8.10471118042824	0.492000000000021\\
8.12600927366202	0.491000000000021\\
8.149096529848	0.490000000000021\\
8.16967485945764	0.489000000000021\\
8.18569579313914	0.488000000000021\\
8.19706415257969	0.487000000000021\\
8.22479739690605	0.48600000000002\\
8.26074938895415	0.48500000000002\\
8.28015291806761	0.48400000000002\\
8.29487179538935	0.483000000000021\\
8.31750166094515	0.48200000000002\\
8.33146297514073	0.48100000000002\\
8.35077916278353	0.48000000000002\\
8.36665887645257	0.47900000000002\\
8.37957512573759	0.47800000000002\\
8.40979000552593	0.47700000000002\\
8.44139560182009	0.47600000000002\\
8.45425888179978	0.47500000000002\\
8.48665538488234	0.47400000000002\\
8.50577479067335	0.47300000000002\\
8.52763232016494	0.47200000000002\\
8.5431691576253	0.47100000000002\\
8.55505982088932	0.47000000000002\\
8.57715106244836	0.46900000000002\\
8.60514409743626	0.46800000000002\\
8.62667848689165	0.46700000000002\\
8.65336235418395	0.46600000000002\\
8.67165008777225	0.46500000000002\\
8.701868285701	0.464000000000019\\
8.71636110126031	0.463000000000019\\
8.7687517383378	0.462000000000019\\
8.79903059799414	0.461000000000019\\
8.84812736835744	0.460000000000019\\
8.86468039041777	0.459000000000019\\
8.91453907030959	0.458000000000019\\
8.93589975402177	0.457000000000019\\
8.94996256008583	0.456000000000019\\
8.9763920124098	0.455000000000019\\
8.98753987910949	0.454000000000019\\
9.00534523560143	0.453000000000019\\
9.04887677547169	0.452000000000019\\
9.07878853266221	0.451000000000019\\
9.10160882727714	0.450000000000019\\
9.11930699804628	0.449000000000019\\
9.12597768022497	0.448000000000019\\
9.14660764988571	0.447000000000019\\
9.1593618814152	0.446000000000019\\
9.17948496569214	0.445000000000019\\
9.19033357910817	0.444000000000019\\
9.20451423213585	0.443000000000019\\
9.22895486481687	0.442000000000019\\
9.24372813608668	0.441000000000019\\
9.2540286828753	0.440000000000019\\
9.27979586345985	0.439000000000018\\
9.31251218457345	0.438000000000018\\
9.33117630721441	0.437000000000018\\
9.34483657721913	0.436000000000018\\
9.3751235128662	0.435000000000018\\
9.38737169977973	0.434000000000018\\
9.40587393616509	0.433000000000018\\
9.43511319514895	0.432000000000018\\
9.4472234659836	0.431000000000018\\
9.48106597057969	0.430000000000018\\
9.51424206943831	0.429000000000018\\
9.53769203092905	0.428000000000018\\
9.56205167162348	0.427000000000018\\
9.57600329650265	0.426000000000018\\
9.60023166043919	0.425000000000018\\
9.64033384126387	0.424000000000018\\
9.6729866750081	0.423000000000018\\
9.69586332800673	0.422000000000018\\
9.71313448937317	0.421000000000018\\
9.7296175502792	0.420000000000017\\
9.76412280896879	0.419000000000018\\
9.80305955689599	0.418000000000017\\
9.83700126734034	0.417000000000018\\
9.88547559531716	0.416000000000017\\
9.9244596527465	0.415000000000017\\
9.94574156564272	0.414000000000017\\
9.96476972977456	0.413000000000017\\
9.97988150458769	0.412000000000017\\
9.99074421153221	0.411000000000017\\
10.0113927319471	0.410000000000017\\
10.034600432154	0.409000000000017\\
10.0550903466511	0.408000000000017\\
10.1271675276598	0.407000000000017\\
10.1400506466151	0.406000000000017\\
10.1774487400138	0.405000000000017\\
10.2000949073408	0.404000000000017\\
10.2139026911801	0.403000000000017\\
10.2708014070473	0.402000000000017\\
10.2942909974571	0.401000000000017\\
10.3147888753846	0.400000000000017\\
10.3679528468917	0.399000000000017\\
10.404740993419	0.398000000000016\\
10.4488938879256	0.397000000000016\\
10.4648269550713	0.396000000000016\\
10.4821737047514	0.395000000000016\\
10.5157626652248	0.394000000000016\\
10.5437935205364	0.393000000000016\\
10.5717690127156	0.392000000000016\\
10.6002203080228	0.391000000000016\\
10.666713819107	0.390000000000016\\
10.7099731656106	0.389000000000016\\
10.7321190874848	0.388000000000016\\
10.7751092685258	0.387000000000016\\
10.8082718324811	0.386000000000016\\
10.8351699058235	0.385000000000016\\
10.8503020906501	0.384000000000016\\
10.8826863088685	0.383000000000016\\
10.9212892216185	0.382000000000016\\
10.9486237727476	0.381000000000016\\
10.9926260826393	0.380000000000016\\
11.0171386846618	0.379000000000016\\
11.0311349755134	0.378000000000016\\
11.0417247968846	0.377000000000016\\
11.0598827939371	0.376000000000016\\
11.0826595902269	0.375000000000016\\
11.0999390361886	0.374000000000015\\
11.1382502531917	0.373000000000015\\
11.1658380406489	0.372000000000015\\
11.2025117769248	0.371000000000015\\
11.2449846211021	0.370000000000015\\
11.2777384779643	0.369000000000015\\
11.3148733391808	0.368000000000015\\
11.3358232836615	0.367000000000015\\
11.3619831723659	0.366000000000015\\
11.3846232057045	0.365000000000015\\
11.4028598430568	0.364000000000015\\
11.4354589160067	0.363000000000015\\
11.46444382781	0.362000000000015\\
11.4824094183588	0.361000000000015\\
11.5115801682356	0.360000000000015\\
11.5286278782291	0.359000000000015\\
11.5953565420878	0.358000000000015\\
11.628951767674	0.357000000000015\\
11.6642325583924	0.356000000000015\\
11.7198354359761	0.355000000000015\\
11.7569478029256	0.354000000000015\\
11.8079329276037	0.353000000000015\\
11.8524463073664	0.352000000000015\\
11.8826241507342	0.351000000000015\\
11.966153531818	0.350000000000015\\
12.0441973786379	0.349000000000014\\
12.0755296001544	0.348000000000014\\
12.1176001613269	0.347000000000014\\
12.169124942928	0.346000000000014\\
12.1910176520657	0.345000000000014\\
12.2383843767858	0.344000000000014\\
12.2606695644245	0.343000000000014\\
12.3162680337984	0.342000000000014\\
12.3500494429432	0.341000000000014\\
12.4004917560588	0.340000000000014\\
12.446922044032	0.339000000000014\\
12.4832919377731	0.338000000000014\\
12.5379468523136	0.337000000000014\\
12.6280909460588	0.336000000000014\\
12.6706157829681	0.335000000000014\\
12.692235373148	0.334000000000014\\
12.7211316107867	0.333000000000014\\
12.7312400200212	0.332000000000013\\
12.775914925802	0.331000000000013\\
12.8348965075924	0.330000000000013\\
12.8470568023505	0.329000000000013\\
12.8814823310841	0.328000000000013\\
12.9456922689319	0.327000000000013\\
12.9671571516411	0.326000000000013\\
13.0350383733625	0.325000000000013\\
13.0690301697792	0.324000000000013\\
13.1201543625318	0.323000000000013\\
13.2189018313727	0.322000000000013\\
13.2778183155127	0.321000000000013\\
13.3110491644729	0.320000000000012\\
13.3478186605409	0.319000000000012\\
13.3921193162513	0.318000000000012\\
13.4381898072863	0.317000000000012\\
13.4920948085261	0.316000000000012\\
13.5272989246126	0.315000000000012\\
13.6041544401563	0.314000000000012\\
13.6492737877345	0.313000000000012\\
13.726158404017	0.312000000000012\\
13.7933178977657	0.311000000000012\\
13.8349934641157	0.310000000000012\\
13.8870656560755	0.309000000000012\\
13.9049806968355	0.308000000000012\\
13.9782398873583	0.307000000000012\\
14.0280726873814	0.306000000000012\\
14.0769930480598	0.305000000000012\\
14.1107856912945	0.304000000000012\\
14.1780779242091	0.303000000000012\\
14.3050348269131	0.302000000000012\\
14.3503205153674	0.301000000000012\\
14.4614223736942	0.300000000000012\\
14.5108672021424	0.299000000000011\\
14.5749750756471	0.298000000000011\\
14.6107187891158	0.297000000000011\\
14.6575861299625	0.296000000000011\\
14.736897225644	0.295000000000011\\
14.7695614104177	0.294000000000011\\
14.819233388949	0.293000000000011\\
14.8810830972781	0.292000000000011\\
14.8973990602612	0.291000000000011\\
14.9367131842176	0.290000000000011\\
14.9697744335143	0.289000000000011\\
15.0376380000512	0.288000000000011\\
15.1075104977352	0.287000000000011\\
15.1523434490932	0.28600000000001\\
15.204422671007	0.28500000000001\\
15.2402329132322	0.28400000000001\\
15.2788084507256	0.28300000000001\\
15.3459820945986	0.28200000000001\\
15.4004354989585	0.28100000000001\\
15.4525157720564	0.28000000000001\\
15.5453133476593	0.27900000000001\\
15.5697656330015	0.27800000000001\\
15.6452544601513	0.27700000000001\\
15.6808143530811	0.27600000000001\\
15.7418719754898	0.27500000000001\\
15.7912136864263	0.27400000000001\\
15.9071401108537	0.27300000000001\\
15.9288958900543	0.27200000000001\\
16.0566875601559	0.27100000000001\\
16.1710776310601	0.27000000000001\\
16.233093260741	0.26900000000001\\
16.2688746917768	0.26800000000001\\
16.3576553386593	0.26700000000001\\
16.4331304711067	0.26600000000001\\
16.4952588478806	0.26500000000001\\
16.5664758468801	0.26400000000001\\
16.650729850563	0.263000000000009\\
16.7190720012867	0.262000000000009\\
16.7617840183627	0.261000000000009\\
16.8076234740704	0.260000000000009\\
16.9416367143059	0.259000000000009\\
17.065042599131	0.258000000000009\\
17.1200068990387	0.257000000000009\\
17.2108825197314	0.256000000000009\\
17.3165729930518	0.255000000000009\\
17.3798618242487	0.254000000000009\\
17.4820540967036	0.253000000000009\\
17.5982710152	0.252000000000009\\
17.6618268973385	0.251000000000009\\
17.8244439078424	0.250000000000009\\
17.8562573700247	0.249000000000009\\
17.9272418352596	0.248000000000009\\
17.9987422183149	0.247000000000009\\
18.0540267477585	0.246000000000009\\
18.1005090552717	0.245000000000009\\
18.1564498637523	0.244000000000009\\
18.2310673128926	0.243000000000009\\
18.2979410920989	0.242000000000009\\
18.4710878088711	0.241000000000009\\
18.6055324826139	0.240000000000009\\
18.6969228967711	0.239000000000008\\
18.9043551454141	0.238000000000008\\
18.9712966612041	0.237000000000008\\
19.0838486025673	0.236000000000008\\
19.1871696235081	0.235000000000008\\
19.2725680961638	0.234000000000008\\
19.3610624004772	0.233000000000008\\
19.4922432504246	0.232000000000008\\
19.6052209369336	0.231000000000008\\
19.7488816062291	0.230000000000008\\
19.7995581065572	0.229000000000008\\
19.9609521214796	0.228000000000008\\
20.0196778571165	0.227000000000008\\
20.1096774541438	0.226000000000008\\
20.2865881124372	0.225000000000008\\
20.5021665945353	0.224000000000008\\
20.5544113428977	0.223000000000008\\
20.7086120754849	0.222000000000008\\
20.7808302005449	0.221000000000008\\
20.9177966647391	0.220000000000008\\
21.0147975151105	0.219000000000008\\
21.0729583358011	0.218000000000008\\
21.1246018390641	0.217000000000008\\
21.1940038737047	0.216000000000008\\
21.3316974522014	0.215000000000008\\
21.4175756030866	0.214000000000008\\
21.490395983649	0.213000000000008\\
21.6717882768883	0.212000000000008\\
21.9832262690894	0.211000000000008\\
22.2136579936899	0.210000000000008\\
22.2833746944649	0.209000000000008\\
22.4807272204771	0.208000000000008\\
22.7292514315783	0.207000000000008\\
22.7914775802433	0.206000000000008\\
22.8743663838356	0.205000000000008\\
22.9998611976646	0.204000000000008\\
23.1062201237963	0.203000000000007\\
23.2585681657591	0.202000000000007\\
23.440079232948	0.201000000000007\\
23.5341024075876	0.200000000000007\\
23.6627458426806	0.199000000000007\\
23.7663682739547	0.198000000000007\\
23.8221788909067	0.197000000000007\\
24.0301815168172	0.196000000000007\\
24.1585089611377	0.195000000000007\\
24.2723057106245	0.194000000000007\\
24.5336627141027	0.193000000000007\\
24.7521391547984	0.192000000000007\\
24.8676208786583	0.191000000000007\\
24.9311666043066	0.190000000000007\\
25.060368119459	0.189000000000007\\
25.3191323038879	0.188000000000007\\
25.5156003064714	0.187000000000007\\
25.8141139378735	0.186000000000007\\
26.0073879579469	0.185000000000007\\
26.0774840294016	0.184000000000007\\
26.1601881527665	0.183000000000007\\
26.5733625449124	0.182000000000007\\
26.8374831061731	0.181000000000007\\
26.936431040863	0.180000000000007\\
27.127459575464	0.179000000000007\\
27.2803795127384	0.178000000000007\\
27.4784678147012	0.177000000000007\\
27.5824176555552	0.176000000000007\\
27.7776107130883	0.175000000000007\\
28.1216054770458	0.174000000000007\\
28.2027525423651	0.173000000000007\\
28.3627570564594	0.172000000000007\\
28.5690717929269	0.171000000000006\\
28.7028383511223	0.170000000000006\\
28.8972600443195	0.169000000000006\\
29.0468879579705	0.168000000000006\\
29.1284778715254	0.167000000000006\\
29.4960340857507	0.166000000000006\\
29.6463985814579	0.165000000000006\\
29.7184484173929	0.164000000000006\\
29.8011981221951	0.163000000000006\\
29.9204028880617	0.162000000000006\\
30.0082256034253	0.161000000000006\\
30.3116194372615	0.160000000000006\\
30.5475007084472	0.159000000000006\\
30.7297454331635	0.158000000000006\\
30.8356497680435	0.157000000000006\\
31.3337556790524	0.156000000000006\\
31.4728109672797	0.155000000000006\\
31.8605587917328	0.154000000000006\\
32.2755014413508	0.153000000000006\\
32.4698919373334	0.152000000000006\\
32.6200627168407	0.151000000000006\\
32.8570110882117	0.150000000000006\\
33.2766628830201	0.149000000000006\\
33.6199937325276	0.148000000000006\\
33.6944638676553	0.147000000000006\\
33.848159333259	0.146000000000006\\
34.0698601850191	0.145000000000006\\
34.7533979837906	0.144000000000006\\
35.1125351309508	0.143000000000006\\
35.6599514942634	0.142000000000006\\
36.1270162513533	0.141000000000006\\
36.7691090107347	0.140000000000006\\
37.0189874676173	0.139000000000006\\
37.3381746024238	0.138000000000006\\
37.8654252032415	0.137000000000006\\
38.230685300023	0.136000000000005\\
38.632353856634	0.135000000000005\\
38.9713774085567	0.134000000000005\\
39.2422426814863	0.133000000000005\\
39.7737450037278	0.132000000000005\\
40.1276602096915	0.131000000000005\\
40.5063540357181	0.130000000000005\\
40.9934782725196	0.129000000000005\\
41.3570224931619	0.128000000000005\\
41.6767546788883	0.127000000000005\\
42.1574171480661	0.126000000000005\\
42.515588698208	0.125000000000005\\
42.795592118706	0.124000000000005\\
43.270247359803	0.123000000000005\\
44.1030498405003	0.122000000000005\\
44.1968580405127	0.121000000000005\\
44.8078195723986	0.120000000000005\\
45.3130982297366	0.119000000000005\\
46.3927166190219	0.118000000000005\\
46.8692351100919	0.117000000000005\\
47.6619079519939	0.116000000000005\\
47.9653275925808	0.115000000000005\\
48.2900102317201	0.114000000000005\\
49.0629760137339	0.113000000000005\\
49.8259247512401	0.112000000000005\\
50.7283202287856	0.111000000000005\\
51.1958179327412	0.110000000000005\\
51.7772652371812	0.109000000000005\\
52.1665996565625	0.108000000000005\\
52.8091598715269	0.107000000000005\\
53.4083577232262	0.106000000000004\\
54.6128351519164	0.105000000000004\\
55.6575097396894	0.104000000000004\\
56.4032315119993	0.103000000000004\\
58.4278304052087	0.102000000000004\\
59.694688888494	0.101000000000004\\
60.8661229673466	0.100000000000004\\
62.4721448553213	0.0990000000000042\\
63.9409334755424	0.0980000000000041\\
65.1179951166744	0.0970000000000041\\
66.7946138508611	0.0960000000000041\\
67.5048239817812	0.095000000000004\\
68.5139604173126	0.094000000000004\\
70.3609176200807	0.093000000000004\\
72.2415105984366	0.0920000000000039\\
73.1855143934301	0.0910000000000039\\
73.8779221189588	0.0900000000000039\\
75.6964455633369	0.0890000000000037\\
77.1170286675225	0.0880000000000037\\
79.5714214792813	0.0870000000000037\\
81.0038705359686	0.0860000000000037\\
82.5722193479969	0.0850000000000036\\
83.7000926284358	0.0840000000000036\\
84.8579244253927	0.0830000000000036\\
86.6186480418173	0.0820000000000036\\
88.2543666830712	0.0810000000000035\\
91.2732710059859	0.0800000000000035\\
94.0482022829031	0.0790000000000035\\
96.2377963589539	0.0780000000000034\\
100.294732901247	0.0770000000000034\\
103.028089575795	0.0760000000000034\\
104.155370234733	0.0750000000000034\\
106.214823337774	0.0740000000000033\\
109.463705952948	0.0730000000000033\\
111.039427299609	0.0720000000000033\\
114.647051942446	0.0710000000000033\\
119.748779971634	0.0700000000000032\\
123.657439353947	0.0690000000000032\\
127.311122255533	0.0680000000000032\\
130.78638613317	0.0670000000000031\\
134.302229128868	0.0660000000000031\\
138.150255374066	0.0650000000000031\\
143.300550606919	0.0640000000000031\\
151.267976719641	0.0630000000000029\\
156.774626174294	0.0620000000000029\\
160.360797133906	0.0610000000000029\\
168.950779140267	0.0600000000000028\\
177.831648570356	0.0590000000000028\\
185.377725694643	0.0580000000000027\\
195.382481109596	0.0570000000000027\\
199.863745956757	0.0560000000000027\\
204.807229179346	0.0550000000000026\\
209.009080536021	0.0540000000000026\\
215.886771806692	0.0530000000000025\\
220.965131815383	0.0520000000000025\\
228.908544102796	0.0510000000000024\\
238.482221204566	0.0500000000000024\\
245.964082665097	0.0490000000000024\\
250.46222483574	0.0480000000000023\\
265.200818013659	0.0470000000000023\\
282.51190274039	0.0460000000000023\\
290.474373614613	0.0450000000000021\\
300.890285969135	0.0440000000000021\\
314.153829552899	0.0430000000000021\\
351.328503289119	0.042000000000002\\
377.485360851362	0.041000000000002\\
390.43354243551	0.0400000000000019\\
447.39064476296	0.0390000000000019\\
480.367834322766	0.0380000000000018\\
562.420216789638	0.0370000000000018\\
596.06160954251	0.0360000000000017\\
634.357550096335	0.0350000000000017\\
704.738486646722	0.0340000000000017\\
732.94822662744	0.0330000000000016\\
807.655598201321	0.0320000000000016\\
892.317159319283	0.0310000000000015\\
998.670564789707	0.0300000000000015\\
1038.95101890341	0.0290000000000014\\
1100.49248444499	0.0280000000000014\\
1156.88639835805	0.0270000000000014\\
1224.40100579328	0.0260000000000012\\
1403.59568220677	0.0250000000000012\\
1540.03061672254	0.0240000000000011\\
1683.34232897975	0.0230000000000011\\
1773.13723952254	0.0220000000000011\\
1962.31828026256	0.021000000000001\\
2282.45542317394	0.020000000000001\\
2455.33736209845	0.0190000000000009\\
2732.93376801947	0.0180000000000009\\
3016.68189947343	0.0170000000000008\\
3301.37765566027	0.0160000000000008\\
3407.84863505354	0.0150000000000008\\
3613.15914120432	0.0140000000000007\\
3863.40955425342	0.0130000000000007\\
4354.63337567702	0.0120000000000006\\
4500.84738165432	0.0110000000000006\\
4996.38343342568	0.0100000000000005\\
5532.63979419089	0.00900000000000045\\
5931.52277971182	0.00800000000000045\\
6261.51619561273	0.00700000000000034\\
6715.06799688804	0.00600000000000034\\
7220.82424424722	0.00500000000000023\\
13113.3949431532	0.00400000000000023\\
14449.6846609933	0.00300000000000011\\
14766.6152410997	0.00200000000000011\\
15807.1611171138	0.001\\
16678.8794915604	0\\
};
\addlegendentry{$K=10$, $G=\;\,5$, $\lrmse =859.3$, $\prmse =0.067$, $\armse =0.054$, $\brmse =4\hspace{-3pt}\times\hspace{-3pt}10^{-4}$, $\gamma=40$}


==> figures/mse_N_2_K_20_G_5_SNR_1000_I_20_Pratio_2_Nratio_1_cs.tex <==
\addplot [color=blue,line width=0.2pt]
  table[row sep=crcr]{%
2.52489739006169e-12	1\\
4.54320825217294e-12	0.999\\
6.25510105502795e-12	0.998\\
7.63058060081213e-12	0.997\\
9.45721437487256e-12	0.996\\
1.00258964834339e-11	0.995\\
1.10823166220824e-11	0.994\\
1.27268340012565e-11	0.993\\
1.32489072038955e-11	0.992\\
1.34958535225004e-11	0.991\\
1.45659042534169e-11	0.99\\
1.59212571457571e-11	0.989\\
1.6853864002934e-11	0.988\\
1.78010682057969e-11	0.987\\
1.80601122722788e-11	0.986\\
1.85519537914928e-11	0.985\\
1.89275995192203e-11	0.984\\
1.94807131947758e-11	0.983\\
1.99628268272956e-11	0.982\\
2.06736826156008e-11	0.981\\
2.13284052214447e-11	0.98\\
2.23011735856548e-11	0.979\\
2.27132006890924e-11	0.978\\
2.33069108464204e-11	0.977\\
2.37394784385644e-11	0.976\\
2.43242181850982e-11	0.975\\
2.45123691662042e-11	0.974\\
2.55866439147212e-11	0.973\\
2.6090835131009e-11	0.972\\
2.67715606168235e-11	0.971\\
2.77148977037888e-11	0.970000000000001\\
2.83520619609247e-11	0.969\\
2.87437222145965e-11	0.968\\
2.92349853415461e-11	0.967000000000001\\
2.96980106498778e-11	0.966000000000001\\
3.01004554875558e-11	0.965000000000001\\
3.04188382505101e-11	0.964000000000001\\
3.0969805374789e-11	0.963000000000001\\
3.16903239074221e-11	0.962000000000001\\
3.20526828309613e-11	0.961000000000001\\
3.25126964512586e-11	0.960000000000001\\
3.32111657601427e-11	0.959000000000001\\
3.38391813465611e-11	0.958000000000001\\
3.41639942263786e-11	0.957000000000001\\
3.48701603947956e-11	0.956000000000001\\
3.6181550547734e-11	0.955000000000001\\
3.70689811561841e-11	0.954000000000001\\
3.73109853790836e-11	0.953000000000001\\
3.76036321033636e-11	0.952000000000001\\
3.79464202155226e-11	0.951000000000001\\
3.83207284877115e-11	0.950000000000001\\
3.89503973779679e-11	0.949000000000001\\
3.95141497400513e-11	0.948000000000001\\
3.98264419922009e-11	0.947000000000001\\
4.01891011353022e-11	0.946000000000001\\
4.04697699202627e-11	0.945000000000001\\
4.09203134610275e-11	0.944000000000001\\
4.14007833012941e-11	0.943000000000001\\
4.20626800407511e-11	0.942000000000001\\
4.26193080942083e-11	0.941000000000001\\
4.35028593157028e-11	0.940000000000001\\
4.37027758831263e-11	0.939000000000001\\
4.45838066988284e-11	0.938000000000001\\
4.50673682071163e-11	0.937000000000001\\
4.61085366686325e-11	0.936000000000001\\
4.67523988943212e-11	0.935000000000001\\
4.74370591248044e-11	0.934000000000001\\
4.79893472981084e-11	0.933000000000001\\
4.87727879189671e-11	0.932000000000001\\
4.91896373414646e-11	0.931000000000001\\
4.95443876826387e-11	0.930000000000001\\
5.03743109854224e-11	0.929000000000001\\
5.11276218411234e-11	0.928000000000001\\
5.16828101301896e-11	0.927000000000001\\
5.22619692137065e-11	0.926000000000001\\
5.25853241898417e-11	0.925000000000001\\
5.3207506736439e-11	0.924000000000001\\
5.39733051397045e-11	0.923000000000001\\
5.52368373097491e-11	0.922000000000001\\
5.62864670197327e-11	0.921000000000001\\
5.68939870107723e-11	0.920000000000001\\
5.75345543673246e-11	0.919000000000001\\
5.85563437433116e-11	0.918000000000001\\
5.87118018613269e-11	0.917000000000001\\
5.96938247644112e-11	0.916000000000001\\
6.03792242713064e-11	0.915000000000001\\
6.0711751823978e-11	0.914000000000001\\
6.09558673419202e-11	0.913000000000001\\
6.13183807663315e-11	0.912000000000001\\
6.19569276152638e-11	0.911000000000001\\
6.27319860254577e-11	0.910000000000001\\
6.29581089261555e-11	0.909000000000001\\
6.35513490358428e-11	0.908000000000001\\
6.42999389881583e-11	0.907000000000001\\
6.46113977973885e-11	0.906000000000001\\
6.5052872408991e-11	0.905000000000001\\
6.55974592955939e-11	0.904000000000001\\
6.69934995153925e-11	0.903000000000001\\
6.76065504086868e-11	0.902000000000001\\
6.88197105746909e-11	0.901000000000001\\
6.94427123988487e-11	0.900000000000001\\
7.0958439155597e-11	0.899000000000001\\
7.13217583990199e-11	0.898000000000001\\
7.19034998490284e-11	0.897000000000001\\
7.28293756901126e-11	0.896000000000001\\
7.32555377143772e-11	0.894800000000001\\
7.36574249171407e-11	0.893800000000001\\
7.45000666670991e-11	0.892800000000001\\
7.50343087260683e-11	0.891800000000001\\
7.55979004398743e-11	0.890800000000001\\
7.60317276171882e-11	0.889800000000001\\
7.64974784022704e-11	0.888800000000001\\
7.6841285995651e-11	0.887800000000001\\
7.75993152411611e-11	0.886800000000001\\
7.86871297989645e-11	0.885800000000001\\
7.92217321831014e-11	0.884800000000001\\
8.00020989663596e-11	0.883800000000001\\
8.11450904059144e-11	0.882800000000001\\
8.16029646872052e-11	0.881800000000001\\
8.19492382324246e-11	0.880800000000001\\
8.27319249736699e-11	0.879800000000001\\
8.35112094927473e-11	0.878800000000001\\
8.4063868741599e-11	0.877800000000001\\
8.47003564181963e-11	0.876800000000001\\
8.58709401827334e-11	0.875800000000001\\
8.63399748796157e-11	0.874800000000001\\
8.67799314476158e-11	0.873800000000001\\
8.72513891146795e-11	0.872800000000001\\
8.77838949560248e-11	0.871800000000001\\
8.89542912501823e-11	0.870800000000001\\
9.00160767157795e-11	0.869800000000001\\
9.09439644146639e-11	0.868800000000001\\
9.13708429502524e-11	0.867800000000001\\
9.18211259613137e-11	0.866800000000001\\
9.26449423205887e-11	0.865800000000001\\
9.33670458561105e-11	0.864800000000001\\
9.36455258458814e-11	0.863800000000001\\
9.39743955275545e-11	0.862800000000001\\
9.44000669660366e-11	0.861800000000001\\
9.47650716822854e-11	0.860800000000001\\
9.57608333060022e-11	0.859800000000001\\
9.65576285702463e-11	0.858800000000001\\
9.74296240729484e-11	0.857800000000001\\
9.83742699428115e-11	0.856800000000001\\
9.90527523061974e-11	0.855800000000001\\
1.0015670698186e-10	0.854800000000001\\
1.00511738918877e-10	0.853800000000001\\
1.00933185606068e-10	0.852800000000001\\
1.01533946445145e-10	0.851800000000001\\
1.02051099274173e-10	0.850800000000001\\
1.02742844248557e-10	0.849800000000001\\
1.0322520710987e-10	0.848800000000001\\
1.03872482815914e-10	0.847800000000001\\
1.04616698832841e-10	0.846800000000001\\
1.05044977032648e-10	0.845800000000001\\
1.05686530657071e-10	0.844800000000001\\
1.06280993940791e-10	0.843800000000001\\
1.06999443188037e-10	0.842800000000001\\
1.07861027617485e-10	0.841800000000001\\
1.08695441694079e-10	0.840800000000001\\
1.09447722332551e-10	0.839800000000001\\
1.10524715848102e-10	0.838800000000001\\
1.11683392002136e-10	0.837800000000001\\
1.11978884114712e-10	0.836800000000001\\
1.12550977736391e-10	0.835800000000001\\
1.1314394091263e-10	0.834800000000001\\
1.13674857339841e-10	0.833800000000001\\
1.14949593102004e-10	0.832800000000001\\
1.15458331285484e-10	0.831800000000001\\
1.1578037806283e-10	0.830800000000001\\
1.16921651629583e-10	0.829800000000001\\
1.17571003650413e-10	0.828800000000001\\
1.18555600248496e-10	0.827800000000001\\
1.19372099926169e-10	0.826800000000001\\
1.19734047005735e-10	0.825800000000001\\
1.20684254417377e-10	0.824800000000002\\
1.21095938806349e-10	0.823800000000002\\
1.21769854598574e-10	0.822800000000002\\
1.23202174296586e-10	0.821800000000002\\
1.23595122874425e-10	0.820800000000002\\
1.23911642012606e-10	0.819800000000002\\
1.24246740509423e-10	0.818800000000002\\
1.25956409869493e-10	0.817800000000002\\
1.26685465808517e-10	0.816800000000002\\
1.2756051071874e-10	0.815800000000002\\
1.28864530671061e-10	0.814800000000002\\
1.29472990854777e-10	0.813800000000002\\
1.30264706477355e-10	0.812800000000002\\
1.30948389663302e-10	0.811800000000002\\
1.31621132764778e-10	0.810800000000002\\
1.32025448415741e-10	0.809800000000002\\
1.32313702136879e-10	0.808800000000002\\
1.33266073853378e-10	0.807800000000002\\
1.34391210786296e-10	0.806800000000002\\
1.34926763473247e-10	0.805800000000002\\
1.35932999095362e-10	0.804800000000002\\
1.36546174615397e-10	0.803800000000002\\
1.37376775747518e-10	0.802800000000002\\
1.38177618255386e-10	0.801800000000002\\
1.38850709026716e-10	0.800800000000002\\
1.4022892394908e-10	0.799800000000002\\
1.41237952453127e-10	0.798800000000002\\
1.42117235403001e-10	0.797800000000002\\
1.43188470563938e-10	0.796800000000002\\
1.43563036908096e-10	0.795800000000002\\
1.44170719053863e-10	0.794800000000002\\
1.4522251197936e-10	0.793800000000002\\
1.46514945877402e-10	0.792800000000002\\
1.4755021162443e-10	0.791800000000002\\
1.49258330145177e-10	0.790800000000002\\
1.50272673610761e-10	0.789800000000002\\
1.51343614518534e-10	0.788800000000002\\
1.52393699591884e-10	0.787800000000002\\
1.53369580157263e-10	0.786800000000002\\
1.53707936546458e-10	0.785800000000002\\
1.53913431677501e-10	0.784800000000002\\
1.54609344861463e-10	0.783800000000002\\
1.554271447975e-10	0.782800000000002\\
1.56411339731346e-10	0.781800000000002\\
1.57520699056431e-10	0.780800000000002\\
1.5831564666512e-10	0.779800000000002\\
1.59180096596513e-10	0.778800000000002\\
1.60225103077782e-10	0.777800000000002\\
1.61681799806829e-10	0.776800000000002\\
1.63044534925417e-10	0.775800000000002\\
1.63903225122943e-10	0.774800000000002\\
1.64238494376213e-10	0.773800000000002\\
1.65007789958078e-10	0.772800000000002\\
1.66167579482367e-10	0.771800000000002\\
1.66747243224582e-10	0.770800000000002\\
1.68184050466732e-10	0.769800000000003\\
1.68948856390379e-10	0.768800000000003\\
1.69376966242003e-10	0.767800000000003\\
1.69709490438066e-10	0.766800000000003\\
1.70188571910668e-10	0.765800000000003\\
1.70867896717581e-10	0.764800000000003\\
1.71882188229349e-10	0.763800000000003\\
1.72206177026343e-10	0.762800000000003\\
1.73171758959926e-10	0.761800000000003\\
1.73669222282495e-10	0.760800000000003\\
1.74318664491265e-10	0.759800000000003\\
1.76678636584358e-10	0.758800000000003\\
1.77437314702321e-10	0.757800000000003\\
1.78172059370084e-10	0.756800000000003\\
1.79700561536558e-10	0.755800000000003\\
1.80864727425538e-10	0.754800000000003\\
1.82479825217749e-10	0.753800000000003\\
1.84149236479164e-10	0.752800000000003\\
1.84783362989052e-10	0.751800000000004\\
1.85377764648104e-10	0.750800000000004\\
1.86514269178527e-10	0.749800000000004\\
1.87933661679769e-10	0.748800000000004\\
1.89603172773053e-10	0.747800000000004\\
1.90769429101731e-10	0.746800000000004\\
1.91347694509969e-10	0.745800000000004\\
1.92225798340178e-10	0.744800000000004\\
1.92910972495223e-10	0.743800000000004\\
1.93362471369992e-10	0.742800000000004\\
1.94446979147928e-10	0.741800000000004\\
1.95170743049263e-10	0.740800000000004\\
1.96119021610587e-10	0.739800000000004\\
1.96486675513594e-10	0.738800000000004\\
1.97061845988343e-10	0.737800000000004\\
1.9889432046494e-10	0.736800000000005\\
1.99443624546578e-10	0.735800000000005\\
2.01921114026053e-10	0.734800000000005\\
2.02228006418165e-10	0.733800000000005\\
2.02880046850799e-10	0.732800000000005\\
2.03640649599705e-10	0.731800000000005\\
2.0445879259359e-10	0.730800000000005\\
2.05161427162263e-10	0.729800000000005\\
2.06619660307903e-10	0.728800000000005\\
2.07900421704709e-10	0.727800000000005\\
2.09100353232516e-10	0.726800000000005\\
2.1065809811793e-10	0.725800000000005\\
2.1176574547093e-10	0.724800000000005\\
2.12791248838054e-10	0.723800000000005\\
2.14373625567601e-10	0.722800000000005\\
2.15298386666171e-10	0.721800000000005\\
2.15889029887275e-10	0.720800000000005\\
2.16708852872467e-10	0.719800000000006\\
2.18298652318752e-10	0.718800000000006\\
2.19921569640209e-10	0.717800000000006\\
2.21076897965179e-10	0.716800000000006\\
2.22366515966016e-10	0.715800000000006\\
2.23516567146384e-10	0.714800000000006\\
2.24193659782379e-10	0.713800000000006\\
2.26074404043039e-10	0.712800000000006\\
2.271009476855e-10	0.711800000000006\\
2.27437451920228e-10	0.710800000000006\\
2.28072738336198e-10	0.709800000000006\\
2.28934044915815e-10	0.708800000000006\\
2.29814990334964e-10	0.707800000000006\\
2.31097805479897e-10	0.706800000000006\\
2.31635635004691e-10	0.705800000000006\\
2.33294243188189e-10	0.704800000000006\\
2.34478615324946e-10	0.703800000000007\\
2.35169479104231e-10	0.702800000000007\\
2.36490854912924e-10	0.701800000000007\\
2.37592605527221e-10	0.700800000000007\\
2.3892005227103e-10	0.699800000000007\\
2.39615609452037e-10	0.698800000000007\\
2.41609407904454e-10	0.697800000000007\\
2.42255314245167e-10	0.696800000000007\\
2.441353851974e-10	0.695800000000007\\
2.46207701750123e-10	0.694800000000007\\
2.47032030279253e-10	0.693800000000007\\
2.47619667258532e-10	0.692800000000007\\
2.48372880931207e-10	0.691800000000007\\
2.50314216059788e-10	0.690800000000007\\
2.51067724168927e-10	0.689800000000007\\
2.51906677346377e-10	0.688800000000007\\
2.53645033074734e-10	0.687800000000007\\
2.54588880131416e-10	0.686800000000007\\
2.55090749668237e-10	0.685800000000007\\
2.5625767414324e-10	0.684800000000007\\
2.57164628574718e-10	0.683800000000007\\
2.58332271717419e-10	0.682800000000007\\
2.5923608659899e-10	0.681800000000007\\
2.61723707532873e-10	0.680800000000007\\
2.62966405290746e-10	0.679800000000007\\
2.64423869566563e-10	0.678800000000008\\
2.6538092665481e-10	0.677800000000008\\
2.66857580896271e-10	0.676800000000008\\
2.67813755247537e-10	0.675800000000008\\
2.69490004248508e-10	0.674800000000008\\
2.71959833261182e-10	0.673800000000008\\
2.7292916360621e-10	0.672800000000008\\
2.75940358148096e-10	0.671800000000008\\
2.77775591259868e-10	0.670800000000008\\
2.78487999131108e-10	0.669800000000008\\
2.79171313140186e-10	0.668800000000008\\
2.81125321719913e-10	0.667800000000008\\
2.82412755888771e-10	0.666800000000008\\
2.83166465259378e-10	0.665800000000008\\
2.85953123720078e-10	0.664800000000008\\
2.88812378625397e-10	0.663800000000008\\
2.90408133179843e-10	0.662800000000008\\
2.91480061499771e-10	0.661800000000009\\
2.93584608860875e-10	0.660800000000009\\
2.9482942831441e-10	0.659800000000009\\
2.95878731782167e-10	0.658800000000009\\
2.96950511142865e-10	0.657800000000009\\
2.98887897692291e-10	0.656800000000009\\
3.00582990965384e-10	0.655800000000009\\
3.02049990336135e-10	0.654800000000009\\
3.03180064711012e-10	0.653800000000009\\
3.04577970710827e-10	0.652800000000009\\
3.06346540558576e-10	0.651800000000009\\
3.08924109204998e-10	0.650800000000009\\
3.09946664391497e-10	0.649800000000009\\
3.11441966844467e-10	0.648800000000009\\
3.1382261719623e-10	0.647800000000009\\
3.16169002785651e-10	0.646800000000009\\
3.20088508022069e-10	0.645800000000009\\
3.2312215835462e-10	0.64480000000001\\
3.26024147360175e-10	0.64380000000001\\
3.26948037207921e-10	0.64280000000001\\
3.29312215326066e-10	0.64180000000001\\
3.30539647972137e-10	0.64080000000001\\
3.32678768930568e-10	0.63980000000001\\
3.34020461434258e-10	0.63880000000001\\
3.35972469369339e-10	0.63780000000001\\
3.37811117294343e-10	0.63680000000001\\
3.38736568553889e-10	0.63580000000001\\
3.39494143847004e-10	0.63480000000001\\
3.42021896226622e-10	0.63380000000001\\
3.45979981148696e-10	0.63280000000001\\
3.4716317645108e-10	0.63180000000001\\
3.48289665501655e-10	0.63080000000001\\
3.5040574476928e-10	0.62980000000001\\
3.53101481593486e-10	0.628800000000011\\
3.5431357942446e-10	0.62780000000001\\
3.55752346892982e-10	0.62680000000001\\
3.57523940227233e-10	0.625800000000011\\
3.59582932338304e-10	0.624800000000011\\
3.61298873059341e-10	0.623800000000011\\
3.62888475047831e-10	0.622800000000011\\
3.64950890887964e-10	0.621800000000011\\
3.6604756524317e-10	0.620800000000011\\
3.67302803225898e-10	0.619800000000011\\
3.68880626795426e-10	0.618800000000011\\
3.71228202319954e-10	0.617800000000011\\
3.71796687297016e-10	0.616800000000011\\
3.73976677003485e-10	0.615800000000011\\
3.75201686256669e-10	0.614800000000012\\
3.76921423876807e-10	0.613800000000012\\
3.78578876618708e-10	0.612800000000012\\
3.79750714530658e-10	0.611800000000012\\
3.82289958374676e-10	0.610800000000012\\
3.83460985964554e-10	0.609800000000012\\
3.84885996815411e-10	0.608800000000012\\
3.86694999584264e-10	0.607800000000012\\
3.89420898110853e-10	0.606800000000012\\
3.90025046000079e-10	0.605800000000012\\
3.92588471540806e-10	0.604800000000012\\
3.95127464975332e-10	0.603800000000013\\
3.98586110811445e-10	0.602800000000013\\
4.00772089848733e-10	0.601800000000013\\
4.02200381216731e-10	0.600800000000013\\
4.0399150462966e-10	0.599800000000013\\
4.06521448731406e-10	0.598800000000013\\
4.07232731509817e-10	0.597800000000013\\
4.09839788549392e-10	0.596800000000013\\
4.11806463447726e-10	0.595800000000013\\
4.13512646823799e-10	0.594800000000013\\
4.14378621588711e-10	0.593800000000013\\
4.16893854143997e-10	0.592800000000014\\
4.1926805714851e-10	0.591800000000014\\
4.24114233577787e-10	0.590800000000014\\
4.26649587447824e-10	0.589800000000014\\
4.33725343276999e-10	0.588800000000014\\
4.35183239614374e-10	0.587800000000014\\
4.36970243381915e-10	0.586800000000014\\
4.37705398481435e-10	0.585800000000014\\
4.40294155529232e-10	0.584800000000014\\
4.4302188576931e-10	0.583800000000014\\
4.4532970153666e-10	0.582800000000014\\
4.46487325152756e-10	0.581800000000014\\
4.48146091571016e-10	0.580800000000015\\
4.49553954117083e-10	0.579800000000015\\
4.50037255732324e-10	0.578800000000015\\
4.510784930006e-10	0.577800000000015\\
4.51833201147657e-10	0.576800000000015\\
4.53168013512751e-10	0.575800000000015\\
4.53844979355315e-10	0.574800000000015\\
4.56031070642323e-10	0.573800000000015\\
4.57035570464098e-10	0.572800000000015\\
4.58410346256682e-10	0.571800000000015\\
4.61954215117143e-10	0.570800000000015\\
4.65855844474025e-10	0.569800000000015\\
4.68049567148842e-10	0.568800000000016\\
4.69318606834152e-10	0.567800000000016\\
4.7212013911549e-10	0.566800000000016\\
4.74644797392586e-10	0.565800000000016\\
4.76981121305683e-10	0.564800000000016\\
4.79077717641265e-10	0.563800000000016\\
4.83975969553604e-10	0.562800000000016\\
4.86899862135178e-10	0.561800000000016\\
4.88393745863612e-10	0.560800000000016\\
4.90690804294452e-10	0.559800000000016\\
4.92988936865836e-10	0.558800000000016\\
4.96600602449483e-10	0.557800000000017\\
5.00905629375029e-10	0.556800000000017\\
5.03250597816494e-10	0.555800000000017\\
5.04730383894356e-10	0.554800000000017\\
5.06141737623908e-10	0.553800000000017\\
5.08092730135355e-10	0.552800000000017\\
5.09992881690733e-10	0.551800000000017\\
5.15129250421414e-10	0.550800000000017\\
5.16712149337428e-10	0.549800000000017\\
5.19243740255655e-10	0.548800000000017\\
5.2215853604223e-10	0.547800000000017\\
5.25078614486248e-10	0.546800000000018\\
5.25511188833514e-10	0.545800000000018\\
5.28380184795365e-10	0.544800000000018\\
5.31356058700586e-10	0.543800000000018\\
5.33657950390734e-10	0.542800000000018\\
5.34581876862229e-10	0.541800000000018\\
5.37428183875986e-10	0.540800000000018\\
5.40695694552255e-10	0.539800000000018\\
5.43103636807714e-10	0.538800000000018\\
5.45345629630891e-10	0.537800000000018\\
5.49500623046466e-10	0.536800000000018\\
5.51296565981141e-10	0.535800000000018\\
5.51974348497006e-10	0.534800000000018\\
5.58303006695771e-10	0.533800000000018\\
5.61968488866078e-10	0.532800000000018\\
5.66325208163313e-10	0.531800000000018\\
5.68857492437979e-10	0.530800000000018\\
5.7132882347628e-10	0.529800000000019\\
5.75379399086211e-10	0.528800000000019\\
5.77276070363143e-10	0.527800000000019\\
5.7972838604185e-10	0.526800000000019\\
5.82177546760894e-10	0.525800000000019\\
5.84797603762188e-10	0.524800000000019\\
5.89577562581253e-10	0.523800000000019\\
5.94309452084206e-10	0.522800000000019\\
5.95911296042446e-10	0.521800000000019\\
5.97307335419511e-10	0.520800000000019\\
6.06076202889169e-10	0.519800000000019\\
6.08512094407173e-10	0.518800000000019\\
6.16080420502666e-10	0.517800000000019\\
6.22524490684818e-10	0.51680000000002\\
6.23569444589557e-10	0.51580000000002\\
6.25950292375268e-10	0.51480000000002\\
6.29097786095209e-10	0.51380000000002\\
6.32038262788613e-10	0.51280000000002\\
6.36188207657259e-10	0.51180000000002\\
6.42345452488212e-10	0.51080000000002\\
6.46182555287338e-10	0.50980000000002\\
6.48998908116689e-10	0.50880000000002\\
6.52607372711329e-10	0.50780000000002\\
6.56367137492098e-10	0.506800000000021\\
6.5773000518267e-10	0.505800000000021\\
6.63239331666263e-10	0.504800000000021\\
6.70075769383484e-10	0.503800000000021\\
6.72996121227284e-10	0.502800000000021\\
6.77260290812178e-10	0.501800000000021\\
6.79485212179928e-10	0.500800000000021\\
6.84876959670027e-10	0.499800000000021\\
6.88125111529756e-10	0.498800000000021\\
6.94492511107833e-10	0.497800000000021\\
6.98164516530722e-10	0.496800000000021\\
7.01492120256287e-10	0.495800000000021\\
7.08530494899005e-10	0.494800000000021\\
7.14450476763046e-10	0.493800000000021\\
7.19134754837223e-10	0.492800000000021\\
7.22245086617768e-10	0.491800000000021\\
7.24105433353798e-10	0.490800000000021\\
7.33416296879544e-10	0.489800000000021\\
7.38580330897795e-10	0.488800000000021\\
7.40122972798131e-10	0.487800000000021\\
7.44199102841061e-10	0.486800000000021\\
7.47224236990754e-10	0.48580000000002\\
7.52944978593259e-10	0.48480000000002\\
7.59176082020232e-10	0.48380000000002\\
7.66992452953389e-10	0.48280000000002\\
7.70741960602105e-10	0.48180000000002\\
7.77303854994466e-10	0.48080000000002\\
7.82538712133758e-10	0.47980000000002\\
7.86799822417128e-10	0.47880000000002\\
7.89164749039079e-10	0.47780000000002\\
7.92695704574611e-10	0.47680000000002\\
7.95778924134539e-10	0.47580000000002\\
7.9900328069679e-10	0.47480000000002\\
8.02026678384937e-10	0.47380000000002\\
8.05133274927239e-10	0.47280000000002\\
8.06909325511074e-10	0.47180000000002\\
8.15142975050631e-10	0.47080000000002\\
8.18833818972368e-10	0.46980000000002\\
8.2245643362977e-10	0.46880000000002\\
8.23879196540721e-10	0.46780000000002\\
8.29578159807965e-10	0.46680000000002\\
8.38102799428505e-10	0.46580000000002\\
8.42624217503467e-10	0.464800000000019\\
8.47252472420782e-10	0.463800000000019\\
8.53249759606279e-10	0.462800000000019\\
8.64208528357887e-10	0.461800000000019\\
8.69545988953963e-10	0.460800000000019\\
8.73228672810464e-10	0.459800000000019\\
8.75931523177286e-10	0.458800000000019\\
8.80206720650696e-10	0.457800000000019\\
8.87345395748355e-10	0.456800000000019\\
8.91300740686702e-10	0.455800000000019\\
8.97157748091397e-10	0.454800000000019\\
9.04006566808564e-10	0.453800000000019\\
9.13486156715108e-10	0.452800000000019\\
9.19576324802745e-10	0.451800000000019\\
9.30826627804194e-10	0.450800000000019\\
9.3331622719828e-10	0.449800000000019\\
9.41063900685521e-10	0.448800000000019\\
9.49921808548725e-10	0.447800000000019\\
9.58142505955726e-10	0.446800000000019\\
9.70545838690067e-10	0.445800000000019\\
9.77228780221067e-10	0.444800000000019\\
9.8219675516434e-10	0.443800000000019\\
9.88606154411325e-10	0.442800000000019\\
9.90254405761043e-10	0.441800000000019\\
9.95570886040679e-10	0.440800000000019\\
1.00307912844064e-09	0.439800000000019\\
1.00815956994342e-09	0.438800000000019\\
1.01124525868777e-09	0.437800000000018\\
1.01588385984144e-09	0.436800000000018\\
1.02416375970164e-09	0.435800000000018\\
1.03595315182424e-09	0.434800000000018\\
1.05606665056229e-09	0.433800000000018\\
1.06468025838468e-09	0.432800000000018\\
1.0667467909718e-09	0.431800000000018\\
1.07820877929675e-09	0.430800000000018\\
1.08188668849435e-09	0.429800000000018\\
1.08637191611459e-09	0.428800000000018\\
1.09830363290081e-09	0.427800000000018\\
1.09955100737065e-09	0.426800000000018\\
1.10719688447138e-09	0.425800000000018\\
1.11315150341073e-09	0.424800000000018\\
1.12115669490865e-09	0.423800000000018\\
1.1262961643711e-09	0.422800000000018\\
1.13108382651288e-09	0.421800000000018\\
1.138905888975e-09	0.420800000000018\\
1.15294103948039e-09	0.419800000000017\\
1.16155489473863e-09	0.418800000000018\\
1.16541945863908e-09	0.417800000000017\\
1.17035619671393e-09	0.416800000000018\\
1.17938872437537e-09	0.415800000000017\\
1.1898221385211e-09	0.414800000000017\\
1.19660092099056e-09	0.413800000000017\\
1.20102128271515e-09	0.412800000000017\\
1.20716109544693e-09	0.411800000000017\\
1.20983582567635e-09	0.410800000000017\\
1.21782564277421e-09	0.409800000000017\\
1.22083006113658e-09	0.408800000000017\\
1.22611563372463e-09	0.407800000000017\\
1.24107179307284e-09	0.406800000000017\\
1.24686407774589e-09	0.405800000000017\\
1.25669155430578e-09	0.404800000000017\\
1.2615254021519e-09	0.403800000000017\\
1.26881243813441e-09	0.402800000000017\\
1.27349270126826e-09	0.401800000000017\\
1.27897755035618e-09	0.400800000000017\\
1.2840331818914e-09	0.399800000000017\\
1.2873495617765e-09	0.398800000000016\\
1.30181621512255e-09	0.397800000000016\\
1.31035481491755e-09	0.396800000000016\\
1.32142134667492e-09	0.395800000000016\\
1.32951198144014e-09	0.394800000000016\\
1.34429840925854e-09	0.393800000000016\\
1.35976375223148e-09	0.392800000000016\\
1.37692406408262e-09	0.391800000000016\\
1.38993334383768e-09	0.390800000000016\\
1.39849105736177e-09	0.389800000000016\\
1.41607662923777e-09	0.388800000000016\\
1.42018962591931e-09	0.387800000000016\\
1.43050239286385e-09	0.386800000000016\\
1.43928506420682e-09	0.385800000000016\\
1.45213252784536e-09	0.384800000000016\\
1.45894245429627e-09	0.383800000000016\\
1.47396742791439e-09	0.382800000000016\\
1.48832468718213e-09	0.381800000000016\\
1.49416745867723e-09	0.380800000000016\\
1.50502639409262e-09	0.379800000000016\\
1.5155540211812e-09	0.378800000000016\\
1.52422832174705e-09	0.377800000000016\\
1.52992282619546e-09	0.376800000000016\\
1.5394615919424e-09	0.375800000000016\\
1.55193013381219e-09	0.374800000000016\\
1.56666599353919e-09	0.373800000000015\\
1.58285768948768e-09	0.372800000000015\\
1.59186572381489e-09	0.371800000000015\\
1.60496849179069e-09	0.370800000000015\\
1.63559861082409e-09	0.369800000000015\\
1.64439353777924e-09	0.368800000000015\\
1.6585926747425e-09	0.367800000000015\\
1.6698908366753e-09	0.366800000000015\\
1.67748398787217e-09	0.365800000000015\\
1.69212554002978e-09	0.364800000000015\\
1.69849751914228e-09	0.363800000000015\\
1.71178031854684e-09	0.362800000000015\\
1.72215957466712e-09	0.361800000000015\\
1.73215693701047e-09	0.360800000000015\\
1.74051924396979e-09	0.359800000000015\\
1.7662000879227e-09	0.358800000000015\\
1.78107733583486e-09	0.357800000000015\\
1.80273483488174e-09	0.356800000000015\\
1.82140442016715e-09	0.355800000000015\\
1.82753552061908e-09	0.354800000000015\\
1.84580286357608e-09	0.353800000000015\\
1.86009892365402e-09	0.352800000000015\\
1.87162844677667e-09	0.351800000000015\\
1.88072501093331e-09	0.350800000000014\\
1.88822255211031e-09	0.349800000000015\\
1.89919420771692e-09	0.348800000000014\\
1.92246869951469e-09	0.347800000000014\\
1.93565489525e-09	0.346800000000014\\
1.94973562994982e-09	0.345800000000014\\
1.97673423893141e-09	0.344800000000014\\
1.98845789422255e-09	0.343800000000014\\
2.00599335322396e-09	0.342800000000014\\
2.01703259252818e-09	0.341800000000014\\
2.04888449234174e-09	0.340800000000014\\
2.07071091238998e-09	0.339800000000014\\
2.08423037447699e-09	0.338800000000014\\
2.0953278737684e-09	0.337800000000014\\
2.11377135152307e-09	0.336800000000014\\
2.12787321308733e-09	0.335800000000014\\
2.14955040523956e-09	0.334800000000014\\
2.1588401085238e-09	0.333800000000014\\
2.17227531551235e-09	0.332800000000014\\
2.20457851302105e-09	0.331800000000013\\
2.22404410353827e-09	0.330800000000013\\
2.23527002225798e-09	0.329800000000013\\
2.25575684483081e-09	0.328800000000013\\
2.27623727788895e-09	0.327800000000013\\
2.28509570626699e-09	0.326800000000013\\
2.29662036892259e-09	0.325800000000013\\
2.32212906895747e-09	0.324800000000013\\
2.34017231775221e-09	0.323800000000013\\
2.35956514403211e-09	0.322800000000013\\
2.39220499337013e-09	0.321800000000013\\
2.41074065531789e-09	0.320800000000013\\
2.43243791590042e-09	0.319800000000013\\
2.46249718340709e-09	0.318800000000013\\
2.48594179431019e-09	0.317800000000013\\
2.49699063604642e-09	0.316800000000012\\
2.51672895292546e-09	0.315800000000013\\
2.54005085161403e-09	0.314800000000012\\
2.56913269425704e-09	0.313800000000012\\
2.59456287868452e-09	0.312800000000012\\
2.60968290758544e-09	0.311800000000012\\
2.62091857086031e-09	0.310800000000012\\
2.64236916959547e-09	0.309800000000012\\
2.66296701062647e-09	0.308800000000012\\
2.68783132344245e-09	0.307800000000012\\
2.70162437225532e-09	0.306800000000012\\
2.72437971851633e-09	0.305800000000012\\
2.7316345774771e-09	0.304800000000012\\
2.75611276795616e-09	0.303800000000012\\
2.77504569031693e-09	0.302800000000012\\
2.79790269944781e-09	0.301800000000012\\
2.82028811659433e-09	0.300800000000012\\
2.82734395294615e-09	0.299800000000012\\
2.8392912815098e-09	0.298800000000012\\
2.86252326703743e-09	0.297800000000011\\
2.89270571155154e-09	0.296800000000011\\
2.91649962233601e-09	0.295800000000011\\
2.94425822039535e-09	0.294800000000011\\
2.97925164036405e-09	0.293800000000011\\
2.99963039099939e-09	0.292800000000011\\
3.01045048565299e-09	0.291800000000011\\
3.01933787983043e-09	0.290800000000011\\
3.04325214583451e-09	0.289800000000011\\
3.07028752483159e-09	0.288800000000011\\
3.09735099077717e-09	0.287800000000011\\
3.11997215864658e-09	0.286800000000011\\
3.14220908328764e-09	0.28580000000001\\
3.15592382036733e-09	0.28480000000001\\
3.1698678131951e-09	0.28380000000001\\
3.18013226045674e-09	0.28280000000001\\
3.20495315430477e-09	0.28180000000001\\
3.22018519004419e-09	0.28080000000001\\
3.24855678626821e-09	0.27980000000001\\
3.27734621034967e-09	0.27880000000001\\
3.32376764630489e-09	0.27780000000001\\
3.35488301913529e-09	0.27680000000001\\
3.37429246442048e-09	0.27580000000001\\
3.38326758121252e-09	0.27480000000001\\
3.40555516683168e-09	0.27380000000001\\
3.42362279424094e-09	0.27280000000001\\
3.43720446946299e-09	0.27180000000001\\
3.45239080423594e-09	0.27080000000001\\
3.48125237512868e-09	0.26980000000001\\
3.50922752845023e-09	0.26880000000001\\
3.55898629157065e-09	0.26780000000001\\
3.57992291507442e-09	0.26680000000001\\
3.59342460746387e-09	0.26580000000001\\
3.6459068828476e-09	0.26480000000001\\
3.66398671187732e-09	0.26380000000001\\
3.68409361934228e-09	0.262800000000009\\
3.70173071541086e-09	0.261800000000009\\
3.73173178680249e-09	0.260800000000009\\
3.76868066195039e-09	0.259800000000009\\
3.82030243214944e-09	0.258800000000009\\
3.85193180535934e-09	0.257800000000009\\
3.90490205617402e-09	0.256800000000009\\
3.92714100536505e-09	0.255800000000009\\
3.93907258393279e-09	0.254800000000009\\
3.95923486968536e-09	0.253800000000009\\
3.9932377013872e-09	0.252800000000009\\
4.04487145091249e-09	0.251800000000009\\
4.09757347309898e-09	0.250800000000009\\
4.10635485637116e-09	0.249800000000009\\
4.13585611246374e-09	0.248800000000009\\
4.1669695152474e-09	0.247800000000009\\
4.18241122091699e-09	0.246800000000009\\
4.20626842621444e-09	0.245800000000009\\
4.23525847269306e-09	0.244800000000009\\
4.29560024965521e-09	0.243800000000009\\
4.3382786898243e-09	0.242800000000009\\
4.36943992182452e-09	0.241800000000009\\
4.42026345719598e-09	0.240800000000009\\
4.44200058153912e-09	0.239800000000009\\
4.46614893167981e-09	0.238800000000008\\
4.51553129139539e-09	0.237800000000008\\
4.57111827887222e-09	0.236800000000008\\
4.61581478014672e-09	0.235800000000008\\
4.64475681836989e-09	0.234800000000008\\
4.66909883831048e-09	0.233800000000008\\
4.69533170925074e-09	0.232800000000008\\
4.74399395252908e-09	0.231800000000008\\
4.78192170808772e-09	0.230800000000008\\
4.80740767481221e-09	0.229800000000008\\
4.8517510657822e-09	0.228800000000008\\
4.87811512257618e-09	0.227800000000008\\
4.89380459573959e-09	0.226800000000008\\
4.90704051318761e-09	0.225800000000008\\
4.93412415257501e-09	0.224800000000008\\
4.97430720059559e-09	0.223800000000008\\
4.99512323586489e-09	0.222800000000008\\
5.03820968665406e-09	0.221800000000008\\
5.06759282870174e-09	0.220800000000008\\
5.10401455755755e-09	0.219800000000008\\
5.13763549605509e-09	0.218800000000008\\
5.17398817885343e-09	0.217800000000008\\
5.20479290175625e-09	0.216800000000008\\
5.23060041157888e-09	0.215800000000008\\
5.26023688044199e-09	0.214800000000008\\
5.2780920453196e-09	0.213800000000008\\
5.32565685735147e-09	0.212800000000008\\
5.33923860298603e-09	0.211800000000008\\
5.39134251352909e-09	0.210800000000008\\
5.41158924220378e-09	0.209800000000008\\
5.44458434999767e-09	0.208800000000008\\
5.46747742396965e-09	0.207800000000008\\
5.49879001337355e-09	0.206800000000008\\
5.5465778233096e-09	0.205800000000008\\
5.59443298585177e-09	0.204800000000007\\
5.6297226666454e-09	0.203800000000007\\
5.67670199216805e-09	0.202800000000007\\
5.70614414191175e-09	0.201800000000007\\
5.7348834345132e-09	0.200800000000007\\
5.79761212710381e-09	0.199800000000007\\
5.86785013370656e-09	0.198800000000007\\
5.92405738605664e-09	0.197800000000007\\
6.00789679042942e-09	0.196800000000007\\
6.0285855902357e-09	0.195800000000007\\
6.05560000121359e-09	0.194800000000007\\
6.09691725857364e-09	0.193800000000007\\
6.11143750192266e-09	0.192800000000007\\
6.18055753642643e-09	0.191800000000007\\
6.22837560692603e-09	0.190800000000007\\
6.25271534600196e-09	0.189800000000007\\
6.29944813875514e-09	0.188800000000007\\
6.32750059044544e-09	0.187800000000007\\
6.34851887520703e-09	0.186800000000007\\
6.36361966762435e-09	0.185800000000007\\
6.42340650274223e-09	0.184800000000007\\
6.45388182641435e-09	0.183800000000007\\
6.52046728557441e-09	0.182800000000007\\
6.54574886273678e-09	0.181800000000007\\
6.57725729228704e-09	0.180800000000007\\
6.6137643972938e-09	0.179800000000007\\
6.64497842214028e-09	0.178800000000007\\
6.69272226659629e-09	0.177800000000007\\
6.7215793637248e-09	0.176800000000007\\
6.76461228288844e-09	0.175800000000007\\
6.79702372840951e-09	0.174800000000007\\
6.83146666308341e-09	0.173800000000007\\
6.87433772477084e-09	0.172800000000007\\
6.91447990689404e-09	0.171800000000007\\
6.96186754562824e-09	0.170800000000007\\
7.02424853204856e-09	0.169800000000007\\
7.07632167979741e-09	0.168800000000007\\
7.14069489844609e-09	0.167800000000006\\
7.1791077402208e-09	0.166800000000006\\
7.22334913173794e-09	0.165800000000006\\
7.25312512466813e-09	0.164800000000006\\
7.29165767621157e-09	0.163800000000006\\
7.31174213415989e-09	0.162800000000006\\
7.337315823331e-09	0.161800000000006\\
7.38129247240989e-09	0.160800000000006\\
7.43311524726595e-09	0.159800000000006\\
7.46416505608912e-09	0.158800000000006\\
7.50440683751697e-09	0.157800000000006\\
7.53092614147443e-09	0.156800000000006\\
7.61038546011518e-09	0.155800000000006\\
7.74771430082828e-09	0.154800000000006\\
7.76004890728729e-09	0.153800000000006\\
7.77999698142223e-09	0.152800000000006\\
7.8608798561331e-09	0.151800000000006\\
7.88916117043827e-09	0.150800000000006\\
7.97948088800256e-09	0.149800000000006\\
8.01065074045702e-09	0.148800000000006\\
8.03584225061281e-09	0.147800000000006\\
8.09317123000993e-09	0.146800000000006\\
8.15917392551968e-09	0.145800000000006\\
8.1861474301866e-09	0.144800000000006\\
8.23574036368759e-09	0.143800000000006\\
8.26197937127086e-09	0.142800000000006\\
8.33674953728859e-09	0.141800000000006\\
8.39291437241439e-09	0.140800000000006\\
8.46380957085005e-09	0.139800000000006\\
8.51367409632101e-09	0.138800000000006\\
8.55474917001278e-09	0.137800000000006\\
8.66191854079082e-09	0.136800000000006\\
8.72769090424646e-09	0.135800000000005\\
8.84983951953991e-09	0.134800000000005\\
8.89966103919876e-09	0.133800000000005\\
8.96138923394094e-09	0.132800000000005\\
9.03552270408952e-09	0.131800000000005\\
9.07635226162633e-09	0.130800000000005\\
9.14688591576202e-09	0.129800000000005\\
9.27437112392751e-09	0.128800000000005\\
9.37681235188293e-09	0.127800000000005\\
9.42039531605625e-09	0.126800000000005\\
9.50823902697592e-09	0.125800000000005\\
9.63490751689763e-09	0.124800000000005\\
9.67584948664571e-09	0.123800000000005\\
9.73269672326814e-09	0.122800000000005\\
9.78864546705131e-09	0.121800000000005\\
9.8936228775e-09	0.120800000000005\\
1.00264368432286e-08	0.119800000000005\\
1.01512775678729e-08	0.118800000000005\\
1.02294075197067e-08	0.117800000000005\\
1.03001330316524e-08	0.116800000000005\\
1.03500529273831e-08	0.115800000000005\\
1.04591546863968e-08	0.114800000000005\\
1.04711265952114e-08	0.113800000000005\\
1.05330666255742e-08	0.112800000000005\\
1.05720132495874e-08	0.111800000000005\\
1.06223827485638e-08	0.110800000000005\\
1.07303614697116e-08	0.109800000000005\\
1.08057662502564e-08	0.108800000000005\\
1.08497659765852e-08	0.107800000000005\\
1.09787359092508e-08	0.106800000000004\\
1.10341467260578e-08	0.105800000000004\\
1.11145588462413e-08	0.104800000000004\\
1.12280466198163e-08	0.103800000000004\\
1.13476015359141e-08	0.102800000000004\\
1.13891121044628e-08	0.101800000000004\\
1.14762724869383e-08	0.100800000000004\\
1.15642045125112e-08	0.0998000000000042\\
1.16248280019819e-08	0.0988000000000041\\
1.17408680873582e-08	0.0978000000000041\\
1.18327826443478e-08	0.0968000000000041\\
1.19361273575083e-08	0.095800000000004\\
1.19996564320936e-08	0.094800000000004\\
1.20968465913903e-08	0.093800000000004\\
1.21780388768399e-08	0.092800000000004\\
1.22761991415839e-08	0.0918000000000039\\
1.2410575925996e-08	0.0908000000000039\\
1.25427222197484e-08	0.0898000000000039\\
1.26468967193983e-08	0.0888000000000038\\
1.27079423209585e-08	0.0878000000000038\\
1.2797472145495e-08	0.0868000000000038\\
1.28561891962377e-08	0.0858000000000037\\
1.29905670866654e-08	0.0848000000000037\\
1.30693425013988e-08	0.0838000000000036\\
1.32832387848645e-08	0.0828000000000035\\
1.33814892325664e-08	0.0818000000000035\\
1.36008044035884e-08	0.0808000000000035\\
1.38706528649852e-08	0.0798000000000035\\
1.39723793930862e-08	0.0788000000000034\\
1.41118305054947e-08	0.0778000000000034\\
1.43095554739922e-08	0.0768000000000034\\
1.44094405678356e-08	0.0758000000000034\\
1.45578727424895e-08	0.0748000000000033\\
1.47698315038024e-08	0.0738000000000033\\
1.50650270866242e-08	0.0728000000000033\\
1.52158647003664e-08	0.0718000000000033\\
1.53644509322418e-08	0.0708000000000032\\
1.56003634857698e-08	0.0698000000000032\\
1.56839548327852e-08	0.0688000000000032\\
1.58160284397956e-08	0.0678000000000031\\
1.59309956644385e-08	0.0668000000000031\\
1.60653613226167e-08	0.0658000000000031\\
1.61675464915231e-08	0.0648000000000031\\
1.6326521837029e-08	0.063800000000003\\
1.67409247881209e-08	0.062800000000003\\
1.69203990879521e-08	0.061800000000003\\
1.70351176205072e-08	0.0608000000000029\\
1.71831677494613e-08	0.0598000000000029\\
1.75112147712988e-08	0.0588000000000028\\
1.76538756264209e-08	0.0578000000000027\\
1.78620440250252e-08	0.0568000000000027\\
1.80151563780627e-08	0.0558000000000026\\
1.83201183375601e-08	0.0548000000000026\\
1.86722512975457e-08	0.0538000000000025\\
1.89768220003614e-08	0.0528000000000025\\
1.9328500009657e-08	0.0518000000000025\\
1.94755633390682e-08	0.0508000000000024\\
1.97227960040963e-08	0.0498000000000024\\
1.98979573650938e-08	0.0488000000000023\\
2.00875873795071e-08	0.0478000000000023\\
2.02078339148562e-08	0.0468000000000023\\
2.04433030087939e-08	0.0458000000000022\\
2.07964422611889e-08	0.0448000000000022\\
2.1060269553254e-08	0.0438000000000022\\
2.13290364202618e-08	0.0428000000000021\\
2.18575933221649e-08	0.0418000000000021\\
2.21063031853886e-08	0.0408000000000019\\
2.2519291966209e-08	0.0398000000000019\\
2.30845608082864e-08	0.0388000000000019\\
2.33716334694595e-08	0.0378000000000018\\
2.37568770520646e-08	0.0368000000000018\\
2.4090609191385e-08	0.0358000000000017\\
2.47974971557206e-08	0.0348000000000017\\
2.51283256756858e-08	0.0338000000000016\\
2.58225797768519e-08	0.0328000000000016\\
2.65798719643204e-08	0.0318000000000015\\
2.72741933758996e-08	0.0308000000000015\\
2.84211896458478e-08	0.0298000000000015\\
2.87825695540526e-08	0.0288000000000014\\
2.98009118437311e-08	0.0278000000000014\\
3.02622259156839e-08	0.0268000000000013\\
3.11849969103909e-08	0.0258000000000013\\
3.19086931073979e-08	0.0248000000000012\\
3.2578519772239e-08	0.0238000000000012\\
3.3504429146341e-08	0.0228000000000012\\
3.44020215130806e-08	0.021800000000001\\
3.50710450752877e-08	0.020800000000001\\
3.61872894577608e-08	0.0198000000000009\\
3.70029635125595e-08	0.0188000000000009\\
4.07977570841469e-08	0.0178000000000009\\
4.57020828082124e-08	0.0168000000000008\\
5.1716376789637e-08	0.0158000000000008\\
5.62181722566451e-08	0.0148000000000007\\
7.47409243733285e-08	0.0138000000000007\\
8.89372651357608e-08	0.0128000000000007\\
1.25679780187629e-07	0.0118000000000006\\
2.23919822567107e-07	0.0108000000000006\\
3.69970086725891e-06	0.00980000000000047\\
1.00602928989464e-05	0.00880000000000047\\
2.85020444197287e-05	0.00780000000000036\\
0.000466891300637564	0.00680000000000036\\
0.00114498786335808	0.00580000000000025\\
0.00287552698104488	0.00480000000000025\\
0.00600143343102173	0.00380000000000014\\
0.053447190796209	0.00280000000000014\\
0.215053940881655	0.00180000000000013\\
302.13957356695	0.000800000000000023\\
};
\addlegendentry{$K=20$, $G=\;\,5$, $\lrmse =9.505$, $\prmse =0.005$, $\armse =0.011$, $\brmse =8\hspace{-3pt}\times\hspace{-3pt}10^{-5}$, $\gamma \rightarrow \infty$}


==> figures/mse_N_2_K_20_G_5_SNR_1000_I_20_Pratio_2_Nratio_2_alpha_2_cs.tex <==
\addplot [color=blue,line width=0.1pt]
  table[row sep=crcr]{%
7.105427357601e-15	1\\
1.63308938774679e-13	0.9978\\
2.34371420084339e-13	0.9936\\
2.82099783974918e-13	0.9892\\
3.24076820333551e-13	0.9858\\
3.51557130126508e-13	0.9822\\
3.72357613997143e-13	0.9792\\
4.21801532856302e-13	0.9762\\
4.54747350886464e-13	0.9726\\
4.75639239174926e-13	0.967800000000001\\
4.92188701274735e-13	0.965000000000001\\
5.14788089466264e-13	0.962600000000001\\
5.33995439242743e-13	0.959600000000001\\
5.59842749328033e-13	0.956600000000001\\
5.73309366159115e-13	0.952000000000001\\
5.88604355912004e-13	0.947800000000001\\
6.02245225434703e-13	0.944000000000001\\
6.33141025046639e-13	0.940400000000001\\
6.43668973480993e-13	0.936800000000001\\
6.71462885293295e-13	0.934000000000001\\
6.89857961396208e-13	0.931200000000001\\
7.0290779065111e-13	0.928000000000001\\
7.14828593574347e-13	0.924800000000001\\
7.38964445190504e-13	0.921200000000001\\
7.7074237983105e-13	0.916400000000001\\
7.9511764041923e-13	0.913600000000001\\
8.03887338846093e-13	0.910200000000001\\
8.21783453071187e-13	0.907200000000002\\
8.38440428196918e-13	0.903600000000001\\
8.59286801531868e-13	0.900400000000001\\
8.82447164727866e-13	0.898000000000001\\
9.09494701772928e-13	0.894400000000001\\
9.22748560908849e-13	0.890600000000001\\
9.33336493195363e-13	0.887600000000001\\
9.44781398777346e-13	0.885200000000001\\
9.59739150230426e-13	0.882600000000001\\
9.73002600439013e-13	0.880200000000001\\
1.0090269762075e-12	0.877200000000001\\
1.02517799317733e-12	0.874600000000001\\
1.03910042738616e-12	0.871200000000001\\
1.05131515159551e-12	0.8676\\
1.06685572399803e-12	0.8652\\
1.09782876710528e-12	0.8616\\
1.12293293645599e-12	0.8588\\
1.14395173781634e-12	0.8558\\
1.15973112787646e-12	0.8514\\
1.17185710042169e-12	0.8486\\
1.18795117038946e-12	0.8456\\
1.20850766196948e-12	0.8424\\
1.23094736076489e-12	0.8394\\
1.25087814721299e-12	0.8366\\
1.26212872323632e-12	0.833200000000001\\
1.28244598416569e-12	0.830000000000001\\
1.29903070069604e-12	0.827000000000001\\
1.31877956825067e-12	0.824600000000001\\
1.35522406650074e-12	0.821400000000001\\
1.36897080878865e-12	0.818200000000001\\
1.39034168667365e-12	0.816000000000001\\
1.4119612329039e-12	0.813400000000001\\
1.44207357152189e-12	0.809400000000001\\
1.46502815924349e-12	0.807200000000001\\
1.48127285677485e-12	0.804000000000001\\
1.49478079595237e-12	0.800400000000001\\
1.50849410939777e-12	0.797800000000001\\
1.52712561682021e-12	0.794800000000001\\
1.54865719262321e-12	0.790600000000001\\
1.56525968725582e-12	0.788000000000001\\
1.58780468648995e-12	0.785400000000001\\
1.60475726869357e-12	0.782800000000001\\
1.62203071720117e-12	0.780600000000001\\
1.65359645140925e-12	0.777200000000001\\
1.6819463601863e-12	0.774200000000001\\
1.70543578738343e-12	0.771600000000001\\
1.71528018679463e-12	0.768800000000002\\
1.73255905953376e-12	0.766400000000002\\
1.75423489886045e-12	0.762800000000002\\
1.77948048104765e-12	0.759600000000002\\
1.79754673591127e-12	0.756400000000002\\
1.81593719892542e-12	0.754200000000002\\
1.82696552201244e-12	0.751600000000002\\
1.84566125597646e-12	0.749400000000002\\
1.86308586951013e-12	0.746400000000002\\
1.88206662768872e-12	0.743600000000002\\
1.91609544693656e-12	0.740400000000002\\
1.9389486191403e-12	0.737200000000002\\
1.95779990682405e-12	0.735000000000002\\
1.97423503173152e-12	0.732400000000002\\
1.99701698540948e-12	0.729800000000003\\
2.02697805362582e-12	0.727400000000003\\
2.0495186137532e-12	0.724400000000003\\
2.07945160171225e-12	0.721000000000003\\
2.10248923148169e-12	0.719000000000003\\
2.12313213247602e-12	0.716800000000003\\
2.142778251365e-12	0.714200000000003\\
2.16079772698643e-12	0.711800000000004\\
2.17866817101103e-12	0.709000000000004\\
2.19142254152317e-12	0.706800000000004\\
2.21196872378292e-12	0.704000000000004\\
2.23152278288583e-12	0.701400000000004\\
2.24873024818095e-12	0.698600000000004\\
2.27533491393222e-12	0.695600000000004\\
2.29143147075165e-12	0.693400000000004\\
2.31196237696113e-12	0.690600000000005\\
2.3299545734287e-12	0.688200000000005\\
2.36099409247109e-12	0.685400000000005\\
2.38352934874598e-12	0.683000000000005\\
2.3982264690095e-12	0.680200000000005\\
2.42263033841707e-12	0.678000000000005\\
2.454161534038e-12	0.675600000000005\\
2.48961845253024e-12	0.673000000000005\\
2.5185006600675e-12	0.670000000000005\\
2.54481453670176e-12	0.667400000000005\\
2.58559462407542e-12	0.663800000000005\\
2.60876614542636e-12	0.661000000000005\\
2.62476304295683e-12	0.658400000000006\\
2.64124132393205e-12	0.656200000000006\\
2.6758703588575e-12	0.653000000000006\\
2.7023052834931e-12	0.650800000000006\\
2.72507729448863e-12	0.648600000000006\\
2.74162709726094e-12	0.646200000000006\\
2.76626615850363e-12	0.643200000000006\\
2.7837319712422e-12	0.640800000000006\\
2.80785776231561e-12	0.638000000000006\\
2.83366723590441e-12	0.635800000000006\\
2.84840134706951e-12	0.633000000000006\\
2.87396750538799e-12	0.631000000000006\\
2.89692595500468e-12	0.628800000000006\\
2.94504321331667e-12	0.626200000000006\\
2.96581593334422e-12	0.624000000000006\\
2.98796738135759e-12	0.621600000000006\\
3.01872808128215e-12	0.619200000000007\\
3.05455909135706e-12	0.616600000000007\\
3.07637927283731e-12	0.613200000000007\\
3.11668375722168e-12	0.610400000000007\\
3.14699048787279e-12	0.608400000000007\\
3.17827918135957e-12	0.606200000000007\\
3.19349241156093e-12	0.603800000000007\\
3.2277102771015e-12	0.601200000000007\\
3.25599182624948e-12	0.598800000000007\\
3.29691829392686e-12	0.596600000000008\\
3.32728280057456e-12	0.594000000000008\\
3.35400444768174e-12	0.592000000000008\\
3.38122793567532e-12	0.590000000000008\\
3.41107879391473e-12	0.587800000000008\\
3.4277335706315e-12	0.585000000000008\\
3.44672738815624e-12	0.582600000000008\\
3.47814842388706e-12	0.580200000000009\\
3.51557130126508e-12	0.577800000000009\\
3.54010047117266e-12	0.575400000000009\\
3.56802839325501e-12	0.573200000000009\\
3.5829394867777e-12	0.570800000000009\\
3.63842286919982e-12	0.568600000000009\\
3.65393104402487e-12	0.566400000000009\\
3.68913350475576e-12	0.56420000000001\\
3.72769572600936e-12	0.56160000000001\\
3.77152978516115e-12	0.55940000000001\\
3.8073423222573e-12	0.55720000000001\\
3.84397709756211e-12	0.55500000000001\\
3.87797535266014e-12	0.55260000000001\\
3.90109478229579e-12	0.550400000000011\\
3.93094564058243e-12	0.548400000000011\\
3.97944532396358e-12	0.546200000000011\\
4.0021157961023e-12	0.544200000000011\\
4.03958387038597e-12	0.542000000000011\\
4.07541942994622e-12	0.539800000000012\\
4.10149985147593e-12	0.537800000000012\\
4.13601793603729e-12	0.535600000000012\\
4.18369107470817e-12	0.533400000000012\\
4.207949023867e-12	0.531400000000013\\
4.24198178889256e-12	0.529000000000013\\
4.28112464668397e-12	0.526400000000013\\
4.32467853782314e-12	0.524000000000013\\
4.3513999137314e-12	0.522000000000013\\
4.41479820414033e-12	0.519000000000013\\
4.47765969359079e-12	0.516800000000014\\
4.5250360589674e-12	0.514800000000014\\
4.57015431544318e-12	0.512600000000014\\
4.62921864213667e-12	0.510200000000014\\
4.67776785886621e-12	0.508200000000014\\
4.76816001636942e-12	0.506200000000015\\
4.79855766098572e-12	0.504200000000015\\
4.85545623513674e-12	0.502200000000015\\
4.92147155953566e-12	0.500000000000015\\
4.96363816085164e-12	0.498000000000015\\
5.02798360366564e-12	0.495800000000015\\
5.0715830827403e-12	0.493600000000015\\
5.1435061812007e-12	0.490800000000015\\
5.18322297397018e-12	0.488800000000015\\
5.22101464435826e-12	0.486800000000015\\
5.25924514790942e-12	0.484800000000015\\
5.28857678983195e-12	0.482800000000015\\
5.33995439242743e-12	0.480600000000014\\
5.37766912714423e-12	0.478400000000014\\
5.41207859675683e-12	0.476200000000014\\
5.45134017841678e-12	0.474200000000014\\
5.52237658573723e-12	0.472000000000014\\
5.57326459413329e-12	0.470000000000014\\
5.60724024463695e-12	0.468000000000014\\
5.6581334948211e-12	0.465800000000014\\
5.72427622058985e-12	0.463600000000014\\
5.79586882886962e-12	0.461400000000014\\
5.81090172795264e-12	0.459400000000014\\
5.8794481127342e-12	0.457400000000014\\
5.94992042563783e-12	0.455200000000014\\
6.00505725385283e-12	0.453000000000014\\
6.03672023417097e-12	0.451000000000014\\
6.0936569221928e-12	0.448800000000014\\
6.14494184568947e-12	0.446600000000014\\
6.22850592458551e-12	0.444400000000013\\
6.28884512750089e-12	0.442400000000013\\
6.3300704652322e-12	0.440400000000013\\
6.39437932704353e-12	0.438400000000013\\
6.45341809721672e-12	0.436400000000013\\
6.5215940981012e-12	0.434400000000013\\
6.59383658785373e-12	0.432400000000013\\
6.67426222508935e-12	0.430200000000013\\
6.73343003372678e-12	0.428000000000013\\
6.76371000833645e-12	0.426000000000013\\
6.83067759646283e-12	0.424000000000013\\
6.88690133199509e-12	0.422000000000013\\
6.97722576043084e-12	0.419800000000013\\
7.05551405377856e-12	0.417800000000013\\
7.14735446490992e-12	0.415600000000013\\
7.19670010062459e-12	0.413400000000013\\
7.25394189050912e-12	0.411400000000013\\
7.32199723102195e-12	0.409200000000013\\
7.39756549094215e-12	0.407000000000013\\
7.50596844695412e-12	0.404800000000013\\
7.56786389257192e-12	0.402800000000013\\
7.65277946916073e-12	0.400600000000013\\
7.7420340002472e-12	0.398400000000012\\
7.83779849059246e-12	0.396400000000012\\
7.8932255752785e-12	0.394400000000012\\
7.98973633031357e-12	0.392400000000012\\
8.07436704646892e-12	0.390400000000012\\
8.12527987547075e-12	0.388400000000012\\
8.20639640053705e-12	0.386200000000012\\
8.28042981749156e-12	0.384000000000012\\
8.33507516052801e-12	0.381800000000012\\
8.415898047734e-12	0.379200000000012\\
8.51594287555638e-12	0.377000000000012\\
8.64024641294898e-12	0.375000000000012\\
8.70743958885626e-12	0.373000000000012\\
8.84422221987585e-12	0.371000000000012\\
8.96992031414554e-12	0.368800000000011\\
9.05872115363902e-12	0.366800000000012\\
9.11499774808324e-12	0.364600000000011\\
9.19287439233359e-12	0.362600000000011\\
9.24295665034963e-12	0.360600000000011\\
9.35501763990661e-12	0.358400000000011\\
9.43091250561811e-12	0.356400000000011\\
9.51060058332602e-12	0.354400000000011\\
9.59564222594693e-12	0.352200000000011\\
9.72342361871392e-12	0.350200000000011\\
9.82273357117741e-12	0.348000000000011\\
9.95267231183625e-12	0.346000000000011\\
1.01027883661295e-11	0.344000000000011\\
1.01951567736687e-11	0.342000000000011\\
1.02750382183887e-11	0.340000000000011\\
1.03754422510818e-11	0.338000000000011\\
1.05606444418357e-11	0.336000000000011\\
1.06552226746873e-11	0.334000000000011\\
1.07963970068562e-11	0.332000000000011\\
1.08660176200456e-11	0.330000000000011\\
1.10328961300289e-11	0.32780000000001\\
1.1123628225688e-11	0.32580000000001\\
1.11789849169963e-11	0.32380000000001\\
1.12871049888905e-11	0.32160000000001\\
1.1351190962911e-11	0.31960000000001\\
1.14168984388256e-11	0.31760000000001\\
1.15317911949953e-11	0.31560000000001\\
1.16161025056907e-11	0.31360000000001\\
1.17499623026599e-11	0.311600000000009\\
1.18234652837072e-11	0.30960000000001\\
1.19043541962634e-11	0.30760000000001\\
1.20059773396199e-11	0.305400000000009\\
1.21326082412972e-11	0.30340000000001\\
1.22449749171776e-11	0.301400000000009\\
1.23505864044099e-11	0.299400000000009\\
1.24869349908713e-11	0.297200000000009\\
1.25860366469422e-11	0.295200000000009\\
1.26813386951552e-11	0.293200000000009\\
1.28017638965132e-11	0.291200000000009\\
1.29046141827907e-11	0.289200000000009\\
1.31383636548541e-11	0.287000000000009\\
1.32622225847024e-11	0.285000000000009\\
1.34281674108479e-11	0.283000000000009\\
1.35330320881194e-11	0.280800000000009\\
1.35993986247467e-11	0.278800000000008\\
1.37579863572712e-11	0.276800000000008\\
1.39037654645444e-11	0.274800000000008\\
1.40713301710898e-11	0.272600000000008\\
1.4210968401585e-11	0.270600000000008\\
1.45305833108709e-11	0.268400000000008\\
1.46610020951904e-11	0.266400000000008\\
1.48605048814562e-11	0.264400000000008\\
1.50729411957582e-11	0.262400000000008\\
1.52404244973374e-11	0.260400000000008\\
1.54199757463422e-11	0.258400000000008\\
1.55054687243694e-11	0.256400000000008\\
1.56960160873746e-11	0.254200000000008\\
1.58963512672609e-11	0.252200000000008\\
1.62184395130017e-11	0.250200000000008\\
1.64359332341515e-11	0.248200000000008\\
1.65998355882439e-11	0.246200000000008\\
1.673756374719e-11	0.244200000000008\\
1.70285891644949e-11	0.242000000000008\\
1.72929461422018e-11	0.240000000000008\\
1.73892556676937e-11	0.238000000000008\\
1.74656434256821e-11	0.236000000000008\\
1.77032574607932e-11	0.234000000000007\\
1.79157119551048e-11	0.232000000000007\\
1.8220510424892e-11	0.230000000000007\\
1.84190220538546e-11	0.228000000000007\\
1.85445719137026e-11	0.226000000000007\\
1.87893941273391e-11	0.224000000000007\\
1.91267757502055e-11	0.222000000000007\\
1.93748523022556e-11	0.220000000000007\\
1.9594083966806e-11	0.218000000000007\\
1.97988165674274e-11	0.216000000000007\\
1.99711406307354e-11	0.213800000000007\\
2.01091578252064e-11	0.211800000000007\\
2.03168907651006e-11	0.209800000000007\\
2.0484857114049e-11	0.207800000000007\\
2.07665277225144e-11	0.205800000000007\\
2.09545112420081e-11	0.203800000000007\\
2.13858207829252e-11	0.201600000000006\\
2.18158050831248e-11	0.199600000000006\\
2.21001956498908e-11	0.197600000000006\\
2.24050338254669e-11	0.195600000000006\\
2.28125607411683e-11	0.193600000000006\\
2.30117050975213e-11	0.191600000000006\\
2.33117799233628e-11	0.189600000000006\\
2.357851036415e-11	0.187600000000006\\
2.41017604192612e-11	0.185600000000006\\
2.43625780459097e-11	0.183600000000006\\
2.49790447336644e-11	0.181600000000006\\
2.55161901624001e-11	0.179600000000006\\
2.59343231775706e-11	0.177600000000006\\
2.62981148897398e-11	0.175600000000006\\
2.67302513018693e-11	0.173600000000006\\
2.70603929837842e-11	0.171600000000006\\
2.74370794064099e-11	0.169600000000006\\
2.77221105355837e-11	0.167600000000006\\
2.8239224658078e-11	0.165600000000006\\
2.8598341510287e-11	0.163600000000005\\
2.884964512377e-11	0.161600000000005\\
2.92826928831312e-11	0.159600000000005\\
2.98526055461554e-11	0.157600000000005\\
3.05173596875654e-11	0.155600000000005\\
3.10004771449623e-11	0.153600000000005\\
3.17774539912852e-11	0.151600000000005\\
3.24013595623426e-11	0.149600000000005\\
3.28248104203092e-11	0.147600000000005\\
3.35238490416753e-11	0.145600000000005\\
3.38453277114054e-11	0.143600000000005\\
3.41148727479683e-11	0.141600000000005\\
3.46896249140853e-11	0.139600000000005\\
3.54236219102867e-11	0.137600000000005\\
3.61358312616262e-11	0.135600000000005\\
3.6741828899237e-11	0.133600000000005\\
3.74698714113888e-11	0.131600000000004\\
3.80843376661004e-11	0.129600000000004\\
3.86781874192091e-11	0.127600000000004\\
3.96209741091418e-11	0.125600000000004\\
4.03009116297994e-11	0.123600000000004\\
4.12323780321112e-11	0.121600000000004\\
4.20844427339471e-11	0.119600000000004\\
4.28068403931981e-11	0.117600000000004\\
4.33288657312793e-11	0.115600000000004\\
4.40485150736212e-11	0.113600000000004\\
4.45090957082578e-11	0.111600000000004\\
4.534637201171e-11	0.109600000000004\\
4.64399338917752e-11	0.107600000000004\\
4.81661025073341e-11	0.105600000000004\\
4.87717858845352e-11	0.103600000000004\\
5.02594276303055e-11	0.101600000000004\\
5.127893933306e-11	0.0996000000000035\\
5.23848498130732e-11	0.0976000000000035\\
5.31102590964915e-11	0.0956000000000033\\
5.40582108810154e-11	0.0936000000000033\\
5.53622289647105e-11	0.0916000000000032\\
5.61426609747082e-11	0.0896000000000032\\
5.70065598441974e-11	0.0876000000000031\\
5.80091545580418e-11	0.0856000000000031\\
5.86485262520958e-11	0.083600000000003\\
5.94547991755751e-11	0.081600000000003\\
6.03762801610271e-11	0.0796000000000029\\
6.1200916411571e-11	0.0776000000000029\\
6.26147481838611e-11	0.0756000000000028\\
6.41136566028089e-11	0.0736000000000028\\
6.60600320817082e-11	0.0716000000000027\\
6.72262292574024e-11	0.0696000000000027\\
6.88658195448168e-11	0.0676000000000025\\
7.09209586959127e-11	0.0656000000000025\\
7.17222104968012e-11	0.0634000000000025\\
7.44609950292927e-11	0.0614000000000023\\
7.69416830587327e-11	0.0594000000000023\\
7.889581906117e-11	0.0574000000000022\\
8.05148452769564e-11	0.0554000000000022\\
8.32085335443905e-11	0.0534000000000021\\
8.52307168680407e-11	0.051400000000002\\
8.79766137278112e-11	0.049400000000002\\
9.18122576836692e-11	0.0474000000000019\\
9.35893057618271e-11	0.0454000000000019\\
9.54932217231057e-11	0.0434000000000018\\
9.76331060230162e-11	0.0414000000000017\\
1.00820292645754e-10	0.0394000000000017\\
1.02092999706873e-10	0.0374000000000015\\
1.04427471632237e-10	0.0354000000000014\\
1.08853366109031e-10	0.0334000000000014\\
1.11875487835819e-10	0.0314000000000013\\
1.15145756446614e-10	0.0294000000000012\\
1.19923300511487e-10	0.0274000000000011\\
1.22045828563305e-10	0.0254000000000011\\
1.262438585163e-10	0.023400000000001\\
1.33843744479441e-10	0.0214000000000009\\
1.36621652475371e-10	0.0194000000000007\\
1.45616089650855e-10	0.0174000000000007\\
1.53493085734816e-10	0.0154000000000006\\
1.60058412992583e-10	0.0134000000000005\\
1.70198916509921e-10	0.0114000000000005\\
1.93469064594285e-10	0.00940000000000041\\
2.27419607391723e-10	0.0074000000000003\\
3.28918027231838e-10	0.00540000000000018\\
2.93257546731559e-06	0.00340000000000018\\
0.00269919455581585	0.00140000000000007\\
};
\addlegendentry{$N=2$,~, $\lrmse =13.19$, $\prmse =0.004$, $\gamma \rightarrow \infty$}


==> figures/mse_N_2_K_20_G_5_SNR_1000_I_20_Pratio_2_Nratio_2_alpha_3.4_cs.tex <==
\addplot [color=blue,line width=0.6pt]
  table[row sep=crcr]{%
1.13686837721616e-13	1\\
1.18097674847168e-13	0.997310020174849\\
1.34064935253613e-13	0.995068370320556\\
1.45661260830821e-13	0.992602555480834\\
1.76495154112988e-13	0.9908092355974\\
1.99078808209974e-13	0.988567585743107\\
2.27373675443232e-13	0.986325935888814\\
2.296108708614e-13	0.983187626092804\\
2.37181889850639e-13	0.980273481282224\\
2.47876578534266e-13	0.977359336471643\\
2.55795384873636e-13	0.971979376821341\\
2.68129870507227e-13	0.969961891952477\\
2.86428933843956e-13	0.966599417171038\\
3.0212691549237e-13	0.963461107375028\\
3.1657051252332e-13	0.961443622506165\\
3.41060513164848e-13	0.958753642681013\\
3.42242702197163e-13	0.954718672943286\\
3.4636680912872e-13	0.951804528132706\\
3.5527136788005e-13	0.949562878278413\\
3.59509347182254e-13	0.946872898453261\\
3.66808009719657e-13	0.944855413584398\\
3.73018018206229e-13	0.943510423671822\\
3.8318285787203e-13	0.940596278861242\\
3.91314921813954e-13	0.93790629903609\\
4.00181302220765e-13	0.936337144138085\\
4.13826335789083e-13	0.932526339385787\\
4.22100661702392e-13	0.931405514458641\\
4.30816891243136e-13	0.929388029589778\\
4.43961293735052e-13	0.926473884779197\\
4.55205087511348e-13	0.924904729881192\\
4.58286294150329e-13	0.919524770230889\\
4.64754157309813e-13	0.917058955391167\\
4.7379136673191e-13	0.914368975566015\\
4.80037224333614e-13	0.912799820668011\\
4.85670383643397e-13	0.910109840842859\\
4.95753157068532e-13	0.908540685944854\\
5.00226627775956e-13	0.906299036090561\\
5.06844133894644e-13	0.904505716207127\\
5.21753229085272e-13	0.899798251513112\\
5.33995439242743e-13	0.897780766644249\\
5.40433031511794e-13	0.894866621833668\\
5.46887162184187e-13	0.893521631921093\\
5.60023081994758e-13	0.89105581708137\\
5.68711676634668e-13	0.888365837256219\\
5.69598729896142e-13	0.886572517372785\\
5.79865563938232e-13	0.881640887693341\\
5.89536412937023e-13	0.879399237839048\\
5.96855898038484e-13	0.877830082941043\\
6.0425383098474e-13	0.87558843308675\\
6.16096278225558e-13	0.874467608159604\\
6.30674225967477e-13	0.872225958305311\\
6.38698482312186e-13	0.869984308451018\\
6.45343374382011e-13	0.868863483523872\\
6.58662001749081e-13	0.867070163640437\\
6.82130278125492e-13	0.862586863931852\\
6.85112070754664e-13	0.860345214077559\\
6.89336322672881e-13	0.858551894194125\\
6.9786185484467e-13	0.854965254427256\\
7.03114260253016e-13	0.853396099529251\\
7.12245996859432e-13	0.851154449674959\\
7.19580208463649e-13	0.849585294776954\\
7.30106431805106e-13	0.846895314951802\\
7.41453983336055e-13	0.845101995068368\\
7.50354660251792e-13	0.842187850257787\\
7.64560162221399e-13	0.840394530374353\\
7.73154085250976e-13	0.838601210490919\\
7.79276225562141e-13	0.837032055592914\\
7.96315232839896e-13	0.833893745796904\\
8.03769573285652e-13	0.830979600986324\\
8.13873899873917e-13	0.827841291190314\\
8.24229573481716e-13	0.824927146379733\\
8.3590755195091e-13	0.822685496525441\\
8.47454404739989e-13	0.821340506612865\\
8.58970937217363e-13	0.819995516700289\\
8.85901765088139e-13	0.818426361802284\\
8.97824942508861e-13	0.81663304191885\\
9.09494701772928e-13	0.815063887020845\\
9.11497836189845e-13	0.812822237166552\\
9.19658896747743e-13	0.809908092355972\\
9.2823781172639e-13	0.806993947545391\\
9.40342307350411e-13	0.804752297691098\\
9.48727559402557e-13	0.802734812822235\\
9.6508340711521e-13	0.80116565792423\\
9.77971156662832e-13	0.799820668011655\\
9.9475983006414e-13	0.798699843084508\\
1.00415552577314e-12	0.797579018157362\\
1.02318770738165e-12	0.795337368303069\\
1.02517799317733e-12	0.793992378390493\\
1.03300305030338e-12	0.791302398565342\\
1.04588053123465e-12	0.789957408652766\\
1.06482480586222e-12	0.787491593813044\\
1.07251948202891e-12	0.785249943958752\\
1.08002495835535e-12	0.784129119031605\\
1.09192641913856e-12	0.781439139206454\\
1.10552777748448e-12	0.780094149293878\\
1.11793123403736e-12	0.778973324366732\\
1.13686837721616e-12	0.777628334454156\\
1.14006133572568e-12	0.775835014570722\\
1.1569416322486e-12	0.774265859672717\\
1.16632944176918e-12	0.772920869760141\\
1.17907282587405e-12	0.771127549876707\\
1.19911323450475e-12	0.770006724949561\\
1.22444471506572e-12	0.768661735036985\\
1.24147900736725e-12	0.766868415153551\\
1.25184644420786e-12	0.764850930284688\\
1.26212872323632e-12	0.762833445415824\\
1.27897692436818e-12	0.760367630576102\\
1.28904281046386e-12	0.758798475678097\\
1.30264499513148e-12	0.757005155794663\\
1.31233223107929e-12	0.755436000896658\\
1.34155285663905e-12	0.754091010984082\\
1.36453808001509e-12	0.752970186056935\\
1.36868035111307e-12	0.75162519614436\\
1.37761483482103e-12	0.750280206231784\\
1.38609113934129e-12	0.749159381304637\\
1.40737693108576e-12	0.747814391392062\\
1.44727631055435e-12	0.746245236494057\\
1.45839653790375e-12	0.744900246581481\\
1.47794597063654e-12	0.743106926698047\\
1.48773464483183e-12	0.741313606814612\\
1.49531688725414e-12	0.739968616902037\\
1.50070932050358e-12	0.73884779197489\\
1.51331007532075e-12	0.737502802062315\\
1.56525968725582e-12	0.73570948217888\\
1.59209543076292e-12	0.734588657251734\\
1.60400202952615e-12	0.733467832324588\\
1.62203071720117e-12	0.731450347455724\\
1.64059994059037e-12	0.730105357543149\\
1.66333789916274e-12	0.728312037659714\\
1.68720613142521e-12	0.726967047747139\\
1.70575029700107e-12	0.725622057834563\\
1.71009200358852e-12	0.724501232907417\\
1.72039403314802e-12	0.723380407980271\\
1.73372427525464e-12	0.722035418067695\\
1.76193108970602e-12	0.720914593140549\\
1.79754673591127e-12	0.719569603227973\\
1.81632291385886e-12	0.718448778300827\\
1.83049930775549e-12	0.716879623402822\\
1.84105996830813e-12	0.715534633490246\\
1.86200160830585e-12	0.713965478592241\\
1.89661678804915e-12	0.712396323694236\\
1.93288521312744e-12	0.71127549876709\\
1.94953038767864e-12	0.709930508854514\\
1.97321184688346e-12	0.708809683927368\\
1.99053446236725e-12	0.707464694014792\\
2.02593166559345e-12	0.705895539116788\\
2.05345621318298e-12	0.704550549204212\\
2.08008276108337e-12	0.703429724277066\\
2.10109301159221e-12	0.702308899349919\\
2.12384539875864e-12	0.701188074422773\\
2.16079772698643e-12	0.699843084510197\\
2.16919282855681e-12	0.697825599641334\\
2.17866817101103e-12	0.696480609728758\\
2.21657447936207e-12	0.695359784801611\\
2.25661929576736e-12	0.694238959874465\\
2.27413639959921e-12	0.693118134947318\\
2.31388326449719e-12	0.691997310020172\\
2.34095526616034e-12	0.690428155122167\\
2.38050109600873e-12	0.689307330195021\\
2.40108781332459e-12	0.688186505267874\\
2.42298458887971e-12	0.687065680340728\\
2.4548197509022e-12	0.685944855413582\\
2.49091597363593e-12	0.684824030486436\\
2.51029831210321e-12	0.683703205559289\\
2.52953213930596e-12	0.682582380632143\\
2.59245877054841e-12	0.681461555704996\\
2.61804868225123e-12	0.68034073077785\\
2.62774036203296e-12	0.679219905850703\\
2.72907616003017e-12	0.678099080923557\\
2.79921374664016e-12	0.67697825599641\\
2.88070534995155e-12	0.675633266083835\\
2.95640430157297e-12	0.674512441156688\\
3.01204965867836e-12	0.673167451244112\\
3.09104873948002e-12	0.672046626316966\\
3.15383540061495e-12	0.670925801389819\\
3.20258566154246e-12	0.669804976462673\\
3.23870336196415e-12	0.668684151535526\\
3.29691829392686e-12	0.66756332660838\\
3.41640296932422e-12	0.666218336695804\\
3.46744855050929e-12	0.665097511768658\\
3.5284152893015e-12	0.663976686841511\\
3.57933038036007e-12	0.662631696928936\\
3.63842286919982e-12	0.66151087200179\\
3.66299080453067e-12	0.660390047074643\\
3.72324393538292e-12	0.659269222147497\\
3.76466972416879e-12	0.65814839722035\\
3.8073423222573e-12	0.657027572293204\\
3.86555003187794e-12	0.655682582380628\\
3.89054591349578e-12	0.654561757453482\\
3.98157616419948e-12	0.653440932526336\\
4.07571673582501e-12	0.652320107599189\\
4.22979024500002e-12	0.651199282672043\\
4.32141437121724e-12	0.650078457744896\\
4.37518961371126e-12	0.648733467832321\\
4.59843584297462e-12	0.647612642905174\\
4.67336359502468e-12	0.646491817978028\\
4.72048573180919e-12	0.645370993050882\\
4.78912129166789e-12	0.644250168123735\\
4.83703761335728e-12	0.64290517821116\\
4.90437164674472e-12	0.641784353284013\\
5.00738577683142e-12	0.640663528356867\\
5.23893138188839e-12	0.63954270342972\\
5.46059373481395e-12	0.638421878502574\\
5.52434982230776e-12	0.637301053575428\\
5.61945425455759e-12	0.636180228648281\\
5.78750034586859e-12	0.635059403721135\\
5.90303236458714e-12	0.633938578793988\\
5.99921966009896e-12	0.632817753866842\\
6.107842260478e-12	0.631696928939696\\
6.20296890051747e-12	0.630576104012549\\
6.36703385865042e-12	0.629455279085403\\
6.46592718316341e-12	0.628334454158256\\
6.54767347830829e-12	0.62721362923111\\
6.6450031106314e-12	0.626092804303964\\
6.76514302306148e-12	0.624971979376817\\
7.0127364384876e-12	0.623851154449671\\
7.37007948038297e-12	0.622730329522525\\
7.55467334651578e-12	0.621609504595379\\
7.73154085250976e-12	0.620488679668232\\
7.83785002234034e-12	0.619367854741086\\
8.03268562776793e-12	0.618247029813939\\
8.24701091978201e-12	0.617126204886793\\
8.51435462011192e-12	0.616005379959647\\
8.7461778743126e-12	0.6148845550325\\
8.98989047685482e-12	0.613539565119925\\
9.43669236651073e-12	0.612418740192778\\
9.61729501550998e-12	0.611073750280203\\
9.87117515865762e-12	0.609952925353056\\
1.01027883661295e-11	0.60883210042591\\
1.03642273154033e-11	0.607711275498763\\
1.05884511315578e-11	0.606590450571617\\
1.09111234937814e-11	0.60546962564447\\
1.1060135768759e-11	0.604348800717324\\
1.13766745696611e-11	0.603227975790178\\
1.1775852541756e-11	0.602107150863031\\
1.24435164678855e-11	0.600986325935885\\
1.29040356341522e-11	0.599865501008738\\
1.3057293373425e-11	0.598744676081592\\
1.3222849045435e-11	0.597623851154445\\
1.34852250846814e-11	0.596503026227299\\
1.37786383680678e-11	0.595382201300153\\
1.4121242741192e-11	0.594261376373006\\
1.43133715262661e-11	0.59314055144586\\
1.44274823282071e-11	0.592019726518713\\
1.48909144825549e-11	0.590898901591567\\
1.52000620013116e-11	0.58977807666442\\
1.55296230730988e-11	0.588657251737274\\
1.59167916815399e-11	0.587536426810127\\
1.63197065134017e-11	0.586415601882981\\
1.67023918274532e-11	0.585294776955835\\
1.69495468161083e-11	0.584173952028688\\
1.72811954621206e-11	0.583053127101542\\
1.7683471651488e-11	0.581932302174395\\
1.78243564749975e-11	0.580811477247249\\
1.79981919610909e-11	0.579690652320103\\
1.85887652283715e-11	0.578569827392956\\
1.93585852466548e-11	0.57744900246581\\
1.98764017984508e-11	0.576328177538663\\
2.07734165346255e-11	0.575207352611516\\
2.14252377191187e-11	0.57408652768437\\
2.16724806208781e-11	0.572965702757224\\
2.20447690178231e-11	0.571844877830077\\
2.22974242913649e-11	0.570724052902931\\
2.31180339569304e-11	0.569603227975785\\
2.33923197743807e-11	0.568482403048638\\
2.41777052324623e-11	0.567361578121492\\
2.46640181712211e-11	0.566240753194346\\
2.50126393873015e-11	0.565119928267199\\
2.55715159913234e-11	0.563999103340053\\
2.61618709054535e-11	0.562878278412906\\
2.66146204741658e-11	0.56175745348576\\
2.71995759248966e-11	0.560636628558614\\
2.75948307445002e-11	0.559515803631467\\
2.80298005118622e-11	0.55839497870432\\
2.81604069802e-11	0.557274153777174\\
2.87403074603095e-11	0.556153328850028\\
2.93881663038602e-11	0.555032503922881\\
3.05181008376994e-11	0.553911678995735\\
3.13778890132911e-11	0.552790854068588\\
3.22600800377125e-11	0.551670029141442\\
3.29997466115433e-11	0.550549204214296\\
3.43727881403078e-11	0.549428379287149\\
3.47973264873611e-11	0.548307554360003\\
3.56716190987719e-11	0.547186729432856\\
3.68350727110031e-11	0.54606590450571\\
3.71047784175042e-11	0.544945079578563\\
3.82097395191336e-11	0.543824254651417\\
3.91535224418958e-11	0.542703429724271\\
4.02761084087807e-11	0.541582604797124\\
4.1872663827667e-11	0.540461779869978\\
4.34459274232186e-11	0.539340954942831\\
4.44429117098661e-11	0.538220130015685\\
4.50199899806347e-11	0.537099305088539\\
4.59378182488549e-11	0.535978480161392\\
4.69748524439426e-11	0.534857655234246\\
4.78626987577424e-11	0.533736830307099\\
4.86181814684657e-11	0.532616005379953\\
4.95577112054207e-11	0.531495180452806\\
5.11436411890927e-11	0.53037435552566\\
5.20816087411329e-11	0.529253530598514\\
5.26970761376125e-11	0.528132705671367\\
5.36831321262341e-11	0.527011880744221\\
5.58795961349512e-11	0.525891055817074\\
5.68710568061948e-11	0.524770230889928\\
5.89629922918215e-11	0.523649405962781\\
6.18086974448105e-11	0.522528581035635\\
6.27017953048904e-11	0.521407756108489\\
6.38920052689054e-11	0.520286931181342\\
6.48312603229309e-11	0.519166106254196\\
6.62126362476026e-11	0.518045281327049\\
6.88181618065679e-11	0.516924456399903\\
7.02209509973179e-11	0.515803631472756\\
7.10491930138127e-11	0.51468280654561\\
7.21637500896444e-11	0.513561981618464\\
7.31497338093775e-11	0.512441156691318\\
7.54634816096276e-11	0.511320331764171\\
7.67690286416377e-11	0.510199506837025\\
7.88629670720251e-11	0.509078681909879\\
8.05865332087121e-11	0.507957856982732\\
8.25200436117775e-11	0.506837032055586\\
8.47436818016888e-11	0.505716207128439\\
8.61517522930901e-11	0.504595382201293\\
8.94260760478569e-11	0.503474557274147\\
9.08298249009312e-11	0.502353732347\\
9.34505849292044e-11	0.501232907419854\\
9.57771124989073e-11	0.500112082492708\\
9.79052274485374e-11	0.498991257565561\\
1.0162420978837e-10	0.497870432638415\\
1.03833560510677e-10	0.496749607711268\\
1.05402858788542e-10	0.495628782784122\\
1.07400566929888e-10	0.494507957856976\\
1.08760416339541e-10	0.493387132929829\\
1.10887521130998e-10	0.492266308002683\\
1.14713853592662e-10	0.491145483075537\\
1.16089963872442e-10	0.49002465814839\\
1.20063110567589e-10	0.488903833221244\\
1.24594190427457e-10	0.487783008294098\\
1.26985100652127e-10	0.486662183366951\\
1.32446748694947e-10	0.485541358439805\\
1.35288574548494e-10	0.484420533512659\\
1.37995618211836e-10	0.483299708585512\\
1.40021021912855e-10	0.482178883658366\\
1.44844819689459e-10	0.481058058731219\\
1.48686675461263e-10	0.479937233804073\\
1.55106239444858e-10	0.478816408876927\\
1.58025726793388e-10	0.477695583949781\\
1.67348733895541e-10	0.476574759022634\\
1.73271509275435e-10	0.475453934095488\\
1.85958779287606e-10	0.474333109168341\\
1.97259098576739e-10	0.473212284241195\\
2.04545229605303e-10	0.472091459314049\\
2.12708075275975e-10	0.470970634386902\\
2.22504225773314e-10	0.469849809459756\\
2.34193397356215e-10	0.46872898453261\\
2.43586220771613e-10	0.467608159605463\\
2.56250378502804e-10	0.466487334678317\\
2.64046437959807e-10	0.465366509751171\\
2.81506678812415e-10	0.464245684824024\\
2.8842351290118e-10	0.463124859896878\\
3.01160672478618e-10	0.462004034969731\\
3.22411463426985e-10	0.460883210042585\\
3.43911421910858e-10	0.459762385115439\\
3.60153285360651e-10	0.458641560188292\\
3.81254965407644e-10	0.457520735261146\\
4.08590890176269e-10	0.456399910334\\
4.33719591980443e-10	0.455279085406853\\
4.57553505218493e-10	0.454158260479707\\
5.05189424441816e-10	0.453037435552561\\
5.53893756868022e-10	0.451916610625414\\
6.42515083659653e-10	0.450795785698268\\
7.07032799030434e-10	0.449674960771122\\
7.98398599832409e-10	0.448554135843975\\
8.95485014519724e-10	0.447433310916829\\
9.88193720792365e-10	0.446312485989683\\
1.05481008356866e-09	0.445191661062536\\
1.13148096617748e-09	0.44407083613539\\
1.39036251056385e-09	0.442950011208244\\
1.57591178939133e-09	0.441829186281097\\
1.75145182507432e-09	0.440708361353951\\
1.88175869575368e-09	0.439587536426805\\
2.00273475451575e-09	0.438466711499658\\
2.14391361176738e-09	0.437345886572512\\
2.23396944131946e-09	0.436225061645366\\
2.41919940989517e-09	0.435104236718219\\
2.51151001202685e-09	0.433983411791073\\
2.60374663947312e-09	0.432862586863926\\
2.73146131038777e-09	0.43174176193678\\
2.98008138708991e-09	0.430620937009634\\
3.05127464091125e-09	0.429500112082488\\
3.18170145863094e-09	0.428379287155341\\
3.28068484649207e-09	0.427258462228195\\
3.46561084207003e-09	0.426137637301048\\
3.55664169949183e-09	0.425016812373902\\
3.6920793577921e-09	0.423895987446756\\
4.4222274189511e-09	0.422775162519609\\
4.71545267304733e-09	0.421654337592463\\
5.10816255549613e-09	0.420533512665317\\
5.55768993504099e-09	0.41941268773817\\
6.00066286771241e-09	0.418291862811024\\
6.41363306405217e-09	0.417171037883878\\
6.86147669065337e-09	0.416050212956731\\
7.22043985571455e-09	0.414929388029585\\
8.00482882580945e-09	0.413808563102439\\
8.63786572826157e-09	0.412687738175292\\
9.10706046358288e-09	0.411566913248146\\
9.52468274273213e-09	0.410446088321\\
1.05265336663453e-08	0.409325263393853\\
1.23445175649352e-08	0.408204438466707\\
1.38194416102654e-08	0.407083613539561\\
1.43018001453672e-08	0.405962788612414\\
1.50689425208806e-08	0.404841963685268\\
1.57288525402677e-08	0.403721138758122\\
1.66441694051972e-08	0.402600313830975\\
1.69502853618323e-08	0.401479488903829\\
1.76829296445834e-08	0.400358663976683\\
1.87484084988997e-08	0.399237839049536\\
1.92879925761215e-08	0.39811701412239\\
1.99671350390255e-08	0.396996189195244\\
2.058523973968e-08	0.395875364268097\\
2.17082109511151e-08	0.394754539340951\\
2.27392772624704e-08	0.393633714413805\\
2.31602301081302e-08	0.392512889486658\\
2.40703467108488e-08	0.391392064559512\\
2.58967883422053e-08	0.390271239632366\\
2.61993895332528e-08	0.389150414705219\\
2.79167418922537e-08	0.388029589778073\\
2.89628873391076e-08	0.386908764850927\\
3.05421263195871e-08	0.38578793992378\\
3.22512211779502e-08	0.384667114996634\\
3.36837086577249e-08	0.383546290069488\\
3.6642598626898e-08	0.382425465142341\\
3.92276869981867e-08	0.381304640215195\\
4.01453061962578e-08	0.380183815288049\\
4.20004644752914e-08	0.379062990360902\\
4.28119460445629e-08	0.377942165433756\\
4.57114642997671e-08	0.37682134050661\\
4.86722487854549e-08	0.375700515579463\\
5.01609449789817e-08	0.374579690652317\\
5.27884871741689e-08	0.373458865725171\\
5.64606738681438e-08	0.372338040798024\\
5.94672891054899e-08	0.371217215870878\\
6.26947025627771e-08	0.370096390943732\\
6.43852570189168e-08	0.368975566016585\\
6.94414638694813e-08	0.367854741089439\\
7.17107032365734e-08	0.366733916162293\\
7.50230673420096e-08	0.365613091235146\\
7.84622397305235e-08	0.364492266308\\
8.34066554271508e-08	0.363371441380854\\
8.64881985330073e-08	0.362250616453707\\
8.89307163616976e-08	0.361129791526561\\
9.50429451606633e-08	0.360008966599415\\
9.71872914136064e-08	0.358888141672268\\
1.01994229875382e-07	0.357767316745122\\
1.05285277178794e-07	0.356646491817976\\
1.0686813164397e-07	0.355525666890829\\
1.12206683857839e-07	0.354404841963683\\
1.14581732457455e-07	0.353284017036537\\
1.16846902444081e-07	0.35216319210939\\
1.18035460536077e-07	0.351042367182244\\
1.2139236011402e-07	0.349921542255098\\
1.25160692313271e-07	0.348800717327951\\
1.28364265950745e-07	0.347679892400805\\
1.33512822556707e-07	0.346559067473659\\
1.42809254643174e-07	0.345438242546512\\
1.47173486370084e-07	0.344317417619366\\
1.51386705981801e-07	0.34319659269222\\
1.57466338082589e-07	0.342075767765073\\
1.64959701758243e-07	0.340954942837927\\
1.68957376723258e-07	0.339834117910781\\
1.77614802525879e-07	0.338713292983634\\
1.83128966780841e-07	0.337592468056488\\
1.85586139890605e-07	0.336471643129342\\
1.92317266250473e-07	0.335350818202195\\
2.02407874080603e-07	0.334229993275049\\
2.11785543150873e-07	0.333109168347903\\
2.14472937636713e-07	0.331988343420756\\
2.19307140673036e-07	0.33086751849361\\
2.22651643741204e-07	0.329746693566464\\
2.35088969527992e-07	0.328625868639317\\
2.41036722987451e-07	0.327505043712171\\
2.52868191336279e-07	0.326384218785025\\
2.59645660235704e-07	0.325263393857878\\
2.68447961963199e-07	0.324142568930732\\
2.79206280589038e-07	0.323021744003586\\
2.84756508092456e-07	0.321900919076439\\
2.93690756541196e-07	0.320780094149293\\
3.00127594724225e-07	0.319659269222147\\
3.12833319603589e-07	0.318538444295001\\
3.2408370645351e-07	0.317417619367854\\
3.34751782448333e-07	0.316296794440708\\
3.42200932644517e-07	0.315175969513562\\
3.50865637970395e-07	0.314055144586415\\
3.56324281543293e-07	0.312934319659269\\
3.65569489053835e-07	0.311813494732122\\
3.69463156844445e-07	0.310692669804976\\
3.78240462231026e-07	0.30957184487783\\
3.83335298792992e-07	0.308451019950684\\
3.93325099436445e-07	0.307330195023537\\
4.02647669972627e-07	0.306209370096391\\
4.13224975796572e-07	0.305088545169245\\
4.23274003672697e-07	0.303967720242098\\
4.30536374047437e-07	0.302846895314952\\
4.35237349517172e-07	0.301726070387806\\
4.39448596238374e-07	0.300605245460659\\
4.48864556957297e-07	0.299484420533513\\
4.55325024440866e-07	0.298363595606367\\
4.59833974317065e-07	0.29724277067922\\
4.71320106762623e-07	0.296121945752074\\
4.79176329446415e-07	0.295001120824928\\
4.85431995076479e-07	0.293880295897781\\
4.88917011111519e-07	0.292759470970635\\
5.03577158978066e-07	0.291638646043489\\
5.1135382937333e-07	0.290517821116342\\
5.1559952865852e-07	0.289396996189196\\
5.25371549889043e-07	0.28827617126205\\
5.33170613092628e-07	0.287155346334903\\
5.38170855194651e-07	0.286034521407757\\
5.43153000038224e-07	0.284913696480611\\
5.55626382208422e-07	0.283792871553464\\
5.62966576266807e-07	0.282672046626318\\
5.79392128711875e-07	0.281551221699172\\
5.91129666730083e-07	0.280430396772025\\
6.10305608443582e-07	0.279309571844879\\
6.18750317782567e-07	0.278188746917733\\
6.30280117344896e-07	0.277067921990586\\
6.42304718449235e-07	0.27594709706344\\
6.49521498766074e-07	0.274826272136294\\
6.69063536366912e-07	0.273705447209148\\
6.81917209378983e-07	0.272584622282001\\
6.89065477024119e-07	0.271463797354855\\
7.04525340949793e-07	0.270342972427709\\
7.18293902770063e-07	0.269222147500562\\
7.2405416355338e-07	0.268101322573416\\
7.32167345203492e-07	0.26698049764627\\
7.50035058731827e-07	0.265859672719123\\
7.59959561949059e-07	0.264738847791977\\
7.68527934951957e-07	0.263618022864831\\
7.77538309208371e-07	0.262497197937684\\
7.87599260360176e-07	0.261376373010538\\
8.04713307327935e-07	0.260255548083392\\
8.16345895157414e-07	0.259134723156245\\
8.2671447424152e-07	0.258013898229099\\
8.34303045852673e-07	0.256893073301953\\
8.43173235291073e-07	0.255772248374806\\
8.49488483758344e-07	0.25465142344766\\
8.55945374221758e-07	0.253530598520514\\
8.66155348603608e-07	0.252409773593367\\
8.79869531527378e-07	0.251288948666221\\
8.934632091327e-07	0.250168123739075\\
9.13661519170203e-07	0.249047298811928\\
9.18860748120669e-07	0.247926473884782\\
9.27495371519471e-07	0.246805648957636\\
9.33650607373928e-07	0.245684824030489\\
9.50327170119474e-07	0.244563999103343\\
9.68146656755566e-07	0.243443174176196\\
9.83188772390825e-07	0.24232234924905\\
9.95664428432998e-07	0.241201524321904\\
1.0155572365563e-06	0.240080699394757\\
1.03682336880315e-06	0.238959874467611\\
1.04605655938414e-06	0.237839049540464\\
1.05293214196424e-06	0.236718224613318\\
1.07543830931233e-06	0.235597399686172\\
1.08766543785806e-06	0.234476574759025\\
1.10726534304307e-06	0.233355749831879\\
1.1350975563007e-06	0.232234924904732\\
1.15580918130118e-06	0.231114099977586\\
1.17151016111057e-06	0.22999327505044\\
1.19438943270389e-06	0.228872450123293\\
1.2106106045426e-06	0.227751625196147\\
1.22390292298642e-06	0.226630800269001\\
1.24859578460425e-06	0.225509975341854\\
1.25701202230065e-06	0.224389150414708\\
1.27020446365368e-06	0.223268325487561\\
1.29450892646298e-06	0.222147500560415\\
1.31633814758597e-06	0.221026675633269\\
1.3316259934838e-06	0.219905850706122\\
1.38075059873411e-06	0.218785025778976\\
1.39991161679601e-06	0.217664200851829\\
1.41969789804883e-06	0.216543375924683\\
1.46525435648921e-06	0.215422550997537\\
1.50352972744133e-06	0.21430172607039\\
1.54613583506153e-06	0.213180901143244\\
1.58425346369804e-06	0.212060076216097\\
1.59086435496919e-06	0.210939251288951\\
1.62672807957789e-06	0.209818426361805\\
1.63806951625317e-06	0.208697601434658\\
1.65020449027498e-06	0.207576776507512\\
1.6743082244513e-06	0.206455951580365\\
1.72167308367485e-06	0.205335126653219\\
1.75941266464779e-06	0.204214301726073\\
1.79951611551977e-06	0.203093476798926\\
1.83458558390742e-06	0.20197265187178\\
1.86595964652991e-06	0.200851826944634\\
1.91801335999089e-06	0.199731002017487\\
1.98585489142736e-06	0.198610177090341\\
2.01698327787764e-06	0.197489352163194\\
2.05268036302057e-06	0.196368527236048\\
2.09063760760197e-06	0.195247702308902\\
2.11607256376023e-06	0.194126877381755\\
2.18074013043107e-06	0.193006052454609\\
2.25038776810346e-06	0.191885227527463\\
2.30967303383705e-06	0.190764402600316\\
2.35934302361725e-06	0.18964357767317\\
2.39496458515324e-06	0.188522752746023\\
2.41316119241773e-06	0.187401927818877\\
2.45898409168975e-06	0.18628110289173\\
2.48903072112239e-06	0.185160277964584\\
2.56502861713564e-06	0.184039453037438\\
2.59017685522364e-06	0.182918628110291\\
2.62997495141657e-06	0.181797803183145\\
2.76350576741186e-06	0.180676978255998\\
2.86642512693768e-06	0.179556153328852\\
2.96177381702138e-06	0.178435328401706\\
3.06342530549991e-06	0.177314503474559\\
3.11634714838656e-06	0.176193678547413\\
3.25588987982303e-06	0.175072853620266\\
3.36793850020312e-06	0.17395202869312\\
3.41298214022222e-06	0.172831203765974\\
3.49701746177448e-06	0.171710378838827\\
3.5462934246648e-06	0.170589553911681\\
3.64951094327624e-06	0.169468728984535\\
3.75547217757541e-06	0.168347904057388\\
3.85572748545486e-06	0.167227079130242\\
3.94646875242646e-06	0.166106254203095\\
4.04724658388011e-06	0.164985429275949\\
4.15374683926963e-06	0.163864604348803\\
4.21183843541414e-06	0.162743779421656\\
4.36423086366047e-06	0.16162295449451\\
4.41922036356443e-06	0.160502129567364\\
4.52247454747663e-06	0.159381304640217\\
4.6040354912472e-06	0.158260479713071\\
4.64953806111032e-06	0.157139654785925\\
4.75588013712478e-06	0.156018829858778\\
4.89089975957237e-06	0.154898004931632\\
5.06110999831955e-06	0.153777180004485\\
5.14806743183948e-06	0.152656355077339\\
5.36271265486719e-06	0.151535530150192\\
5.45210707455323e-06	0.150414705223046\\
5.55815028674691e-06	0.1492938802959\\
5.71560850718143e-06	0.148173055368753\\
5.95233739191769e-06	0.147052230441607\\
6.03646189539439e-06	0.145931405514461\\
6.11356007395231e-06	0.144810580587314\\
6.4503100410902e-06	0.143689755660168\\
6.72458716377034e-06	0.142568930733021\\
6.94868131667417e-06	0.141448105805875\\
7.12046423700997e-06	0.140327280878729\\
7.36958449320064e-06	0.139206455951582\\
7.59268773333302e-06	0.138085631024436\\
7.80504029538614e-06	0.136964806097289\\
8.01084303906875e-06	0.135843981170143\\
8.38537162679881e-06	0.134723156242997\\
8.48823502164509e-06	0.13360233131585\\
8.7758458034291e-06	0.132481506388704\\
8.93061698985949e-06	0.131360681461558\\
9.05873248558693e-06	0.130239856534411\\
9.13423000778839e-06	0.129119031607265\\
9.4639982063435e-06	0.127998206680118\\
9.65572235037835e-06	0.126877381752972\\
1.00179187613121e-05	0.125756556825826\\
1.03595040329853e-05	0.124635731898679\\
1.05245490243057e-05	0.123514906971533\\
1.07165589631645e-05	0.122394082044387\\
1.10526578858001e-05	0.12127325711724\\
1.12717724878328e-05	0.120152432190094\\
1.16314779653165e-05	0.119031607262947\\
1.18836429627701e-05	0.117910782335801\\
1.19640407453909e-05	0.116789957408654\\
1.21484450730022e-05	0.115669132481508\\
1.24921569022173e-05	0.114548307554362\\
1.28215617689703e-05	0.113427482627215\\
1.29424031935951e-05	0.112306657700069\\
1.32506659718864e-05	0.111185832772922\\
1.34806064453897e-05	0.110065007845776\\
1.38302845506526e-05	0.10894418291863\\
1.42572300460338e-05	0.107823357991483\\
1.456735609261e-05	0.106702533064337\\
1.48628362941148e-05	0.105581708137191\\
1.56178544527087e-05	0.104460883210044\\
1.59000414762326e-05	0.103340058282898\\
1.63992221988443e-05	0.102219233355751\\
1.72356033628804e-05	0.101098408428605\\
1.77003313713418e-05	0.0999775835014586\\
1.82807385445076e-05	0.0988567585743122\\
1.86865766435143e-05	0.0977359336471658\\
1.92150869154592e-05	0.0966151087200194\\
1.96179266146994e-05	0.0954942837928731\\
1.98923415919156e-05	0.0943734588657267\\
2.02050702610971e-05	0.0932526339385802\\
2.07838231583157e-05	0.0921318090114338\\
2.10766915703892e-05	0.0910109840842874\\
2.15303966456259e-05	0.089890159157141\\
2.19753303152666e-05	0.0887693342299947\\
2.25736292801337e-05	0.0876485093028483\\
2.31611559811146e-05	0.0865276843757019\\
2.36314882148963e-05	0.0854068594485555\\
2.39181266595612e-05	0.0842860345214091\\
2.43924955561162e-05	0.0831652095942627\\
2.46312493972539e-05	0.0820443846671163\\
2.54512013200963e-05	0.0809235597399699\\
2.6001345642499e-05	0.0798027348128235\\
2.69896644091743e-05	0.0786819098856771\\
2.72036908454524e-05	0.0775610849585308\\
2.75192045832704e-05	0.0764402600313844\\
2.83088577773295e-05	0.0753194351042379\\
2.87179521144818e-05	0.0741986101770915\\
2.95481560299286e-05	0.0730777852499451\\
3.01961550370714e-05	0.0719569603227987\\
3.14601855353667e-05	0.0708361353956524\\
3.20805593729765e-05	0.069715310468506\\
3.23755414875953e-05	0.0685944855413596\\
3.28658153958137e-05	0.0674736606142132\\
3.37142007677435e-05	0.0663528356870668\\
3.46774500953612e-05	0.0652320107599204\\
3.61151955176604e-05	0.064111185832774\\
3.79259645514649e-05	0.0629903609056276\\
3.82044732062606e-05	0.0618695359784812\\
3.90844065337101e-05	0.0607487110513348\\
4.00264494897977e-05	0.0596278861241885\\
4.07038597796182e-05	0.058507061197042\\
4.21837395247373e-05	0.0573862362698956\\
4.34808994843178e-05	0.0562654113427492\\
4.43269614505254e-05	0.0551445864156028\\
4.54442807379196e-05	0.0540237614884564\\
4.66265230313437e-05	0.0529029365613101\\
4.80503624202674e-05	0.0517821116341637\\
4.98479402322989e-05	0.0506612867070173\\
5.22291885562559e-05	0.0495404617798708\\
5.38365154510714e-05	0.0484196368527244\\
5.53212672678617e-05	0.0472988119255781\\
5.6348974935109e-05	0.0461779869984317\\
5.76825810473539e-05	0.0450571620712853\\
6.00006017659469e-05	0.0439363371441389\\
6.07662413136435e-05	0.0428155122169925\\
6.50539222071925e-05	0.041694687289846\\
6.75527303422807e-05	0.0405738623626997\\
6.90849969074512e-05	0.0394530374355533\\
7.13382303691733e-05	0.0383322125084069\\
7.68651739941534e-05	0.0372113875812605\\
7.92210884799815e-05	0.0360905626541141\\
8.15057268380132e-05	0.0349697377269678\\
8.42265958107501e-05	0.0338489127998214\\
8.56484582273661e-05	0.0327280878726749\\
8.88343775182957e-05	0.0316072629455285\\
9.08522885150847e-05	0.0304864380183821\\
9.71691656108791e-05	0.0293656130912358\\
0.000100018443852462	0.0282447881640894\\
0.000101915955238097	0.0271239632369429\\
0.000107798907454266	0.0260031383097965\\
0.000111878044994242	0.0248823133826501\\
0.000116445896488368	0.0237614884555037\\
0.000129680715092367	0.0226406635283574\\
0.000139439496102696	0.021519838601211\\
0.000150716066212241	0.0203990136740645\\
0.000169952123891708	0.0192781887469181\\
0.00017876125926567	0.0181573638197717\\
0.000228950401902898	0.0170365388926254\\
0.000328944482540013	0.015915713965479\\
0.000648995390176783	0.0147948890383325\\
0.00186222207853477	0.0136740641111861\\
0.00860392956660599	0.0125532391840397\\
0.0806298100110785	0.0114324142568933\\
14.4988595376509	0.010311589329747\\
60.6797164940808	0.00919076440260047\\
131.507855530199	0.00806993947545409\\
218.491350443469	0.00694911454830771\\
529.041315181901	0.00582828962116133\\
1086.15684268478	0.00470746469401495\\
1413.43455523179	0.00358663976686846\\
1552.40470254885	0.00246581483972208\\
1649.24262005884	0.0013449899125757\\
2446.73099141547	0.00022416498542932\\
};
\addlegendentry{$N=2$,~, $\lrmse =94.17$, $\prmse =0.015$, $\armse =0.028$, $\brmse =3\hspace{-3pt}\times\hspace{-3pt}10^{-4}$, $\gamma \rightarrow \infty$}


==> figures/mse_N_2_K_20_G_5_SNR_40_I_20_Pratio_2_Nratio_1_cs.tex <==
\addplot [color=blue, dashed,line width=0.6pt]
  table[row sep=crcr]{%
0.0259132649530224	1\\
0.0259132649530224	0.999324324324324\\
0.0339697428049308	0.998648648648649\\
0.0461343934603397	0.997972972972973\\
0.0517095630831873	0.997297297297297\\
0.0521544349804292	0.996621621621622\\
0.0522447022882867	0.995945945945946\\
0.0526579126935798	0.99527027027027\\
0.052772581932691	0.994594594594595\\
0.0532845414433845	0.993918918918919\\
0.0543996564279004	0.993243243243243\\
0.0546697910546455	0.992567567567568\\
0.0546924102814615	0.991891891891892\\
0.0577731641379093	0.991216216216216\\
0.0582286855921402	0.99054054054054\\
0.0582332511187664	0.989864864864865\\
0.0596285739192182	0.989189189189189\\
0.0600077212863887	0.988513513513513\\
0.0603908635072678	0.987837837837838\\
0.0625362227399033	0.987162162162162\\
0.0627636260304324	0.986486486486486\\
0.0628491492373313	0.985810810810811\\
0.063071194120347	0.985135135135135\\
0.064471287794792	0.984459459459459\\
0.0645806956668101	0.983783783783784\\
0.0647666161303729	0.983108108108108\\
0.0652674206153528	0.982432432432432\\
0.0657547113756153	0.981756756756757\\
0.0665360580512596	0.981081081081081\\
0.0665884986422282	0.980405405405405\\
0.0668399450283013	0.97972972972973\\
0.0682288014213744	0.979054054054054\\
0.0701991732403336	0.978378378378378\\
0.0716775368119457	0.977702702702702\\
0.0725297802117349	0.977027027027027\\
0.0727436695228145	0.976351351351351\\
0.0730983655469086	0.975675675675675\\
0.0736910385492142	0.975\\
0.0739283061211141	0.974324324324324\\
0.075061846426365	0.973648648648648\\
0.075810708833019	0.972972972972972\\
0.0761150229881689	0.972297297297297\\
0.0761286160445376	0.971621621621621\\
0.0769003620676231	0.970945945945945\\
0.0777153899739915	0.97027027027027\\
0.0788297976124173	0.969594594594594\\
0.0792462189020897	0.968918918918918\\
0.0796925725266732	0.968243243243243\\
0.0802642475917854	0.967567567567567\\
0.0803463696891224	0.966891891891891\\
0.0811237537515946	0.966216216216216\\
0.081246350470594	0.96554054054054\\
0.0812584898618051	0.964864864864864\\
0.0825646576193794	0.964189189189189\\
0.0826930719921826	0.963513513513513\\
0.082721564793215	0.962837837837837\\
0.0835869843445749	0.962162162162161\\
0.0849055867347487	0.961486486486486\\
0.0850128311395457	0.96081081081081\\
0.0858627368608544	0.960135135135134\\
0.0858692278156385	0.959459459459459\\
0.0859618338506587	0.958783783783783\\
0.0860107093367029	0.958108108108107\\
0.0863602001690801	0.957432432432432\\
0.0866509495037553	0.956756756756756\\
0.0868288664447322	0.95608108108108\\
0.0869101820304014	0.955405405405405\\
0.0873842555358529	0.954729729729729\\
0.0876736268227448	0.954054054054053\\
0.0877053113164049	0.953378378378378\\
0.0885089021979163	0.952702702702702\\
0.0886432707618841	0.952027027027026\\
0.0887548386347448	0.951351351351351\\
0.088806024671503	0.950675675675675\\
0.088823040309642	0.949999999999999\\
0.0888928689733143	0.949324324324324\\
0.0901559539433246	0.948648648648648\\
0.0904754226967641	0.947972972972972\\
0.0905144786542806	0.947297297297297\\
0.0906451608062006	0.946621621621621\\
0.0920991964566161	0.945945945945945\\
0.0926100553173126	0.94527027027027\\
0.0928521314911324	0.944594594594594\\
0.0930303183650316	0.943918918918918\\
0.0945023888991836	0.943243243243243\\
0.0945345451179769	0.942567567567567\\
0.0945524146577758	0.941891891891891\\
0.0949269689386643	0.941216216216215\\
0.095370135399722	0.94054054054054\\
0.0957998245955535	0.939864864864864\\
0.0958214791447604	0.939189189189188\\
0.0962630165292737	0.938513513513513\\
0.0965494302909953	0.937837837837837\\
0.0965502970973103	0.937162162162162\\
0.0968626675407727	0.936486486486486\\
0.0972221799071613	0.93581081081081\\
0.0972357057123334	0.935135135135135\\
0.0978729183519971	0.934459459459459\\
0.0985249437593545	0.933783783783783\\
0.0986172894029381	0.933108108108108\\
0.0986370982766685	0.932432432432432\\
0.0996510913020338	0.931756756756756\\
0.0999688656868119	0.931081081081081\\
0.100051117036246	0.930405405405405\\
0.100073179856151	0.929729729729729\\
0.100331700943623	0.929054054054054\\
0.100788960989727	0.928378378378378\\
0.100799107320541	0.927702702702702\\
0.101295040588932	0.927027027027027\\
0.101496807647808	0.926351351351351\\
0.102001650027856	0.925675675675675\\
0.102407312142519	0.925\\
0.10285729088825	0.924324324324324\\
0.103308574135792	0.923648648648648\\
0.103828247761244	0.922972972972973\\
0.104077724604279	0.922297297297297\\
0.104452789852963	0.921621621621621\\
0.105140980636118	0.920945945945946\\
0.105333529990339	0.92027027027027\\
0.105914437454691	0.919594594594594\\
0.106002561622675	0.918918918918919\\
0.106563165596938	0.918243243243243\\
0.106816711928448	0.917567567567567\\
0.107648652461555	0.916891891891891\\
0.107851418867039	0.916216216216216\\
0.108019993455404	0.91554054054054\\
0.108339851338794	0.914864864864865\\
0.108484848435282	0.914189189189189\\
0.108528066176637	0.913513513513513\\
0.108647055441518	0.912837837837837\\
0.108878928772126	0.912162162162162\\
0.109229268620916	0.911486486486486\\
0.109446432936636	0.910810810810811\\
0.109651016358684	0.910135135135135\\
0.110124224005662	0.909459459459459\\
0.111072498332087	0.908783783783783\\
0.111286705192907	0.908108108108108\\
0.11148559902329	0.907432432432432\\
0.111765742710184	0.906756756756756\\
0.113027410968147	0.906081081081081\\
0.113093166135305	0.905405405405405\\
0.113189860949325	0.904729729729729\\
0.113394718207575	0.904054054054053\\
0.11347410534643	0.903378378378378\\
0.113544151157768	0.902702702702702\\
0.113757835169933	0.902027027027027\\
0.113892976900161	0.901351351351351\\
0.114118685365523	0.900675675675675\\
0.114490281937693	0.9\\
0.115337113308907	0.899324324324324\\
0.115380360531455	0.898648648648648\\
0.115589301318209	0.897972972972973\\
0.116053294882801	0.897297297297297\\
0.116253107114258	0.896621621621621\\
0.116260755899239	0.895945945945945\\
0.117037888596406	0.89527027027027\\
0.117224120836779	0.894594594594594\\
0.117389084394838	0.893918918918918\\
0.117402141583715	0.893243243243243\\
0.117563425711227	0.892567567567567\\
0.117636705236476	0.891891891891891\\
0.118027138993839	0.891216216216216\\
0.118129635344915	0.89054054054054\\
0.118495068628388	0.889864864864864\\
0.119168197402238	0.889189189189189\\
0.119509582175976	0.888513513513513\\
0.119817201662148	0.887837837837837\\
0.119958252672971	0.887162162162161\\
0.120101228042465	0.886486486486486\\
0.120311201843459	0.88581081081081\\
0.120326280693907	0.885135135135135\\
0.120684448954177	0.884459459459459\\
0.120997852202381	0.883783783783783\\
0.121284476320718	0.883108108108108\\
0.121555251003438	0.882432432432432\\
0.121720982369884	0.881756756756756\\
0.121919911392378	0.881081081081081\\
0.122017366653672	0.880405405405405\\
0.122365331139812	0.879729729729729\\
0.122934318631257	0.879054054054053\\
0.123102396669181	0.878378378378378\\
0.12313323319859	0.877702702702702\\
0.123312670306601	0.877027027027027\\
0.123706490812778	0.876351351351351\\
0.123952216050184	0.875675675675675\\
0.124204175893732	0.875\\
0.124232417288042	0.874324324324324\\
0.124470570864913	0.873648648648648\\
0.125607768310541	0.872972972972973\\
0.125742604160835	0.872297297297297\\
0.126999924596045	0.871621621621621\\
0.127021384295383	0.870945945945946\\
0.127057752896463	0.87027027027027\\
0.12706254739149	0.869594594594594\\
0.127277275294044	0.868918918918919\\
0.127746500856325	0.868243243243243\\
0.128037958709521	0.867567567567567\\
0.128129225598873	0.866891891891892\\
0.128525854082826	0.866216216216216\\
0.128700996070481	0.86554054054054\\
0.129442491710109	0.864864864864865\\
0.129530976591681	0.864189189189189\\
0.130359993493684	0.863513513513513\\
0.130588306342061	0.862837837837838\\
0.130601513361092	0.862162162162162\\
0.130879479423139	0.861486486486486\\
0.130884413799571	0.860810810810811\\
0.1321967145366	0.860135135135135\\
0.132264012946886	0.859459459459459\\
0.132915069018611	0.858783783783784\\
0.132929036574269	0.858108108108108\\
0.133331808533278	0.857432432432432\\
0.133429805214548	0.856756756756757\\
0.133866092082835	0.856081081081081\\
0.133981124406691	0.855405405405405\\
0.134146636108728	0.854729729729729\\
0.134179197515717	0.854054054054054\\
0.134242129629784	0.853378378378378\\
0.13425215599142	0.852702702702702\\
0.134283249475395	0.852027027027027\\
0.134411721935542	0.851351351351351\\
0.135174613142712	0.850675675675675\\
0.135186912692623	0.849999999999999\\
0.135269908284559	0.849324324324324\\
0.135311943645098	0.848648648648648\\
0.135554321060065	0.847972972972972\\
0.135946913856722	0.847297297297297\\
0.136291292920899	0.846621621621621\\
0.136312308151794	0.845945945945945\\
0.137007878711019	0.84527027027027\\
0.137121793332938	0.844594594594594\\
0.1373533284833	0.843918918918918\\
0.137478537218362	0.843243243243243\\
0.137724767024142	0.842567567567567\\
0.137974801855391	0.841891891891891\\
0.138097921454004	0.841216216216216\\
0.138421100062915	0.84054054054054\\
0.138727725968933	0.839864864864864\\
0.13906181226913	0.839189189189189\\
0.139315579323739	0.838513513513513\\
0.139476207102114	0.837837837837837\\
0.139554798856032	0.837162162162161\\
0.139769491917097	0.836486486486486\\
0.14003711409697	0.83581081081081\\
0.140058835654735	0.835135135135134\\
0.140463308863655	0.834459459459459\\
0.140714819495357	0.833783783783783\\
0.14071788739933	0.833108108108107\\
0.141175028132834	0.832432432432431\\
0.141941225416871	0.831756756756756\\
0.14224397368266	0.83108108108108\\
0.142274147721602	0.830405405405404\\
0.142584256312874	0.829729729729729\\
0.142832437332893	0.829054054054053\\
0.143578303881267	0.828378378378377\\
0.143788435081661	0.827702702702702\\
0.143874940067686	0.827027027027026\\
0.144168363335775	0.82635135135135\\
0.144583312641299	0.825675675675675\\
0.144867666353038	0.824999999999999\\
0.145113109660199	0.824324324324323\\
0.14531988532063	0.823648648648648\\
0.145494109613624	0.822972972972972\\
0.145711907047528	0.822297297297296\\
0.145744682299353	0.821621621621621\\
0.145925641366135	0.820945945945945\\
0.146018720007343	0.820270270270269\\
0.14629193896598	0.819594594594594\\
0.146466297375809	0.818918918918918\\
0.146757237303742	0.818243243243242\\
0.147403819198744	0.817567567567566\\
0.14766570071046	0.816891891891891\\
0.14832268075519	0.816216216216215\\
0.148429800124275	0.815540540540539\\
0.149758040227491	0.814864864864864\\
0.149762925092611	0.814189189189188\\
0.149843710712562	0.813513513513512\\
0.150297913806609	0.812837837837837\\
0.150334058726533	0.812162162162161\\
0.150608281497005	0.811486486486485\\
0.150656034991953	0.81081081081081\\
0.150975280572417	0.810135135135134\\
0.151037809873331	0.809459459459458\\
0.151284848931132	0.808783783783782\\
0.151512175952898	0.808108108108107\\
0.151541054353881	0.807432432432431\\
0.152112035170833	0.806756756756755\\
0.153385301933942	0.80608108108108\\
0.153455731751105	0.805405405405404\\
0.153778233849302	0.804729729729728\\
0.153914063759706	0.804054054054053\\
0.154100892812449	0.803378378378377\\
0.154256959716021	0.802702702702701\\
0.154994775146323	0.802027027027026\\
0.155104335534025	0.80135135135135\\
0.155298223255661	0.800675675675674\\
0.155350143215201	0.799999999999999\\
0.155382293905362	0.799324324324323\\
0.155717434678317	0.798648648648647\\
0.155730966756831	0.797972972972972\\
0.155731687921788	0.797297297297296\\
0.156024639713338	0.79662162162162\\
0.156334283317619	0.795945945945945\\
0.156624967423115	0.795270270270269\\
0.156673251121296	0.794594594594593\\
0.157146627665668	0.793918918918918\\
0.157180870680645	0.793243243243242\\
0.157248258406742	0.792567567567566\\
0.157332228710591	0.791891891891891\\
0.157677555619694	0.791216216216215\\
0.158126086419929	0.790540540540539\\
0.158481040184505	0.789864864864864\\
0.158492341265618	0.789189189189188\\
0.158779695405246	0.788513513513512\\
0.158845413064447	0.787837837837837\\
0.158940782336054	0.787162162162161\\
0.15917646063977	0.786486486486485\\
0.15932740020825	0.78581081081081\\
0.159434832607299	0.785135135135134\\
0.159473545206549	0.784459459459458\\
0.159606465086863	0.783783783783783\\
0.15970327622983	0.783108108108107\\
0.159707738245849	0.782432432432431\\
0.159933176493823	0.781756756756756\\
0.160130442525769	0.78108108108108\\
0.160174527548127	0.780405405405404\\
0.160266634735453	0.779729729729729\\
0.160545560409361	0.779054054054053\\
0.16077937232805	0.778378378378377\\
0.160789613674802	0.777702702702701\\
0.161587378198488	0.777027027027026\\
0.161670151332396	0.77635135135135\\
0.161694926669321	0.775675675675675\\
0.161725716152681	0.774999999999999\\
0.161797861775647	0.774324324324323\\
0.162499970349807	0.773648648648647\\
0.162532320005684	0.772972972972972\\
0.162956106306664	0.772297297297296\\
0.16361121131492	0.771621621621621\\
0.164191410431617	0.770945945945945\\
0.164734189490038	0.770270270270269\\
0.164881158396262	0.769594594594593\\
0.165094294822392	0.768918918918918\\
0.16536181381407	0.768243243243242\\
0.165853704486773	0.767567567567566\\
0.166565939851913	0.76689189189189\\
0.166795766209444	0.766216216216215\\
0.166881371945651	0.765540540540539\\
0.166942850802492	0.764864864864864\\
0.167088075432187	0.764189189189188\\
0.167245104663262	0.763513513513512\\
0.167548631978234	0.762837837837837\\
0.16781446044305	0.762162162162161\\
0.16782526361713	0.761486486486485\\
0.16826631078918	0.76081081081081\\
0.168321399695659	0.760135135135134\\
0.168520103879235	0.759459459459458\\
0.168525716409161	0.758783783783783\\
0.168814001875996	0.758108108108107\\
0.168955996412881	0.757432432432431\\
0.169341817381253	0.756756756756755\\
0.169809028194295	0.75608108108108\\
0.170253704219477	0.755405405405404\\
0.170277275943777	0.754729729729728\\
0.170369316508251	0.754054054054053\\
0.170405986252185	0.753378378378377\\
0.170430428975588	0.752702702702701\\
0.17059150577837	0.752027027027026\\
0.171262647901736	0.75135135135135\\
0.171473290508341	0.750675675675674\\
0.171506000266284	0.749999999999999\\
0.171680933656898	0.749324324324323\\
0.17195245634632	0.748648648648647\\
0.172329262196126	0.747972972972972\\
0.172618051895413	0.747297297297296\\
0.17302135091795	0.74662162162162\\
0.173091396526002	0.745945945945944\\
0.173143752698529	0.745270270270269\\
0.173348569868658	0.744594594594593\\
0.173439227143976	0.743918918918917\\
0.173986028720412	0.743243243243242\\
0.174127203834071	0.742567567567566\\
0.174219527967474	0.741891891891891\\
0.174323120602711	0.741216216216215\\
0.174403765625948	0.740540540540539\\
0.174491293161876	0.739864864864864\\
0.174749728450061	0.739189189189188\\
0.174797274649871	0.738513513513512\\
0.174984723186719	0.737837837837837\\
0.174988544978199	0.737162162162161\\
0.17500756557638	0.736486486486485\\
0.175023467299426	0.735810810810809\\
0.175216106548255	0.735135135135134\\
0.175228575522245	0.734459459459458\\
0.175334598759572	0.733783783783782\\
0.175389734478617	0.733108108108107\\
0.175520415019844	0.732432432432431\\
0.175687639205071	0.731756756756755\\
0.175823864426558	0.73108108108108\\
0.176278808849018	0.730405405405404\\
0.176292231540442	0.729729729729728\\
0.176487409309161	0.729054054054053\\
0.176742310677091	0.728378378378377\\
0.17695787251152	0.727702702702701\\
0.177067672493548	0.727027027027025\\
0.177106736277229	0.72635135135135\\
0.178041986410831	0.725675675675674\\
0.178347196092497	0.724999999999999\\
0.178882375819302	0.724324324324323\\
0.178915539214385	0.723648648648647\\
0.179002760725727	0.722972972972972\\
0.179343456542202	0.722297297297296\\
0.179865354516782	0.72162162162162\\
0.179968451094141	0.720945945945945\\
0.180122753710403	0.720270270270269\\
0.180210418410961	0.719594594594593\\
0.180210705681656	0.718918918918917\\
0.180434899739105	0.718243243243242\\
0.180787847093745	0.717567567567566\\
0.181097232102136	0.716891891891891\\
0.181244355303871	0.716216216216215\\
0.181675891715098	0.715540540540539\\
0.181908102150739	0.714864864864863\\
0.182099683260723	0.714189189189188\\
0.182236311151586	0.713513513513512\\
0.182389805112978	0.712837837837836\\
0.182565365361712	0.712162162162161\\
0.182984820734246	0.711486486486485\\
0.182987265917983	0.710810810810809\\
0.183193846337557	0.710135135135133\\
0.18347208625365	0.709459459459458\\
0.183821157659298	0.708783783783782\\
0.184428650573259	0.708108108108107\\
0.185021503649193	0.707432432432431\\
0.185147594981253	0.706756756756755\\
0.185211301579472	0.706081081081079\\
0.185800036223885	0.705405405405404\\
0.185934560598994	0.704729729729728\\
0.186060411892337	0.704054054054052\\
0.186261665037914	0.703378378378377\\
0.186995643924266	0.702702702702701\\
0.18722642568815	0.702027027027025\\
0.187376683820123	0.70135135135135\\
0.187397059126017	0.700675675675674\\
0.187441634657606	0.699999999999998\\
0.187493434598197	0.699324324324322\\
0.187498084685703	0.698648648648647\\
0.187581846731742	0.697972972972971\\
0.187627736537085	0.697297297297295\\
0.187850497993	0.69662162162162\\
0.187886340858069	0.695945945945944\\
0.187940565885557	0.695270270270268\\
0.18797586606224	0.694594594594592\\
0.188539058421867	0.693918918918917\\
0.188643430081407	0.693243243243241\\
0.188894429397397	0.692567567567565\\
0.189018665908455	0.69189189189189\\
0.189079993422679	0.691216216216214\\
0.189152238546332	0.690540540540538\\
0.189153002112139	0.689864864864863\\
0.18932449663917	0.689189189189187\\
0.189593450328649	0.688513513513511\\
0.18980888705445	0.687837837837835\\
0.189884662324185	0.68716216216216\\
0.190001988560759	0.686486486486484\\
0.19008231748998	0.685810810810809\\
0.190329636586156	0.685135135135133\\
0.190511177432948	0.684459459459457\\
0.191196945314046	0.683783783783781\\
0.191284471961446	0.683108108108106\\
0.191345878761681	0.68243243243243\\
0.191433658723038	0.681756756756754\\
0.191437563826354	0.681081081081079\\
0.191504145305967	0.680405405405403\\
0.191540426475457	0.679729729729727\\
0.191669491295413	0.679054054054052\\
0.191750708394691	0.678378378378376\\
0.191836384151467	0.6777027027027\\
0.191944857881114	0.677027027027025\\
0.191969492553784	0.676351351351349\\
0.192069857067565	0.675675675675673\\
0.192384213596249	0.674999999999997\\
0.192444354829366	0.674324324324322\\
0.192457677875749	0.673648648648646\\
0.192538552981039	0.672972972972971\\
0.192627836207199	0.672297297297295\\
0.193478438395621	0.671621621621619\\
0.193520247985328	0.670945945945943\\
0.193534585133605	0.670270270270268\\
0.193717466650586	0.669594594594592\\
0.193882132093479	0.668918918918917\\
0.19409429670602	0.668243243243241\\
0.194101895271204	0.667567567567565\\
0.194556429376476	0.666891891891889\\
0.194876912419413	0.666216216216214\\
0.194942320508422	0.665540540540538\\
0.195304657026476	0.664864864864863\\
0.195787610477601	0.664189189189187\\
0.195835400524377	0.663513513513511\\
0.195897329587687	0.662837837837836\\
0.195914843193146	0.66216216216216\\
0.195945548712862	0.661486486486484\\
0.19595680929684	0.660810810810808\\
0.19628275097494	0.660135135135133\\
0.196554346191968	0.659459459459457\\
0.196857722935951	0.658783783783781\\
0.196928893432519	0.658108108108106\\
0.197100867932923	0.65743243243243\\
0.197375099705196	0.656756756756754\\
0.197483435949423	0.656081081081079\\
0.197522160168743	0.655405405405403\\
0.197933585132222	0.654729729729727\\
0.197947658521837	0.654054054054052\\
0.198139767147898	0.653378378378376\\
0.198260819297945	0.6527027027027\\
0.19828800962503	0.652027027027025\\
0.198329709071274	0.651351351351349\\
0.198336960063052	0.650675675675673\\
0.198420635696538	0.649999999999997\\
0.198501972962652	0.649324324324322\\
0.198985072205191	0.648648648648646\\
0.198994592461195	0.64797297297297\\
0.199055284308594	0.647297297297295\\
0.199097060663062	0.646621621621619\\
0.19948138855268	0.645945945945943\\
0.199757083474193	0.645270270270268\\
0.199936026422416	0.644594594594592\\
0.200124985588429	0.643918918918917\\
0.20031030113523	0.643243243243241\\
0.200691267213754	0.642567567567565\\
0.200700692766413	0.641891891891889\\
0.20093544728196	0.641216216216214\\
0.201391594911994	0.640540540540538\\
0.201549667104182	0.639864864864862\\
0.201636003558056	0.639189189189187\\
0.202132780934428	0.638513513513511\\
0.202133275176152	0.637837837837835\\
0.202647200007912	0.637162162162159\\
0.202662818969867	0.636486486486484\\
0.20285352094708	0.635810810810808\\
0.203036599070325	0.635135135135133\\
0.203057094213091	0.634459459459457\\
0.203223068688172	0.633783783783781\\
0.203340861709914	0.633108108108105\\
0.203944762852694	0.63243243243243\\
0.204117573055632	0.631756756756754\\
0.204462484700903	0.631081081081078\\
0.20454050692217	0.630405405405403\\
0.204777811101303	0.629729729729727\\
0.204905179047916	0.629054054054051\\
0.204907277845578	0.628378378378376\\
0.205074231917438	0.6277027027027\\
0.205622005180018	0.627027027027024\\
0.206084063379228	0.626351351351349\\
0.206132792179025	0.625675675675673\\
0.206198314394804	0.624999999999997\\
0.206469896725162	0.624324324324322\\
0.206513624016937	0.623648648648646\\
0.20667657998021	0.62297297297297\\
0.206845878464813	0.622297297297295\\
0.207016833441429	0.621621621621619\\
0.207107004264869	0.620945945945943\\
0.207288890769052	0.620270270270268\\
0.207339128364397	0.619594594594592\\
0.207544804793055	0.618918918918916\\
0.207560896896986	0.618243243243241\\
0.207682937321953	0.617567567567565\\
0.207688062022625	0.616891891891889\\
0.207769631206719	0.616216216216214\\
0.208029097454103	0.615540540540538\\
0.208059639177034	0.614864864864862\\
0.208098556301008	0.614189189189187\\
0.208263805965897	0.613513513513511\\
0.208372114648719	0.612837837837835\\
0.208710383825564	0.61216216216216\\
0.209157883627392	0.611486486486484\\
0.209243447091847	0.610810810810808\\
0.209436474690813	0.610135135135133\\
0.209644618621669	0.609459459459457\\
0.209655796211696	0.608783783783781\\
0.210103472945102	0.608108108108106\\
0.210802011139582	0.60743243243243\\
0.211375629063892	0.606756756756754\\
0.21150331406494	0.606081081081079\\
0.211630334760132	0.605405405405403\\
0.211989789019447	0.604729729729727\\
0.212138729968344	0.604054054054052\\
0.212542123785914	0.603378378378376\\
0.212709011739415	0.6027027027027\\
0.212919190378894	0.602027027027025\\
0.213095399336674	0.601351351351349\\
0.21376176610332	0.600675675675673\\
0.213931144548426	0.599999999999998\\
0.213966124393441	0.599324324324322\\
0.214038588929324	0.598648648648646\\
0.214374534324655	0.597972972972971\\
0.214418966940509	0.597297297297295\\
0.214563999859821	0.596621621621619\\
0.214747331675239	0.595945945945944\\
0.214758215121415	0.595270270270268\\
0.2149415025624	0.594594594594592\\
0.215289519776059	0.593918918918917\\
0.21542355160456	0.593243243243241\\
0.215553594838349	0.592567567567565\\
0.215603959799379	0.59189189189189\\
0.215865612813207	0.591216216216214\\
0.216046821264315	0.590540540540538\\
0.216199769396175	0.589864864864862\\
0.216393007327945	0.589189189189187\\
0.216441190543163	0.588513513513511\\
0.216729767244939	0.587837837837835\\
0.216885488882401	0.58716216216216\\
0.217026710869826	0.586486486486484\\
0.217296046918207	0.585810810810809\\
0.217358203320092	0.585135135135133\\
0.217951947796532	0.584459459459457\\
0.218549807398177	0.583783783783781\\
0.219015666729702	0.583108108108106\\
0.219116899495915	0.58243243243243\\
0.219188636432981	0.581756756756755\\
0.219365082980983	0.581081081081079\\
0.219417452920954	0.580405405405403\\
0.219628949085411	0.579729729729727\\
0.219959971771147	0.579054054054052\\
0.220215973304486	0.578378378378376\\
0.220477836002991	0.5777027027027\\
0.220658773336574	0.577027027027025\\
0.220819513814148	0.576351351351349\\
0.220832027649698	0.575675675675673\\
0.220999166435721	0.574999999999998\\
0.221247000369692	0.574324324324322\\
0.221817082885616	0.573648648648646\\
0.222089805362233	0.572972972972971\\
0.222573834511044	0.572297297297295\\
0.223521785361878	0.571621621621619\\
0.223640536689807	0.570945945945944\\
0.223718915145664	0.570270270270268\\
0.223950172700304	0.569594594594592\\
0.224004343487858	0.568918918918917\\
0.224333037223969	0.568243243243241\\
0.224519228130821	0.567567567567565\\
0.224659630260845	0.56689189189189\\
0.224670825227596	0.566216216216214\\
0.225012197258671	0.565540540540538\\
0.225387474784839	0.564864864864863\\
0.225488853240317	0.564189189189187\\
0.225654524731917	0.563513513513511\\
0.225713145548243	0.562837837837835\\
0.225765050510544	0.56216216216216\\
0.2259146728897	0.561486486486484\\
0.226132994209697	0.560810810810808\\
0.226651869271044	0.560135135135133\\
0.226676331558519	0.559459459459457\\
0.226879090279858	0.558783783783781\\
0.227006861366315	0.558108108108106\\
0.227124646371687	0.55743243243243\\
0.227224062479834	0.556756756756754\\
0.227550293095023	0.556081081081079\\
0.227593819965884	0.555405405405403\\
0.227698511240958	0.554729729729727\\
0.228356042384892	0.554054054054052\\
0.228357857528026	0.553378378378376\\
0.228430190793863	0.5527027027027\\
0.228796733881155	0.552027027027024\\
0.229101937067095	0.551351351351349\\
0.229663001599764	0.550675675675673\\
0.229668327860297	0.549999999999997\\
0.229768448124447	0.549324324324322\\
0.230203492319754	0.548648648648646\\
0.230390364294699	0.54797297297297\\
0.231180249165799	0.547297297297295\\
0.231817536510162	0.546621621621619\\
0.232471560598394	0.545945945945943\\
0.232637841431641	0.545270270270268\\
0.232673077093379	0.544594594594592\\
0.232796953701123	0.543918918918916\\
0.232894665121682	0.543243243243241\\
0.233764124386408	0.542567567567565\\
0.233938163204206	0.541891891891889\\
0.233973505061378	0.541216216216214\\
0.2340207918863	0.540540540540538\\
0.234076964030372	0.539864864864862\\
0.234265881196988	0.539189189189186\\
0.234801558301207	0.538513513513511\\
0.235023517675123	0.537837837837835\\
0.235469865735992	0.53716216216216\\
0.235506288579974	0.536486486486484\\
0.235839491228036	0.535810810810808\\
0.235885955370323	0.535135135135132\\
0.236010983267088	0.534459459459457\\
0.236054862553613	0.533783783783781\\
0.236084192205585	0.533108108108105\\
0.236806881233591	0.53243243243243\\
0.236882420508026	0.531756756756754\\
0.237208352126408	0.531081081081078\\
0.237232728412173	0.530405405405402\\
0.237375701595581	0.529729729729727\\
0.237383192225469	0.529054054054051\\
0.237415727038922	0.528378378378375\\
0.238046106323265	0.5277027027027\\
0.238213140210212	0.527027027027024\\
0.238247732985204	0.526351351351348\\
0.238435434131354	0.525675675675673\\
0.238744980817916	0.524999999999997\\
0.238980064285515	0.524324324324321\\
0.239035747399368	0.523648648648646\\
0.239473770776351	0.52297297297297\\
0.240666608118146	0.522297297297294\\
0.240706776430806	0.521621621621618\\
0.240759879080807	0.520945945945943\\
0.241025140795001	0.520270270270267\\
0.241153612231722	0.519594594594591\\
0.24135083782428	0.518918918918916\\
0.241394521269542	0.51824324324324\\
0.241835844394978	0.517567567567564\\
0.241951249367659	0.516891891891889\\
0.24223098597959	0.516216216216213\\
0.242257607095326	0.515540540540537\\
0.242338297835761	0.514864864864862\\
0.242462751150166	0.514189189189186\\
0.242530752240515	0.51351351351351\\
0.242888834010177	0.512837837837835\\
0.242893460165926	0.512162162162159\\
0.243089540928518	0.511486486486483\\
0.243266378314251	0.510810810810808\\
0.243533162395898	0.510135135135132\\
0.243896364808522	0.509459459459456\\
0.244351383363094	0.508783783783781\\
0.244579693104878	0.508108108108105\\
0.244655244077694	0.507432432432429\\
0.244791680070094	0.506756756756754\\
0.244906661246048	0.506081081081078\\
0.244942708470138	0.505405405405402\\
0.244946911864377	0.504729729729727\\
0.245342249314303	0.504054054054051\\
0.245547425873581	0.503378378378375\\
0.245838534029787	0.5027027027027\\
0.245955389470726	0.502027027027024\\
0.246096976090437	0.501351351351348\\
0.246129496782384	0.500675675675673\\
0.246431807526517	0.499999999999997\\
0.246609823407039	0.499324324324321\\
0.24661799385352	0.498648648648646\\
0.246665872624103	0.49797297297297\\
0.246873748584901	0.497297297297294\\
0.247170494626931	0.496621621621619\\
0.247701540353353	0.495945945945943\\
0.247982385877998	0.495270270270267\\
0.248081101327685	0.494594594594592\\
0.248434920992481	0.493918918918916\\
0.249162633964907	0.49324324324324\\
0.249249083455138	0.492567567567565\\
0.249282085222289	0.491891891891889\\
0.249310561204949	0.491216216216213\\
0.249472418777684	0.490540540540538\\
0.24952242633621	0.489864864864862\\
0.249640571032263	0.489189189189186\\
0.249762929893909	0.488513513513511\\
0.249842577934952	0.487837837837835\\
0.250055279818644	0.487162162162159\\
0.250988027315358	0.486486486486484\\
0.251010582034329	0.485810810810808\\
0.251069866907731	0.485135135135132\\
0.251253674270569	0.484459459459457\\
0.252062077956202	0.483783783783781\\
0.252259307998594	0.483108108108105\\
0.252495363711238	0.48243243243243\\
0.252549029128367	0.481756756756754\\
0.252910834152983	0.481081081081078\\
0.252990075045745	0.480405405405403\\
0.253008506216589	0.479729729729727\\
0.25307178331691	0.479054054054051\\
0.25315884570477	0.478378378378375\\
0.253220996879387	0.4777027027027\\
0.253349403652062	0.477027027027024\\
0.253811313313341	0.476351351351349\\
0.254858938056705	0.475675675675673\\
0.255112488794388	0.474999999999997\\
0.255281992621639	0.474324324324322\\
0.255477620261117	0.473648648648646\\
0.255668075303474	0.47297297297297\\
0.255764346969336	0.472297297297295\\
0.255912496444508	0.471621621621619\\
0.256506897807184	0.470945945945943\\
0.256644449691422	0.470270270270267\\
0.257526116322109	0.469594594594592\\
0.257669179573996	0.468918918918916\\
0.25793702547448	0.468243243243241\\
0.258292529766163	0.467567567567565\\
0.25840498039872	0.466891891891889\\
0.258513405838425	0.466216216216214\\
0.25883220436146	0.465540540540538\\
0.25897725289981	0.464864864864862\\
0.259597008511154	0.464189189189187\\
0.259855408555803	0.463513513513511\\
0.259979153813662	0.462837837837835\\
0.260150694578488	0.462162162162159\\
0.260273775117022	0.461486486486484\\
0.261010254712507	0.460810810810808\\
0.26127947452601	0.460135135135132\\
0.2622394747657	0.459459459459457\\
0.262279108808739	0.458783783783781\\
0.262480563337206	0.458108108108106\\
0.262580334228954	0.45743243243243\\
0.263002339970322	0.456756756756754\\
0.263072773131066	0.456081081081078\\
0.263412848306868	0.455405405405403\\
0.263415893500449	0.454729729729727\\
0.263709458357461	0.454054054054051\\
0.263818815614867	0.453378378378376\\
0.264667221592862	0.4527027027027\\
0.264697673957362	0.452027027027024\\
0.264723749746684	0.451351351351349\\
0.265082671782272	0.450675675675673\\
0.265548468513812	0.449999999999998\\
0.265656469110676	0.449324324324322\\
0.265728581105478	0.448648648648646\\
0.265903449896222	0.44797297297297\\
0.265925107788601	0.447297297297295\\
0.265976176150743	0.446621621621619\\
0.26655118978637	0.445945945945943\\
0.267142520391788	0.445270270270268\\
0.267340648576722	0.444594594594592\\
0.26738953970155	0.443918918918916\\
0.267652870442477	0.443243243243241\\
0.268077132420651	0.442567567567565\\
0.268143360368637	0.441891891891889\\
0.268223189834384	0.441216216216214\\
0.26957194936745	0.440540540540538\\
0.269700159123601	0.439864864864862\\
0.269717168265382	0.439189189189187\\
0.270444854427098	0.438513513513511\\
0.270494594638513	0.437837837837835\\
0.2707802359671	0.43716216216216\\
0.270798240352992	0.436486486486484\\
0.270983702418938	0.435810810810808\\
0.271126876102623	0.435135135135133\\
0.271423828240437	0.434459459459457\\
0.271623892559929	0.433783783783781\\
0.272011695620171	0.433108108108106\\
0.272139317606424	0.43243243243243\\
0.272717254568416	0.431756756756754\\
0.272753783972413	0.431081081081079\\
0.273027109610529	0.430405405405403\\
0.273809430878518	0.429729729729727\\
0.273873761825389	0.429054054054052\\
0.274153178946342	0.428378378378376\\
0.274985450242008	0.4277027027027\\
0.275080474728629	0.427027027027025\\
0.275208874509485	0.426351351351349\\
0.27532020217951	0.425675675675673\\
0.275355540209451	0.424999999999998\\
0.27555521776973	0.424324324324322\\
0.275775409423951	0.423648648648646\\
0.275880331711876	0.422972972972971\\
0.276101574345651	0.422297297297295\\
0.276318078902787	0.421621621621619\\
0.276367412923838	0.420945945945944\\
0.277413766419516	0.420270270270268\\
0.277811239671112	0.419594594594592\\
0.277822851231238	0.418918918918917\\
0.277872404905383	0.418243243243241\\
0.278021562655157	0.417567567567565\\
0.278083021471803	0.41689189189189\\
0.278098595527242	0.416216216216214\\
0.278489653926156	0.415540540540538\\
0.278511493113335	0.414864864864863\\
0.278710409602637	0.414189189189187\\
0.278880384309682	0.413513513513511\\
0.279145173199514	0.412837837837836\\
0.279396305823412	0.41216216216216\\
0.280049006180677	0.411486486486484\\
0.280809971559743	0.410810810810809\\
0.280883429956369	0.410135135135133\\
0.281007645503175	0.409459459459457\\
0.28105405164837	0.408783783783782\\
0.281306590213524	0.408108108108106\\
0.281355779980686	0.40743243243243\\
0.2815900039557	0.406756756756755\\
0.281708024357171	0.406081081081079\\
0.281828812269804	0.405405405405403\\
0.282551050372366	0.404729729729728\\
0.282866389528546	0.404054054054052\\
0.283043591436254	0.403378378378376\\
0.28342118706037	0.402702702702701\\
0.283490189883691	0.402027027027025\\
0.283742067508989	0.401351351351349\\
0.284154892807898	0.400675675675674\\
0.284275048035408	0.399999999999998\\
0.284481516517808	0.399324324324322\\
0.284567918947504	0.398648648648647\\
0.2850048782974	0.397972972972971\\
0.285230264257326	0.397297297297295\\
0.285650210282068	0.39662162162162\\
0.285985957909952	0.395945945945944\\
0.286630273963993	0.395270270270268\\
0.287014649342055	0.394594594594593\\
0.287048575983433	0.393918918918917\\
0.287529460729725	0.393243243243241\\
0.287768265472602	0.392567567567566\\
0.287847629655358	0.39189189189189\\
0.288899584735411	0.391216216216214\\
0.289342083082798	0.390540540540539\\
0.28937192030742	0.389864864864863\\
0.28938720047285	0.389189189189187\\
0.289540242682281	0.388513513513512\\
0.289843206927185	0.387837837837836\\
0.290541099555236	0.38716216216216\\
0.29065807781967	0.386486486486485\\
0.291200627396083	0.385810810810809\\
0.291358905286108	0.385135135135133\\
0.291571173634243	0.384459459459458\\
0.292180539916654	0.383783783783782\\
0.292227683222479	0.383108108108106\\
0.292405019329182	0.382432432432431\\
0.29271228160048	0.381756756756755\\
0.29307216589531	0.381081081081079\\
0.293189225213033	0.380405405405404\\
0.293197180032608	0.379729729729728\\
0.293341575006915	0.379054054054052\\
0.294186567346389	0.378378378378377\\
0.294310121703285	0.377702702702701\\
0.29436948387567	0.377027027027025\\
0.29444988135847	0.37635135135135\\
0.294726708458856	0.375675675675674\\
0.294736377502053	0.374999999999998\\
0.295573296360613	0.374324324324323\\
0.295613659986981	0.373648648648647\\
0.295968028002388	0.372972972972971\\
0.295991281770496	0.372297297297296\\
0.296138523051847	0.37162162162162\\
0.296406312149217	0.370945945945944\\
0.296759060329372	0.370270270270268\\
0.296938968651556	0.369594594594593\\
0.297283528007071	0.368918918918917\\
0.297436353818079	0.368243243243242\\
0.29763555855342	0.367567567567566\\
0.297687581898078	0.36689189189189\\
0.297911506245516	0.366216216216215\\
0.298212101471226	0.365540540540539\\
0.298653813660496	0.364864864864863\\
0.298817674345827	0.364189189189188\\
0.299250775787152	0.363513513513512\\
0.299286210513094	0.362837837837836\\
0.299341537262317	0.36216216216216\\
0.299667764644481	0.361486486486485\\
0.29983619609793	0.360810810810809\\
0.299836848751273	0.360135135135134\\
0.301029146233048	0.359459459459458\\
0.301090732848387	0.358783783783782\\
0.30112797557724	0.358108108108107\\
0.302187801832988	0.357432432432431\\
0.302210918039236	0.356756756756755\\
0.3022168475619	0.356081081081079\\
0.303311307553424	0.355405405405404\\
0.303424093955738	0.354729729729728\\
0.30418337053905	0.354054054054052\\
0.304571188725673	0.353378378378377\\
0.304801572536299	0.352702702702701\\
0.305489393716003	0.352027027027025\\
0.305538568553337	0.35135135135135\\
0.306057440634321	0.350675675675674\\
0.306278741620239	0.349999999999999\\
0.306577281827662	0.349324324324323\\
0.306713076190134	0.348648648648647\\
0.306867091940152	0.347972972972971\\
0.307011168892248	0.347297297297296\\
0.30757994485993	0.34662162162162\\
0.307901745304752	0.345945945945944\\
0.309642712784971	0.345270270270269\\
0.310405346018535	0.344594594594593\\
0.31145562331502	0.343918918918917\\
0.311536671580461	0.343243243243242\\
0.312199036836506	0.342567567567566\\
0.312242541004858	0.341891891891891\\
0.312928584166882	0.341216216216215\\
0.313531121263458	0.340540540540539\\
0.314111761659182	0.339864864864863\\
0.314244302125475	0.339189189189188\\
0.314700109535946	0.338513513513512\\
0.314787193812197	0.337837837837836\\
0.31508301560445	0.337162162162161\\
0.315110855489432	0.336486486486485\\
0.315598248480573	0.335810810810809\\
0.315734290200861	0.335135135135134\\
0.316002025121255	0.334459459459458\\
0.316240706398773	0.333783783783782\\
0.316541446812232	0.333108108108107\\
0.31674956924562	0.332432432432431\\
0.316895648682109	0.331756756756755\\
0.317041831990383	0.33108108108108\\
0.31713120134241	0.330405405405404\\
0.31780535875643	0.329729729729728\\
0.318371653692285	0.329054054054053\\
0.319016690398174	0.328378378378377\\
0.319037181274395	0.327702702702701\\
0.319123403111341	0.327027027027026\\
0.320060784519564	0.32635135135135\\
0.32014036831782	0.325675675675674\\
0.320390771726306	0.324999999999999\\
0.320928041619566	0.324324324324323\\
0.321341688144565	0.323648648648647\\
0.321524205383346	0.322972972972972\\
0.321753533367544	0.322297297297296\\
0.322656043638681	0.32162162162162\\
0.323123866545357	0.320945945945945\\
0.323844567609565	0.320270270270269\\
0.323941222366244	0.319594594594593\\
0.324004033703293	0.318918918918918\\
0.324038948108653	0.318243243243242\\
0.324260619859601	0.317567567567566\\
0.324351559241268	0.316891891891891\\
0.324722757733521	0.316216216216215\\
0.32479573907341	0.315540540540539\\
0.324925825077977	0.314864864864864\\
0.325365593191844	0.314189189189188\\
0.325840996490598	0.313513513513512\\
0.326009971998653	0.312837837837837\\
0.326598703268216	0.312162162162161\\
0.326645479397842	0.311486486486485\\
0.327136647398732	0.31081081081081\\
0.327732205595353	0.310135135135134\\
0.328222443024228	0.309459459459458\\
0.329348011402933	0.308783783783783\\
0.329429596175823	0.308108108108107\\
0.329514383594774	0.307432432432431\\
0.330045662076216	0.306756756756756\\
0.330548819169607	0.30608108108108\\
0.330698270910739	0.305405405405404\\
0.330902841011038	0.304729729729729\\
0.331368144052283	0.304054054054053\\
0.331696701682034	0.303378378378377\\
0.332180258701071	0.302702702702702\\
0.334258973565954	0.302027027027026\\
0.33466655834032	0.30135135135135\\
0.33481481868498	0.300675675675675\\
0.335434644329691	0.299999999999999\\
0.3355140842148	0.299324324324323\\
0.335932008562629	0.298648648648648\\
0.335934232039578	0.297972972972972\\
0.336126438698923	0.297297297297296\\
0.336713076700947	0.296621621621621\\
0.336905325092109	0.295945945945945\\
0.337271293874785	0.295270270270269\\
0.337294400569548	0.294594594594594\\
0.337436852260052	0.293918918918918\\
0.337737132499959	0.293243243243242\\
0.337920520151703	0.292567567567567\\
0.338004546768476	0.291891891891891\\
0.338420434479256	0.291216216216215\\
0.338450512702521	0.29054054054054\\
0.338887272169202	0.289864864864864\\
0.338968514968031	0.289189189189188\\
0.339931591700613	0.288513513513513\\
0.340816923142806	0.287837837837837\\
0.340964170374244	0.287162162162161\\
0.341120248214922	0.286486486486486\\
0.341178278980603	0.28581081081081\\
0.341203041649412	0.285135135135134\\
0.341234589399033	0.284459459459459\\
0.341292100630132	0.283783783783783\\
0.34189009421992	0.283108108108107\\
0.342309312849742	0.282432432432432\\
0.34275103311225	0.281756756756756\\
0.343231712841341	0.28108108108108\\
0.343754523597819	0.280405405405405\\
0.344075610822076	0.279729729729729\\
0.34437351779061	0.279054054054053\\
0.34450733227637	0.278378378378378\\
0.344823993658341	0.277702702702702\\
0.344950646582412	0.277027027027026\\
0.345073212596571	0.276351351351351\\
0.345396585264031	0.275675675675675\\
0.346624754140664	0.274999999999999\\
0.346803209967706	0.274324324324324\\
0.347358150783503	0.273648648648648\\
0.347703820986709	0.272972972972972\\
0.347911316000047	0.272297297297297\\
0.348249403886197	0.271621621621621\\
0.348673869131491	0.270945945945945\\
0.348904775537066	0.27027027027027\\
0.349748457847128	0.269594594594594\\
0.350361006748914	0.268918918918918\\
0.350538001522576	0.268243243243243\\
0.351217880725356	0.267567567567567\\
0.351527326911926	0.266891891891891\\
0.351781076705727	0.266216216216216\\
0.352112573086664	0.26554054054054\\
0.352227005619	0.264864864864864\\
0.352415763222002	0.264189189189189\\
0.352744799516002	0.263513513513513\\
0.352819794406571	0.262837837837837\\
0.353166227387884	0.262162162162161\\
0.353497728475792	0.261486486486486\\
0.353551405969876	0.26081081081081\\
0.353648000004822	0.260135135135135\\
0.355214054977854	0.259459459459459\\
0.355408258737675	0.258783783783783\\
0.355801742616973	0.258108108108108\\
0.356133880135101	0.257432432432432\\
0.356160363747285	0.256756756756756\\
0.356200797074779	0.256081081081081\\
0.356918949494502	0.255405405405405\\
0.358308508520551	0.254729729729729\\
0.35954113320716	0.254054054054053\\
0.360060425111412	0.253378378378378\\
0.360695808700267	0.252702702702702\\
0.361079966735815	0.252027027027027\\
0.361400092335176	0.251351351351351\\
0.361517873639179	0.250675675675675\\
0.362960723112451	0.249999999999999\\
0.363254860141901	0.249324324324324\\
0.365214791127095	0.248648648648648\\
0.365696861416759	0.247972972972972\\
0.366301541497985	0.247297297297297\\
0.367960173773217	0.246621621621621\\
0.368467950505108	0.245945945945945\\
0.368851371009732	0.24527027027027\\
0.368987699585928	0.244594594594594\\
0.369259529905085	0.243918918918918\\
0.369566979619125	0.243243243243243\\
0.369701070293766	0.242567567567567\\
0.369758854655694	0.241891891891891\\
0.370081099203378	0.241216216216216\\
0.370153556132824	0.24054054054054\\
0.37145744562977	0.239864864864864\\
0.372590887536966	0.239189189189189\\
0.372775723448404	0.238513513513513\\
0.372951430561962	0.237837837837837\\
0.373093313586612	0.237162162162162\\
0.374629021866903	0.236486486486486\\
0.374929539863017	0.23581081081081\\
0.375347294120607	0.235135135135135\\
0.375586580556162	0.234459459459459\\
0.375968907394127	0.233783783783783\\
0.376788543136916	0.233108108108108\\
0.377040211400758	0.232432432432432\\
0.377072559261486	0.231756756756756\\
0.377111694524973	0.231081081081081\\
0.377579901682259	0.230405405405405\\
0.378020225564597	0.229729729729729\\
0.378538365875481	0.229054054054054\\
0.379338979121279	0.228378378378378\\
0.379663620978206	0.227702702702702\\
0.381411389779368	0.227027027027027\\
0.381657576679024	0.226351351351351\\
0.383511604428231	0.225675675675675\\
0.383865397193455	0.225\\
0.385035409067977	0.224324324324324\\
0.385919707631364	0.223648648648648\\
0.386720306959711	0.222972972972973\\
0.387745127858555	0.222297297297297\\
0.388264347308381	0.221621621621621\\
0.389335022657023	0.220945945945946\\
0.389650762448087	0.22027027027027\\
0.389789596523186	0.219594594594594\\
0.390520471029551	0.218918918918918\\
0.390984200482047	0.218243243243243\\
0.391070132814995	0.217567567567567\\
0.392697071665965	0.216891891891892\\
0.392879506957682	0.216216216216216\\
0.393244789735291	0.21554054054054\\
0.393675764105572	0.214864864864864\\
0.394423452159221	0.214189189189189\\
0.39447502562434	0.213513513513513\\
0.395017707139012	0.212837837837837\\
0.397132034522209	0.212162162162162\\
0.397922160359281	0.211486486486486\\
0.399429680287835	0.21081081081081\\
0.400298568426101	0.210135135135135\\
0.400360811048487	0.209459459459459\\
0.400434005695453	0.208783783783783\\
0.400583970461425	0.208108108108108\\
0.402000474618622	0.207432432432432\\
0.402463587944713	0.206756756756756\\
0.402598721243765	0.206081081081081\\
0.402847057782718	0.205405405405405\\
0.402908251507338	0.204729729729729\\
0.403079251988322	0.204054054054054\\
0.403696054870037	0.203378378378378\\
0.405310587356359	0.202702702702702\\
0.405928953865756	0.202027027027027\\
0.407635704123426	0.201351351351351\\
0.408884457541921	0.200675675675675\\
0.408889919097641	0.2\\
0.408915778713412	0.199324324324324\\
0.409256201829175	0.198648648648648\\
0.410459344616961	0.197972972972973\\
0.410672445635011	0.197297297297297\\
0.411214519776089	0.196621621621621\\
0.411292111822804	0.195945945945946\\
0.411784481482811	0.19527027027027\\
0.413100514507545	0.194594594594594\\
0.413552975404789	0.193918918918919\\
0.41496423078757	0.193243243243243\\
0.415975721258554	0.192567567567567\\
0.416370577056888	0.191891891891892\\
0.417537057224046	0.191216216216216\\
0.417810260609653	0.19054054054054\\
0.418763918214055	0.189864864864865\\
0.419031381492559	0.189189189189189\\
0.420246311357293	0.188513513513513\\
0.420368275661342	0.187837837837838\\
0.420581394032654	0.187162162162162\\
0.420900743704793	0.186486486486486\\
0.422612224993661	0.185810810810811\\
0.423638441027758	0.185135135135135\\
0.423638934637582	0.184459459459459\\
0.423966180032191	0.183783783783783\\
0.424302806406677	0.183108108108108\\
0.424740254828342	0.182432432432432\\
0.425068369786979	0.181756756756757\\
0.428348366129381	0.181081081081081\\
0.428558379214078	0.180405405405405\\
0.428606889542514	0.179729729729729\\
0.429222209151918	0.179054054054054\\
0.429273741685417	0.178378378378378\\
0.430377501642227	0.177702702702702\\
0.430592628593773	0.177027027027027\\
0.434474684241243	0.176351351351351\\
0.434569520028325	0.175675675675675\\
0.434771194177595	0.175\\
0.435267517310763	0.174324324324324\\
0.435355509577654	0.173648648648648\\
0.436728772031346	0.172972972972973\\
0.437821993658754	0.172297297297297\\
0.438089551631539	0.171621621621621\\
0.438616364773489	0.170945945945946\\
0.438791275744228	0.17027027027027\\
0.440690406299755	0.169594594594594\\
0.442352656823581	0.168918918918919\\
0.442780704511318	0.168243243243243\\
0.444909831255652	0.167567567567567\\
0.445488480441832	0.166891891891892\\
0.445914760011393	0.166216216216216\\
0.446318778487065	0.16554054054054\\
0.446685813175742	0.164864864864865\\
0.447468369956368	0.164189189189189\\
0.44788180225246	0.163513513513513\\
0.44820077093805	0.162837837837838\\
0.448932684919483	0.162162162162162\\
0.449731610624655	0.161486486486486\\
0.450108309810351	0.160810810810811\\
0.451852841168207	0.160135135135135\\
0.453514813719337	0.159459459459459\\
0.454899910548235	0.158783783783784\\
0.455393540679947	0.158108108108108\\
0.45809714085356	0.157432432432432\\
0.458141266181219	0.156756756756757\\
0.458206190481825	0.156081081081081\\
0.458943983915872	0.155405405405405\\
0.459418181836737	0.15472972972973\\
0.459608409310772	0.154054054054054\\
0.462013593565948	0.153378378378378\\
0.462745046245458	0.152702702702703\\
0.467292047777392	0.152027027027027\\
0.467408698250309	0.151351351351351\\
0.467662677432119	0.150675675675676\\
0.4687023766999	0.15\\
0.468881495646837	0.149324324324324\\
0.470250791783811	0.148648648648649\\
0.470427364900696	0.147972972972973\\
0.470437224405546	0.147297297297297\\
0.471146911867635	0.146621621621622\\
0.471645597042548	0.145945945945946\\
0.471818814213333	0.14527027027027\\
0.47299671209099	0.144594594594595\\
0.476305833035333	0.143918918918919\\
0.476582262809779	0.143243243243243\\
0.476857869507184	0.142567567567568\\
0.477430355903579	0.141891891891892\\
0.477816547060879	0.141216216216216\\
0.479410205850588	0.140540540540541\\
0.479437625349565	0.139864864864865\\
0.479757268450602	0.139189189189189\\
0.481030818644987	0.138513513513514\\
0.482232689986005	0.137837837837838\\
0.484914836611835	0.137162162162162\\
0.48492117257259	0.136486486486487\\
0.484981796198712	0.135810810810811\\
0.486514794718654	0.135135135135135\\
0.486524389717565	0.13445945945946\\
0.486671076046039	0.133783783783784\\
0.487642257534262	0.133108108108108\\
0.487644109990727	0.132432432432433\\
0.488899777736551	0.131756756756757\\
0.489783535661193	0.131081081081081\\
0.492014367619281	0.130405405405406\\
0.492782011971298	0.12972972972973\\
0.492847673142401	0.129054054054054\\
0.494422520273778	0.128378378378379\\
0.495421150251645	0.127702702702703\\
0.495980357039383	0.127027027027027\\
0.49675385114603	0.126351351351351\\
0.497081101423214	0.125675675675676\\
0.499549204439586	0.125\\
0.500502681813804	0.124324324324324\\
0.500505610274437	0.123648648648649\\
0.502412509016818	0.122972972972973\\
0.502834773390975	0.122297297297297\\
0.506930546145505	0.121621621621622\\
0.507624501568975	0.120945945945946\\
0.508998569531934	0.12027027027027\\
0.509670328068054	0.119594594594595\\
0.51322725929467	0.118918918918919\\
0.51514532049833	0.118243243243243\\
0.515635517383576	0.117567567567568\\
0.516439748750718	0.116891891891892\\
0.517063207508041	0.116216216216216\\
0.517427182125867	0.115540540540541\\
0.518131989505086	0.114864864864865\\
0.518201126743417	0.114189189189189\\
0.520462751165129	0.113513513513514\\
0.520690122461567	0.112837837837838\\
0.52089412883941	0.112162162162162\\
0.521116216259833	0.111486486486487\\
0.521936421069995	0.110810810810811\\
0.523121203439642	0.110135135135135\\
0.523838537995039	0.10945945945946\\
0.523973431086877	0.108783783783784\\
0.526237185288723	0.108108108108108\\
0.528387358997419	0.107432432432433\\
0.53109759533464	0.106756756756757\\
0.53218491281512	0.106081081081081\\
0.53447688676735	0.105405405405406\\
0.537963531234533	0.10472972972973\\
0.538032132068648	0.104054054054054\\
0.538099801139371	0.103378378378378\\
0.539961714046732	0.102702702702703\\
0.54005074520029	0.102027027027027\\
0.541815446461453	0.101351351351352\\
0.542553750077985	0.100675675675676\\
0.542576694294636	0.1\\
0.545078786376522	0.0993243243243245\\
0.546604768118884	0.0986486486486488\\
0.547451714842572	0.0979729729729731\\
0.548524008106509	0.0972972972972974\\
0.548664235784669	0.0966216216216218\\
0.551187771878738	0.0959459459459461\\
0.55167759834795	0.0952702702702704\\
0.551848842283893	0.0945945945945947\\
0.555792438480691	0.093918918918919\\
0.557750713259591	0.0932432432432434\\
0.558683538237169	0.0925675675675677\\
0.563676362121288	0.0918918918918921\\
0.564209777066965	0.0912162162162163\\
0.565574491112629	0.0905405405405406\\
0.566307142022886	0.089864864864865\\
0.571452784097273	0.0891891891891893\\
0.573050648753349	0.0885135135135137\\
0.575860138882354	0.0878378378378379\\
0.57726812128013	0.0871621621621623\\
0.577537619039637	0.0864864864864866\\
0.578929481686287	0.0858108108108109\\
0.584415821986639	0.0851351351351353\\
0.592681193806009	0.0844594594594595\\
0.59928353806297	0.0837837837837839\\
0.599465303210486	0.0831081081081082\\
0.601607264748547	0.0824324324324325\\
0.602144853610623	0.0817567567567569\\
0.602554715060754	0.0810810810810811\\
0.602605326179391	0.0804054054054055\\
0.602611052811161	0.0797297297297298\\
0.603287090531344	0.0790540540540542\\
0.603708640609989	0.0783783783783785\\
0.605320714582974	0.0777027027027029\\
0.606796045345287	0.0770270270270271\\
0.608094057138937	0.0763513513513515\\
0.608325653228258	0.0756756756756758\\
0.60938777736945	0.0750000000000002\\
0.612322463875611	0.0743243243243245\\
0.618873169070683	0.0736486486486487\\
0.620256185691886	0.0729729729729731\\
0.621165990192576	0.0722972972972974\\
0.624647429094516	0.0716216216216218\\
0.625195367173234	0.0709459459459461\\
0.626250940545374	0.0702702702702704\\
0.629277266889977	0.0695945945945947\\
0.631231483120565	0.068918918918919\\
0.631323955367042	0.0682432432432434\\
0.632513078063931	0.0675675675675677\\
0.632954807511197	0.066891891891892\\
0.635513313086044	0.0662162162162163\\
0.63897019291807	0.0655405405405407\\
0.642255520231957	0.064864864864865\\
0.643004858926715	0.0641891891891893\\
0.645940036036888	0.0635135135135136\\
0.649391311837765	0.0628378378378379\\
0.650133519401801	0.0621621621621623\\
0.650237243670419	0.0614864864864866\\
0.653751353377843	0.060810810810811\\
0.653778460951069	0.0601351351351352\\
0.657990165842331	0.0594594594594595\\
0.663353722445936	0.0587837837837839\\
0.666254739912149	0.0581081081081082\\
0.668399627525456	0.0574324324324326\\
0.672197621411077	0.0567567567567568\\
0.673381702822847	0.0560810810810812\\
0.678873912294336	0.0554054054054055\\
0.680195018993023	0.0547297297297298\\
0.680388581302396	0.0540540540540542\\
0.682580508497471	0.0533783783783784\\
0.683064229915056	0.0527027027027028\\
0.685204707223431	0.0520270270270271\\
0.689184501370022	0.0513513513513515\\
0.701259954040495	0.0506756756756758\\
0.708511607319582	0.05\\
0.709460358987994	0.0493243243243244\\
0.709595822506609	0.0486486486486487\\
0.716530928725355	0.0479729729729731\\
0.718324103257477	0.0472972972972974\\
0.721784052613968	0.0466216216216218\\
0.723986665090767	0.045945945945946\\
0.726094777604532	0.0452702702702703\\
0.727924307910418	0.0445945945945947\\
0.728312477273088	0.043918918918919\\
0.729491000775532	0.0432432432432434\\
0.735809579344905	0.0425675675675676\\
0.743144716782395	0.041891891891892\\
0.745072650796908	0.0412162162162163\\
0.746174726937168	0.0405405405405407\\
0.752006371450486	0.039864864864865\\
0.752380192964211	0.0391891891891892\\
0.754875562009758	0.0385135135135136\\
0.755024631757642	0.0378378378378379\\
0.759064314079966	0.0371621621621623\\
0.770472321714284	0.0364864864864866\\
0.771469741836539	0.0358108108108108\\
0.776842521823143	0.0351351351351352\\
0.78087760569512	0.0344594594594595\\
0.782769581057107	0.0337837837837839\\
0.783230864674768	0.0331081081081082\\
0.798753490425121	0.0324324324324325\\
0.801302113094575	0.0317567567567568\\
0.802520394735476	0.0310810810810812\\
0.822327522172694	0.0304054054054055\\
0.82466762488274	0.0297297297297298\\
0.82705030703634	0.0290540540540541\\
0.829177541203314	0.0283783783783784\\
0.830127901685554	0.0277027027027028\\
0.833160560662631	0.0270270270270271\\
0.840689978256791	0.0263513513513514\\
0.848549222416459	0.0256756756756757\\
0.856354144251005	0.025\\
0.856990494730905	0.0243243243243244\\
0.873850232057276	0.0236486486486487\\
0.885452347331731	0.0229729729729731\\
0.909049092743344	0.0222972972972973\\
0.916513872570269	0.0216216216216216\\
0.91918466395884	0.020945945945946\\
0.930298827553538	0.0202702702702703\\
0.977270644020666	0.0195945945945947\\
0.992216474669012	0.0189189189189189\\
1.01959284250081	0.0182432432432433\\
1.02165405918119	0.0175675675675676\\
1.06767003627049	0.0168918918918919\\
1.08857290661301	0.0162162162162163\\
1.10488803085007	0.0155405405405405\\
1.14636008082137	0.0148648648648649\\
1.15784432863468	0.0141891891891892\\
1.20235308199745	0.0135135135135136\\
1.20373770600345	0.0128378378378379\\
1.2042040711094	0.0121621621621621\\
1.20534391452092	0.0114864864864865\\
1.25538617998722	0.0108108108108108\\
1.26552061141545	0.0101351351351352\\
1.30815584299299	0.00945945945945947\\
1.33897028795771	0.00878378378378386\\
1.46499151141983	0.00810810810810814\\
1.51139829913487	0.00743243243243241\\
1.52010943492158	0.0067567567567568\\
1.61807752612448	0.00608108108108107\\
1.70801468044587	0.00540540540540546\\
1.78147631853848	0.00472972972972974\\
1.85498806265531	0.00405405405405401\\
1.86042815389099	0.0033783783783784\\
1.90485496447081	0.00270270270270268\\
2.44161294332638	0.00202702702702706\\
3.46750867887049	0.00135135135135134\\
374.347158170592	0.000675675675675724\\
414.80582356199	0\\
};
\addlegendentry{$K=20$, $G=\;\,5$, $\lrmse =10.28$, $\prmse =0.026$, $\armse =0.011$, $\brmse =5\hspace{-3pt}\times\hspace{-3pt}10^{-5}$, $\gamma=40$}


==> figures/mse_N_2_K_20_G_5_SNR_40_I_20_Pratio_2_Nratio_2_alpha_2_cs.tex <==
\addplot [color=blue, dashed,line width=0.6pt]
  table[row sep=crcr]{%
0.0373151376033766	1\\
0.0760602844505477	0.997999199679872\\
0.0888773147407979	0.995998399359744\\
0.0972351236436132	0.993997599039616\\
0.105049584682633	0.991996798719488\\
0.117562516046031	0.98999599839936\\
0.124787160597866	0.987995198079232\\
0.133840260386755	0.985994397759104\\
0.138155122348336	0.983993597438975\\
0.141318442472819	0.981992797118847\\
0.143823606010757	0.979991996798719\\
0.146981325344854	0.977991196478591\\
0.155208624737019	0.975990396158463\\
0.158159243591432	0.973989595838335\\
0.162265096432143	0.971988795518207\\
0.167779996977337	0.969987995198079\\
0.171162099999805	0.967987194877951\\
0.173618264836939	0.965986394557824\\
0.176871625390805	0.963985594237695\\
0.180447583285903	0.961984793917567\\
0.181677308881592	0.959983993597439\\
0.183844548264418	0.957983193277311\\
0.187062746993993	0.955982392957183\\
0.191131343318914	0.953981592637055\\
0.193767372977587	0.951980792316927\\
0.195241534243254	0.949979991996799\\
0.198246356553969	0.947979191676671\\
0.20358436359807	0.945978391356542\\
0.205527015471158	0.943977591036414\\
0.208038437402837	0.941976790716286\\
0.210510700512622	0.939975990396158\\
0.213827955901961	0.93797519007603\\
0.215751680810469	0.935974389755902\\
0.217894381359538	0.933973589435774\\
0.220274007687605	0.931972789115646\\
0.2224195876342	0.929971988795518\\
0.224036266231024	0.92797118847539\\
0.225775987500976	0.925970388155262\\
0.228928653725302	0.923969587835134\\
0.230712439517883	0.921968787515006\\
0.231917290757706	0.919967987194878\\
0.233142892575056	0.91796718687475\\
0.234839793311586	0.915966386554621\\
0.236333912878198	0.913965586234494\\
0.237288646847731	0.911964785914365\\
0.239503963227392	0.909963985594237\\
0.241992749371976	0.907963185274109\\
0.243904786028826	0.905962384953981\\
0.246856819627116	0.903961584633853\\
0.248039244925873	0.901960784313725\\
0.249147395554048	0.899959983993597\\
0.250674555364341	0.897959183673469\\
0.252158104128592	0.895958383353341\\
0.254677592769306	0.893957583033212\\
0.257010554163675	0.891956782713084\\
0.258108309277724	0.889955982392956\\
0.259231691137088	0.887955182072828\\
0.260736478649392	0.8859543817527\\
0.263266487958514	0.883953581432572\\
0.265857413289728	0.881952781112444\\
0.268188169720886	0.879951980792316\\
0.269812347546386	0.877951180472188\\
0.272114797865946	0.87595038015206\\
0.273285574536809	0.873949579831932\\
0.274987738325248	0.871948779511804\\
0.275977148277242	0.869947979191676\\
0.278369813666775	0.867947178871548\\
0.279520671375081	0.86594637855142\\
0.28123992502895	0.863945578231292\\
0.282348257873676	0.861944777911164\\
0.284452832255676	0.859943977591036\\
0.285757677044324	0.857943177270908\\
0.286741573288588	0.85594237695078\\
0.288922413341155	0.853941576630652\\
0.290373689742793	0.851940776310524\\
0.291787303091333	0.849939975990396\\
0.29304189811527	0.847939175670268\\
0.294325533423779	0.845938375350139\\
0.297346737676364	0.843937575030011\\
0.298335060089159	0.841936774709883\\
0.29912312324921	0.839935974389755\\
0.300434323950467	0.837935174069628\\
0.301595863874814	0.8359343737495\\
0.303331864609226	0.833933573429371\\
0.304563892457353	0.831932773109243\\
0.306168441547838	0.829931972789115\\
0.307777777645952	0.827931172468987\\
0.309055848240244	0.825930372148859\\
0.310208522351207	0.823929571828731\\
0.31144996229533	0.821928771508603\\
0.31262846836069	0.819927971188475\\
0.314123932933981	0.817927170868347\\
0.314979703918538	0.81592637054822\\
0.316796489604659	0.813925570228092\\
0.318113218088459	0.811924769907964\\
0.319440739393168	0.809923969587836\\
0.320899728280465	0.807923169267707\\
0.322851347764084	0.805922368947579\\
0.324454166425064	0.803921568627451\\
0.32605004579499	0.801920768307323\\
0.328007720843373	0.799919967987195\\
0.329339929164551	0.797919167667067\\
0.330777934230759	0.795918367346939\\
0.331994167123224	0.793917567026811\\
0.332890818569	0.791916766706683\\
0.334927545401627	0.789915966386555\\
0.335586350596698	0.787915166066427\\
0.336900235649436	0.785914365746299\\
0.339174603979827	0.783913565426171\\
0.340119424476658	0.781912765106043\\
0.341881505355188	0.779911964785915\\
0.343005923831864	0.777911164465787\\
0.344929144620393	0.775910364145659\\
0.346457841702469	0.773909563825531\\
0.347818682908654	0.771908763505403\\
0.349201390672127	0.769907963185275\\
0.350045358718856	0.767907162865147\\
0.351201763157732	0.765906362545019\\
0.352717118341148	0.763905562224891\\
0.355060991795128	0.761904761904763\\
0.356112573596019	0.759903961584635\\
0.358052397373918	0.757903161264507\\
0.359082411743009	0.755902360944379\\
0.360327069960911	0.753901560624251\\
0.361802300541009	0.751900760304123\\
0.362808617799426	0.749899959983995\\
0.36380046222993	0.747899159663867\\
0.365589522997448	0.745898359343739\\
0.367311885724908	0.743897559023611\\
0.368967885865222	0.741896758703483\\
0.370272457251827	0.739895958383355\\
0.372519551565327	0.737895158063227\\
0.374044957376121	0.735894357743099\\
0.374945218631111	0.733893557422971\\
0.37632485923712	0.731892757102843\\
0.377686421180383	0.729891956782715\\
0.378999594523942	0.727891156462587\\
0.379732571396441	0.725890356142459\\
0.380776042325184	0.723889555822331\\
0.38177261279244	0.721888755502203\\
0.383533201065486	0.719887955182075\\
0.384940675047256	0.717887154861947\\
0.386378129896469	0.715886354541819\\
0.387170545855421	0.713885554221692\\
0.388347644935523	0.711884753901564\\
0.3894729437885	0.709883953581435\\
0.390221839522982	0.707883153261307\\
0.391197714431383	0.705882352941179\\
0.392147038155787	0.703881552621051\\
0.393393379978398	0.701880752300923\\
0.394608698957518	0.699879951980795\\
0.395719837219525	0.697879151660667\\
0.397840398599282	0.69587835134054\\
0.399295261788312	0.693877551020412\\
0.400361458933934	0.691876750700284\\
0.402320672456506	0.689875950380155\\
0.403759141576842	0.687875150060027\\
0.405058209407952	0.6858743497399\\
0.406045564146959	0.683873549419772\\
0.407436175764929	0.681872749099644\\
0.409556869912953	0.679871948779516\\
0.41062549400718	0.677871148459388\\
0.41265555641553	0.67587034813926\\
0.414428778867969	0.673869547819132\\
0.415418122546753	0.671868747499004\\
0.417543365284792	0.669867947178876\\
0.418540499772753	0.667867146858748\\
0.419863884572737	0.66586634653862\\
0.421362713165669	0.663865546218492\\
0.422435185575511	0.661864745898364\\
0.423085355165654	0.659863945578236\\
0.424612828904278	0.657863145258109\\
0.425316226816791	0.655862344937981\\
0.426989106876172	0.653861544617853\\
0.429012884077518	0.651860744297725\\
0.430558782712195	0.649859943977597\\
0.432046283777967	0.647859143657469\\
0.433558251528436	0.645858343337341\\
0.434951048177031	0.643857543017213\\
0.435820435541284	0.641856742697085\\
0.437407659299073	0.639855942376957\\
0.439257625562932	0.637855142056829\\
0.44045178664876	0.635854341736701\\
0.441369468675247	0.633853541416573\\
0.442290432859773	0.631852741096444\\
0.443506894305069	0.629851940776317\\
0.446231566105322	0.627851140456189\\
0.4475104020268	0.625850340136061\\
0.448930397274926	0.623849539815933\\
0.450351568137282	0.621848739495804\\
0.452833098084281	0.619847939175676\\
0.453934769040415	0.617847138855548\\
0.455246307020705	0.61584633853542\\
0.456799928774475	0.613845538215293\\
0.458063358169879	0.611844737895165\\
0.459861536359574	0.609843937575037\\
0.461520888685835	0.607843137254909\\
0.46319878708425	0.605842336934781\\
0.464347367918126	0.603841536614652\\
0.467378716009178	0.601840736294525\\
0.469210507100445	0.599839935974397\\
0.470664094865184	0.597839135654269\\
0.471888701895939	0.595838335334141\\
0.473246995862432	0.593837535014013\\
0.474386491593518	0.591836734693885\\
0.477193126850441	0.589835934373757\\
0.478136373152651	0.587835134053629\\
0.47949123348694	0.585834333733501\\
0.481476670867543	0.583833533413374\\
0.48363159664466	0.581832733093246\\
0.485147357450675	0.579831932773118\\
0.486395936267404	0.57783113245299\\
0.488079658118957	0.575830332132862\\
0.489435219574861	0.573829531812734\\
0.490601747005136	0.571828731492606\\
0.492098420017602	0.569827931172479\\
0.493102993218105	0.56782713085235\\
0.495005203859804	0.565826330532223\\
0.496842486159858	0.563825530212095\\
0.498464118235311	0.561824729891967\\
0.500964108686487	0.559823929571839\\
0.502646436361181	0.557823129251711\\
0.504187612906056	0.555822328931583\\
0.504828748449481	0.553821528611456\\
0.506368850673813	0.551820728291328\\
0.507611528946522	0.5498199279712\\
0.509324946168319	0.547819127651072\\
0.510359902681609	0.545818327330944\\
0.511293641180663	0.543817527010816\\
0.512731324912918	0.541816726690688\\
0.514144387074758	0.539815926370561\\
0.516358056024905	0.537815126050433\\
0.517394995034421	0.535814325730305\\
0.518867546889822	0.533813525410177\\
0.519914289030544	0.531812725090049\\
0.521739222777775	0.529811924769921\\
0.523035526696759	0.527811124449793\\
0.523949748287236	0.525810324129665\\
0.525558619732528	0.523809523809537\\
0.52760131068214	0.521808723489409\\
0.528475035328977	0.519807923169281\\
0.530051541755435	0.517807122849153\\
0.531630893691048	0.515806322529025\\
0.532271880472435	0.513805522208897\\
0.533762294746542	0.511804721888769\\
0.535406564027133	0.509803921568641\\
0.536797207426152	0.507803121248513\\
0.539733089906803	0.505802320928385\\
0.5417261790148	0.503801520608258\\
0.544384498050072	0.501800720288129\\
0.545352438535898	0.499799919968001\\
0.546912630296833	0.497799119647873\\
0.548151935240558	0.495798319327745\\
0.549636909164097	0.493797519007617\\
0.55168729885815	0.491796718687489\\
0.553342662007975	0.489795918367361\\
0.555080956070422	0.487795118047233\\
0.556587349243804	0.485794317727104\\
0.558056880834246	0.483793517406977\\
0.559277505447232	0.481792717086848\\
0.561702161154489	0.47979191676672\\
0.563835392538538	0.477791116446592\\
0.565722170343581	0.475790316126464\\
0.568726032774755	0.473789515806336\\
0.570313648483624	0.471788715486208\\
0.572357962000782	0.46978791516608\\
0.573809096317712	0.467787114845951\\
0.575923924962175	0.465786314525823\\
0.578064671716092	0.463785514205695\\
0.579909365797582	0.461784713885567\\
0.581615264668149	0.459783913565439\\
0.583572222511314	0.457783113245311\\
0.585407868848304	0.455782312925183\\
0.5869160773852	0.453781512605055\\
0.589502077286732	0.451780712284927\\
0.591353995698741	0.449779911964798\\
0.59252031703204	0.447779111644671\\
0.594104637701206	0.445778311324542\\
0.595515886050836	0.443777511004414\\
0.596821979185638	0.441776710684286\\
0.598482442270976	0.439775910364158\\
0.601515635208101	0.43777511004403\\
0.603890421213657	0.435774309723902\\
0.60578426924672	0.433773509403774\\
0.607616658850284	0.431772709083646\\
0.610675426365691	0.429771908763517\\
0.612118153898186	0.427771108443389\\
0.613497155267459	0.425770308123261\\
0.615328289974459	0.423769507803133\\
0.617840014862422	0.421768707483005\\
0.619485388324247	0.419767907162877\\
0.621181739204097	0.417767106842749\\
0.623427936219349	0.41576630652262\\
0.625544765434083	0.413765506202493\\
0.627017972550464	0.411764705882364\\
0.628505487820778	0.409763905562236\\
0.63068940858967	0.407763105242108\\
0.63294581295096	0.40576230492198\\
0.634367891184313	0.403761504601852\\
0.637377517808627	0.401760704281724\\
0.63939584255574	0.399759903961595\\
0.641770314290693	0.397759103641467\\
0.644780996882165	0.395758303321339\\
0.647366258271061	0.393757503001211\\
0.649627091997584	0.391756702681083\\
0.652476536731909	0.389755902360955\\
0.655438825780701	0.387755102040827\\
0.657394969917752	0.385754301720699\\
0.661330563727227	0.383753501400571\\
0.663373993683186	0.381752701080442\\
0.665039729096329	0.379751900760314\\
0.667373408059282	0.377751100440186\\
0.67029276979918	0.375750300120058\\
0.672673850231415	0.37374949979993\\
0.674714240656333	0.371748699479802\\
0.676763025276183	0.369747899159673\\
0.679943201111539	0.367747098839545\\
0.682296828770502	0.365746298519417\\
0.684525261465092	0.363745498199289\\
0.686270382510486	0.361744697879161\\
0.690110996138428	0.359743897559033\\
0.691405161012426	0.357743097238905\\
0.694498816194971	0.355742296918776\\
0.696349282328029	0.353741496598648\\
0.698923641876335	0.35174069627852\\
0.701070469639196	0.349739895958392\\
0.703411369844605	0.347739095638264\\
0.705603060664969	0.345738295318135\\
0.707955532693019	0.343737494998007\\
0.710021572647718	0.341736694677879\\
0.712484465615247	0.339735894357751\\
0.7136927536861	0.337735094037623\\
0.715389166375046	0.335734293717494\\
0.71770139056136	0.333733493397366\\
0.721488031427562	0.331732693077238\\
0.722914791286467	0.32973189275711\\
0.725181803368305	0.327731092436982\\
0.727687087607304	0.325730292116853\\
0.730308282021504	0.323729491796725\\
0.734107050857046	0.321728691476597\\
0.735905833196278	0.319727891156469\\
0.738327557298227	0.317727090836341\\
0.740206853982487	0.315726290516213\\
0.742303886673085	0.313725490196084\\
0.746523407015106	0.311724689875956\\
0.748594509104061	0.309723889555828\\
0.752322492762508	0.3077230892357\\
0.754907158298421	0.305722288915572\\
0.758815496869437	0.303721488595444\\
0.761943968445428	0.301720688275316\\
0.764505402855718	0.299719887955187\\
0.767068080626705	0.297719087635059\\
0.77116953381473	0.295718287314931\\
0.776687765032618	0.293717486994803\\
0.778944035688133	0.291716686674675\\
0.780958480000592	0.289715886354546\\
0.784831696931639	0.287715086034418\\
0.789533096852609	0.28571428571429\\
0.792449956106558	0.283713485394162\\
0.796151206655562	0.281712685074034\\
0.798326767157885	0.279711884753906\\
0.800003580476849	0.277711084433778\\
0.803477319478973	0.27571028411365\\
0.805032042868548	0.273709483793522\\
0.806665690283962	0.271708683473393\\
0.810945327151696	0.269707883153265\\
0.816545238787852	0.267707082833137\\
0.819649384921062	0.265706282513009\\
0.822971212720541	0.263705482192881\\
0.827078342594427	0.261704681872752\\
0.834109684968606	0.259703881552624\\
0.836356236228646	0.257703081232496\\
0.840925668527231	0.255702280912368\\
0.844397459383509	0.25370148059224\\
0.849368897167011	0.251700680272112\\
0.85161597781622	0.249699879951984\\
0.856668607050939	0.247699079631855\\
0.859441563642652	0.245698279311727\\
0.863480412021902	0.243697478991599\\
0.869142681866699	0.241696678671471\\
0.872124655090535	0.239695878351343\\
0.874596701341453	0.237695078031215\\
0.877851725182395	0.235694277711087\\
0.880546284076838	0.233693477390959\\
0.88342025234637	0.231692677070831\\
0.88841385994475	0.229691876750703\\
0.890696668164971	0.227691076430575\\
0.89745190647511	0.225690276110447\\
0.901101918746919	0.223689475790319\\
0.907801798936789	0.221688675470191\\
0.912783755415095	0.219687875150062\\
0.91638025609497	0.217687074829934\\
0.919968453382461	0.215686274509806\\
0.921801185441218	0.213685474189678\\
0.924216588337042	0.21168467386955\\
0.92828500834285	0.209683873549422\\
0.931724752513513	0.207683073229294\\
0.937477310487011	0.205682272909166\\
0.941347150330636	0.203681472589038\\
0.946043014343359	0.20168067226891\\
0.950384477250386	0.199679871948782\\
0.953832692259439	0.197679071628654\\
0.957096415222285	0.195678271308526\\
0.9608180083649	0.193677470988398\\
0.96436937757653	0.19167667066827\\
0.971127448755657	0.189675870348141\\
0.974976388439087	0.187675070028013\\
0.978646370248636	0.185674269707885\\
0.981987767566881	0.183673469387757\\
0.985968389128228	0.181672669067629\\
0.992954170819967	0.179671868747501\\
0.997132532456814	0.177671068427373\\
1.00234905815229	0.175670268107245\\
1.00736196586629	0.173669467787117\\
1.01147835330714	0.171668667466989\\
1.01610531593405	0.169667867146861\\
1.02080577757355	0.167667066826733\\
1.02835073000814	0.165666266506605\\
1.04140048824442	0.163665466186477\\
1.04574003225403	0.161664665866349\\
1.05490467306304	0.159663865546221\\
1.05879121074678	0.157663065226093\\
1.06307096669593	0.155662264905965\\
1.06889678749637	0.153661464585837\\
1.07667706631902	0.151660664265708\\
1.08120334600404	0.14965986394558\\
1.08644925783252	0.147659063625452\\
1.09116163371566	0.145658263305324\\
1.09730037835647	0.143657462985196\\
1.10332003206487	0.141656662665068\\
1.1098285212507	0.13965586234494\\
1.1152015415269	0.137655062024812\\
1.12179945171755	0.135654261704684\\
1.12592268733851	0.133653461384556\\
1.14079545092497	0.131652661064428\\
1.14591318179621	0.1296518607443\\
1.15298864524728	0.127651060424172\\
1.16389016077832	0.125650260104044\\
1.17130273142848	0.123649459783916\\
1.17881251594518	0.121648659463788\\
1.18623024912322	0.11964785914366\\
1.19870767061782	0.117647058823532\\
1.20460105985273	0.115646258503404\\
1.21199275670431	0.113645458183276\\
1.22236699422477	0.111644657863147\\
1.23834955735142	0.109643857543019\\
1.24166243186871	0.107643057222891\\
1.2503459556262	0.105642256902763\\
1.26064752276336	0.103641456582635\\
1.26691561937684	0.101640656262507\\
1.27632878022439	0.0996398559423788\\
1.28693004532754	0.0976390556222507\\
1.29590101670866	0.0956382553021227\\
1.30364140810314	0.0936374549819945\\
1.318347625991	0.0916366546618664\\
1.3294751841811	0.0896358543417384\\
1.33734928168074	0.0876350540216102\\
1.34851656468376	0.0856342537014821\\
1.36218981035501	0.0836334533813541\\
1.38437926123274	0.0816326530612259\\
1.39723766167063	0.0796318527410979\\
1.41101164562249	0.0776310524209698\\
1.42736724672643	0.0756302521008417\\
1.44413474329696	0.0736294517807136\\
1.4718316432672	0.0716286514605855\\
1.48749958171185	0.0696278511404574\\
1.49954083278701	0.0676270508203293\\
1.51108337063727	0.0656262505002012\\
1.5420053566805	0.063625450180073\\
1.56381823773059	0.061624649859945\\
1.58218257067572	0.0596238495398169\\
1.60821297057902	0.0576230492196887\\
1.63009667398983	0.0556222488995607\\
1.65643546923156	0.0536214485794326\\
1.68075521743574	0.0516206482593046\\
1.69537604059483	0.0496198479391765\\
1.71138204169448	0.0476190476190484\\
1.75124566473841	0.0456182472989203\\
1.80064020349087	0.0436174469787922\\
1.84160538723258	0.0416166466586642\\
1.89818726987054	0.0396158463385361\\
1.9366527426519	0.037615046018408\\
1.97706174816705	0.03561424569828\\
2.03126148858313	0.0336134453781519\\
2.06782231724511	0.0316126450580239\\
2.11666312991298	0.0296118447378957\\
2.19850905550684	0.0276110444177676\\
2.25454879942296	0.0256102440976396\\
2.37852513875065	0.0236094437775115\\
2.45089670878162	0.0216086434573833\\
2.60192065223369	0.0196078431372553\\
2.78539758083498	0.0176070428171272\\
3.0433775889806	0.0156062424969992\\
3.42366960144872	0.013605442176871\\
4.12783934087638	0.0116046418567429\\
5.8049897761065	0.00960384153661487\\
13.0668895317031	0.00760304121648669\\
19.0670009877433	0.00560224089635863\\
32.3630707350974	0.00360144057623057\\
163.787637445477	0.00160064025610251\\
};
\addlegendentry{$N=2$,~, $\lrmse =18.18$, $\prmse =0.009$, $\gamma=40$}


==> figures/mse_N_2_K_20_G_5_SNR_40_I_20_Pratio_2_Nratio_2_alpha_3.4_cs.tex <==
\addplot [color=blue, dashed,line width=0.6pt]
  table[row sep=crcr]{%
0.0258689993853216	1\\
0.0324530534222959	0.998851366873421\\
0.0382031477192825	0.997702733746841\\
0.0414330912039657	0.996554100620262\\
0.049101363102056	0.995405467493683\\
0.0508182951176195	0.994256834367103\\
0.0521167851935904	0.993108201240524\\
0.0543572173830561	0.991959568113944\\
0.0557051145691693	0.990810934987365\\
0.0580540122533509	0.989662301860786\\
0.0594669350893162	0.988513668734206\\
0.0608356010585981	0.987365035607627\\
0.0626319339609425	0.986216402481047\\
0.0631407826180573	0.985067769354468\\
0.063911401743128	0.983919136227889\\
0.0648078978724496	0.982770503101309\\
0.0658407638613719	0.98162186997473\\
0.0663357827836157	0.980473236848151\\
0.067964862657651	0.979324603721571\\
0.0698538768509242	0.978175970594992\\
0.0711796406007192	0.977027337468412\\
0.0721295293792541	0.975878704341833\\
0.0732062526900508	0.974730071215253\\
0.0739596953033419	0.973581438088674\\
0.0759727298794029	0.972432804962094\\
0.0769388568378884	0.971284171835515\\
0.0784603064954183	0.970135538708936\\
0.0790689133786235	0.968986905582356\\
0.0801313309692121	0.967838272455777\\
0.0809735874500427	0.966689639329197\\
0.0818279808861504	0.965541006202618\\
0.0827260421517428	0.964392373076039\\
0.0839496322851026	0.963243739949459\\
0.0843536620633129	0.96209510682288\\
0.0859021411549573	0.960946473696301\\
0.0868497369304053	0.959797840569721\\
0.0871603013270681	0.958649207443142\\
0.0878361973657688	0.957500574316562\\
0.0884585318309064	0.956351941189983\\
0.0887104718644333	0.955203308063404\\
0.089713159056676	0.954054674936824\\
0.0902319138132827	0.952906041810245\\
0.0910940838099511	0.951757408683666\\
0.0915961457488854	0.950608775557086\\
0.0922962497162182	0.949460142430507\\
0.0929792870200601	0.948311509303927\\
0.0938162055139899	0.947162876177348\\
0.0944192712723615	0.946014243050769\\
0.0952532441844779	0.944865609924189\\
0.0957176762387093	0.94371697679761\\
0.0961723846010606	0.942568343671031\\
0.0965529223481238	0.941419710544451\\
0.0969461104271861	0.940271077417872\\
0.0972656684921201	0.939122444291293\\
0.0979828399609126	0.937973811164713\\
0.0982603961980808	0.936825178038134\\
0.0991368127352998	0.935676544911555\\
0.100317420889466	0.934527911784976\\
0.10065529953056	0.933379278658396\\
0.101336839771369	0.932230645531817\\
0.102068145274561	0.931082012405237\\
0.102532839241395	0.929933379278658\\
0.103273012664681	0.928784746152079\\
0.104157857216547	0.927636113025499\\
0.105261150392751	0.92648747989892\\
0.106056333176426	0.92533884677234\\
0.107308778282352	0.924190213645761\\
0.10777704309801	0.923041580519182\\
0.108441859566005	0.921892947392602\\
0.108965789084613	0.920744314266023\\
0.109695213031642	0.919595681139443\\
0.110173345890228	0.918447048012864\\
0.111137864723155	0.917298414886285\\
0.111471274514586	0.916149781759705\\
0.11196939276464	0.915001148633126\\
0.112403689787297	0.913852515506547\\
0.113179922668919	0.912703882379967\\
0.113567202662277	0.911555249253388\\
0.113821011505866	0.910406616126809\\
0.114089001482784	0.909257983000229\\
0.114280703296483	0.90810934987365\\
0.115212873900232	0.906960716747071\\
0.115931802642808	0.905812083620491\\
0.116350169945221	0.904663450493912\\
0.117088573396237	0.903514817367333\\
0.117252361697154	0.902366184240753\\
0.117720845122945	0.901217551114174\\
0.117955570353342	0.900068917987594\\
0.118978498477255	0.898920284861015\\
0.119581504107244	0.897771651734435\\
0.119811549522835	0.896623018607856\\
0.120157239607891	0.895474385481277\\
0.120576830873208	0.894325752354697\\
0.121030062615029	0.893177119228118\\
0.121383370514872	0.892028486101538\\
0.122015546781358	0.890879852974959\\
0.122385817383254	0.88973121984838\\
0.12266499927013	0.8885825867218\\
0.123181424514979	0.887433953595221\\
0.123568346732705	0.886285320468641\\
0.123798937235346	0.885136687342062\\
0.124199627622447	0.883988054215483\\
0.12505480699994	0.882839421088903\\
0.125548097005011	0.881690787962324\\
0.126111822216044	0.880542154835744\\
0.126796950246673	0.879393521709165\\
0.127324462008461	0.878244888582586\\
0.127691116427986	0.877096255456007\\
0.128091995350456	0.875947622329427\\
0.128470538558927	0.874798989202848\\
0.12876807501834	0.873650356076269\\
0.129283719665105	0.872501722949689\\
0.129837480195921	0.87135308982311\\
0.130047917174232	0.87020445669653\\
0.130558118755722	0.869055823569951\\
0.130704935018182	0.867907190443371\\
0.131513151493697	0.866758557316792\\
0.132029456484828	0.865609924190213\\
0.132442132995113	0.864461291063633\\
0.132890769353683	0.863312657937054\\
0.133098329119126	0.862164024810475\\
0.133464857877693	0.861015391683895\\
0.13393546605765	0.859866758557316\\
0.134205735358497	0.858718125430737\\
0.134500181228045	0.857569492304157\\
0.134865570209527	0.856420859177578\\
0.135297701867304	0.855272226050999\\
0.135530787091638	0.85412359292442\\
0.136685247966642	0.85297495979784\\
0.137013350016713	0.851826326671261\\
0.137092132326164	0.850677693544682\\
0.137479262109431	0.849529060418102\\
0.137850847985452	0.848380427291523\\
0.13798226200102	0.847231794164943\\
0.138315726373934	0.846083161038364\\
0.138773546659099	0.844934527911784\\
0.139467745230323	0.843785894785205\\
0.139751071262119	0.842637261658626\\
0.140424105707859	0.841488628532046\\
0.14088269514894	0.840339995405467\\
0.141678225979962	0.839191362278888\\
0.14199672397581	0.838042729152308\\
0.142373762753131	0.836894096025729\\
0.142779764458828	0.83574546289915\\
0.143507825117506	0.83459682977257\\
0.144142391824565	0.833448196645991\\
0.144748026098236	0.832299563519412\\
0.145328716317803	0.831150930392832\\
0.145617792529702	0.830002297266253\\
0.145777129215801	0.828853664139674\\
0.146160900782436	0.827705031013094\\
0.146447087302463	0.826556397886515\\
0.146845837692192	0.825407764759936\\
0.147172162054004	0.824259131633356\\
0.14751732613708	0.823110498506777\\
0.147957091412867	0.821961865380198\\
0.148319898232906	0.820813232253619\\
0.148664065202783	0.819664599127039\\
0.148932240881523	0.81851596600046\\
0.14962380582688	0.817367332873881\\
0.149937380675644	0.816218699747301\\
0.150343710322181	0.815070066620722\\
0.150585436516664	0.813921433494142\\
0.150918794206525	0.812772800367563\\
0.151286047776124	0.811624167240984\\
0.15222777717804	0.810475534114404\\
0.152970525376261	0.809326900987825\\
0.153339857005784	0.808178267861245\\
0.153876847993569	0.807029634734666\\
0.154080503788507	0.805881001608087\\
0.154328303435415	0.804732368481508\\
0.154980914006138	0.803583735354928\\
0.155256776044749	0.802435102228349\\
0.155724714406644	0.80128646910177\\
0.156011021647528	0.80013783597519\\
0.156541955031192	0.798989202848611\\
0.156722053503316	0.797840569722032\\
0.157159415478805	0.796691936595453\\
0.157600382429436	0.795543303468873\\
0.157996363220734	0.794394670342294\\
0.158609579426537	0.793246037215715\\
0.158918708318805	0.792097404089135\\
0.159136290463945	0.790948770962556\\
0.159459852027156	0.789800137835976\\
0.159595724300298	0.788651504709397\\
0.159830431257137	0.787502871582818\\
0.160143335530219	0.786354238456238\\
0.160549151935547	0.785205605329659\\
0.160815545905777	0.78405697220308\\
0.161296791870702	0.7829083390765\\
0.161568043571246	0.781759705949921\\
0.161924029006242	0.780611072823342\\
0.162295435589648	0.779462439696762\\
0.162942037304863	0.778313806570183\\
0.163134722233368	0.777165173443604\\
0.16354207092831	0.776016540317024\\
0.16408448661732	0.774867907190445\\
0.164647509749023	0.773719274063866\\
0.165082141227609	0.772570640937286\\
0.16528638602137	0.771422007810707\\
0.165628459478199	0.770273374684127\\
0.165786554674656	0.769124741557548\\
0.16613762641117	0.767976108430969\\
0.166828526450686	0.76682747530439\\
0.167056320391644	0.76567884217781\\
0.167816853380514	0.764530209051231\\
0.168216351202521	0.763381575924652\\
0.168569125860584	0.762232942798072\\
0.169102727883786	0.761084309671493\\
0.169296558523409	0.759935676544914\\
0.169543837188015	0.758787043418334\\
0.169746046980461	0.757638410291755\\
0.170289071974753	0.756489777165176\\
0.170898474258081	0.755341144038596\\
0.171158407046282	0.754192510912017\\
0.171731399139392	0.753043877785438\\
0.172301704857633	0.751895244658859\\
0.172968815287395	0.750746611532279\\
0.173376759213648	0.7495979784057\\
0.17383784394016	0.748449345279121\\
0.174128198864952	0.747300712152541\\
0.174411986287089	0.746152079025962\\
0.174645052746072	0.745003445899383\\
0.174961129177612	0.743854812772803\\
0.175266880870594	0.742706179646224\\
0.175658765098146	0.741557546519645\\
0.176047694806914	0.740408913393065\\
0.176701785698935	0.739260280266486\\
0.177026314460397	0.738111647139907\\
0.177318446058379	0.736963014013327\\
0.177675732060953	0.735814380886748\\
0.178123644981083	0.734665747760168\\
0.17858782839484	0.733517114633589\\
0.179000274358406	0.73236848150701\\
0.179253263705652	0.73121984838043\\
0.179435171252522	0.730071215253851\\
0.180110207315944	0.728922582127272\\
0.180458497303145	0.727773949000692\\
0.181046464299437	0.726625315874113\\
0.181352978101051	0.725476682747533\\
0.181508041227761	0.724328049620954\\
0.181614876969239	0.723179416494375\\
0.181793407543403	0.722030783367796\\
0.18198412325581	0.720882150241216\\
0.182695359194445	0.719733517114637\\
0.183106887608823	0.718584883988057\\
0.183451847997766	0.717436250861478\\
0.183953424867026	0.716287617734899\\
0.184372152097709	0.715138984608319\\
0.184764245075563	0.71399035148174\\
0.185177123866173	0.712841718355161\\
0.185610576593435	0.711693085228581\\
0.185927245806575	0.710544452102002\\
0.186155700346347	0.709395818975422\\
0.186578656263082	0.708247185848843\\
0.186925178316518	0.707098552722264\\
0.187213308051661	0.705949919595685\\
0.187476437014374	0.704801286469105\\
0.187776651219685	0.703652653342526\\
0.188098066399304	0.702504020215947\\
0.188510189494346	0.701355387089368\\
0.188677044008696	0.700206753962788\\
0.188803587813225	0.699058120836209\\
0.188999513450731	0.697909487709629\\
0.189478412392549	0.69676085458305\\
0.189843062315673	0.69561222145647\\
0.190254010733067	0.694463588329891\\
0.190459723451967	0.693314955203312\\
0.191019969148143	0.692166322076732\\
0.191364844798211	0.691017688950153\\
0.191517627616445	0.689869055823574\\
0.191875029511737	0.688720422696995\\
0.192195427537931	0.687571789570415\\
0.1925627997106	0.686423156443836\\
0.19293401272754	0.685274523317257\\
0.193312997038886	0.684125890190677\\
0.193502896359497	0.682977257064098\\
0.193723493510459	0.681828623937519\\
0.193958215305444	0.68067999081094\\
0.194642291288971	0.67953135768436\\
0.195056598548978	0.678382724557781\\
0.195397431306877	0.677234091431202\\
0.195734629100494	0.676085458304622\\
0.196070140101478	0.674936825178043\\
0.196231370946259	0.673788192051464\\
0.196614059033647	0.672639558924884\\
0.196941850063411	0.671490925798305\\
0.197201773953578	0.670342292671726\\
0.197677680449612	0.669193659545147\\
0.198029606533134	0.668045026418567\\
0.198202242962546	0.666896393291988\\
0.198325918858559	0.665747760165409\\
0.19852664149616	0.66459912703883\\
0.198853654031587	0.66345049391225\\
0.199268726146437	0.662301860785671\\
0.199538558493366	0.661153227659092\\
0.199994282981714	0.660004594532512\\
0.200204781029433	0.658855961405933\\
0.200353119393435	0.657707328279354\\
0.200617986259771	0.656558695152774\\
0.201110118596622	0.655410062026195\\
0.201517355791618	0.654261428899616\\
0.201965752249777	0.653112795773036\\
0.202170621081259	0.651964162646457\\
0.202607950323251	0.650815529519878\\
0.202954488773747	0.649666896393298\\
0.203281789270708	0.648518263266719\\
0.204002783755779	0.64736963014014\\
0.20420769817197	0.646220997013561\\
0.204672313116614	0.645072363886981\\
0.204917032755587	0.643923730760402\\
0.20525859283527	0.642775097633823\\
0.205535263432315	0.641626464507244\\
0.205845492936118	0.640477831380664\\
0.20609664252929	0.639329198254085\\
0.206605272870288	0.638180565127506\\
0.206946880473539	0.637031932000927\\
0.207208944673706	0.635883298874347\\
0.207493111263404	0.634734665747768\\
0.207727622240941	0.633586032621189\\
0.207892828498584	0.63243739949461\\
0.20837753953341	0.63128876636803\\
0.208676703212102	0.630140133241451\\
0.209254807876198	0.628991500114872\\
0.20955209181255	0.627842866988292\\
0.209911913794697	0.626694233861713\\
0.210304655760144	0.625545600735134\\
0.211034462378884	0.624396967608555\\
0.211333213567898	0.623248334481975\\
0.211616533054796	0.622099701355396\\
0.212055628121273	0.620951068228817\\
0.212690450146735	0.619802435102238\\
0.213117332303853	0.618653801975658\\
0.213255625964436	0.617505168849079\\
0.213598927798387	0.616356535722499\\
0.213989726583394	0.61520790259592\\
0.214171252787456	0.614059269469341\\
0.214548650913337	0.612910636342761\\
0.214884230896464	0.611762003216182\\
0.215086129724879	0.610613370089603\\
0.21557964681721	0.609464736963024\\
0.215696329585159	0.608316103836444\\
0.215836687121938	0.607167470709865\\
0.216345845479626	0.606018837583286\\
0.216449907645611	0.604870204456706\\
0.216583298708435	0.603721571330127\\
0.216827642656238	0.602572938203548\\
0.217155322352193	0.601424305076968\\
0.21755671606622	0.600275671950389\\
0.218125600262477	0.59912703882381\\
0.218672552624723	0.597978405697231\\
0.218861087943699	0.596829772570651\\
0.219022949886558	0.595681139444072\\
0.219135612188652	0.594532506317492\\
0.219254458682299	0.593383873190913\\
0.219781606896449	0.592235240064333\\
0.220384343913741	0.591086606937754\\
0.220904295317299	0.589937973811175\\
0.221059558856629	0.588789340684595\\
0.221477217530657	0.587640707558016\\
0.222046553574197	0.586492074431437\\
0.22259325601562	0.585343441304857\\
0.222821116617133	0.584194808178278\\
0.223376572911799	0.583046175051699\\
0.223665093629523	0.581897541925119\\
0.224057843758093	0.58074890879854\\
0.224222582275897	0.579600275671961\\
0.224552690490856	0.578451642545382\\
0.224811176276106	0.577303009418802\\
0.225121309775936	0.576154376292223\\
0.225423058628298	0.575005743165643\\
0.225866643408872	0.573857110039064\\
0.226291870865459	0.572708476912484\\
0.226581956343426	0.571559843785905\\
0.226947247023191	0.570411210659326\\
0.227368191437505	0.569262577532747\\
0.227727412949448	0.568113944406167\\
0.22832999723914	0.566965311279588\\
0.228585692921418	0.565816678153009\\
0.229165973028955	0.56466804502643\\
0.229759899962779	0.56351941189985\\
0.230157799073475	0.562370778773271\\
0.230505877562282	0.561222145646692\\
0.230871809661844	0.560073512520113\\
0.231271112957126	0.558924879393533\\
0.231747176697718	0.557776246266954\\
0.231935398535021	0.556627613140375\\
0.232637634506271	0.555478980013795\\
0.233031823371269	0.554330346887216\\
0.233689258353767	0.553181713760637\\
0.234067163709632	0.552033080634057\\
0.234801725309826	0.550884447507478\\
0.234954056962653	0.549735814380899\\
0.235352462848984	0.548587181254319\\
0.23583072890208	0.54743854812774\\
0.236237495661589	0.546289915001161\\
0.237066398748789	0.545141281874581\\
0.237382731798415	0.543992648748002\\
0.237561462636383	0.542844015621422\\
0.238169526814661	0.541695382494843\\
0.238726852533482	0.540546749368263\\
0.238917208046398	0.539398116241684\\
0.239161173692242	0.538249483115105\\
0.239667566329196	0.537100849988525\\
0.239970510571843	0.535952216861946\\
0.240512216005435	0.534803583735367\\
0.240991541004583	0.533654950608788\\
0.241211462305766	0.532506317482208\\
0.241669645934351	0.531357684355629\\
0.241929831924256	0.53020905122905\\
0.242077883949863	0.529060418102471\\
0.242455069515893	0.527911784975891\\
0.242820872899422	0.526763151849312\\
0.24302284875879	0.525614518722732\\
0.243535248360908	0.524465885596153\\
0.244308168020872	0.523317252469574\\
0.244906824631456	0.522168619342995\\
0.245038313767381	0.521019986216415\\
0.245439248770917	0.519871353089836\\
0.245607076155098	0.518722719963257\\
0.245835537362318	0.517574086836677\\
0.246516902831053	0.516425453710098\\
0.246853891732637	0.515276820583518\\
0.247177264270591	0.514128187456939\\
0.247731380468938	0.51297955433036\\
0.248157793951545	0.51183092120378\\
0.248695973434549	0.510682288077201\\
0.248828535767027	0.509533654950622\\
0.249084193901132	0.508385021824042\\
0.249385006630951	0.507236388697463\\
0.24969416753746	0.506087755570884\\
0.24999713989129	0.504939122444305\\
0.250499711233941	0.503790489317725\\
0.250950633579268	0.502641856191146\\
0.25132696228956	0.501493223064567\\
0.251568922322502	0.500344589937988\\
0.251896228677718	0.499195956811408\\
0.252217718169222	0.498047323684829\\
0.252387386410997	0.496898690558249\\
0.252645425973226	0.49575005743167\\
0.252820107223637	0.494601424305091\\
0.253311949283093	0.493452791178511\\
0.253616628523612	0.492304158051932\\
0.254452585873504	0.491155524925352\\
0.254670054237816	0.490006891798773\\
0.25498690089285	0.488858258672193\\
0.255347294454736	0.487709625545614\\
0.25565997095484	0.486560992419035\\
0.256212914290134	0.485412359292455\\
0.256619791443984	0.484263726165876\\
0.257301849679687	0.483115093039296\\
0.257401670032786	0.481966459912717\\
0.258139793021829	0.480817826786138\\
0.258379010122158	0.479669193659558\\
0.258578671883092	0.478520560532979\\
0.258875486746712	0.477371927406399\\
0.25956769655716	0.47622329427982\\
0.260075949737536	0.475074661153241\\
0.260727415514132	0.473926028026661\\
0.261101057882192	0.472777394900082\\
0.261901510473263	0.471628761773502\\
0.262193881062306	0.470480128646923\\
0.262883578612	0.469331495520344\\
0.263083974283655	0.468182862393764\\
0.263621811441132	0.467034229267185\\
0.263958807701903	0.465885596140605\\
0.264385440360109	0.464736963014026\\
0.264566489055725	0.463588329887447\\
0.265100116779277	0.462439696760867\\
0.265560916708127	0.461291063634288\\
0.266237078768791	0.460142430507708\\
0.266814608449321	0.458993797381129\\
0.267261371372233	0.457845164254549\\
0.268158613953469	0.45669653112797\\
0.268693067719487	0.455547898001391\\
0.26906743990426	0.454399264874811\\
0.269761664978864	0.453250631748232\\
0.270257970080703	0.452101998621652\\
0.270681405595711	0.450953365495073\\
0.271263941784444	0.449804732368494\\
0.271930736950243	0.448656099241915\\
0.272178595404502	0.447507466115335\\
0.272668037645669	0.446358832988756\\
0.272969907301678	0.445210199862176\\
0.273352063681641	0.444061566735597\\
0.273831314991197	0.442912933609017\\
0.27415380180864	0.441764300482438\\
0.274553615575102	0.440615667355859\\
0.275334381282881	0.439467034229279\\
0.275795744539422	0.4383184011027\\
0.27624305549549	0.43716976797612\\
0.277366761554278	0.436021134849541\\
0.278078219279806	0.434872501722961\\
0.27832183839815	0.433723868596382\\
0.278884279303597	0.432575235469803\\
0.279025824834571	0.431426602343223\\
0.279326525652523	0.430277969216644\\
0.279727039599768	0.429129336090064\\
0.280367081039638	0.427980702963485\\
0.280928953251022	0.426832069836905\\
0.281051280140406	0.425683436710326\\
0.281422539077499	0.424534803583747\\
0.281803463158144	0.423386170457167\\
0.282145966852571	0.422237537330588\\
0.282757551086561	0.421088904204008\\
0.283249863307991	0.419940271077429\\
0.283578617947345	0.41879163795085\\
0.283733978184407	0.41764300482427\\
0.283922421958739	0.416494371697691\\
0.284481182501573	0.415345738571111\\
0.284745709771522	0.414197105444532\\
0.285320875259903	0.413048472317952\\
0.285757457415201	0.411899839191373\\
0.286346611382446	0.410751206064794\\
0.286832621223726	0.409602572938214\\
0.287531588012876	0.408453939811635\\
0.287933232239366	0.407305306685055\\
0.288487849865282	0.406156673558476\\
0.288824373875377	0.405008040431896\\
0.289299158499323	0.403859407305317\\
0.28978301746734	0.402710774178737\\
0.290189919139185	0.401562141052158\\
0.29106978095951	0.400413507925579\\
0.291690605340853	0.399264874798999\\
0.292244940820382	0.39811624167242\\
0.292710972500868	0.39696760854584\\
0.292908592625913	0.395818975419261\\
0.294111670686285	0.394670342292681\\
0.294270235444219	0.393521709166102\\
0.294512036713399	0.392373076039522\\
0.294672516957002	0.391224442912943\\
0.294897932966948	0.390075809786363\\
0.295559757128083	0.388927176659784\\
0.295713322517069	0.387778543533205\\
0.296598510311687	0.386629910406625\\
0.296886582412645	0.385481277280046\\
0.297145898180735	0.384332644153466\\
0.298035482889946	0.383184011026887\\
0.298325449586638	0.382035377900307\\
0.298972935058683	0.380886744773728\\
0.299356477336855	0.379738111647149\\
0.300024520048891	0.378589478520569\\
0.300963702602897	0.37744084539399\\
0.301209322448272	0.37629221226741\\
0.302235360107774	0.375143579140831\\
0.302565450843053	0.373994946014251\\
0.302838981661914	0.372846312887672\\
0.303323063139952	0.371697679761093\\
0.304191106916891	0.370549046634513\\
0.304946874579518	0.369400413507934\\
0.305487452698983	0.368251780381354\\
0.305837576533053	0.367103147254775\\
0.306746657110898	0.365954514128195\\
0.307571084536461	0.364805881001616\\
0.308450052996787	0.363657247875037\\
0.308833896339704	0.362508614748457\\
0.308963056581692	0.361359981621878\\
0.309461069031531	0.360211348495298\\
0.310126306932538	0.359062715368719\\
0.31037933951389	0.357914082242139\\
0.311250225023922	0.35676544911556\\
0.311441270648324	0.355616815988981\\
0.311787314560454	0.354468182862401\\
0.312009966881481	0.353319549735822\\
0.312757529873604	0.352170916609242\\
0.313568528438296	0.351022283482663\\
0.314296368149718	0.349873650356084\\
0.314818694127498	0.348725017229504\\
0.315239602637369	0.347576384102925\\
0.316046151464358	0.346427750976345\\
0.316635313900946	0.345279117849766\\
0.317208040519442	0.344130484723186\\
0.317840991480813	0.342981851596607\\
0.318086002459436	0.341833218470028\\
0.318545354909671	0.340684585343448\\
0.318887742577123	0.339535952216869\\
0.319434212553095	0.338387319090289\\
0.320565225636076	0.33723868596371\\
0.321593984878319	0.33609005283713\\
0.321861904493682	0.334941419710551\\
0.322511666763552	0.333792786583971\\
0.323147200454519	0.332644153457392\\
0.323985319470843	0.331495520330813\\
0.324387847547511	0.330346887204233\\
0.325188517106173	0.329198254077654\\
0.325686568406508	0.328049620951074\\
0.326538847408955	0.326900987824495\\
0.327163665986357	0.325752354697916\\
0.328080478182688	0.324603721571336\\
0.329220492487698	0.323455088444757\\
0.329527732552782	0.322306455318177\\
0.330139757779986	0.321157822191598\\
0.330985427805688	0.320009189065019\\
0.331519272663235	0.318860555938439\\
0.33196252729951	0.31771192281186\\
0.333129402070586	0.31656328968528\\
0.333676232982051	0.315414656558701\\
0.334466518928331	0.314266023432122\\
0.335099827703732	0.313117390305542\\
0.335365643954402	0.311968757178963\\
0.335762203830748	0.310820124052383\\
0.336407115877958	0.309671490925804\\
0.33684977287438	0.308522857799225\\
0.337318271165432	0.307374224672645\\
0.337886012064549	0.306225591546066\\
0.338171609663412	0.305076958419486\\
0.338635127875401	0.303928325292907\\
0.339699781679787	0.302779692166327\\
0.340416735513965	0.301631059039748\\
0.341001435948326	0.300482425913168\\
0.341577569825707	0.299333792786589\\
0.341949364319978	0.298185159660009\\
0.342687631297076	0.29703652653343\\
0.343355607482785	0.295887893406851\\
0.343559106523128	0.294739260280271\\
0.344147375623938	0.293590627153692\\
0.344471678575448	0.292441994027112\\
0.344793429591607	0.291293360900533\\
0.345531415649464	0.290144727773954\\
0.34668466944508	0.288996094647374\\
0.347141822839814	0.287847461520795\\
0.34801504624618	0.286698828394215\\
0.348575462518126	0.285550195267636\\
0.349513961064812	0.284401562141056\\
0.349955692739655	0.283252929014477\\
0.350990899323541	0.282104295887897\\
0.35152640947775	0.280955662761318\\
0.352515931064966	0.279807029634739\\
0.352919975040718	0.278658396508159\\
0.353285546768034	0.27750976338158\\
0.354117430770493	0.276361130255\\
0.355040838612235	0.275212497128421\\
0.355256819270955	0.274063864001841\\
0.356143552081116	0.272915230875262\\
0.35720731975079	0.271766597748682\\
0.358231297994931	0.270617964622103\\
0.359227804807461	0.269469331495524\\
0.359873027275012	0.268320698368944\\
0.360828187334205	0.267172065242365\\
0.361722090220083	0.266023432115785\\
0.362369461212913	0.264874798989206\\
0.363467608516983	0.263726165862626\\
0.365493979666905	0.262577532736047\\
0.366195949041518	0.261428899609468\\
0.367380454902447	0.260280266482888\\
0.367868173067815	0.259131633356309\\
0.368788904704018	0.257983000229729\\
0.369191440609626	0.25683436710315\\
0.370385000433906	0.25568573397657\\
0.370735212202787	0.254537100849991\\
0.372494424492847	0.253388467723412\\
0.373278365793477	0.252239834596832\\
0.374423380007754	0.251091201470253\\
0.375103178392313	0.249942568343673\\
0.37584065563373	0.248793935217094\\
0.376407716911998	0.247645302090514\\
0.377255396586359	0.246496668963935\\
0.377730923099434	0.245348035837356\\
0.379146408817001	0.244199402710776\\
0.379519538390024	0.243050769584197\\
0.380174231552204	0.241902136457618\\
0.381523819327619	0.240753503331038\\
0.382254706604364	0.239604870204459\\
0.38389292159908	0.23845623707788\\
0.384234580649814	0.2373076039513\\
0.386186605265717	0.236158970824721\\
0.387677433483849	0.235010337698141\\
0.388443469531728	0.233861704571562\\
0.389543336087207	0.232713071444983\\
0.39010636615933	0.231564438318403\\
0.391151639643601	0.230415805191824\\
0.391636296040623	0.229267172065245\\
0.392965342949071	0.228118538938665\\
0.39438657013504	0.226969905812086\\
0.395055035059003	0.225821272685506\\
0.396531771764371	0.224672639558927\\
0.398068794223207	0.223524006432348\\
0.398750065135896	0.222375373305768\\
0.399630582061095	0.221226740179189\\
0.400515053559778	0.220078107052609\\
0.401341644089077	0.21892947392603\\
0.402215594554384	0.217780840799451\\
0.402709557340975	0.216632207672871\\
0.404408662910019	0.215483574546292\\
0.405473318836812	0.214334941419713\\
0.406142708053742	0.213186308293133\\
0.408036341562398	0.212037675166554\\
0.408926909480081	0.210889042039974\\
0.410403078735065	0.209740408913395\\
0.411722635716317	0.208591775786816\\
0.412817166893237	0.207443142660236\\
0.413906197348466	0.206294509533657\\
0.414684440542754	0.205145876407078\\
0.415725760711221	0.203997243280498\\
0.416595331083299	0.202848610153919\\
0.418018335352007	0.201699977027339\\
0.419421693242214	0.20055134390076\\
0.420631380937298	0.199402710774181\\
0.421436158499143	0.198254077647601\\
0.423177149667481	0.197105444521022\\
0.424550863329668	0.195956811394443\\
0.42610474233877	0.194808178267863\\
0.427308650822107	0.193659545141284\\
0.429562401824285	0.192510912014704\\
0.430023649250843	0.191362278888125\\
0.430880205145039	0.190213645761546\\
0.431958996560647	0.189065012634966\\
0.433456058032955	0.187916379508387\\
0.434721226585928	0.186767746381807\\
0.435496820474826	0.185619113255228\\
0.436387059829528	0.184470480128649\\
0.437449929335138	0.183321847002069\\
0.438427973301081	0.18217321387549\\
0.440681064671469	0.181024580748911\\
0.442932211475319	0.179875947622331\\
0.444475745745577	0.178727314495752\\
0.445289361690166	0.177578681369172\\
0.446731787547501	0.176430048242593\\
0.447394875826889	0.175281415116014\\
0.448543279956576	0.174132781989434\\
0.449633629649736	0.172984148862855\\
0.451773712695437	0.171835515736275\\
0.453373781820572	0.170686882609696\\
0.454314099789668	0.169538249483117\\
0.455794952728784	0.168389616356537\\
0.458249095214861	0.167240983229958\\
0.459029266774512	0.166092350103379\\
0.460487691659726	0.164943716976799\\
0.462394883111475	0.16379508385022\\
0.464246089304639	0.162646450723641\\
0.467209245080738	0.161497817597061\\
0.469032090681582	0.160349184470482\\
0.469600148125361	0.159200551343903\\
0.471272060953012	0.158051918217323\\
0.472291468876449	0.156903285090744\\
0.473111420800151	0.155754651964164\\
0.475493244311785	0.154606018837585\\
0.476876185388771	0.153457385711006\\
0.478387913949117	0.152308752584426\\
0.479359106856998	0.151160119457847\\
0.481092627879686	0.150011486331268\\
0.483523401263865	0.148862853204688\\
0.486570587506092	0.147714220078109\\
0.488566731989506	0.14656558695153\\
0.489697015036279	0.14541695382495\\
0.491289312707202	0.144268320698371\\
0.493299498413807	0.143119687571791\\
0.495002832693203	0.141971054445212\\
0.49714775691542	0.140822421318633\\
0.499575393584164	0.139673788192053\\
0.500618620619028	0.138525155065474\\
0.501756735641492	0.137376521938894\\
0.502540453760895	0.136227888812315\\
0.505264825154501	0.135079255685736\\
0.506595635449359	0.133930622559156\\
0.509673996707197	0.132781989432577\\
0.511549616738414	0.131633356305998\\
0.512822630419481	0.130484723179418\\
0.516133892741447	0.129336090052839\\
0.516760912584302	0.12818745692626\\
0.518199915868201	0.12703882379968\\
0.520532960121274	0.125890190673101\\
0.523160995146309	0.124741557546522\\
0.524154910046465	0.123592924419942\\
0.526042235596256	0.122444291293363\\
0.528378720903705	0.121295658166783\\
0.530291099049936	0.120147025040204\\
0.533050409199254	0.118998391913625\\
0.537468305326578	0.117849758787045\\
0.539260928236248	0.116701125660466\\
0.542887500072715	0.115552492533886\\
0.545117059634945	0.114403859407307\\
0.547783411280025	0.113255226280728\\
0.549925758431436	0.112106593154148\\
0.552000532655817	0.110957960027569\\
0.553787147310239	0.109809326900989\\
0.556436048055486	0.10866069377441\\
0.55986101406287	0.107512060647831\\
0.562952605261032	0.106363427521251\\
0.565269344450092	0.105214794394672\\
0.573157474409493	0.104066161268092\\
0.575532418487667	0.102917528141513\\
0.577817656280727	0.101768895014934\\
0.58002700587994	0.100620261888354\\
0.582356488222805	0.099471628761775\\
0.586604076224534	0.0983229956351955\\
0.589410827506349	0.0971743625086161\\
0.597454356093526	0.0960257293820368\\
0.600665596068084	0.0948770962554574\\
0.603278332317554	0.0937284631288779\\
0.605478203014828	0.0925798300022986\\
0.60863888204484	0.0914311968757192\\
0.612385343253753	0.0902825637491399\\
0.620686725672144	0.0891339306225605\\
0.624140288141003	0.0879852974959811\\
0.628716660824256	0.0868366643694016\\
0.632912922626212	0.0856880312428223\\
0.636281322896003	0.0845393981162429\\
0.638508328814799	0.0833907649896635\\
0.642093477495012	0.082242131863084\\
0.649063148150854	0.0810934987365047\\
0.65034669187184	0.0799448656099253\\
0.65438267844532	0.0787962324833459\\
0.660334142145485	0.0776475993567665\\
0.663949746107254	0.0764989662301871\\
0.666489923690344	0.0753503331036077\\
0.670202249552548	0.0742016999770283\\
0.673170420279887	0.0730530668504489\\
0.677946966916054	0.0719044337238695\\
0.680085411057655	0.0707558005972901\\
0.683893782702187	0.0696071674707107\\
0.686915883493503	0.0684585343441313\\
0.697872878065334	0.067309901217552\\
0.702705885922662	0.0661612680909726\\
0.709127218161424	0.0650126349643931\\
0.71708485726187	0.0638640018378137\\
0.720160635561645	0.0627153687112343\\
0.724560523074051	0.061566735584655\\
0.728376158775242	0.0604181024580756\\
0.737751513559035	0.0592694693314961\\
0.743426441686495	0.0581208362049168\\
0.746510319692269	0.0569722030783374\\
0.758053786522772	0.0558235699517581\\
0.768033317547038	0.0546749368251787\\
0.773455978615636	0.0535263036985992\\
0.785679408121857	0.0523776705720199\\
0.796781901223051	0.0512290374454405\\
0.803006626108592	0.0500804043188612\\
0.808665492669327	0.0489317711922818\\
0.822177528909014	0.0477831380657023\\
0.829605961861661	0.046634504939123\\
0.832346779910045	0.0454858718125436\\
0.844336850654799	0.0443372386859643\\
0.858519546830092	0.0431886055593849\\
0.868788567918324	0.0420399724328054\\
0.887265285676109	0.0408913393062261\\
0.89990793344802	0.0397427061796467\\
0.909633906074548	0.0385940730530674\\
0.918870637766866	0.037445439926488\\
0.938301431672483	0.0362968067999085\\
0.973798338600861	0.0351481736733292\\
0.977429308561494	0.0339995405467498\\
1.00785363071963	0.0328509074201704\\
1.02300855886196	0.0317022742935911\\
1.04417640182305	0.0305536411670116\\
1.07228618039099	0.0294050080404323\\
1.14720517741653	0.0282563749138529\\
1.17676225824908	0.0271077417872735\\
1.20333865673967	0.0259591086606942\\
1.26032315406951	0.0248104755341148\\
1.32134180593969	0.0236618424075353\\
1.3851854109475	0.022513209280956\\
1.48195505648423	0.0213645761543766\\
1.57442211285048	0.0202159430277972\\
1.66746305003488	0.0190673099012179\\
1.80472345600379	0.0179186767746384\\
1.87820242699243	0.016770043648059\\
2.02802600433276	0.0156214105214797\\
2.91815260744147	0.0144727773949003\\
5.11224290696707	0.0133241442683208\\
46.8999746548672	0.0121755111417415\\
116.956626462557	0.0110268780151621\\
124.098516434589	0.00987824488858269\\
163.366805179846	0.00872961176200338\\
297.241823943989	0.00758097863542395\\
684.538570813024	0.00643234550884453\\
1207.50023638638	0.00528371238226522\\
1347.34896757408	0.00413507925568579\\
1470.99558570416	0.00298644612910637\\
1585.89124501358	0.00183781300252706\\
1807.65632923678	0.000689179875947632\\
};
\addlegendentry{$N=2$,~, $\lrmse =101.5$, $\prmse =0.033$, $\armse =0.045$, $\brmse =3\hspace{-3pt}\times\hspace{-3pt}10^{-4}$, $\gamma=40$}


==> figures/mse_N_2_K_50_G_11_SNR_40_I_20_Pratio_2_Nratio_1_cs.tex <==
\addplot [color=green, dashed,line width=0.6pt]
  table[row sep=crcr]{%
0.00998262084019069	1\\
0.014018340673161	0.999\\
0.0168326077006397	0.998\\
0.0184869530491045	0.997\\
0.0208190954483676	0.996\\
0.0223088293557577	0.995\\
0.0240203234376834	0.994\\
0.0252592800972367	0.993\\
0.0263963861355148	0.992\\
0.0272016901688068	0.991\\
0.0274561107911052	0.99\\
0.0280185845993738	0.989\\
0.02901280632812	0.988\\
0.0299165360953748	0.987\\
0.0303188303077597	0.986\\
0.0307710646791647	0.985\\
0.0317241722732009	0.984\\
0.0323039487646204	0.983\\
0.0330925294442834	0.982\\
0.0333771591878439	0.981\\
0.0339533507740229	0.98\\
0.0343741108601549	0.979\\
0.0351864121775369	0.978\\
0.0359523954022211	0.977\\
0.0363303745155174	0.976\\
0.0368492876607701	0.975\\
0.0371835012903507	0.974\\
0.0378223068563734	0.973\\
0.0383521665310432	0.972\\
0.0385873922285112	0.971\\
0.0387128084603111	0.970000000000001\\
0.0393607946592701	0.969\\
0.0399108284413562	0.968\\
0.0402736317922847	0.967000000000001\\
0.0405682239781974	0.966000000000001\\
0.0410570159742525	0.965000000000001\\
0.0412089381935591	0.964000000000001\\
0.0413674966646878	0.963000000000001\\
0.0417940515845065	0.962000000000001\\
0.0421844824937029	0.961000000000001\\
0.0424389414538499	0.960000000000001\\
0.0426311480748466	0.959000000000001\\
0.0430280633150143	0.958000000000001\\
0.0433775497983125	0.957000000000001\\
0.0437282363793503	0.956000000000001\\
0.0439122745265269	0.955000000000001\\
0.0442726876635161	0.954000000000001\\
0.0445466750833142	0.953000000000001\\
0.0446985593580679	0.952000000000001\\
0.0448685104000731	0.951000000000001\\
0.0451955145411576	0.950000000000001\\
0.0455244086276029	0.949000000000001\\
0.0459098357313223	0.948000000000001\\
0.046150906244277	0.947000000000001\\
0.0463849642931483	0.946000000000001\\
0.0467710806117702	0.945000000000001\\
0.047062061828548	0.944000000000001\\
0.0471647042043441	0.943000000000001\\
0.0472692590999202	0.942000000000001\\
0.0476481483272932	0.941000000000001\\
0.0477829929395648	0.940000000000001\\
0.048121810485985	0.939000000000001\\
0.0484128073836355	0.938000000000001\\
0.0486065065747389	0.937000000000001\\
0.0490182107572311	0.936000000000001\\
0.0492934100771481	0.935000000000001\\
0.0495584666627639	0.934000000000001\\
0.0497473939362868	0.933000000000001\\
0.0500111328691165	0.932000000000001\\
0.0503344713307975	0.931000000000001\\
0.0504687258446333	0.930000000000001\\
0.0505976206157717	0.929000000000001\\
0.0508800034701355	0.928000000000001\\
0.0509737443277396	0.927000000000001\\
0.0511578386055533	0.926000000000001\\
0.0514904723991851	0.925000000000001\\
0.0517452716614385	0.924000000000001\\
0.0519867899214288	0.923000000000001\\
0.052202769618464	0.922000000000001\\
0.0523012463152684	0.921000000000001\\
0.0523933203982294	0.920000000000001\\
0.0526009334421936	0.919000000000001\\
0.0527511305204126	0.918000000000001\\
0.0528833714206314	0.917000000000001\\
0.0531027073748546	0.916000000000001\\
0.0534075462268122	0.915000000000001\\
0.0537512625987006	0.914000000000001\\
0.0539852348444682	0.913000000000001\\
0.0542135602756417	0.912000000000001\\
0.054338863408665	0.911000000000001\\
0.0544283511562654	0.910000000000001\\
0.0546359433420743	0.909000000000001\\
0.0547300317493062	0.908000000000001\\
0.0548212792842359	0.907000000000001\\
0.0549252529444506	0.906000000000001\\
0.0551042305927079	0.905000000000001\\
0.0552125797144424	0.904000000000001\\
0.055322316831162	0.903000000000001\\
0.0556242302843246	0.902000000000001\\
0.0557998650742053	0.901000000000001\\
0.055999469726443	0.900000000000001\\
0.0562462071314491	0.899000000000001\\
0.056572562069618	0.898000000000001\\
0.0567718809307446	0.897000000000001\\
0.0569830240418096	0.896000000000001\\
0.0570781372787501	0.895000000000001\\
0.0572420106506109	0.894000000000001\\
0.0572810545174306	0.893000000000001\\
0.0574107620513682	0.892000000000001\\
0.0576318056643169	0.891000000000001\\
0.0578461867611279	0.890000000000001\\
0.058130387292921	0.889000000000001\\
0.0582669120440771	0.888000000000001\\
0.0584204769316806	0.887000000000001\\
0.0585928284628056	0.886000000000001\\
0.0587049938075136	0.885000000000001\\
0.0590059322720746	0.884000000000001\\
0.0591466996081228	0.883000000000001\\
0.0592676981535683	0.882000000000001\\
0.0593992262165593	0.881000000000001\\
0.0594661445582179	0.880000000000001\\
0.0597614201903491	0.879000000000001\\
0.0600342902879546	0.878000000000001\\
0.0602606495001364	0.877000000000001\\
0.0604334699413439	0.876000000000001\\
0.0605489404713238	0.875000000000001\\
0.0608051641417552	0.874000000000001\\
0.0609876079530432	0.873000000000001\\
0.0610793423778779	0.872000000000001\\
0.061273048481267	0.871000000000001\\
0.0613232990497638	0.870000000000001\\
0.0615129546502866	0.869000000000001\\
0.0616871676945273	0.868000000000002\\
0.0618332421639148	0.867000000000001\\
0.0621124126883665	0.866000000000001\\
0.0623913201976055	0.865000000000001\\
0.06255919118905	0.864000000000001\\
0.0627639494065459	0.863000000000001\\
0.0628888417406868	0.862000000000002\\
0.0630525190164084	0.861000000000002\\
0.063298479815591	0.860000000000001\\
0.0634741128419496	0.859000000000001\\
0.0636473642578913	0.858000000000001\\
0.0638221375175318	0.857000000000001\\
0.0638686229767809	0.856000000000001\\
0.0641228228144298	0.855000000000002\\
0.0643125985697441	0.854000000000002\\
0.0644462423258393	0.853000000000001\\
0.0645860404323141	0.852000000000001\\
0.0647532910398118	0.851000000000001\\
0.0648367719968188	0.850000000000001\\
0.0649881100884924	0.849000000000001\\
0.0651872569136249	0.848000000000001\\
0.0652736427328197	0.847000000000001\\
0.0655691058117571	0.846000000000001\\
0.0656584444611978	0.845000000000001\\
0.0657736812934335	0.844000000000001\\
0.0659605862081218	0.843000000000001\\
0.0660849499048536	0.842000000000001\\
0.066364671757328	0.841000000000001\\
0.066544179341392	0.840000000000001\\
0.0667001765900297	0.839000000000001\\
0.0669291906982404	0.838000000000002\\
0.0670296735889203	0.837000000000002\\
0.0671649251012743	0.836000000000002\\
0.0673569747258259	0.835000000000001\\
0.0674513870465218	0.834000000000001\\
0.0676296844297209	0.833000000000001\\
0.0678943476832459	0.832000000000001\\
0.0680281950084408	0.831000000000001\\
0.0681782149135132	0.830000000000001\\
0.0683729685315369	0.829000000000001\\
0.0685133300173582	0.828000000000001\\
0.0686185434667854	0.827000000000001\\
0.0687517744553034	0.826000000000002\\
0.0688589270125705	0.825000000000002\\
0.0690508749277098	0.824000000000002\\
0.0692528839718403	0.823000000000002\\
0.0693379243967079	0.822000000000002\\
0.0695185665982595	0.821000000000002\\
0.0697868085493185	0.820000000000002\\
0.0698914189787351	0.819000000000002\\
0.070083193748287	0.818000000000002\\
0.0702096425480791	0.817000000000002\\
0.0703327119092276	0.816000000000002\\
0.0704721496255612	0.815000000000002\\
0.0706327422371648	0.814000000000002\\
0.0707869798830435	0.813000000000002\\
0.0711084161696322	0.812000000000002\\
0.0711479825649932	0.811000000000002\\
0.0712905417627574	0.810000000000002\\
0.0714581006079262	0.809000000000002\\
0.0716086910544135	0.808000000000002\\
0.0718444728313122	0.807000000000002\\
0.0720459812192418	0.806000000000002\\
0.0722550556476416	0.805000000000002\\
0.0724275580021294	0.804000000000002\\
0.0725898834842334	0.803000000000002\\
0.0728092312721772	0.802000000000002\\
0.0728756704140774	0.801000000000002\\
0.0730639748674362	0.800000000000002\\
0.0731412496474245	0.799000000000002\\
0.0732360252638087	0.798000000000002\\
0.0733609134745651	0.797000000000002\\
0.0736452449601084	0.796000000000002\\
0.0736924603248227	0.795000000000002\\
0.0738595083354638	0.794000000000002\\
0.0740124637334492	0.793000000000002\\
0.0740894235786881	0.792000000000002\\
0.0742757379845264	0.791000000000002\\
0.0744576783669368	0.790000000000002\\
0.0745321092778407	0.789000000000002\\
0.0747069669727796	0.788000000000002\\
0.074850427193638	0.787000000000002\\
0.074985602651747	0.786000000000002\\
0.0751104713803495	0.785000000000002\\
0.0752210490759332	0.784000000000002\\
0.0754074276222254	0.783000000000002\\
0.0755204809792553	0.782000000000002\\
0.0756807480808824	0.781000000000002\\
0.0758313239515064	0.780000000000002\\
0.0759846552240972	0.779000000000002\\
0.0761383412256614	0.778000000000002\\
0.0762494314807202	0.777000000000002\\
0.0764570934443114	0.776000000000002\\
0.0766415644208781	0.775000000000002\\
0.0766735623415471	0.774000000000002\\
0.0768054674230752	0.773000000000002\\
0.0768922522170995	0.772000000000002\\
0.0770629931978344	0.771000000000003\\
0.0771254784015096	0.770000000000003\\
0.0772582925818284	0.769000000000003\\
0.077422708535118	0.768000000000003\\
0.0776595787155624	0.767000000000003\\
0.0777522838882922	0.766000000000003\\
0.0778116584010762	0.765000000000003\\
0.0779988845646395	0.764000000000003\\
0.0782056396079814	0.763000000000003\\
0.0783833279057558	0.762000000000003\\
0.0784755846377884	0.761000000000003\\
0.0785157104605668	0.760000000000003\\
0.0785820676449355	0.759000000000003\\
0.078640565158117	0.758000000000003\\
0.0787933589078113	0.757000000000003\\
0.0789110633093357	0.756000000000003\\
0.0790434256091182	0.755000000000004\\
0.0791299595595105	0.754000000000004\\
0.079210945768199	0.753000000000004\\
0.0793775264625919	0.752000000000004\\
0.0795228097844545	0.751000000000004\\
0.0795852919824798	0.750000000000004\\
0.0797351342783282	0.749000000000004\\
0.07984252116775	0.748000000000004\\
0.0799631343170075	0.747000000000004\\
0.080037462754485	0.746000000000004\\
0.0801160582719576	0.745000000000004\\
0.0801589900629193	0.744000000000004\\
0.0803047811103022	0.743000000000004\\
0.0804249547861374	0.742000000000004\\
0.0806220018426233	0.741000000000004\\
0.0807103024839418	0.740000000000004\\
0.0807877778211004	0.739000000000004\\
0.0808922826456993	0.738000000000005\\
0.0809560778592022	0.737000000000005\\
0.0810978140273111	0.736000000000005\\
0.0811675840087992	0.735000000000005\\
0.081312172072543	0.734000000000005\\
0.0814155056225313	0.733000000000005\\
0.0815835667303622	0.732000000000005\\
0.0816728010108561	0.731000000000005\\
0.0817045729361273	0.730000000000005\\
0.0817287438038854	0.729000000000005\\
0.0818011922787603	0.728000000000005\\
0.0819694397100135	0.727000000000005\\
0.0820527586816173	0.726000000000005\\
0.082141902132698	0.725000000000006\\
0.0823165425879297	0.724000000000006\\
0.0824300907106459	0.723000000000006\\
0.0824952875950456	0.722000000000006\\
0.0825716520256155	0.721000000000006\\
0.0829039463094095	0.720000000000006\\
0.0829787339592725	0.719000000000006\\
0.0830608188164763	0.718000000000006\\
0.0831419084107953	0.717000000000006\\
0.0832189513109011	0.716000000000006\\
0.0833246189767955	0.715000000000006\\
0.0836362512495428	0.714000000000006\\
0.0838264481787346	0.713000000000006\\
0.0839364194880442	0.712000000000006\\
0.0840694956217963	0.711000000000006\\
0.0842468400427362	0.710000000000006\\
0.0843023314743384	0.709000000000006\\
0.084471795750289	0.708000000000006\\
0.0844975239341219	0.707000000000007\\
0.0846453175219932	0.706000000000007\\
0.0847030408994551	0.705000000000007\\
0.0848207251997433	0.704000000000007\\
0.0850025115561589	0.703000000000007\\
0.0852489403348154	0.702000000000007\\
0.0854407276113352	0.701000000000007\\
0.0855222231669757	0.700000000000007\\
0.0856748682370744	0.699000000000007\\
0.0858379707268283	0.698000000000007\\
0.0858623335581222	0.697000000000007\\
0.0859728718184884	0.696000000000007\\
0.0861335318871709	0.695000000000007\\
0.0862160912647176	0.694000000000007\\
0.0863206529364857	0.693000000000007\\
0.0864179689747835	0.692000000000007\\
0.0867123700178808	0.691000000000007\\
0.0867462813055476	0.690000000000007\\
0.0868645544147423	0.689000000000007\\
0.0869625556166012	0.688000000000007\\
0.087076974033907	0.687000000000007\\
0.0872391935549825	0.686000000000007\\
0.0874595575505797	0.685000000000007\\
0.0875706187422577	0.684000000000007\\
0.0876804729002482	0.683000000000007\\
0.08778329669268	0.682000000000007\\
0.087887593218016	0.681000000000007\\
0.0879334654868315	0.680000000000007\\
0.0881789125658253	0.679000000000008\\
0.088281308206485	0.678000000000008\\
0.0885327186856662	0.677000000000008\\
0.0886600706053402	0.676000000000008\\
0.0888072759398378	0.675000000000008\\
0.0890261536505536	0.674000000000008\\
0.0890920699847655	0.673000000000008\\
0.0892776942648534	0.672000000000008\\
0.0894120940369112	0.671000000000008\\
0.089625525624251	0.670000000000008\\
0.0898424178057275	0.669000000000008\\
0.0899349361077959	0.668000000000008\\
0.0899768936525071	0.667000000000008\\
0.090110362779766	0.666000000000008\\
0.0901408105141364	0.665000000000008\\
0.0902350749464931	0.664000000000008\\
0.0903171277803748	0.663000000000009\\
0.0904154023742476	0.662000000000009\\
0.0904684141101808	0.661000000000009\\
0.0905617840508252	0.660000000000009\\
0.0906997852111256	0.659000000000009\\
0.0908208396962784	0.658000000000009\\
0.0909315034711532	0.657000000000009\\
0.0910386673574315	0.656000000000009\\
0.0912496921805001	0.655000000000009\\
0.0914156912562026	0.654000000000009\\
0.0915832009844502	0.653000000000009\\
0.0918282569379224	0.652000000000009\\
0.0918845049523837	0.651000000000009\\
0.0920117922862093	0.650000000000009\\
0.0921634977080603	0.649000000000009\\
0.0923347818844135	0.64800000000001\\
0.0924343682930625	0.64700000000001\\
0.0925782231316908	0.64600000000001\\
0.0926425554042306	0.64500000000001\\
0.0927223064622985	0.64400000000001\\
0.092886794309299	0.64300000000001\\
0.0929815136979654	0.64200000000001\\
0.0930788029731778	0.64100000000001\\
0.0931431006697402	0.64000000000001\\
0.0932666021128726	0.63900000000001\\
0.0934462521837067	0.63800000000001\\
0.0935572330212554	0.63700000000001\\
0.0937384737803449	0.63600000000001\\
0.0938957149687017	0.63500000000001\\
0.0940419476817117	0.63400000000001\\
0.0942185307840757	0.63300000000001\\
0.0943181099168325	0.63200000000001\\
0.0943969961249429	0.63100000000001\\
0.094530579290226	0.630000000000011\\
0.0946267141548903	0.629000000000011\\
0.0947555351650526	0.628000000000011\\
0.0949404176569328	0.627000000000011\\
0.0950246172945388	0.626000000000011\\
0.0951107467573497	0.625000000000011\\
0.09521861702721	0.624000000000011\\
0.0953906260987769	0.623000000000011\\
0.0955587024652718	0.622000000000011\\
0.0957056324623813	0.621000000000011\\
0.0958060749601736	0.620000000000011\\
0.0959065923405781	0.619000000000011\\
0.0959590131837333	0.618000000000011\\
0.0960583127704606	0.617000000000011\\
0.0962608261299645	0.616000000000012\\
0.0963373974311141	0.615000000000012\\
0.0964888184830323	0.614000000000012\\
0.0966038055440991	0.613000000000012\\
0.0967702821412762	0.612000000000012\\
0.0969660474634956	0.611000000000012\\
0.097067195976488	0.610000000000012\\
0.0972751912978059	0.609000000000012\\
0.0974236036199522	0.608000000000012\\
0.0975474003041397	0.607000000000012\\
0.0976282373515425	0.606000000000012\\
0.0977313065590486	0.605000000000013\\
0.0978931448089796	0.604000000000013\\
0.09801511652868	0.603000000000013\\
0.0981036211441486	0.602000000000013\\
0.0983432996740729	0.601000000000013\\
0.0985009824177944	0.600000000000013\\
0.0985674349660675	0.599000000000013\\
0.0985928570001762	0.598000000000013\\
0.0987213638195349	0.597000000000013\\
0.0989852383051902	0.596000000000013\\
0.0991062199711269	0.595000000000013\\
0.099184037642328	0.594000000000014\\
0.0993656970512693	0.593000000000014\\
0.099676563243942	0.592000000000014\\
0.0998913219136837	0.591000000000014\\
0.100072470593366	0.590000000000014\\
0.100127862057472	0.589000000000014\\
0.100374147513629	0.588000000000014\\
0.10053258461061	0.587000000000014\\
0.100695317252946	0.586000000000014\\
0.100808895913243	0.585000000000014\\
0.100887122207769	0.584000000000014\\
0.1009938721284	0.583000000000015\\
0.101309391710367	0.582000000000015\\
0.10139328541491	0.581000000000015\\
0.101592128786671	0.580000000000015\\
0.101727527892937	0.579000000000015\\
0.101868261685893	0.578000000000015\\
0.101976379156943	0.577000000000015\\
0.102205002184454	0.576000000000015\\
0.102280014333758	0.575000000000015\\
0.102522596089442	0.574000000000015\\
0.102588753657503	0.573000000000015\\
0.102730433683611	0.572000000000015\\
0.102812317834061	0.571000000000015\\
0.102970107368641	0.570000000000015\\
0.103042016457668	0.569000000000015\\
0.103327936835981	0.568000000000016\\
0.103406519491483	0.567000000000015\\
0.103631113898621	0.566000000000016\\
0.103828735114492	0.565000000000016\\
0.103927827448041	0.564000000000016\\
0.104008316459653	0.563000000000016\\
0.104091387340414	0.562000000000016\\
0.104488700814601	0.561000000000016\\
0.104554535016842	0.560000000000016\\
0.104681079273932	0.559000000000016\\
0.104852926581034	0.558000000000016\\
0.105162238755213	0.557000000000017\\
0.105212228941373	0.556000000000017\\
0.105386058704197	0.555000000000017\\
0.105602798221474	0.554000000000017\\
0.10586859793722	0.553000000000017\\
0.105926184835974	0.552000000000017\\
0.106021114325479	0.551000000000017\\
0.106110224209852	0.550000000000017\\
0.106218785841696	0.549000000000017\\
0.106406689474572	0.548000000000017\\
0.10656268037218	0.547000000000018\\
0.106679330240875	0.546000000000018\\
0.106771072498395	0.545000000000018\\
0.106884156437993	0.544000000000018\\
0.106999169306761	0.543000000000018\\
0.107038872201266	0.542000000000018\\
0.107077381387553	0.541000000000018\\
0.107212187366065	0.540000000000018\\
0.107287275235346	0.539000000000018\\
0.107341782291466	0.538000000000018\\
0.10751324883365	0.537000000000018\\
0.107610588125868	0.536000000000018\\
0.1077197382993	0.535000000000018\\
0.107875416329037	0.534000000000018\\
0.10793623088425	0.533000000000018\\
0.108052571138783	0.532000000000018\\
0.108138020237042	0.531000000000018\\
0.108248263807164	0.530000000000019\\
0.108280331119306	0.529000000000019\\
0.108445314836705	0.528000000000019\\
0.108561547575855	0.527000000000019\\
0.108638463522754	0.526000000000019\\
0.10880111448164	0.525000000000019\\
0.109012240594052	0.524000000000019\\
0.109165023806214	0.523000000000019\\
0.109319485767396	0.522000000000019\\
0.109373066963075	0.521000000000019\\
0.109542012144811	0.520000000000019\\
0.109676858829746	0.519000000000019\\
0.109756019072294	0.518000000000019\\
0.10983177680587	0.51700000000002\\
0.109918307136577	0.51600000000002\\
0.110082150182974	0.51500000000002\\
0.110382192634598	0.51400000000002\\
0.110565417451403	0.51300000000002\\
0.110714433180257	0.51200000000002\\
0.110786057116094	0.51100000000002\\
0.110949733339133	0.51000000000002\\
0.111010440042381	0.50900000000002\\
0.111173516649048	0.50800000000002\\
0.111264119993785	0.507000000000021\\
0.111408335567968	0.506000000000021\\
0.111494619674856	0.505000000000021\\
0.111612038985372	0.504000000000021\\
0.111712532311806	0.503000000000021\\
0.111858577117781	0.502000000000021\\
0.111969956622785	0.501000000000021\\
0.112103086952102	0.500000000000021\\
0.112232927522069	0.499000000000021\\
0.112299908466357	0.498000000000021\\
0.112368932468397	0.497000000000021\\
0.112548965852898	0.496000000000021\\
0.112760325364501	0.495000000000021\\
0.112847683532425	0.494000000000021\\
0.11313100783849	0.493000000000021\\
0.113298601496836	0.492000000000021\\
0.113376081896723	0.491000000000021\\
0.113631404308902	0.490000000000021\\
0.113768631291498	0.489000000000021\\
0.113921263482196	0.488000000000021\\
0.11407554441994	0.487000000000021\\
0.114204291920245	0.48600000000002\\
0.114248803427173	0.48500000000002\\
0.1143911394954	0.48400000000002\\
0.114507405255278	0.483000000000021\\
0.114562994439629	0.48200000000002\\
0.11474840102968	0.48100000000002\\
0.114807451772203	0.48000000000002\\
0.114958390735284	0.47900000000002\\
0.115106571490349	0.47800000000002\\
0.115251051905302	0.47700000000002\\
0.115365512627636	0.47600000000002\\
0.115508078547642	0.47500000000002\\
0.115770443057022	0.47400000000002\\
0.115861907174241	0.47300000000002\\
0.11593382899432	0.47200000000002\\
0.116060030805618	0.47100000000002\\
0.116145580284102	0.47000000000002\\
0.116408388349688	0.46900000000002\\
0.116471425173665	0.46800000000002\\
0.116703176634911	0.46700000000002\\
0.116778476869699	0.46600000000002\\
0.116856321478499	0.46500000000002\\
0.117012681639905	0.464000000000019\\
0.117086967084848	0.463000000000019\\
0.117190573427642	0.462000000000019\\
0.117370351337416	0.461000000000019\\
0.11752326235475	0.460000000000019\\
0.117781022409827	0.459000000000019\\
0.117875974168453	0.458000000000019\\
0.118032885902975	0.457000000000019\\
0.118262865093181	0.456000000000019\\
0.118478228903076	0.455000000000019\\
0.118572620145916	0.454000000000019\\
0.118742315605059	0.453000000000019\\
0.118798086729977	0.452000000000019\\
0.119028066615243	0.451000000000019\\
0.11915728307313	0.450000000000019\\
0.119340128938027	0.449000000000019\\
0.119414025352942	0.448000000000019\\
0.119541364226052	0.447000000000019\\
0.119731160881677	0.446000000000019\\
0.119842555832074	0.445000000000019\\
0.120020835821861	0.444000000000019\\
0.120267438787865	0.443000000000019\\
0.120541479914809	0.442000000000019\\
0.120655007212906	0.441000000000019\\
0.120838334944684	0.440000000000019\\
0.120877421618558	0.439000000000018\\
0.121006566071928	0.438000000000018\\
0.121240319764975	0.437000000000018\\
0.121466741266701	0.436000000000018\\
0.121718952010594	0.435000000000018\\
0.121828346896119	0.434000000000018\\
0.121926125199638	0.433000000000018\\
0.122145965072998	0.432000000000018\\
0.122208644188106	0.431000000000018\\
0.122356727699423	0.430000000000018\\
0.122507550921443	0.429000000000018\\
0.122687946764075	0.428000000000018\\
0.122776276104308	0.427000000000018\\
0.123004984581264	0.426000000000018\\
0.123134606541002	0.425000000000018\\
0.123188680023589	0.424000000000018\\
0.123283262460353	0.423000000000018\\
0.123611589205609	0.422000000000018\\
0.123798501881816	0.421000000000018\\
0.123886469813484	0.420000000000017\\
0.123944003616969	0.419000000000018\\
0.124098059807652	0.418000000000017\\
0.12427129977547	0.417000000000018\\
0.124399840977814	0.416000000000017\\
0.12455614005569	0.415000000000017\\
0.124663857920112	0.414000000000017\\
0.124798735834721	0.413000000000017\\
0.124929471078784	0.412000000000017\\
0.125001602548755	0.411000000000017\\
0.125080683126968	0.410000000000017\\
0.125230097803733	0.409000000000017\\
0.125391346835029	0.408000000000017\\
0.125595701623431	0.407000000000017\\
0.12574804884408	0.406000000000017\\
0.125938450464266	0.405000000000017\\
0.126316604064119	0.404000000000017\\
0.126443416931196	0.403000000000017\\
0.126596503215807	0.402000000000017\\
0.126771125583544	0.401000000000017\\
0.127043780888085	0.400000000000017\\
0.127293845732218	0.399000000000017\\
0.127401387303348	0.398000000000016\\
0.127675878075608	0.397000000000016\\
0.127750568511223	0.396000000000016\\
0.128047471559795	0.395000000000016\\
0.12813356042932	0.394000000000016\\
0.128226050337777	0.393000000000016\\
0.128412301502425	0.392000000000016\\
0.128496415124951	0.391000000000016\\
0.128686634182015	0.390000000000016\\
0.128934978808476	0.389000000000016\\
0.129191079882404	0.388000000000016\\
0.129306230429464	0.387000000000016\\
0.129359943981663	0.386000000000016\\
0.129511237282792	0.385000000000016\\
0.129608455477593	0.384000000000016\\
0.129795287921729	0.383000000000016\\
0.130024075834731	0.382000000000016\\
0.130096264841924	0.381000000000016\\
0.130291807144332	0.380000000000016\\
0.13037786732312	0.379000000000016\\
0.130591127448633	0.378000000000016\\
0.130793240357344	0.377000000000016\\
0.130964871137643	0.376000000000016\\
0.131166805127236	0.375000000000016\\
0.13128230684662	0.374000000000015\\
0.131478322540625	0.373000000000015\\
0.13166159739887	0.372000000000015\\
0.131775234381818	0.371000000000015\\
0.13197767826682	0.370000000000015\\
0.132113815253868	0.369000000000015\\
0.132237627124466	0.368000000000015\\
0.132434127594324	0.367000000000015\\
0.132660893583233	0.366000000000015\\
0.132828199692995	0.365000000000015\\
0.132961809486537	0.364000000000015\\
0.133045846644127	0.363000000000015\\
0.133176830465418	0.362000000000015\\
0.133435910779144	0.361000000000015\\
0.133545340679006	0.360000000000015\\
0.133802892962416	0.359000000000015\\
0.134053075614359	0.358000000000015\\
0.134232622911905	0.357000000000015\\
0.134380676026424	0.356000000000015\\
0.134598713681831	0.355000000000015\\
0.134756609056581	0.354000000000015\\
0.134856306273511	0.353000000000015\\
0.135060697074667	0.352000000000015\\
0.135151026881733	0.351000000000015\\
0.135335101495206	0.350000000000015\\
0.135598031996767	0.349000000000014\\
0.135709272051946	0.348000000000014\\
0.135861760068555	0.347000000000014\\
0.13595473474162	0.346000000000014\\
0.136063910386514	0.345000000000014\\
0.136124988064503	0.344000000000014\\
0.136187941034926	0.343000000000014\\
0.136359264327217	0.342000000000014\\
0.136418312096935	0.341000000000014\\
0.136488156903561	0.340000000000014\\
0.136685683930699	0.339000000000014\\
0.136826674556329	0.338000000000014\\
0.136890451113299	0.337000000000014\\
0.137044786411256	0.336000000000014\\
0.137192420683493	0.335000000000014\\
0.137327713545375	0.334000000000014\\
0.137742511267834	0.333000000000014\\
0.137816667207091	0.332000000000013\\
0.137979535496234	0.331000000000013\\
0.138270739984677	0.330000000000013\\
0.138569534167538	0.329000000000013\\
0.139003133943015	0.328000000000013\\
0.139131257119838	0.327000000000013\\
0.139401456656994	0.326000000000013\\
0.139499346694055	0.325000000000013\\
0.139621970048572	0.324000000000013\\
0.13989341763632	0.323000000000013\\
0.140058062862427	0.322000000000013\\
0.140311733808546	0.321000000000013\\
0.140386281670319	0.320000000000012\\
0.140464653341256	0.319000000000012\\
0.14060721375546	0.318000000000012\\
0.14092683647331	0.317000000000012\\
0.141179154952917	0.316000000000012\\
0.141344837630848	0.315000000000012\\
0.141609463466166	0.314000000000012\\
0.141790387710695	0.313000000000012\\
0.141952536996124	0.312000000000012\\
0.14206731848338	0.311000000000012\\
0.142257498934389	0.310000000000012\\
0.142490223710838	0.309000000000012\\
0.142796856416344	0.308000000000012\\
0.143008474898981	0.307000000000012\\
0.143195441111357	0.306000000000012\\
0.143373464076831	0.305000000000012\\
0.143473546654273	0.304000000000012\\
0.143545148433589	0.303000000000012\\
0.143637330234722	0.302000000000012\\
0.143767479961261	0.301000000000012\\
0.143873585413593	0.300000000000012\\
0.143993365925026	0.299000000000011\\
0.144114098411316	0.298000000000011\\
0.144258630324047	0.297000000000011\\
0.144425071671095	0.296000000000011\\
0.144719131629907	0.295000000000011\\
0.144958892218547	0.294000000000011\\
0.145143425679131	0.293000000000011\\
0.145291608866873	0.292000000000011\\
0.145451862739295	0.291000000000011\\
0.145657848567547	0.290000000000011\\
0.145877336911887	0.289000000000011\\
0.146049214669611	0.288000000000011\\
0.1463454031739	0.287000000000011\\
0.146542334294847	0.28600000000001\\
0.146613223414896	0.28500000000001\\
0.146799606622313	0.28400000000001\\
0.147009622250971	0.28300000000001\\
0.147198995202602	0.28200000000001\\
0.147345573133936	0.28100000000001\\
0.147498392442402	0.28000000000001\\
0.14780598413679	0.27900000000001\\
0.147965474623678	0.27800000000001\\
0.148134266069082	0.27700000000001\\
0.148219344505639	0.27600000000001\\
0.148330378399106	0.27500000000001\\
0.148701421064256	0.27400000000001\\
0.148831510237173	0.27300000000001\\
0.148955586132592	0.27200000000001\\
0.149070846268492	0.27100000000001\\
0.14927301596061	0.27000000000001\\
0.149499045199855	0.26900000000001\\
0.149794149009436	0.26800000000001\\
0.150122836457341	0.26700000000001\\
0.150398203852343	0.26600000000001\\
0.150547937089771	0.26500000000001\\
0.150650165142706	0.26400000000001\\
0.150949423522946	0.263000000000009\\
0.15112534989759	0.262000000000009\\
0.15125760440008	0.261000000000009\\
0.151624238068591	0.260000000000009\\
0.151825611538097	0.259000000000009\\
0.152155033189004	0.258000000000009\\
0.152351581260757	0.257000000000009\\
0.152703346433843	0.256000000000009\\
0.153099800561741	0.255000000000009\\
0.153207193738016	0.254000000000009\\
0.153578976435572	0.253000000000009\\
0.154025940277483	0.252000000000009\\
0.154294356572559	0.251000000000009\\
0.154534010774802	0.250000000000009\\
0.154657467386763	0.249000000000009\\
0.154972891836967	0.248000000000009\\
0.155183223293896	0.247000000000009\\
0.155418346777488	0.246000000000009\\
0.155808366507442	0.245000000000009\\
0.156043041536326	0.244000000000009\\
0.156206088599592	0.243000000000009\\
0.156356266071822	0.242000000000009\\
0.156445997285899	0.241000000000009\\
0.156630762260542	0.240000000000009\\
0.156925467377947	0.239000000000008\\
0.157361516706912	0.238000000000008\\
0.157441732163987	0.237000000000008\\
0.157838267744161	0.236000000000008\\
0.158122727223983	0.235000000000008\\
0.158317365983172	0.234000000000008\\
0.158501223394895	0.233000000000008\\
0.158656195722047	0.232000000000008\\
0.159117718198756	0.231000000000008\\
0.159372887888018	0.230000000000008\\
0.159555532178143	0.229000000000008\\
0.15982289634905	0.228000000000008\\
0.160095449902492	0.227000000000008\\
0.160263819638816	0.226000000000008\\
0.160818149773741	0.225000000000008\\
0.161134549859777	0.224000000000008\\
0.16127334762533	0.223000000000008\\
0.161532632963148	0.222000000000008\\
0.161774312501655	0.221000000000008\\
0.161930104881657	0.220000000000008\\
0.162425577802723	0.219000000000008\\
0.162818773024214	0.218000000000008\\
0.16317538114071	0.217000000000008\\
0.163548051914473	0.216000000000008\\
0.163717789796918	0.215000000000008\\
0.164126569235815	0.214000000000008\\
0.164272183882505	0.213000000000008\\
0.164382559748003	0.212000000000008\\
0.164566317984157	0.211000000000008\\
0.164786240310009	0.210000000000008\\
0.16502723769962	0.209000000000008\\
0.165277562075846	0.208000000000008\\
0.165512350087254	0.207000000000008\\
0.165711492095182	0.206000000000008\\
0.165965183914014	0.205000000000008\\
0.166395640427164	0.204000000000008\\
0.166708596075487	0.203000000000007\\
0.166992292329647	0.202000000000007\\
0.167320048474103	0.201000000000007\\
0.167644851064296	0.200000000000007\\
0.167871220375261	0.199000000000007\\
0.168446660985329	0.198000000000007\\
0.168652761541551	0.197000000000007\\
0.168811950616215	0.196000000000007\\
0.169000402642334	0.195000000000007\\
0.169251035263031	0.194000000000007\\
0.169458041702405	0.193000000000007\\
0.169769938089007	0.192000000000007\\
0.169932803483856	0.191000000000007\\
0.170339938619911	0.190000000000007\\
0.170785811298709	0.189000000000007\\
0.171227184910394	0.188000000000007\\
0.171490248008009	0.187000000000007\\
0.171886511905038	0.186000000000007\\
0.172309775417684	0.185000000000007\\
0.172417811129659	0.184000000000007\\
0.172690149820422	0.183000000000007\\
0.173034412647253	0.182000000000007\\
0.173200908305157	0.181000000000007\\
0.173355334531188	0.180000000000007\\
0.173806903701858	0.179000000000007\\
0.174366714965439	0.178000000000007\\
0.174566954595783	0.177000000000007\\
0.174809843950677	0.176000000000007\\
0.175122354513147	0.175000000000007\\
0.175425976725569	0.174000000000007\\
0.175676625711945	0.173000000000007\\
0.175916962578011	0.172000000000007\\
0.176129978520741	0.171000000000006\\
0.176530684713122	0.170000000000006\\
0.17680031800126	0.169000000000006\\
0.177281924927897	0.168000000000006\\
0.177675288686738	0.167000000000006\\
0.177927389781892	0.166000000000006\\
0.178754095542111	0.165000000000006\\
0.179443795234908	0.164000000000006\\
0.180047004081533	0.163000000000006\\
0.18015614740788	0.162000000000006\\
0.180598262350843	0.161000000000006\\
0.180910074411287	0.160000000000006\\
0.181417902168856	0.159000000000006\\
0.182124388883111	0.158000000000006\\
0.182510882685847	0.157000000000006\\
0.18319564062093	0.156000000000006\\
0.183452167791796	0.155000000000006\\
0.183784103673057	0.154000000000006\\
0.18423164677739	0.153000000000006\\
0.18459026307898	0.152000000000006\\
0.184850187954959	0.151000000000006\\
0.185063195197568	0.150000000000006\\
0.185432005587529	0.149000000000006\\
0.185987372157063	0.148000000000006\\
0.186347917669034	0.147000000000006\\
0.186540501372672	0.146000000000006\\
0.187102993639484	0.145000000000006\\
0.187292189284714	0.144000000000006\\
0.187716509022442	0.143000000000006\\
0.188254664308281	0.142000000000006\\
0.188507272803394	0.141000000000006\\
0.189158435313312	0.140000000000006\\
0.189582046156031	0.139000000000006\\
0.189861052204591	0.138000000000006\\
0.190335160784501	0.137000000000006\\
0.190620994218233	0.136000000000005\\
0.190816911346785	0.135000000000005\\
0.191097313253905	0.134000000000005\\
0.191428032332185	0.133000000000005\\
0.192119546938152	0.132000000000005\\
0.192503515394147	0.131000000000005\\
0.192941280712148	0.130000000000005\\
0.193614030337923	0.129000000000005\\
0.193899320847094	0.128000000000005\\
0.19448056659778	0.127000000000005\\
0.195036987085228	0.126000000000005\\
0.195470840097069	0.125000000000005\\
0.195768721466571	0.124000000000005\\
0.196104281074917	0.123000000000005\\
0.196723643570824	0.122000000000005\\
0.197357316650495	0.121000000000005\\
0.198190585148357	0.120000000000005\\
0.198844313903159	0.119000000000005\\
0.199125899240422	0.118000000000005\\
0.19965181227919	0.117000000000005\\
0.200196187899606	0.116000000000005\\
0.200446756451897	0.115000000000005\\
0.20098610730995	0.114000000000005\\
0.201426847416772	0.113000000000005\\
0.201670621905931	0.112000000000005\\
0.202201976245976	0.111000000000005\\
0.202466325023093	0.110000000000005\\
0.202635769215511	0.109000000000005\\
0.203128369164416	0.108000000000005\\
0.203850290072386	0.107000000000005\\
0.204819044745844	0.106000000000004\\
0.205316608493589	0.105000000000004\\
0.205979170145322	0.104000000000004\\
0.206848746875078	0.103000000000004\\
0.207623415068016	0.102000000000004\\
0.208363212639356	0.101000000000004\\
0.208939672620161	0.100000000000004\\
0.209828320517869	0.0990000000000042\\
0.21000474011804	0.0980000000000041\\
0.210572994383825	0.0970000000000041\\
0.211419690587546	0.0960000000000041\\
0.212268703830771	0.095000000000004\\
0.212555009267969	0.094000000000004\\
0.213671509910918	0.093000000000004\\
0.214068815901457	0.0920000000000039\\
0.214318464907646	0.0910000000000039\\
0.214911659056426	0.0900000000000039\\
0.215179110285184	0.0890000000000037\\
0.215516489447413	0.0880000000000037\\
0.216765878142786	0.0870000000000037\\
0.217642130569281	0.0860000000000037\\
0.218195280865054	0.0850000000000036\\
0.219294943113844	0.0840000000000036\\
0.22014395251485	0.0830000000000036\\
0.220713495439887	0.0820000000000036\\
0.221158216204753	0.0810000000000035\\
0.221487188929582	0.0800000000000035\\
0.222178112704461	0.0790000000000035\\
0.222831710987268	0.0780000000000034\\
0.223425701567319	0.0770000000000034\\
0.223816840991447	0.0760000000000034\\
0.224901986652821	0.0750000000000034\\
0.226116456647775	0.0740000000000033\\
0.227058929405626	0.0730000000000033\\
0.22772174671557	0.0720000000000033\\
0.228538457876947	0.0710000000000033\\
0.229527599981817	0.0700000000000032\\
0.230200246652322	0.0690000000000032\\
0.230875135887859	0.0680000000000032\\
0.23152226120211	0.0670000000000031\\
0.232048195864483	0.0660000000000031\\
0.232470656085368	0.0650000000000031\\
0.233381956026846	0.0640000000000031\\
0.234384415001651	0.0630000000000029\\
0.235782054986474	0.0620000000000029\\
0.236270614988101	0.0610000000000029\\
0.236934557437619	0.0600000000000028\\
0.237517064810163	0.0590000000000028\\
0.238586841179905	0.0580000000000027\\
0.239279772153196	0.0570000000000027\\
0.241578077447509	0.0560000000000027\\
0.243259656127995	0.0550000000000026\\
0.243981917078244	0.0540000000000026\\
0.244792358032102	0.0530000000000025\\
0.245849618425614	0.0520000000000025\\
0.248213388425355	0.0510000000000024\\
0.250251903205275	0.0500000000000024\\
0.251990218565207	0.0490000000000024\\
0.254152651043796	0.0480000000000023\\
0.255473057515195	0.0470000000000023\\
0.257042109282529	0.0460000000000023\\
0.259334856084646	0.0450000000000021\\
0.259547912211176	0.0440000000000021\\
0.26076272532037	0.0430000000000021\\
0.261764804373418	0.042000000000002\\
0.262383163484584	0.041000000000002\\
0.265786456436554	0.0400000000000019\\
0.267257936710202	0.0390000000000019\\
0.268415699386236	0.0380000000000018\\
0.269459611268782	0.0370000000000018\\
0.270761089375344	0.0360000000000017\\
0.276050457807973	0.0350000000000017\\
0.277535091294387	0.0340000000000017\\
0.280534080950497	0.0330000000000016\\
0.284101322853031	0.0320000000000016\\
0.287158499856468	0.0310000000000015\\
0.289376168672598	0.0300000000000015\\
0.290238927107002	0.0290000000000014\\
0.292907235616769	0.0280000000000014\\
0.296821888260454	0.0270000000000014\\
0.301423239670587	0.0260000000000012\\
0.307026023072487	0.0250000000000012\\
0.310094456384535	0.0240000000000011\\
0.311118704011314	0.0230000000000011\\
0.313585448338207	0.0220000000000011\\
0.31743542641871	0.021000000000001\\
0.323708608207357	0.020000000000001\\
0.32729713257042	0.0190000000000009\\
0.331697476996142	0.0180000000000009\\
0.334796634943001	0.0170000000000008\\
0.341281835134675	0.0160000000000008\\
0.346766619016718	0.0150000000000008\\
0.350933640831662	0.0140000000000007\\
0.355507157340918	0.0130000000000007\\
0.362545264479673	0.0120000000000006\\
0.368451506439122	0.0110000000000006\\
0.374874351500414	0.0100000000000005\\
0.385154586871104	0.00900000000000045\\
0.391136062804896	0.00800000000000045\\
0.40075229547609	0.00700000000000034\\
0.413788621171867	0.00600000000000034\\
0.434841491248191	0.00500000000000023\\
0.449663503957686	0.00400000000000023\\
0.490223989750752	0.00300000000000011\\
0.565241699664405	0.00200000000000011\\
1.35689293601357	0.001\\
102.870072631472	0\\
};
\addlegendentry{$K=50$, $G=11$, $\lrmse =1.945$, $\prmse =0.013$, $\armse =0.004$, $\brmse =3\hspace{-3pt}\times\hspace{-3pt}10^{-5}$, $\gamma=40$}


==> figures/mse_N_3_K_20_G_5_SNR_1000_I_20_Pratio_2_Nratio_2_alpha_2_cs.tex <==
\addplot [color=green,line width=0.6pt]
  table[row sep=crcr]{%
2.66936731587288	1\\
21.9576529804951	0.997009569377991\\
31.3704254827051	0.994019138755981\\
40.8472140860817	0.991028708133971\\
55.7647992741641	0.988038277511962\\
59.5587963204456	0.985047846889952\\
67.2562768908865	0.982057416267943\\
75.3214132616101	0.979066985645933\\
86.3842738463209	0.976076555023924\\
94.0192174331755	0.973086124401914\\
98.8988653483051	0.970095693779905\\
103.177663244121	0.967105263157895\\
109.785017218267	0.964114832535885\\
116.068077409561	0.961124401913876\\
119.884262039874	0.958133971291866\\
124.921573899942	0.955143540669857\\
130.758783084533	0.952153110047847\\
135.055933481833	0.949162679425838\\
139.518501496416	0.946172248803828\\
147.046446232253	0.943181818181818\\
151.817883707906	0.940191387559809\\
157.99357971992	0.937200956937799\\
164.568155628235	0.934210526315789\\
167.517667125576	0.93122009569378\\
171.580137489093	0.92822966507177\\
173.924318707804	0.92523923444976\\
178.430043984247	0.922248803827751\\
183.570239184474	0.919258373205741\\
186.375415179303	0.916267942583731\\
189.485805678981	0.913277511961722\\
194.93099235244	0.910287081339712\\
198.323098249864	0.907296650717702\\
202.901474427983	0.904306220095693\\
205.994512216748	0.901315789473683\\
208.997930900035	0.898325358851674\\
212.203783899021	0.895334928229664\\
214.813484334153	0.892344497607654\\
220.083307211433	0.889354066985645\\
224.457829034859	0.886363636363635\\
227.707729084259	0.883373205741625\\
232.063145132325	0.880382775119616\\
234.639241378032	0.877392344497606\\
237.584138103273	0.874401913875597\\
241.348798059249	0.871411483253587\\
245.705508604968	0.868421052631577\\
247.623545907115	0.865430622009568\\
250.518072323887	0.862440191387558\\
254.886578428823	0.859449760765548\\
259.507776403714	0.856459330143539\\
264.291714264024	0.853468899521529\\
266.715150343754	0.850478468899519\\
270.529951693266	0.84748803827751\\
274.487019676504	0.8444976076555\\
280.876181103551	0.84150717703349\\
284.910234242987	0.838516746411481\\
289.894006832707	0.835526315789471\\
293.251915454906	0.832535885167461\\
298.183620160876	0.829545454545452\\
304.464280444891	0.826555023923442\\
308.644659306487	0.823564593301432\\
312.28694110398	0.820574162679423\\
315.519130136048	0.817583732057413\\
319.728764485132	0.814593301435403\\
324.032167332271	0.811602870813394\\
329.114814924553	0.808612440191384\\
335.618613432232	0.805622009569374\\
340.980457026963	0.802631578947365\\
346.574201716486	0.799641148325355\\
354.312156984092	0.796650717703346\\
357.354987636779	0.793660287081336\\
367.057437005045	0.790669856459326\\
373.370557452102	0.787679425837317\\
383.392580733707	0.784688995215307\\
388.994894976927	0.781698564593297\\
398.728823822875	0.778708133971288\\
405.809935062567	0.775717703349278\\
409.448001694007	0.772727272727268\\
424.886270012764	0.769736842105259\\
431.918224398888	0.766746411483249\\
437.327561228341	0.763755980861239\\
443.808811325	0.76076555023923\\
452.08801052923	0.75777511961722\\
458.161912093496	0.75478468899521\\
464.801000554817	0.751794258373201\\
472.565397342569	0.748803827751191\\
481.651928628041	0.745813397129181\\
486.665124335847	0.742822966507172\\
492.717617128283	0.739832535885162\\
500.6246731073	0.736842105263152\\
509.950907507863	0.733851674641143\\
517.928149919043	0.730861244019133\\
524.12744366118	0.727870813397123\\
531.644779957829	0.724880382775114\\
539.902866605712	0.721889952153104\\
550.924791880651	0.718899521531094\\
559.092803340129	0.715909090909085\\
569.23638158086	0.712918660287075\\
576.946652067266	0.709928229665066\\
585.351376431543	0.706937799043056\\
592.923789933441	0.703947368421046\\
598.24405426576	0.700956937799037\\
609.278370300935	0.697966507177027\\
621.458741206426	0.694976076555017\\
625.48068300589	0.691985645933008\\
632.438802651955	0.688995215310998\\
639.929388525829	0.686004784688988\\
646.214005127073	0.683014354066979\\
654.915169132035	0.680023923444969\\
661.546861568809	0.677033492822959\\
668.432582685019	0.67404306220095\\
675.161206044011	0.67105263157894\\
682.767725837431	0.66806220095693\\
687.798256704773	0.665071770334921\\
695.4719674423	0.662081339712911\\
702.823095914327	0.659090909090901\\
707.185854548255	0.656100478468892\\
713.852677696448	0.653110047846882\\
719.188998284359	0.650119617224872\\
723.815430000696	0.647129186602863\\
729.541301661811	0.644138755980853\\
733.461410032639	0.641148325358843\\
737.339755173741	0.638157894736834\\
741.466828115274	0.635167464114824\\
747.336444843757	0.632177033492815\\
752.489889767611	0.629186602870805\\
758.723007066955	0.626196172248795\\
764.274401334113	0.623205741626786\\
768.40624352522	0.620215311004776\\
772.610842639771	0.617224880382766\\
776.723177639699	0.614234449760757\\
784.00768175424	0.611244019138747\\
787.658647695016	0.608253588516737\\
791.10208843083	0.605263157894728\\
798.262323124445	0.602272727272718\\
804.189467329148	0.599282296650708\\
810.589088859669	0.596291866028699\\
815.696945155686	0.593301435406689\\
818.543263197943	0.590311004784679\\
825.343439120686	0.58732057416267\\
830.282150121148	0.58433014354066\\
835.697244099041	0.58133971291865\\
838.815730700318	0.578349282296641\\
846.405673108727	0.575358851674631\\
849.797008278473	0.572368421052621\\
855.001572591151	0.569377990430612\\
858.369823254662	0.566387559808602\\
865.488354016254	0.563397129186592\\
869.366296557199	0.560406698564583\\
873.36271650858	0.557416267942573\\
878.846713055697	0.554425837320563\\
881.680710879197	0.551435406698554\\
885.999461386728	0.548444976076544\\
889.453010489711	0.545454545454535\\
894.405887129793	0.542464114832525\\
902.254518346518	0.539473684210515\\
909.298635269176	0.536483253588506\\
913.410063201499	0.533492822966496\\
916.968346347665	0.530502392344486\\
922.593302130072	0.527511961722477\\
928.230766851681	0.524521531100467\\
932.5915176011	0.521531100478457\\
936.217539117032	0.518540669856448\\
939.435690576563	0.515550239234438\\
943.083012283431	0.512559808612428\\
946.301636124231	0.509569377990419\\
950.547787691911	0.506578947368409\\
955.509264164505	0.503588516746399\\
962.132099667518	0.50059808612439\\
968.316261585315	0.49760765550238\\
970.852888150362	0.494617224880371\\
973.895526561991	0.491626794258361\\
976.86253982543	0.488636363636352\\
982.420948482761	0.485645933014342\\
984.783141355794	0.482655502392332\\
986.933678012292	0.479665071770323\\
990.744758569531	0.476674641148313\\
993.140103777398	0.473684210526304\\
996.72859329752	0.470693779904294\\
1000.80934625891	0.467703349282285\\
1003.22563771308	0.464712918660275\\
1005.63178392253	0.461722488038266\\
1008.54565472557	0.458732057416256\\
1012.19223997061	0.455741626794247\\
1014.54968203252	0.452751196172237\\
1016.34250815631	0.449760765550228\\
1019.41733676167	0.446770334928218\\
1021.4157958024	0.443779904306209\\
1025.49009695709	0.440789473684199\\
1027.27041836949	0.437799043062189\\
1030.37001532113	0.43480861244018\\
1033.35056035384	0.43181818181817\\
1036.19207355483	0.428827751196161\\
1039.42162892698	0.425837320574151\\
1042.47674845886	0.422846889952142\\
1044.49846713146	0.419856459330132\\
1048.13087860776	0.416866028708123\\
1050.95388805059	0.413875598086113\\
1054.34320232647	0.410885167464104\\
1057.82666357988	0.407894736842094\\
1060.31153307825	0.404904306220085\\
1063.43976875478	0.401913875598075\\
1064.78900894578	0.398923444976066\\
1066.88401510299	0.395933014354056\\
1069.00925016912	0.392942583732047\\
1072.13576592185	0.389952153110037\\
1076.03852606079	0.386961722488028\\
1080.4029433535	0.383971291866018\\
1082.60024819948	0.380980861244008\\
1085.70967167449	0.377990430621999\\
1088.47514357466	0.374999999999989\\
1090.47778181371	0.37200956937798\\
1092.196928116	0.36901913875597\\
1095.16209796821	0.366028708133961\\
1096.45598854314	0.363038277511951\\
1097.77330946937	0.360047846889941\\
1100.25820406419	0.357057416267932\\
1103.1837493892	0.354066985645922\\
1105.73708037166	0.351076555023913\\
1107.74269385907	0.348086124401903\\
1109.71233466288	0.345095693779894\\
1110.88174128651	0.342105263157884\\
1112.47755113947	0.339114832535875\\
1113.58327015694	0.336124401913865\\
1115.99285733512	0.333133971291856\\
1117.40593757637	0.330143540669846\\
1118.84306785441	0.327153110047836\\
1120.93084955695	0.324162679425827\\
1122.86872189987	0.321172248803817\\
1123.7670175192	0.318181818181808\\
1127.3725742494	0.315191387559798\\
1128.84808656085	0.312200956937789\\
1131.15461184534	0.309210526315779\\
1132.79032056943	0.306220095693769\\
1135.20235579623	0.30322966507176\\
1137.09116206973	0.30023923444975\\
1139.21938087798	0.297248803827741\\
1140.7655505679	0.294258373205731\\
1142.17573672296	0.291267942583722\\
1144.64922955221	0.288277511961712\\
1146.78310812622	0.285287081339703\\
1149.4136857675	0.282296650717693\\
1153.460096944	0.279306220095684\\
1156.0260019216	0.276315789473674\\
1158.69910496894	0.273325358851665\\
1160.59025476963	0.270334928229655\\
1162.60496795016	0.267344497607646\\
1166.52547319778	0.264354066985636\\
1169.35063267645	0.261363636363627\\
1171.63204829024	0.258373205741617\\
1174.07828235448	0.255382775119608\\
1177.16159704924	0.252392344497598\\
1178.72210871859	0.249401913875589\\
1181.45697773667	0.246411483253579\\
1183.74421191244	0.24342105263157\\
1186.56053689572	0.24043062200956\\
1188.44074243213	0.237440191387551\\
1190.52413558503	0.234449760765541\\
1192.85152943278	0.231459330143532\\
1194.84862958466	0.228468899521522\\
1197.07443426932	0.225478468899513\\
1201.0830036338	0.222488038277503\\
1204.0357426228	0.219497607655494\\
1208.24635822146	0.216507177033484\\
1212.10881114378	0.213516746411475\\
1215.91483754457	0.210526315789466\\
1219.87912264303	0.207535885167456\\
1222.03188347069	0.204545454545447\\
1224.27252323581	0.201555023923437\\
1227.38972752486	0.198564593301428\\
1231.40413717647	0.195574162679419\\
1236.20578639735	0.192583732057409\\
1241.07828548087	0.1895933014354\\
1246.07137910001	0.18660287081339\\
1251.54956394979	0.183612440191381\\
1256.62004360591	0.180622009569371\\
1261.88455549629	0.177631578947362\\
1266.29604700791	0.174641148325352\\
1277.111679601	0.171650717703343\\
1282.17543766085	0.168660287081334\\
1285.60911620767	0.165669856459324\\
1289.05778927692	0.162679425837315\\
1293.18037904652	0.159688995215305\\
1297.43648500657	0.156698564593296\\
1300.69728362902	0.153708133971286\\
1308.2236461982	0.150717703349277\\
1312.58956085606	0.147727272727268\\
1317.46606112693	0.144736842105258\\
1325.17262957024	0.141746411483249\\
1335.20629485788	0.138755980861239\\
1339.71962182905	0.13576555023923\\
1347.90538074183	0.13277511961722\\
1361.0268487407	0.129784688995211\\
1371.93573486928	0.126794258373202\\
1385.02156063354	0.123803827751192\\
1392.7350722091	0.120813397129183\\
1403.51590422503	0.117822966507173\\
1409.15369982603	0.114832535885164\\
1415.21834379303	0.111842105263154\\
1422.59768068277	0.108851674641145\\
1437.68716387169	0.105861244019135\\
1452.98075193798	0.102870813397126\\
1468.08442246587	0.0998803827751163\\
1480.43306389845	0.0968899521531068\\
1491.53847405778	0.0938995215310974\\
1504.91928369357	0.0909090909090879\\
1514.47325842472	0.0879186602870784\\
1532.3627829669	0.0849282296650689\\
1552.83855380545	0.0819377990430594\\
1568.238250256	0.0789473684210499\\
1593.75030097315	0.0759569377990404\\
1610.24338129203	0.0729665071770309\\
1625.25242990057	0.0699760765550215\\
1639.4056373985	0.0669856459330119\\
1661.41359633663	0.0639952153110025\\
1693.77280224569	0.0610047846889931\\
1722.47815159417	0.0580143540669836\\
1768.6710736809	0.0550239234449741\\
1790.7788904708	0.0520334928229647\\
1816.70138423168	0.0490430622009552\\
1844.05030987662	0.0460526315789458\\
1883.88584983639	0.0430622009569362\\
1931.18746522829	0.0400717703349268\\
1962.28010490702	0.0370813397129174\\
1994.18965388157	0.034090909090908\\
2074.34527197251	0.0311004784688985\\
2121.37885301385	0.028110047846889\\
2203.33303041704	0.0251196172248795\\
2267.54040155714	0.0221291866028701\\
2392.50567974399	0.0191387559808607\\
2563.13173223774	0.0161483253588511\\
2714.31765389853	0.0131578947368417\\
2804.47154708251	0.0101674641148322\\
};
\addlegendentry{$N=3$,~, $\lrmse =679.9$, $\prmse =0.277$, $\gamma \rightarrow \infty$}


==> figures/mse_N_3_K_20_G_5_SNR_40_I_20_Pratio_2_Nratio_2_alpha_2_cs.tex <==
\addplot [color=green, dashed,line width=0.6pt]
  table[row sep=crcr]{%
16.2257314107414	1\\
70.4643438799427	0.992248062015504\\
135.354762460411	0.984496124031008\\
164.875954102285	0.976744186046512\\
183.546024744745	0.968992248062016\\
205.177495570469	0.96124031007752\\
219.666351993176	0.953488372093024\\
234.661382439448	0.945736434108527\\
247.357190592141	0.937984496124031\\
266.757984962084	0.930232558139535\\
275.112782807783	0.922480620155039\\
285.451596443796	0.914728682170543\\
312.081293223598	0.906976744186047\\
321.634082488046	0.899224806201551\\
342.407983458446	0.891472868217055\\
368.763211992892	0.883720930232558\\
384.80272530724	0.875968992248062\\
404.588537471258	0.868217054263566\\
442.039322731376	0.86046511627907\\
475.709754182941	0.852713178294574\\
506.265827010677	0.844961240310078\\
518.000239651074	0.837209302325582\\
553.985138753973	0.829457364341086\\
577.532781869805	0.82170542635659\\
601.774225990192	0.813953488372094\\
634.817690762437	0.806201550387597\\
647.882183309485	0.798449612403101\\
669.783601098101	0.790697674418605\\
691.490453460935	0.782945736434109\\
709.028150586008	0.775193798449613\\
723.541611932239	0.767441860465117\\
744.105763858518	0.759689922480621\\
753.838845796538	0.751937984496125\\
762.874110160436	0.744186046511629\\
778.070583255648	0.736434108527133\\
790.389954881157	0.728682170542637\\
803.812469978558	0.720930232558141\\
816.685883688357	0.713178294573645\\
829.925518282293	0.705426356589149\\
838.171145358414	0.697674418604653\\
849.662574022145	0.689922480620157\\
862.459419641671	0.682170542635661\\
874.99176522049	0.674418604651165\\
883.772689393227	0.666666666666669\\
893.274217434129	0.658914728682173\\
904.656823559984	0.651162790697677\\
921.020606578667	0.643410852713181\\
929.547512891527	0.635658914728685\\
938.724497993642	0.627906976744189\\
946.187219757654	0.620155038759693\\
956.718001706304	0.612403100775197\\
961.722479629691	0.604651162790701\\
975.910296050296	0.596899224806205\\
984.650777528961	0.589147286821709\\
996.878660975063	0.581395348837213\\
1004.11460191954	0.573643410852717\\
1010.87948452966	0.565891472868221\\
1016.36177571758	0.558139534883725\\
1020.45387422671	0.550387596899229\\
1027.19057141447	0.542635658914733\\
1035.41287254008	0.534883720930238\\
1042.79702290501	0.527131782945742\\
1050.43146634788	0.519379844961246\\
1056.70130015342	0.51162790697675\\
1061.69034649746	0.503875968992254\\
1064.23406539684	0.496124031007758\\
1067.38519012918	0.488372093023262\\
1076.93265297528	0.480620155038765\\
1080.93905912346	0.472868217054269\\
1090.1149509189	0.465116279069773\\
1094.31784763155	0.457364341085277\\
1099.50806204276	0.449612403100781\\
1102.90165946052	0.441860465116285\\
1108.81447623299	0.434108527131788\\
1111.68516760207	0.426356589147292\\
1114.45718805334	0.418604651162796\\
1118.23240066004	0.4108527131783\\
1121.38894884413	0.403100775193803\\
1124.9489941507	0.395348837209307\\
1127.40210335067	0.387596899224811\\
1132.7420427879	0.379844961240315\\
1137.36946835389	0.372093023255818\\
1141.52132740234	0.364341085271322\\
1146.30404442631	0.356589147286826\\
1148.85934667911	0.34883720930233\\
1154.30464660456	0.341085271317834\\
1157.71676767586	0.333333333333337\\
1164.07088496515	0.325581395348841\\
1168.60803288346	0.317829457364345\\
1176.7852553323	0.310077519379849\\
1181.53867014898	0.302325581395353\\
1184.86089588831	0.294573643410856\\
1187.01746952434	0.28682170542636\\
1193.70771020307	0.279069767441864\\
1197.8411644676	0.271317829457368\\
1203.46526967147	0.263565891472871\\
1206.97582400544	0.255813953488375\\
1210.86904624822	0.248062015503879\\
1214.88064171527	0.240310077519383\\
1222.73742606856	0.232558139534886\\
1228.73299781857	0.22480620155039\\
1237.36924248697	0.217054263565894\\
1240.35306912674	0.209302325581398\\
1246.52250965803	0.201550387596902\\
1260.13038269748	0.193798449612405\\
1269.97638449125	0.186046511627909\\
1281.34801465601	0.178294573643413\\
1291.71901464962	0.170542635658917\\
1305.17282180932	0.162790697674421\\
1312.57773226521	0.155038759689925\\
1321.85205407072	0.147286821705428\\
1329.95185386235	0.139534883720932\\
1352.89760440233	0.131782945736436\\
1378.3336558074	0.12403100775194\\
1404.45794638264	0.116279069767444\\
1425.0055377682	0.108527131782947\\
1445.7777995356	0.100775193798451\\
1480.52130701036	0.0930232558139549\\
1503.7386375715	0.0852713178294586\\
1531.35791137636	0.0775193798449625\\
1557.68984467147	0.0697674418604662\\
1606.48649635927	0.06201550387597\\
1685.93546099682	0.0542635658914737\\
1741.88367686807	0.0465116279069775\\
1796.52230241497	0.0387596899224812\\
1916.16994125681	0.031007751937985\\
2001.50172538483	0.0232558139534887\\
2334.14804117784	0.0155038759689925\\
2757.45065853079	0.00775193798449625\\
};
\addlegendentry{$N=3$,~, $\lrmse =724.3$, $\prmse =0.288$, $\gamma=40$}


==> mytikz.code.tex <==
% -------------------------------------------------------------------------
% This library provides figures customized for my diessrtation. 
% Copyright 2017 by Ehsan Zandi
% -------------------------------------------------------------------------
\usepackage{xstring}
\usepackage{xparse}
\makeatletter
\pgfdeclareshape{fusion}
{
	\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
		\inheritanchorborder[from=rectangle]
		\inheritanchor[from=rectangle]{center}
	\inheritanchor[from=rectangle]{north}
	\inheritanchor[from=rectangle]{south}
	\inheritanchor[from=rectangle]{west}
	\inheritanchor[from=rectangle]{east}
	\backgroundpath{% this is new
		% store lower right in xa/ya and upper right in xb/yb
			\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
			\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
			% construct main path
\def\xshift{20}
\def\yshift{12}
%%%% the base
		\pgfpathmoveto{\pgfpoint{1.15*\xshift+\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{1.15*\xshift+\pgf@xa}{-1.25*\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.75*\xshift+\pgf@xa}{-1.25*\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.75*\xshift+\pgf@xa}{-1.75*\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.75*\xshift+\pgf@xb}{-1.75*\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-0.75*\xshift+\pgf@xb}{-1.25*\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-1.15*\xshift+\pgf@xb}{-1.25*\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-1.15*\xshift+\pgf@xb}{\pgf@ya}}
		\pgfpathclose
   \pgfusepath{fill}
%% the frame
			\pgfsetcornersarced{\pgfpoint{5pt}{5pt}}
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathclose
%% the fusion rule		
		\pgfsetcornersarced{\pgfpoint{0pt}{0pt}}
		\pgfpathmoveto{\pgfpoint{\xshift+\pgf@xa}{\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-\xshift+\pgf@xb}{\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{-\xshift+\pgf@xb}{-\yshift+\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\xshift+\pgf@xa}{-\yshift+\pgf@yb}}
		\pgfpathclose
		\pgfpathmoveto{\pgfpoint{\xshift+\pgf@xa}{\yshift+\pgf@ya}}
		\pgfpathlineto{\pgfpoint{0.5*\xshift+\pgf@xa}{\yshift+\pgf@ya}}
		\pgfpathmoveto{\pgfpoint{-\xshift+\pgf@xb}{-\yshift+\pgf@yb}}
		\pgfpathlineto{\pgfpoint{-0.5*\xshift+\pgf@xb}{-\yshift+\pgf@yb}}
		\pgfpathclose
	}
}
\pgfdeclareshape{sensor}
{
	\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
		\inheritanchorborder[from=rectangle]
		\inheritanchor[from=rectangle]{center}
	\inheritanchor[from=rectangle]{north}
	\inheritanchor[from=rectangle]{south}
	\inheritanchor[from=rectangle]{west}
	\inheritanchor[from=rectangle]{east}
	\backgroundpath{% this is new
		% store lower right in xa/ya and upper right in xb/yb
			\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
			\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
			% construct main path

%%%% the base
		\def\xmin{( \pgf@xa+\pgf@xb)/2}
		\def\dy{0.4*(\pgf@yb-\pgf@ya)}
		\def\dx{0.4*(\pgf@xb-\pgf@xa)}

		\pgfpathmoveto{\pgfpoint{\xmin}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\xmin}{\pgf@yb+2*\dy}}

		\pgfpathmoveto{\pgfpoint{\xmin}{\pgf@yb+\dy}}
		\pgfpathlineto{\pgfpoint{\xmin+\dx}{\pgf@yb+2*\dy}}

		\pgfpathmoveto{\pgfpoint{\xmin}{\pgf@yb+\dy}}
		\pgfpathlineto{\pgfpoint{\xmin-\dx}{\pgf@yb+2*\dy}}
%% the frame
		\pgfsetcornersarced{\pgfpoint{0pt}{0pt}}
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathclose
	}
}
\newcommand{\insertchap}[1]{
	\IfFileExists{chapters/#1.tex}{
		\def\chappath{chapters}
	  \import{\chappath/}{#1}
	}{
		\def\chappath{chapters/#1}
    \import{\chappath/}{chap_main.tex}
	}
}

\NewDocumentCommand \insertsec { o m }
{
  \IfNoValueTF {#1}
  {\def\secpath{\chappath/sections}}
  {\def\secpath{\chappath/sections/#1}}
  \def\filename{\secpath/#2.tex}
  \input{\filename}
  }
\NewDocumentCommand \insertsubsec{m}{
  \def\filename@insertsubsec{\secpath/#1.tex}
  \input{\filename@insertsubsec}}

%\newcommand{\insertsec}[2]{
%  \IfFileExists{\chappath/sections/#2} {\def\secpath{\chappath/sections/}} {\def\secpath{\chappath/sections/#2}}  %%%% if the subfolder does not exist
%  %%%%%%it looks for the file in the current folder
%	%\subimport{\secpath}{#1.tex}
%	\input{\secpath/#1.tex}
%}

\NewDocumentCommand \insertfig { o m o }
{
  \IfNoValueTF {#1}
  {\def\figsize@insertfig{1}}
  {\def\figsize@insertfig{#1}}

  \IfNoValueTF {#3}
  {\def\filename@insertfig{\secpath/figures/#2}}
  {\def\filename@insertfig{\chappath/sections/#3/figures/#2}}

	\IfEndWith{\filename@insertfig}{.tex}
	{\scalebox{\figsize@insertfig}{\input{\filename@insertfig}}}
	{\includegraphics[width=\figsize@insertfig\textwidth]{\filename@insertfig}}
}


==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

